Efficient IoT Inference via Context-Awareness

While existing strategies to execute deep learning-based classification on low-power platforms assume the models are trained on all classes of interest, this paper posits that adopting context-awareness i.e. narrowing down a classification task to the current deployment context consisting of only recent inference queries can substantially enhance performance in resource-constrained environments. We propose a new paradigm, CACTUS, for scalable and efficient context-aware classification where a micro-classifier recognizes a small set of classes relevant to the current context and, when context change happens (e.g., a new class comes into the scene), rapidly switches to another suitable micro-classifier. CACTUS features several innovations, including optimizing the training cost of context-aware classifiers, enabling on-the-fly context-aware switching between classifiers, and balancing context switching costs and performance gains via simple yet effective switching policies. We show that CACTUS achieves significant benefits in accuracy, latency, and compute budget across a range of datasets and IoT platforms.

==> Backup/Feb8/Case.tex <==
\section{Case for Context-aware Micro-classifiers}
\label{case_context}
There are many methods exist to reduce the computational cost of executing classifiers of IoT devices. We argue that each of these have their limitations when scaled down to small processors/resources, and it is generally beneficial to have classifiers with fewer classes.

\mypara{Limits of alternate approaches:} There are a number of existing approaches for optimizing deep learning models for embedded MCUs  \cite{cheng2017survey} including model compression techniques such as weight quantization, weight sparsification, compact filters and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand}, and early exit methods where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers \cite{teerapittayanon2016branchynet, kaya2019shallow,Fleet-Mobicom23}. But all these approaches improve in accuracy and performance if fewer classes are used. 

\begin{itemize}
\item \emph{Graph: Accuracy vs Size.} Show that a 10 or 20 class classifier will lose accuracy quickly if squeezed below some threshold size for either method (under some resource constraints in terms of number of layers/parameters)

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/Acc_vs_Model_Size.png}
%     \caption{Accuracy Drops as the model gets smaller (Places Dataset)}
%     \label{fig:accuracy_vs_model_size}
% \end{figure}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/STL_All_Config.png}
    \caption{Accuracy Drops when models get squeezed and resolution is decreased}
    \label{fig:accuracy_vs_size}
\end{figure}


\item Fewer classes is better. Classifiers with fewer classes is better from performance perspective.
\end{itemize}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/STL_Acc_vs_Classes.png}
    \caption{Accuracy Drops as the classifier coverage increases (STL Dataset)}
    \label{fig:accuracy_vs_classes}
\end{figure}

\mypara{Temporal correlation in classes} In many static deployments, there is significant temporal stability and context change is not frequent. 
\begin{itemize}
    \item \emph{Graph: Median #classes vs Temporal window.} For different temporal windows (30min, 1hr, 2hr, 3 hr, etc), show the median number of classes that occur. Use camera-trap dataset.
\end{itemize}


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/CDF_Temporal.png}
    \caption{CDF for number of unique classes in different temporal windows (Camera Trap Dataset)}
    \label{fig:CDF_Temporal}
\end{figure}


\mypara{Our idea: Context-aware Micro-classifiers.} To scale down in resources, our idea is to use context-aware $\mu$Classifiers combined with context change detection. Context-aware $\mu$Classifiers consume less resources and can offer \textcolor{red}{higher accuracy} in resource-constrained settings. But they introduce new problem --- need to switch to a different set of classes when detecting that the context has changed. However, as shown above, there is temporal consistency, so context don't change very frequently for static sensor deployments.


==> Backup/Jun23/Design.tex <==
\section{\myname{} Design Overview}
\label{des_over}

We now have an effective similarity metric that can measure the compressibility of a set of classes. With this building block, we can now design a practical system that uses context-aware $\mu Classifiers$. But instantiating such a system in practice presents three challenges. 

\subsection{Challenges}
\label{challenge}
\mypara{Challenge 1: Minimizing training overhead.}
The first challenge is reducing overhead for training a huge number of $\mu$Classifiers. 
For example, if there are 20 classes and we consider 3-class $\mu$classifiers, there are $C^{20}_3 = 1140$ $\mu$Classifers. Furthermore, each 3-class combination will need to be optimized by model compression for which we need to determine the best configuration (e.g. quantization, pruning, resolution, etc). 
If we consider 100 configurations per $\mu$Classifier, then 114K models need to be trained. 

\mypara{Challenge 2: Detecting context switch.} 
A second key challenge is designing an accurate detector that can precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. Since context change detection lies on the critical path of every prediction, the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 

\mypara{Challenge 3: Addressing storage constraints.}
An IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. 
If the IoT device is connected to an edge-cloud, it may be possible to train a $\mu$Classifier \emph{on-demand} and download the learned weights during run-time. 
But this incurs high communication overhead and only works for devices connected to an edge-cloud. 
Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead.

\subsection{\myname{} Overview}
\label{sec:overview}

\myname{} comprises three main components.
During the training phase, the \textit{Configuration Predictor} leverages the ``similarity'' between classes and a kNN model to efficiently identify the suitable configuration of the $\mu$Classifier for each subset of classes. 
The \textit{Budget-limited $\mu$Classifier Selector} selects a smaller subset of $\mu$Classifiers to train and store on device from 
% among the set of $C^N_m$ combinations 
among all possible candidates
to achieve high coverage, high accuracy, and low computational costs while meeting the storage requirements. 
These steps happen offline and are shown in Figure~\ref{fig:offline}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/offline.png}
    \caption{Similarity-based configuration prediction and budget-limited $\mu$Classifier selection}
    \label{fig:offline}
\end{figure}

\begin{figure*}[t!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_v6.png}
    \caption{Context-Aware Switching in the proposed \myname{} architecture. (CCD: Context change detection, FE: Feature extractor)}
    \label{framework_all}
\end{figure*}

At run-time, \textit{context-aware switching} occurs in two steps.
To detect context changes, we augment the \emph{$\mu$Classifier} with an additional lightweight \textit{Context Change Detector} head. 
The \textit{Context Change Detector} head rapidly detects if the input frame is a new class without determining which is the new class. 
If context change is detected, \myname{} executes the \textit{all-class model}, a heavyweight classification module, that determines which classes are present in the scene. 
If a new class is detected, it triggers a ``model switch'' to load a new context-specific $\mu$Classifier. Figure~\ref{framework_all} illustrates switching at run-time.

% \mypara{\myname{} in practice.} \myname{} can be instantiated both for local and cloud-assisted IoT deployment. 

% When the IoT device is operating autonomously, we pre-load a subset of $\mu$Classifiers selected by the budget-limited $\mu$Classifier selection process on the device prior to deployment. During inference, the choice of the all-class model to run for context change detection depends on available resources. 
% On low-end IoT platforms (e.g. with MCU), the all-class model also needs to be resource-constrained and hence a lightweight model like EfficientNet can be used. 
% On heterogeneous multi-core processors (e.g. NXP's i.MX \cite{URL:iMX}), a more computationally heavy model like ResNet \cite{resnet-50} can be used to leverage the more powerful cores.

% When an IoT device is operating with edge-cloud support, it locally executes the $\mu$Classifier.  
% It transmits images to the edge-cloud when a context change is detected. 
% The edge-cloud uses a powerful model like ResNet-50 to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. 
% The parameters of the trained model are then downloaded to the IoT device. 
% To reduce the frequency with which model parameters need to be downloaded via a wireless link, a smaller set of  $\mu$Classifiers selected via the budget-limited $\mu$Classifier selection procedure can be cached on the IoT device.

We now describe these components in more detail.

\section{Configuration Prediction}
\label{sec:configuration-prediction}

Our idea is to design a lightweight configuration selector that can identify the best configuration of the $\mu$Classifier without requiring so many models to be trained. We note that the ``best configuration'' is defined based on application needs, i.e.  the available resources and accuracy tolerance for the application. 
For example, when resources are a priority (e.g. highly constrained IoT devices), then there may be more tolerance for lower accuracy. 
In the rest of the paper, we refer to the best configuration as the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$ (as defined for the application). 

A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions: (1) \textit{What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? }, and (2) \textit{How to quickly identify the most efficient yet accurate $\mu$Classifier, given any subset of classes?}

% \begin{enumerate}
%     \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
%     \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
% \end{enumerate}

\subsection{Multi-Dimensional Configuration Space}
\HG{we might be able to get rid of this section.. having a configuration space of both model size and resolution do not sound really special. }
To make the problem tractable, we look at which configuration parameters provide the large dynamic range of resource-accuracy tradeoffs for $\mu$Classifiers.

We find that two methods are particularly effective for configuring $\mu$Classifiers --- image resolution and filter pruning. Varying the resolution of the image that we provide as input to the $\mu$Classifier is particularly effective because a) the computation complexity of a feature extractor decreases quadratically as resolution (height and width) decreases, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. Filter pruning with different sparsity ratios to control the computation complexity of the feature extractor is also effective. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and pruning level scales down better as compute decreases compared to varying only the pruning level. Each point shows the average accuracy across all 3-class subsets of 10 classes.  We see that varying both resolution and pruning level provides us configurations with lower computation costs while accuracy remains in a reasonable range. Pruning performs poorly in the low FLOPs regime since it requires very high pruning levels which leads to very low accuracies.

\begin{figure}[h]
    \includegraphics[width=0.4\textwidth]{figures/res_size_vs_size_V3.png}
    \caption{Configuring resolution and model size (by varying the pruning level) provides us a large dynamic range in resource-accuracy tradeoffs for configuring $\mu$Classifiers. (Camera Trap dataset is used.)}
    \label{res_size_vs_size}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}

We now have two pieces of the puzzle: a) an effective inter-class similarity metric that accurately tracks resource-accuracy trade-offs of a $\mu$Classifier, and b) a narrower parameter space of resolution and model size as the two parameters that we tune. Given these, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


% \mypara{Similarity-directed sampling.} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration of the remaining combinations accurately. This is critical to ensure the performance of kNN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a \textbf{similarity-directed sampling} scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the kNN.
Compared to random sampling, our empirical evaluation on three datasets demonstrates that similarity-directed sampling can reduce 25-66\% of samples while getting similar prediction accuracy.  

We note that an alternate approach to using a kNN-based configuration selecter is to use Neural Architecture Search (NAS \cite{NAS1,NAS2}). This is a possible option, however, our method is considerably lighter weight since we can quickly decide which classes to use in a $\mu Classifer$ based on similarity, and then cheaply determine which configuration parameters to use via the kNN.

\section{Budget-limited $\mu$C selection}
% \HG{we do not have an evaluation section corresponding to the classifier selection component} 
So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for an $m$-class combination. 
However, in practice, an IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. 
Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead. This raises another question:
\textit{How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes?}
% \begin{enumerate}
%     \item How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes.
% \end{enumerate}


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to cover all classes that can possibly occur in a scene, and achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of covering as many classes as possible is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifier should work in any possible context. 

The problem can be re-phrased as a combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is minimized while each model meets a target accuracy threshold and the collection meets some class coverage requirement. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{salkin1975knapsack}. 
We next elaborate on our greedy algorithm to approximate the optimal solution. 

% \M{Our solution has a different objective in comparison to the stated problem. The Problem says we want to maximize accuracy s.t a budget limit. But our approach aims to minimize computation s.t that the accuracy over a threshold. Do you agree?}
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training of the $\mu$Classifiers.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
If this is the case, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. Since the selection is based on kNN prediction, we again need to go through the process of training the newly selected model to check if the accuracy requirement ($Acc_{thr}$) is satisfied.
% In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
% As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If so, the replacement happens; otherwise, the process repeats and the next lightest $\mu$Classifier will be selected and trained. 
% and checked until the replacement happens. 
% Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
This process continues until the $Acc_{thr}$ threshold is met. 
In our experience, kNN has high accuracy, hence the number of times a $\mu$Classifier in the selected set needs to be replaced is very low.

\mypara{Optimizing storage requirements:} 
Since $\mu$Classifiers that operate on the same model size (same pruning level) share the same model weights, we can further reduce storage requirements by storing one feature extractor per model size, and then only storing the classification and context change detection heads for each chosen $\mu$Classifier. 

% only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

% \subsection{Local and Edge-cloud} 

% We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

% \mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

% The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
% Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

% During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

% On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

% \mypara{Edge-cloud assisted IoT devices.} 
% Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
% The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

% Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
% The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change:} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computationally intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the $\mu$Classifier as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching:} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. Once this is determined, we use a simple technique where the last $p$ predictions made by the pipeline are observed and the farthest predicted class among the previous set of classes is substituted by the new ones. 

As described in \S\ref{sec:overview}, the \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Jun23/DesignOverview.tex <==
\section{Design Overview}
\label{des_over}

While context-aware $\mu$Classifiers consume \emph{less resources} and offer \emph{higher accuracy} in resource-constrained settings, instantiating such a system in practice presents three challenges. 

\subsection{Challenges}
\label{challenge}
\mypara{Challenge 1: Minimizing training overhead.}
The first challenge is reducing overhead for training a huge number of $\mu$Classifiers. 
For example, if there are 20 classes and we consider 3-class $\mu$classifiers, there are $C^{20}_3 = 1140$ $\mu$Classifers. Furthermore, each 3-class combination will need to be optimized by model compression for which we need to determine the best configuration (e.g. quantization, pruning, resolution, etc). 
% This configuration space is quite large and requires us to train models with different choices per 3-class combination to determine the $\mu$Classifier that offers the best accuracy and computation tradeoff. 
If we consider 100 configurations per $\mu$Classifier, then 114K models need to be trained. 
% When the search space is larger, for example, 100 classes in ImageNet \cite{}, this increases to 16 million 3-class models.

\mypara{Challenge 2: Detecting context switch.} 
A second key challenge is designing an accurate detector that can precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. Since context change detection lies on the critical path of every prediction, the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 


\mypara{Challenge 3: Addressing storage constraints.}
% The large number of $\mu$Classifiers raises not just a training challenge but also a storage challenge.
An IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. 
If the IoT device is connected to an edge-cloud, it may be possible to train a $\mu$Classifier \emph{on-demand} and download the learned weights during run-time. 
But this incurs high communication overhead and only works for devices connected to an edge-cloud. 
Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead.

\subsection{\myname{} Overview}
\label{sec:overview}
% We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}. 

% \mypara{\myname{} contributions:} Our work has three major contributions. First, we develop a similarity-aware model configuration predictor to reduce training overhead. 
% The core building block for our method is a \emph{similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
% We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

% Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
% This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the rate to invoke the heavyweight classifier.

% Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
% Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

\myname{} comprises three main components.
During the training phase, the \textit{Configuration Predictor} leverages the ``similarity'' between classes and a kNN model to efficiently identify the suitable configuration of the $\mu$Classifier for each subset of classes. 
The \textit{Budget-limited $\mu$Classifier Selector} selects a smaller subset of $\mu$Classifiers to train and store on device from 
% among the set of $C^N_m$ combinations 
among all possible candidates
to achieve high coverage, high accuracy, and low computational costs while meeting the storage requirements. 
These steps happen offline and are shown in Figure~\ref{fig:offline}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/offline.png}
    \caption{Similarity-based configuration prediction and budget-limited $\mu$Classifier selection}
    \label{fig:offline}
\end{figure}

\begin{figure*}[t!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_v6.png}
    \caption{Context-Aware Switching in the proposed \myname{} architecture. (CCD: Context change detection, FE: Feature extractor)}
    \label{framework_all}
\end{figure*}

At run-time, \textit{context-aware switching} occurs in two steps.
To detect context changes, we augment the \emph{$\mu$Classifier} with an additional lightweight \textit{Context Change Detector} head. 
The \textit{Context Change Detector} head rapidly detects if the input frame is a new class without determining which is the new class. 
If context change is detected, \myname{} executes the \textit{all-class model}, a heavyweight classification module, that determines which classes are present in the scene. 
If a new class is detected, it triggers a ``model switch'' to load a new context-specific $\mu$Classifier. Figure~\ref{framework_all} illustrates switching at run-time.

\mypara{\myname{} in practice.} \myname{} can be instantiated both for local and cloud-assisted IoT deployment. 

When the IoT device is operating autonomously, we pre-load a subset of $\mu$Classifiers selected by the budget-limited $\mu$Classifier selection process on the device prior to deployment. During inference, the choice of the all-class model to run for context change detection depends on available resources. 
On low-end IoT platforms (e.g. with MCU), the all-class model also needs to be resource-constrained and hence a lightweight model like EfficientNet can be used. 
On heterogeneous multi-core processors (e.g. NXP's i.MX \cite{URL:iMX}), a more computationally heavy model like ResNet \cite{resnet-50} can be used to leverage the more powerful cores.

When an IoT device is operating with edge-cloud support, it locally executes the $\mu$Classifier.  
It transmits images to the edge-cloud when a context change is detected. 
The edge-cloud uses a powerful model like ResNet-50 to determine whether a new class needs to be added to the $\mu$Classifier. 
It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. 
The parameters of the trained model are then downloaded to the IoT device. 
To reduce the frequency with which model parameters need to be downloaded via a wireless link, a smaller set of  $\mu$Classifiers selected via the budget-limited $\mu$Classifier selection procedure can be cached on the IoT device.

We now describe these components in more detail.




% \paragraph{Configuration Selector} 
% This component determines the optimal architecture configuration of a \textit{$\mu$Classifier} to achieve both high computation efficiency and task accuracy for a arbitrary subset of classes. 
% It leverages a k-NN model that takes as input a vector representation for a subset of classes, and predict its appropriate \textit{$\mu$Classifier} configuration.
% % We represent a subset of classes as the mean and standard deviation of pair-wise class similarities, which captures how difficult it is to achieve high accuracy for the subset.
% Since not all \textit{$\mu$Classifiers} can be stored on a device, the configuration selector also determines the set of \textit{$\mu$Classifiers} that need to be loaded on device to optimize on-device efficiency.
%  % leverages a greedy approach to select a set of \textit{$\mu$Classifiers} that can fit on device and achieve target task accuracy and the lowest computation cost. \HG{note that I put the selection of subset of mini-classifier here.}



% % We considered several levels of image size downsampling and model size to create a configuration space. Unimportant filters in convolutional layers are pruned to compress the model. 

% % The output vector of the oracle's feature extractor is considered to represent a class and the similarity between two classes is measured using the cosine distance of their vectors. statistics such as mean and std are extracted from pair-wise similarities of a set of classes. Since all possible pair-wise similarities only need to be computed once and k-NN inference is quite fast, the runtime overhead of predicting a configuration is negligible. For training the k-NN we sample a few sets of classes from different levels of hardness/similarity. To make a dataset, we extract the mentioned statistics as the input and label each set of classes with a configuration based on predefined criteria.

% \paragraph{$\mu$Classifier Constructor} 
% This module materializes a well-trained $\mu$Classifier based on the selected configuration by the k-NN. 
% A $\mu$Classifier has a feature extractor, one class label classification head, and a context change detection head. 
% The $\mu$Classifier constructor initializes the feature extractor of the  $\mu$Classifier using parameters that are trained on all classes of the dataset, and trains only the classification and detection heads using the subset of classes. 
% Freezing the feature extractor has two benefits. (1) It makes the training process faster since the computation of the heads are much more lightweight compared to that of the feature extractor. (2) $\mu$Classifiers with the same configuration can share the same feature extractor, reducing space of storing $\mu$Classifiers on device.   


% % The feature extractor of the $\mu$Classifier is previously fine-tuned on all classes of the dataset and will be initialized with these weights. 
% % The feature extractor is kept frozen during training of the classification and context change detector heads. The training process is quite fast as the major part of the $\mu$Classifier is frozen. 
% % The classification and context change detector heads are quantized and then transmitted to the IoT alongside the feature extractor ID. The feature extractor ID notifies the IoT which of the pre-stored feature extractors should be loaded on the IoT.

% \paragraph{$\mu$Classifier-based Predictor}
% This module executes $\mu$Classifiers on device to predict the label of an input image and detect whether a context change happens. 
% If a context change is detected, the input image will be sent to another module \textit{new class detector} to further identify which new class appears.
% In case a new class appear, the predictor will load another $\mu$Classifier that covers the new class and the other recently appeared classes to make predictions.  


 
 
% % This part of the RASCAM architecture is responsible for detecting the new context which is essentially any class other than the current target classes. On the IoT side, there is a convolutional network called $\mu$Classifier with two output heads. One head does the classification task and the other decides whether the context has changed in the current frame or not. 

% % The context change detector is a regressor and it is trained to output a number close to 1 whenever the context changes and a number close to 0 in case the current frame contains an object from the current target classes. Its architecture is shown in Figure \ref{framework1}.

% \paragraph{New Class Detector} 
% This module executes a model that is trained on all classes to identify the class of an input image. 
% We refer to the model as a \textit{all-class model}.  
% If network is available, the module can be placed on the cloud: whenever a context change is detected by the $\mu$Classifier, the image will be compressed and transmitted to the cloud so that the module can execute the all-class model to predict the class label. 
% The class label will be sent back to the device for the device to make the decision on switching $\mu$Classifiers. 
% If the module is placed on the device due to the lack of network connections, it loads the all-class model from storage and executes it locally. 

% The oracle is a powerful model that covers all classes in the dataset. It is fed with the frame as the input and predicts its label. If the predicted class is not in the covered set of classes by the current $\mu$Classifier, the process of preparing a new $\mu$Classifier will be started by the micro-classifier configuration selector module.


% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/framework_iot_v2.png}
%     \caption{IoT node framework}
%     \label{framework1}
% \end{figure}




% Next, we explain the three key components in more detail. 

==> Backup/Jun23/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant activity in recent years in optimizing deep learning methods for low-power embedded systems and IoT devices (e.g. \cite{lai2018enable, warden2019tinyml,mazumder2021survey}). 
%  vlin2021memory
% While there is great diversity in the computational capabilities (e.g. low-power microcontrollers, neural architectures and heterogeneous multi-core processors) and communication capabilities (e.g. BLE and WiFi) of these devices, they share the constraint that they are heavily resource constrained. 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.

% \mypara{Squeezing deep learning models on IoT platforms.} 
Prior approaches to squeeze deep learning models fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. 
% Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. 
%Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 
% 
The second category is partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud~\cite{kang2017neurosurgeon,teerapittayanon2017distributed,choi2018deep, cohen2020lightweight, huang2020clio, itahara2021packet}
% 
The third category is early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations include model compression, partitioning, and early-exit.}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference and its challenges:} 
We argue that one dimension that has not been explored in prior efforts is \emph{context-aware inference}. 
Our endeavor in developing context-aware inference models draws inspiration from the remarkable efficiency of the human brain, particularly, how humans employ working memory. Working memory, a fundamental cognitive mechanism, serves as a mental workspace where individuals can manipulate and process information relevant to the task at hand. Unlike an inexhaustible reservoir, it has a limited capacity. In fact, working memory is often estimated to have a fixed capacity (of approximately three or four items’ worth of information) \cite{luck1997capacity}. Despite this constraint, humans utilize this capacity judiciously. They have a knack for bringing into their working memory only the information that holds relevance for the current context. This discerning selection of information is immensely advantageous as it prevents the cognitive system from getting overwhelmed by the vast expanse of knowledge a human possesses, as much of this knowledge is often extraneous to the immediate task.

What if we borrowed idea of working memory from human cognition and integrated it into our deep learning models? We advocate for an approach that emulates the human working memory by constructing multiple, petite, context-aware classifiers (we refer to these as \textit{$\mu$Classifiers}). Each of these \textit{$\mu$Classifiers} would be akin to a segment of working memory, specialized in handling specific types of information or tasks. Based on the task at hand, the system would dynamically bring the appropriate classifiers into memory, just as humans selectively populate their working memory with relevant information.

% We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. 

What makes context-aware inference particularly effective and relevant in IoT settings is that, in many applications, the context can remain fairly static for extended periods.
For instance, a trail camera positioned in a forest may primarily observe the same set of animals. Similarly, a doorbell camera in a residential area is likely to capture the same types of vehicles and individuals recurrently. Context-aware inference could be beneficial in various other applications such as industrial monitoring systems where machinery states change infrequently, or in smart agriculture where monitoring conditions may remain constant over long growing seasons. This idea holds even greater significance in environments where compute and memory resources are scarce, such as in many IoT devices.


% We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a subset of the overall set of classes, making it more resource-efficient and accurate.

% This paradigm shift necessitates a change in a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

Translating the intuitive concept of using working memory into a practical neural network model presents a plethora of challenges. Human working memory operates on a foundation of sophisticated semantic knowledge, however, our current capability in capturing context within neural networks is considerably more constrained. Thus, the first challenge is how to judiciously group classes into the current context to achieve optimal performance from a computational perspective,

% The first is that we need to minimize training overhead given the large number of $\mu$Classifiers. For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class $\mu$Classifiers and $C^{20}_4$ (4845) four-class $\mu$Classifiers that are possible (if we go with the parallel of human working memory holding three or four chunks of information). 
% In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. %It is impractical to pre-train and optimize a huge number of $\mu$Classifers.
%As we show later, the optimal parameters depend greatly upon the specific set of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to detect context change so that we can switch to the appropriate $\mu$Classifier for the new context when an entity that is not in the class set of the current $\mu$Classifier enters the scene. In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier.

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the lowest computation while meeting the desired accuracy, coverage across classes of interest, and not exceeding available storage. 

\mypara{The \myname{} approach:} We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}.\footnote{\myname{} connotes the back-and-forth nature of switching between $\mu$Classifiers depending on context.}

Our work has three major contributions. First, we develop a similarity-aware kNN-based model configuration predictor to reduce training overhead. 
The core building block for our method is an \emph{inter-class similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the frequency of invoking the heavyweight classifier.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

% In this paper, we present a novel solution that addresses these problems. 
% %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
% First, we define a inter-class similarity metric that captures the similarity of classes and the hardness of distinguishing them.
% A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
% %The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
% Second, we add a regression head to the $\mu$Classifier as the second output head to detect context changes. 
% Since the classification and regression heads share a feature extractor, the overhead for context change detection is negligible. 
% %The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.
% Third, we present a budget-limited $\mu$Classifier selector that selects the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
%     \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
%     \label{fig:our-approach}
% \end{figure}

We implement \myname{} by modifying EfficientNet-B0 \cite{efficientnet} and conduct extensive evaluation across three datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}) and multiple IoT processors (Risc-V(GAP8) \cite{URL:GAP8} and low-end ARM 11 \cite{URL:Arm11} to high-end Cortex-A77 \cite{URL:Cortex-A77}). We show that:
\begin{itemize}
    \item \myname{} can provide up to 13$\times$ reduction in computational cost while outperforming all-class EfficientNet-B0 across a wide range of desired accuracy thresholds. 
    \item Our inter-class similarity metric captures the hardness of a set of classes in a $\mu$Classifier very well (0.86-0.97 Pearson's coefficient between classification accuracy and our metric).
    \item \myname{}'s context change detector has 10-20\% fewer false positives and false negatives than an alternate lightweight detector that uses similar FLOPs. It has only  3-7\% higher false positives and false negatives than a heavyweight detector that uses 2-4$\times$ more FLOPs. 
    \item End-to-end results on the Raspberry Pi Zero W and GAP8 IoT processors show that \myname{} can achieve 1.2$\times$ -- 4.4$\times$ speed-up and up to $5\%$ gain in accuracy compared to all-class EfficientNet. We also show that our greedy algorithm that selects a subset of $\mu$Classifiers to balance accuracy, FLOPs, and coverage under storage constraints has up to 1.4$\times$ speed-up compared to a solely coverage-focused method.
    
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Jun23/Similarity.tex <==
\section{Inter-class Similarity}

So far, we have shown that keeping the context reasonably small (e.g. focusing on three classes) can provide significant performance benefits. However, an intriguing question emerges: does the selection of which three classes are chosen carry significance from a resource optimization perspective? In other words, are some groups of classes more compressible than others?

\subsection{Choice of context matters}

\DG{Is there a generic way to validate this without specifically describing our approach?}

Indeed, we show that selection of classes within a $\mu$Classifier is of paramount importance, as different groups of three classes can exhibit different levels of compressibility when subjected to various model compression techniques such as pruning, quantization, or early exiting. \DG{correct?} Intuitively, this can be understood by considering the inherent characteristics of the classes in question.

Imagine that the classes are representative of different animals that might be captured by a trail camera. When the classes consist of animals with similar features, textures, or behaviors, the classifier faces a more challenging task in distinguishing between them. For instance, if the three classes represent a deer, an elk, and a moose, the classifier has to contend with the fact that all three animals have somewhat similar body shapes, sizes, and features. Consequently, the model may need to employ more computational resources to scrutinize subtle distinctions and achieve a comparable level of accuracy.

In contrast, if the classes are composed of animals that are markedly disparate in features, they are more easily distinguishable, and the classifier can make decisions with less computational effort. For example, consider a group comprising a deer, a rabbit and a racoon. These animals are drastically different in size, appearance, and behavior, making them easier to classify with higher confidence.

In essence, the inter-class similarities or differences play a significant role in determining the computational resources needed by the $\mu$Classifier. When designing a context-aware system, careful consideration should be given to the grouping of classes, taking into account the inherent characteristics of the data to optimize performance and resource utilization.

% For example, we could contemplate several $\mu$Classifier designs. One approach, based on temporal co-occurrence, might be to simply load a $\mu$Classifier for the three most recently observed classes. On the other hand, a more meticulous design could involve selecting the three classes that yield the best performance based on certain criteria or metrics. The crux here lies in discerning whether there is a substantial performance difference between these options. We start by analyzing and comparing the efficacy of these designs to provide insights into the optimization of context-aware neural network models.

\subsection{Similarity metric}

How can we capture the compressibility of a group of classes? As we describe later, such a metric is necessary to quickly determine which $\mu Classifiers$ to select and what configuration to use to train it.

To achieve this, we define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities would also share a similar $\mu$Classifier configuration. 

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

We note that the above metric was chosen after careful consideration of several alternate measures of similarity including using a ``confusion matrix'' and XXX \DG{what else?}. We show empirical results comparing these metrics in \S\ref{}.

\subsection{Similarity as proxy for compressibility} 

We now look at whether the similarity metric that we have defined captures the essential resource-accuracy tradeoffs in grouping classes into a $\mu Classifier$. 

Figure~\ref{heatmap} shows that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to the similarity among classes (darker $\implies$ higher accuracy). X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolutions) sorted from least to most compute complexity. We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models. \DG{Since this comes before we discuss the configuration space, can we make the heatmap more generic i.e. not specific to size/resolution but pick one dimension, for example, pruning or early exit or something else that a reader would naturally expect.}}
    \label{heatmap}
\end{figure}

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.}
    \label{fig:kNN-training}
\end{figure}


==> Backup/Jun24/Case.tex <==
\begin{figure*}[t]%
    \centering
    \subfloat[\centering Fewer classes is better\label{fig:accuracy_vs_classes}]{{\includegraphics[width=.32\textwidth]{figures/Acc_vs_Classes.png}}}%
    \subfloat[\centering Pruning does not reduce gap (STL-10) \label{fig:accuracy_vs_size}]{{\includegraphics[width=.335\textwidth]{figures/STL_All_Config_V3.png}}}%
    % \qquad
    \subfloat[\centering Early exit does not reduce gap \label{fig:early_exit accuracy_vs_size}]{{\includegraphics[width=.32\textwidth]{figures/Early_Exit_Acc_Vs_Classes.png}}}%
    \caption{Context-aware $\mu$Classifiers can provide substantial performance advantages. (a)  shows that accuracy drop is substantial as \#classes increases; (b) shows that model compression expands this gap further and (c) shows a similar trend for early-exit models. \HG{need to change the color of figure (a) and (c); the current drawing makes people naturally comparing the blue and orange curves.}}
\label{knn_performance}
\end{figure*}

\section{Case for $\mu$Classifiers}
\label{case_context}

In this section, we compare two designs for squeezing DNNs on IoT devices ---  the canonical method of training and compressing an \textit{all-class model} and our approach of using a \textit{$\mu$Classifier} that has fewer classes. 

\mypara{Observation 1: Using fewer classes has significant performance benefits.} 
Intuitively, if a classifier has fewer classes than another, it should be more accurate given the same resources. 
But how much is this gain in accuracy?

To answer this, we look at the accuracy of the EfficientNet-B0 on different subsets of classes from STL-10 \cite{STL10} and Camera Trap dataset~\cite{Camera_trap_enonkishu,Camera_trap_camdeboo} (See \S\ref{experiment_setting} for details on the datasets).
Figure~\ref{fig:accuracy_vs_classes} shows the average accuracy across all 3-class subsets of the 10 classes, the 4-class subsets, and so on till all 10 classes. 
Post-training dynamic range quantization~\cite{dynamicq} is applied to all models. 

We see that accuracy increases steadily as the number of classes decreases: the overall increase is by about 5\% and 13\% for STL-10 and Camera Trap respectively when we go from 10 classes to 3 classes. 
This indicates the substantial accuracy advantage of $\mu$Classifiers over an all-class model given the same DNN architecture.

\mypara{Observation 2: Model compression does not diminish the advantage of $\mu$Classifiers.} 
In Figure~\ref{fig:accuracy_vs_classes}, we used EfficientNet-B0 with quantization but did not apply other techniques that are available for optimizing deep learning models for embedded MCUs (e.g. weight sparsification, filter pruning, and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand,cheng2017survey}). 
We now ask whether these techniques can bridge the accuracy gap between $\mu$Classifiers and the all-class model.

Figure~\ref{fig:accuracy_vs_size} shows the performance gap between 10-class and 3-class EfficientNet after model pruning and quantization on the STL-10 dataset. 
We apply filter pruning~\cite{str_p1} which reduces the number of filters in each layer based on $\ell_1$ norm. The accuracy of each orange point that represents a 3-class model is computed by averaging the accuracy of all 3-class subsets. 
We see that the accuracy gap between the $\mu$Classifier and all-class classifier increases as resources reduce (5\% at 148 MFLOPs to 11.5\% at 70 MFLOPs).  
The result highlights that model optimization techniques cannot diminish the accuracy advantage of $\mu$Classifiers over the all-class model. 
In other words, $\mu$Classifiers achieves higher computation efficiency than all-class model given the same target accuracy.  

\mypara{Observation 3: The benefits hold for early exit models.} 
Another approach to reduce the computational requirements of executing models on IoT devices is to use early exit, where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers~\cite{teerapittayanon2016branchynet, kaya2019shallow, fleet2023}. 
This is an orthogonal dimension to the idea of limiting the number of classes, so we augment $\mu Classifiers$ with early exit capability. 
We compare the performance of a $\mu$Classifier with early-exit capability against an all-class models with early exit.  


Figure~\ref{fig:early_exit accuracy_vs_size} shows the average accuracy across all 3-class subsets of 10 classes, 4-class subsets, and so on till all 10 classes after applying quantization and adding two early exit branches (stages 4 and 6) to the EfficientNet-B0. 
We see that accuracy increases with a decreasing number of classes. 
In particular, 3-class $\mu$Classifiers has 5\% and 12\% higher accuracy compared to all-class models for STL-10 and Camera Trap datasets respectively. 
Thus, the performance advantages of $\mu$Classifiers remain even if we augment the model with early exits.


==> Backup/Jun24/Design.tex <==
\section{Configuration Prediction}
\label{sec:configuration-prediction}

With similariyy as a building block, we can now design a practical method to reduce the training overhead for $\mu Classifiers$.

Our idea is to design a lightweight configuration selector that can identify the best configuration of the $\mu$Classifier without requiring so many models to be trained. We note that the ``best configuration'' is defined based on application needs, i.e.  the available resources and accuracy tolerance for the application. 
For example, when resources are a priority (e.g. highly constrained IoT devices), then there may be more tolerance for lower accuracy. 
In the rest of the paper, we refer to the best configuration as the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$ (as defined for the application). 

A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions: (1) \textit{What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? }, and (2) \textit{How to quickly identify the most efficient yet accurate $\mu$Classifier, given any subset of classes?}

% \begin{enumerate}
%     \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
%     \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
% \end{enumerate}

\subsection{Multi-Dimensional Configuration Space}
\HG{we might be able to get rid of this section.. having a configuration space of both model size and resolution do not sound really special. }
To make the problem tractable, we look at which configuration parameters provide the large dynamic range of resource-accuracy tradeoffs for $\mu$Classifiers.

We find that two methods are particularly effective for configuring $\mu$Classifiers --- image resolution and filter pruning. Varying the resolution of the image that we provide as input to the $\mu$Classifier is particularly effective because a) the computation complexity of a feature extractor decreases quadratically as resolution (height and width) decreases, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. Filter pruning with different sparsity ratios to control the computation complexity of the feature extractor is also effective. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and pruning level scales down better as compute decreases compared to varying only the pruning level. Each point shows the average accuracy across all 3-class subsets of 10 classes.  We see that varying both resolution and pruning level provides us configurations with lower computation costs while accuracy remains in a reasonable range. Pruning performs poorly in the low FLOPs regime since it requires very high pruning levels which leads to very low accuracies.

\begin{figure}[h]
    \includegraphics[width=0.4\textwidth]{figures/res_size_vs_size_V3.png}
    \caption{Configuring resolution and model size (by varying the pruning level) provides us a large dynamic range in resource-accuracy tradeoffs for configuring $\mu$Classifiers. (Camera Trap dataset is used.)}
    \label{res_size_vs_size}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}

We now have two pieces of the puzzle: a) an effective inter-class similarity metric that accurately tracks resource-accuracy trade-offs of a $\mu$Classifier, and b) a narrower parameter space of resolution and model size as the two parameters that we tune. Given these, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


% \mypara{Similarity-directed sampling.} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration of the remaining combinations accurately. This is critical to ensure the performance of kNN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a \textbf{similarity-directed sampling} scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the kNN.
Compared to random sampling, our empirical evaluation on three datasets demonstrates that similarity-directed sampling can reduce 25-66\% of samples while getting similar prediction accuracy.  

We note that an alternate approach to using a kNN-based configuration selecter is to use Neural Architecture Search (NAS \cite{NAS1,NAS2}). This is a possible option, however, our method is considerably lighter weight since we can quickly decide which classes to use in a $\mu Classifer$ based on similarity, and then cheaply determine which configuration parameters to use via the kNN.

\section{Budget-limited $\mu$C selection}
% \HG{we do not have an evaluation section corresponding to the classifier selection component} 
So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for an $m$-class combination. 
However, in practice, an IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. 
Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead. This raises another question:
\textit{How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes?}
% \begin{enumerate}
%     \item How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes.
% \end{enumerate}


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to cover all classes that can possibly occur in a scene, and achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of covering as many classes as possible is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifier should work in any possible context. 

The problem can be re-phrased as a combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is minimized while each model meets a target accuracy threshold and the collection meets some class coverage requirement. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{salkin1975knapsack}. 
We next elaborate on our greedy algorithm to approximate the optimal solution. 

% \M{Our solution has a different objective in comparison to the stated problem. The Problem says we want to maximize accuracy s.t a budget limit. But our approach aims to minimize computation s.t that the accuracy over a threshold. Do you agree?}
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training of the $\mu$Classifiers.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
If this is the case, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. Since the selection is based on kNN prediction, we again need to go through the process of training the newly selected model to check if the accuracy requirement ($Acc_{thr}$) is satisfied.
% In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
% As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If so, the replacement happens; otherwise, the process repeats and the next lightest $\mu$Classifier will be selected and trained. 
% and checked until the replacement happens. 
% Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
This process continues until the $Acc_{thr}$ threshold is met. 
In our experience, kNN has high accuracy, hence the number of times a $\mu$Classifier in the selected set needs to be replaced is very low.

\mypara{Optimizing storage requirements:} 
Since $\mu$Classifiers that operate on the same model size (same pruning level) share the same model weights, we can further reduce storage requirements by storing one feature extractor per model size, and then only storing the classification and context change detection heads for each chosen $\mu$Classifier. 

% only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

% \subsection{Local and Edge-cloud} 

% We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

% \mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

% The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
% Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

% During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

% On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

% \mypara{Edge-cloud assisted IoT devices.} 
% Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
% The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

% Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
% The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change:} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computationally intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the $\mu$Classifier as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching:} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. Once this is determined, we use a simple technique where the last $p$ predictions made by the pipeline are observed and the farthest predicted class among the previous set of classes is substituted by the new ones. 

As described in \S\ref{sec:overview}, the \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Jun24/DesignOverview.tex <==
\section{\myname{} Design Overview}
\label{des_over}

So far, we have shown that keeping the context reasonably small (e.g. focusing on three classes) can provide significant performance benefits. 
However, instantiating such a system in practice presents three challenges

\subsection{Challenges}
\label{challenge}
% \mypara{Challenge 1: Deciding which classes to group.} The first challenge is deciding which classes to group into a $\mu$Classifier to get best performance --- we find that this matters from a computational perspective and different choices lead to vastly different resource usage to achieve the same target accuracy. 

\mypara{Challenge 1: Identifying resource-efficient $\mu$Classifers for every possible context.}
The first challenge is to identify the most resource-efficient $\mu$Classifers for every possible context that reaches a target accuracy. 
The total number of contexts grows exponentially with the total number of classes. 
For example, if there are 40 classes and we consider 3-class $\mu$classifiers, there are $C^{40}_3 = 9880$ $\mu$Classifers. 
And what's worse, the optimal configurations of the $\mu$Classifer depends on the difficulty level of the context.  
A context whose classes have similar patterns or features would be harder to recognize and need to use a $\mu$Classifier that has higher model capacity.  
If we consider 10 configurations per $\mu$Classifier, then nearly 100K models need to be trained to identify the optimal $\mu$Classifers for all possible contexts. 


\mypara{Challenge 2: Detecting context switch.} 
The second key challenge is designing an accurate detector that can precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. 
Since context change detection lies on the critical path of every prediction, 
the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 

\mypara{Challenge 3: Robustness to connectivity.}
The third key challenge is operating in different communication regimes. For example, when connectivity is strong, we can train new $\mu Classifiers$ on-demand in the cloud and download the learned weights during run-time when a new context arises. But when cloud-assistance is unavailable or bandwidth too limited, then a subset of $\mu$Classifiers need to be pre-trained and stored locally in the limited IoT storage.

\begin{figure*}[t!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_v7.png}
    \caption{Context-Aware Switching in \myname{}. In case the communication or cloud is not available, the framework relies on cached/stored $\mu$Classifiers. (CCD: Context change detection, FE: Feature extractor)}
    \label{framework_all}
\end{figure*}


\subsection{\myname{} Overview}
\label{sec:overview}



\myname{} executes context-aware $\mu$Classifiers for a prediction task deployed on a device and dynamically switches between $\mu$Classifiers to handle context changes.  
It comprises three main components.


The first component \textit{Configuration Predictor} identifies the suitable configuration of the $\mu$Classifier for each context, i.e., a subset of classes.  
It addresses the first challenge by representing a context based on an \textit{inter-class similarity} metric. 
The metric estimates the difficulty in classifying the set of classes in a context and allows a simple k-nearest neighbor approach to rapidly predict the optimal configuration of a $\mu$Classifier. 

 
The second component \textit{context-aware switching} enables the device to seamlessly switch between $\mu$Classifiers based on context changes. 
It occurs in two steps to address the second challenge. 
To detect context changes, we augment $\mu$Classifiers with an additional lightweight \textit{Context Change Detector} head. 
The \textit{Context Change Detector} head rapidly detects if the input frame is a new class without determining which is the new class. 
If context change is detected, \myname{} executes the \textit{all-class model}, a heavyweight classification module, that determines which classes are present in the scene. 
If a new class is detected, it triggers a ``model switch'' to load a new $\mu$Classifier. 
Figure~\ref{framework_all} illustrates switching at run-time.

The last component \textit{Budget-limited $\mu$Classifier Selector} selects a smaller subset of $\mu$Classifiers to train and store on device from among all possible candidates. 
It addresses the third challenge by allowing devices to switch between $\mu$Classifiers locally during run-time when cloud assistance is unavailable.  

\mypara{Usage scenarios.} \myname{} supports two types of usage scenarios depending on the availability of cloud assistance.

When the cloud assistance is available, \myname{} instantiates the first two components: context-aware switching detects changes in context and requests a $\mu$Classifier for the new context. \myname{} cloud executes the Configuration Predictor to rapidly identify the suitable configuration of the $\mu$Classifier, then trains the $\mu$Classifier and downloads the well-trained model to the device to handle the new context. These are cached on-device and the next time the same context occurs, the cached model can be used as shown in Figure~\ref{framework_all}

For unattended operation i.e. no cloud availability, \myname{} relies on locally stored $\mu$Classifiers. At installation time, the Budget-limited $\mu$Classifier Selector and Configuration Predictor are used to select the optimal set of  $\mu$Classifiers to store on the device such that context-aware switching can happen locally. 



If times when connectivity is available, additiionl $\mu$Classifiers may be downloaded and cached on-device.
 
%  executes Configuration Predictor to identify the suitable configurations for all possible contexts offline. 
% It then uses Budget-limited $\mu$Classifier Selector to select the optimal set of  $\mu$Classifiers to install on the device such that context-aware switching can happen locally. 



\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/offline.png}
    \caption{Similarity-based configuration prediction and budget-limited $\mu$Classifier selection}
    \label{fig:offline}
\end{figure}


We now describe these components in more detail.



==> Backup/Jun24/Evaluation.tex <==
\section{Evaluation}
We first describe the implementation and experiment settings, and then evaluate the components of \myname{} over datasets and real platforms. 
% We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Implementation}

\mypara{IoT processors:} 
We implement the \myname{} pipeline on three different IoT devices --- Raspberry Pi 4B, Raspberry Pi Zero W, and GAP8. We generate \textbf{TensorFlow Lite} models using the default optimization and int-8 quantization to reduce the model size and execution latency. On all the platforms, we profile the execution latency of models of different configurations on different datasets.

For profiling on Raspberry Pi 4B and Zero W, we utilize the \textbf{TVM} framework \cite{TVM} to tune the operator implementations to reduce the execution latency for the Arm Cores. 

For profiling on GAP8, we use the GAP8 tool chain \cite{URL:GAP8_tool} to transform the \textbf{TensorFlow Lite} models into C code by fusing the operations. 

\mypara{Training:} An NVIDIA Tesla M40 24GB GPU was used for training models and as the edge-cloud in some of our experiments. 

\mypara{Open source code:} If accepted, we will make our code on all the above platforms openly available.

\subsection{Experiment Settings}
\label{experiment_setting}

\begin{comment}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resolution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\end{comment}

\mypara{Dataset:}
\label{dataset}
We use three datasets, Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}, STL-10 \cite{STL10}, and Places365 \cite{PLACES365}.
Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images, each time in a sequence of three. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two snapshot projects, Enonkishu \cite{Camera_trap_enonkishu} and Camdeboo \cite{Camera_trap_camdeboo}, were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species were picked from the Snapshot Camdeboo dataset (both from cameras in the African savannah) to get a total of ten species. The dataset has labels over 3-frame image sequences (i.e. the label would be for a species even if it is present in one of the frames), which leads to erroneous labels for several individual frames. Hence, accuracy is lower across all methods for this dataset.

STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 

PLACES365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 

% Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10 species classes + 1 empty class to be close to the real-world setting. As mentioned, Camera Trap images form a sequence of 3 frames and the labels in each sequence are the same. However, sometimes one or more frames in the sequence do not show any species in the scene as they have left the scene. Hence, those frames are wrongly labeled as that species. It leads to non-accurate labels which lower the accuracy of the classification task.}

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation i.e. each $\mu$Classifier has 3 places, objects, or species depending on the dataset. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_classes}) but also requires the most switching between contexts. 
So, it helps us evaluate the upper limits of how a nimble context-aware system can be designed with $\mu$Classifiers. 
%By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. %Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

\mypara{The configuration space of $\mu$Classifiers:}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that besides the EfficientNet-B0 we get a total of four feature extractor architectures.  
%The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The range of image resolutions is considered 58-96, 130-256, and 100-320 for STL-10, PLACES365, and Camera Trap datasets respectively. For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
The two heads use two Fully Connected layers. Feature extractors are fine-tuned once on all classes, and then frozen during the training of the two heads of $\mu$Classifiers.

\mypara{Inter-class similarity metric:}
The configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of ResNet-50 to extract the embedding of images from a class and average the embeddings into a single vector to be used for computing the inter-class similarities. 


\mypara{KNN-based configuration selection:}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector, and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in \S\ref{sec:knn}) to get 200 3-class combination samples from 1140 combinations ($C^{20}_3$) in the PLACES365 dataset, and 40 out of 120 combinations ($C^{10}_3$) for the STL-10 and Camera Trap datasets. 
For each sampled 3-class combination, we train $\mu$Classifiers with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 

After collecting the training data, we use the kNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved.


\mypara{Context-aware switching.} 
As discussed in \S\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect the context change. 
It is trained to output a value close to 0 for the target classes of the $\mu$Classifier and a value around 1 for other classes. 
We used $0.5$, $0.6$, and $0.45$ as the decision boundary for STL-10, Camera Trap, and PLACES365 datasets respectively.
% 
Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50 for its high classification accuracy if higher resources are available (e.g. cloud offload or heterogeneous multi-core processor) and uses EfficientNet-B0 otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on the target dataset.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance of Configuration Prediction with different accuracy thresholds.}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}

This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in lighter $\mu$Classifiers and thus less FLOPs. 

We compared the classification accuracy and computation cost of the predicted configuration (\myname{}) against the following baselines: (a) \textbf{All-Class EfficientNet}, which uses the well-trained EfficientNet-B0 with all the classes and full image resolution, (b) \myname{} \textbf{(Highest FLOPs)}, which uses the $\mu$Classifier that has same classes as \myname{} predicts but uses full image resolution and no pruning (and hence computationally the most expensive), and (c) \myname{} \textbf{(Oracle)} i.e. the $\mu$Classifier that meets the target accuracy threshold with minimum FLOPs (which would be selected by an omniscient scheme rather than the kNN-based method we use). We note that training the Oracle is not scalable --- it takes a total of 40, 120, and 300 hours longer than our approach for the STL-10, Camera Trap, and PLACES365 respectively.
% , and would take longer on larger datasets.

Figure~\ref{knn_performance} shows how different target accuracy thresholds affect the classification accuracy and the computation costs for our methods and baselines. We sweep over target accuracy thresholds for the curves but the dotted horizontal line shows a specific choice of target accuracy that we use in the rest of this paper (chosen as described in \S\ref{experiment_setting}). 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   

We see that \myname{} (the orange curve) can cover a wide trade-off region between accuracy and computational cost --- accuracies vary by 3.5-8.8\% and compute by 3.9$\times$ to 13$\times$. Across this range, the accuracy is nearly as good as the \myname{} (Oracle) which shows that the kNN together with the inter-class similarity metric works well in selecting the best configuration. 

In contrast, All-Class EfficientNet (red star) and 3-class EfficientNet (green star) are point solutions. We compare these models against a specific instance of \myname{}, i.e. the point where the dotted line intersects the \myname{} curve (orange) based on the threshold we choose. 
This configuration of \myname{} is 0.8-10\% more accurate than All-Class EfficientNet and requires $53\%$ to $75\%$ less computation to hit the target accuracy. 
When comparing against \myname{} (Highest FLOPs), we see that \myname{} achieves 53-75\% computation savings while sacrificing 1.5-4.3\% classification accuracy. 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

% We now compare \myname{} against {all-class EfficientNet} (red star). \myname{} is between 5.1\% -- 12.3\% more accurate and requires 53\% to $74.79\%$ less computation to hit the target accuracy (horizontal dotted line).

% When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
% For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_vs_sim_eval}]{{\includegraphics[width=.24\textwidth]{figures/Accuracy_Vs_Similarity.png}}}%
    \subfloat[\centering \label{fig:comp_gain_Vs_Similarity}]{{\includegraphics[width=.235\textwidth]{figures/comp_gain_Vs_Similarity.png}}}%
    \caption{(a) We select a representative configuration and show how its accuracy varies with inter-class similarity. 
    (b) The relation between the computational complexity of the predicted $\mu$Classifiers and the inter-class similarity. We see that both accuracy and computation gain (over All-Class EfficientNet or Highest FLOPs $\mu$Classifier) drop as similarity increases. Thus, our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes. Similarity is normalized to [0, 1] in both figures.}
% \label{}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.25\textwidth]{figures/Accuracy_Vs_Similarity.png}
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
%     \label{acc_vs_sim_eval}
% \end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/comp_gain_Vs_Similarity.png}
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
%     \label{speedup_vs_sim_eval}
% \end{figure}

\mypara{Effectiveness of the inter-class similarity metric:} We now examine the effectiveness of the proposed inter-class similarity metric in quantifying the difficulty level of differentiating a set of classes. 
% Recall that our underlying assumption in the configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold. Thus, two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. We now ask whether this is indeed the case i.e. can the difficulty level can be quantified by our proposed inter-class similarity metric? 

Figure~\ref{fig:acc_vs_sim_eval} illustrates how the accuracy of a representative $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
% 
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.86-0.97$), indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure~\ref{fig:comp_gain_Vs_Similarity} looks at this relation from another performance dimension --- computation gain. The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-class similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class EfficientNet/\myname{} (Highest FLOPs) and the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the similarity-aware kNN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
\myname{} $\mu$C + regression head & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
\myname{} $\mu$C + maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\  
\myname{} (Oracle) $\mu$C + regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
\myname{} (Highest FLOPs) $\mu$C + regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\ \hline

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
% An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. 
A false positive (FP) that wrongly predicts a context change would introduce additional cost whereas a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot detect the context change. 
To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.

Table~\ref{fpfnt} compares the context-change detection performance of \myname{} against several baselines: a) the same $\mu$Classifier as \myname{} but with a different approach for context change detection based on maximum probability \cite{maxsoft1}, b) the \myname{} (Oracle) $\mu$Classifier with regression head and c) the \myname{} (Highest FLOPs) with regression head as a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.

\myname{}'s use of a regression head is much more accurate compared to the baseline that uses the maximum probability. The FP and FN rates of our approach are $10-20\%$ lower than the baseline. \myname{} is quite close to the Oracle $\mu$Classifer as well. There is a gap in performance between \myname{} and \myname{} \textbf{(Highest FLOPs)} (2-4\% for Camera Trap and PLACES365, and 6-7\% for STL-10) but this is to be expected since we are operating with a lower target accuracy, and have considerable computational gains.
These values can be further lowered by increasing the $Acc_{thr}$ explained in \S\ref{sec:configuration-prediction} as it directly affects the predicted configuration and therefore FP and FN rates. 

\begin{table*}[t]
% \scalebox{0.55}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) \\
%   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) \\ 
  \midrule
\myname{} & 88.5\% & 229.1 & 382.0 & 93.5\% & 88.9 & 94.1 & 95.4\% & 291.0 & 512.4 \\
\myname{} (Oracle) & 88.8\% & 227.8 & 355.4 & 93.8\% & 90.6 & 96.2 & 95.7\% & 292.6 & 511.6\\
\myname{} (Highest FLOPs) & 91.4\% & 842.6 & 1854.7 & 95.9\% & 120.7 & 137.6 & 96.8\% & 534.4 & 1168.4\\
All-Class EfficientNet (full res) & 82.0\% & 833.4 & 1844.0 & 92.1\% & 107.9 & 124.5 & 90.4\% & 521.1 & 1162.1 \\
All-Class EfficientNet-Early Exit & 81.0\% & 450.0 & 916.6 & 91.9\% & 100.1 & 108.9 & 90.1\% & 417.2 & 883.2 \\
All-Class EfficientNet-Pruned(30\%) & 76.2\% & 676.6 & 1092.1 & 84.3\% & 89.0 & 95.5 & 84.9\% & 377.7 & 587.1 \\
FAST \cite{FAST} & 82.9\% & 801.6 & 1730.4 & 92.8\% & 108.9 & 124.4 & 91.0\% & 501.6 & 1091.7 \\
\midrule
\end{tabular}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/diff_context_change.png}
%     \caption{\myname{} performance with different context change rate in Edge-Cloud assisted setting. The blue curves show the end-to-end latency for PLACES365 and STL-10 datasets. The red curves show the accuracy for the two mentioned datasets.} 
%     \label{diff_context_change}
% \end{figure}

% \begin{table*}[t]
% %\scalebox{1}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% & \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c|}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8\\ 
%   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}
%     &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c}{(ms)}\\ 
%   \midrule
% Greedy Selection & 80.92\% & 266.76 & - & 81.55\% & 267.41 & - & 81.65\% & 288.84 & - & 81.97\% & 305.16 & -\\
% Random Selection & 81.30\% & 352.60 & - & 81.22\% & 369.33 & - & 81.31\% & 357.06 & - & 81.53\% & 369.34 & - \\

% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}
% \caption{End-To-End performance of Local inference; $3\%$ Context change rate}
% \label{local_end-to-end}
% \end{table*}


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:speedup_local}]{{\includegraphics[width=.24\textwidth]{figures/speedup_local.png}}}%
    \subfloat[\centering \label{fig:acc_local}]{{\includegraphics[width=.235\textwidth]{figures/acc_local.png}}}%
    \caption{(a) The greedy selector picks better $\mu$Classifiers resulting in speedup over coverage-based selection (on Rasp. Pi0; GAP8 results are similar). (b) Even with only 10 $\mu$Classifiers i.e. 8.3\% of all $C^{10}_3$ 3-class subsets, accuracy is nearly as high All-class EfficientNet but with 3$\times$ speedup.}
% \label{}
\end{figure}

\subsection{End-to-End Evaluation}
In order to evaluate the end-to-end performance of \myname{}, we need to evaluate on a dataset that has context change and over a real embedded platform. The Camera Trap dataset provides us with a real-world temporal flow with context changes but other datasets are not temporal. We sequence test sets from the Places and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. Specifically, we find that the context change rate is $3\%$ for the Camera Trap dataset when considering 3-class $\mu$Classifiers. We use this to synthesize a test set with 3\% context change for the PLACES365 and STL-10 datasets and use this in our evaluation unless noted differently.

% If we consider $m$-class combinations, the context changes whenever a frame represents a class different from the last $m$ distinct classes. 
% Consider the case when $m=3$ i.e. 3-class combinations. Let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

% Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is $n=\lceil{CCR\times |TS|}\rceil$.


To generate a test set with temporal flow, we randomly construct a sequence of 3-class combinations, where every two consecutive combinations show a context change of a single class. To match the context change rate to 3\%, we persist the current context for an appropriate time by picking random samples from the current context. 

% In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantees n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  

% In the 3-class combination setting the context change rate is $3\%$ for the Camera Trap dataset. As this dataset has a temporal flow and it shows a real-world use case for \myname{}, its intrinsic context change rate is considered for evaluating all three datasets unless noted differently.



%  \begin{algorithm}
%         \caption{Generating a sequence of contexts}
%         \label{Alg3}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$TS$: Original test set)
%         \\$CCR$: Context change rate
%         \\$S$: List of all m-class combinations\\     
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $n = \lceil{CCR\times |TS|}\rceil$
%             \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
%             \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
%             \While{$|C|\neq n$}
%             \State $New_C = random\_choice(S)$ \Comment{New context candidate}
%             \If {$|New_C\cap Curr_C|==m-1$}
%               \State $C=C\cup New_C$
%               \State $Curr_C=New_C$
%             \EndIf
%             \EndWhile
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: A sequence of $n$ contexts  
% \end{flushleft}           
%     \end{algorithm}

\mypara{Edge-Cloud Assisted Inference:} First, we look at an edge-cloud assisted system that uses ResNet-50 as the all-class model in the cloud to predict the label of the new context. The IoT communicates via WiFi with data rate of $10$ Mbps. The reported latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices. We assumed no $\mu$Classifiers are cached on the device which is the \emph{worst-case scenario} as it requires more transmission and increases the overall latency. We report average latencies over the test set. Note that for the Camera Trap dataset, the lack of enough training samples and inaccurate labels results in lower accuracy for both EfficientNet and ResNet-50, and hence the difference in accuracy between \myname{} and All-Class EfficientNet is very small. 

% . As a result, thResNet-50 only gains 0.2\% over All-Class EfficientNet. We employed ResNet-50 as the all-class model in the cloud to be consistent with the other two datasets. ResNet-50 is the bottleneck in the pipeline for the Camera Trap dataset as it was not possible to achieve a noticeable accuracy.}

Table \ref{End-to-end-online} shows the end-to-end results on two devices. When compared to All-class EfficientNet, \myname{} has comparable or higher accuracy (5\% higher for the PLACES365 dataset) but offers substantial computational gains (latency speedup of $1.2-3.5\times$ for the Pi0 and $1.3-4.4\times$ for the GAP8). When compared to Highest FLOPs $\mu$Classifier, \myname{} has $1.4-3\%$ less accuracy but similar speedup as above. \myname{}'s performance is also very close to the Oracle $\mu$Classifier. Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 

We also evaluated how our end-to-end results change as the context change rates increase from 3\% to 9\% on the STL-10 and PLACES365 datasets. \myname{} maintains its advantage in terms of accuracy and latency even with higher context change rates. For example, on the Raspberry Pi Zero W, the latency increases by about 8-13\% and accuracy slightly decreases by about 1\%.

% Figure \ref{diff_context_change} shows how the end-to-end results change on the Raspberry Pi Zero W as the context change rates increase from 3\% to 9\%. The latency slowly increases from 88.9 to 100.6 and 297 to 316.4 milliseconds for the STL-10 and PLACES365 datasets respectively. Also, accuracy slightly decreases from 93.6 to 92.7 and 96 to 94.9 for the STL-10 and PLACES365 datasets respectively. Overall, \myname{} keeps its advantage in terms of accuracy and latency even with higher context change rates.

% On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

% When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less accuracy but $2.6\times$ speedup, and c) For the STL-10 dataset, 
% \M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}

\mypara{Local inference:} 
This section evaluates the performance of local inference when All-Class EfficientNet is executed on the local device. The main difference is the use of a greedy selection method that selects classifiers that achieve coverage over all classes of interest while also having high accuracy and low FLOPs. 

We compare our greedy selection method against Coverage-based selection which uses the kNN for selecting the best configuration for all $\mu$Classifiers but randomly selects among these with only coverage as the constraint. We show results for the Camera Trap dataset as this dataset is more challenging; trends are similar for others.

Figure~\ref{fig:speedup_local} shows the end-to-end results with different numbers of stored $\mu$Classifiers (averages over 20 runs are reported). We see that on the Raspberry Pi Zero W platform, we have 1.25$\times$ -- 1.4$\times$ speedup over Coverage-based selection when the number of stored $\mu$Classifiers increases from 10 to 50 (trend on the GAP8 is similar).

Figure~\ref{fig:acc_local} shows the end-to-end accuracy with respect to the different numbers of $\mu$Classifiers (picked by the Greedy selector) on the device. Even with only 10 $\mu$Classifiers i.e. 8.3\% of all $C^{10}_3$ 3-class subsets, we see that the accuracy drop is only 0.3\% but we have 3$\times$ speedup in latency.  

% Overall, We can achieve marginally higher accuracy (0.4\%) than Random selection as well, but the main advantage is in the selection of low-cost $\mu$Classifiers. Results follow a similar trend for the GAP8.

% Table \ref{local_end-to-end} shows that the accuracy increases as we store more $\mu$Classifiers on the device. Also, only 40 $\mu$Classifiers are needed to be stored on the device to achieve the same accuracy as the All-Class EfficientNet (Table \ref{End-to-end-online}) while we still gain 3$\times$ speedup.

% On the Raspberry Pi Zero-W platform, the latency slightly increases by selecting more $\mu$Classifiers. The reason is that the computation cost of the selected $\mu$Classifiers slightly increase as we expand the number of picked $\mu$Classifiers. For instance, it is expected that any other $\mu$Classifier have a higher computation cost than the chosen 20 $\mu$Classifiers as the greedy selector aims to pick the lightest $\mu$Classifiers. Although storing a high number of $\mu$Classifiers helps the device to lower the number of execution of the all-class model, it doesn't necessarily lead to lower latency in comparison to storing a small number of $\mu$Classifiers. It is due to the fact that the computation cost of the selected $\mu$Classifiers dominates the latency. In case we employ a more complex model like ResNet50 as the all-class model on the device, its computation cost may dominate the computation cost of the $\mu$Classifiers.


% \mypara{Case study: Trail camera} We implemented an end-to-end use case of \myname{} inference pipeline for detecting animals observed by a trail camera for the Raspberry Pi Zero W. This is a common use-case for low-power IoT platforms which wakeup upon detecting that there is movement in the scene. The video in \cite{} shows an example where we use the Camera Trap datasets \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} as input and locally store 40 $\mu$Classifiers for switching.

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}








% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}


% \subsection{Case study: Trail camera} 

% We briefly provide some end-to-end memory benchmarks from an end-to-end implementation. In order to better visualize how the \myname{} pipeline works, we built a demo on the Raspberry Pi 4B running at $1$ GHz. The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows a working end-to-end system.

% In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 
% We resize the captured images into $4$ different sizes: $100$, $160$, $240$, $320$ depending on configuration parameters and use the corresponding feature extractors and $\mu$Classifiers to generate the classification results and regression results. 

% For the regression results, we use a threshold of $0.6$ to trigger the context change. When the regression results are smaller than $0.6$, we consider the current context might not be appropriate anymore and trigger the full model to do the inference again. The full model is latency-heavy on the Raspberry Pi 4B which will cost more than $600$ ms. The all-class model uses the image of the size $320$ as input and will generate the classification results of $11$ classes. Based on the classification results, we will find the most proper context. We find the new combinations of 3-class in a First-In-First-Out(\textbf{FIFO}) manner by removing the oldest classes and adding the latest predicted classes. If the new combination has no valid $\mu$Classifiers, we will iteratively remove the second and third oldest classes instead of the first one. If there is no valid combination using the heuristic, we will randomly sample one valid combination containing the predicted class. 

% When the regression results are larger than the threshold, we will remain on the current context and accept the predicted $3$-class results. Overall, we find out that we could achieve $82\%$ accuracy and $16\%$ rate of triggering the all-class models.

\mypara{Case study: Trail camera.} While resource usage depends on the number of models and configurations, we provide end-to-end memory benchmarks for one implementation instance on the Raspberry Pi 4B running at $1$ GHz. The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. A video\footnote{\url{https://anonymous.4open.science/r/ZIGZAG-F7E0/README.md}} is provided to show a working end-to-end system.

In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint of the models is $28$ MB and that of the feature extractors and all-class model is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 


==> Backup/Jun24/Similarity-0.tex <==
\section{Inter-class Similarity}

The first question we ask is whether the selection of which set of  classes are chosen in a $\mu Classifier$ carries significance from a resource optimization perspective? In other words, are some groups of classes more compressible than others when subjected to various model compression techniques such as pruning, quantization, or early exiting?

% \subsection{Choice of context matters}

% \DG{Is there a generic way to validate this without specifically describing our approach?}

% Indeed, we show that selection of classes within a $\mu$Classifier is of paramount importance, as different groups of three classes can exhibit different levels of compressibility when subjected to various model compression techniques such as pruning, quantization, or early exiting. \DG{correct?} \M{True} 

Indeed, we show that selection of classes within a $\mu$Classifier can dramatically impact compressibility. Intuitively, this can be understood by considering the inherent characteristics of the classes in question.

Imagine that the classes are representative of different animals that might be captured by a trail camera. When the classes consist of animals with similar features, textures, or behaviors, the classifier faces a more challenging task in distinguishing between them. For instance, if the three classes represent a deer, an elk, and a moose, the classifier has to contend with the fact that all three animals have somewhat similar body shapes, sizes, and features. Consequently, the model may need to employ more computational resources to scrutinize subtle distinctions and achieve a comparable level of accuracy.

In contrast, if the classes are composed of animals that are markedly disparate in features, they are more easily distinguishable, and the classifier can make decisions with less computational effort. For example, consider a group comprising a deer, a rabbit and a racoon. These animals are drastically different in size, appearance, and behavior, making them easier to classify with higher confidence.

In essence, the inter-class similarities or differences play a significant role in determining the computational resources needed by the $\mu$Classifier. When designing a context-aware system, careful consideration should be given to the grouping of classes, taking into account the inherent characteristics of the data to optimize performance and resource utilization.

% For example, we could contemplate several $\mu$Classifier designs. One approach, based on temporal co-occurrence, might be to simply load a $\mu$Classifier for the three most recently observed classes. On the other hand, a more meticulous design could involve selecting the three classes that yield the best performance based on certain criteria or metrics. The crux here lies in discerning whether there is a substantial performance difference between these options. We start by analyzing and comparing the efficacy of these designs to provide insights into the optimization of context-aware neural network models.

\subsection{Similarity metric}

How can we capture this intuition in a metric? Such a metric is necessary to quickly determine which $\mu Classifiers$ to select and what configuration to use to train it.

To achieve this, we define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities would also share a similar $\mu$Classifier configuration. 

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

We note that the above metric was chosen after careful consideration of several alternate measures of similarity. We show empirical results comparing these metrics in \S\ref{}.

\subsection{Similarity as proxy for compressibility} 

We now look at whether the similarity metric that we have defined captures the essential resource-accuracy tradeoffs in grouping classes into a $\mu Classifier$. 

Figure~\ref{heatmap} shows that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to the similarity among classes (darker $\implies$ higher accuracy). X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (constructed by varying model size and image resolutions) sorted from least to most compute complexity. We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models.}
    \label{heatmap}
\end{figure}

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.}
    \label{fig:kNN-training}
\end{figure}


==> Backup/Jun24/Similarity.tex <==
\section{Inter-class Similarity}

At the core of our configuration prediction method is a ``similarity'' metric that captures the similarity between the set of  classes chosen in a $\mu Classifier$ which in turn correlates with how much computational resources the model requires.

% \subsection{Choice of context matters}

% \DG{Is there a generic way to validate this without specifically describing our approach?}

% Indeed, we show that selection of classes within a $\mu$Classifier is of paramount importance, as different groups of three classes can exhibit different levels of compressibility when subjected to various model compression techniques such as pruning, quantization, or early exiting. \DG{correct?} \M{True} 

Intuitively, the manner in which similarity and resource needs relate can be understood by considering the inherent characteristics of the classes in question. Imagine that the classes are representative of different animals that might be captured by a trail camera. When the classes consist of animals with similar features, textures, or behaviors, the classifier faces a more challenging task in distinguishing between them. For instance, if the three classes represent a deer, an elk, and a moose, the classifier has to contend with the fact that all three animals have somewhat similar body shapes, sizes, and features. Consequently, the model may need to employ more computational resources to scrutinize subtle distinctions and achieve a comparable level of accuracy.

In contrast, if the classes are composed of animals that are markedly disparate in features, they are more easily distinguishable, and the classifier can make decisions with less computational effort. For example, consider a group comprising a deer, a rabbit and a racoon. These animals are drastically different in size, appearance, and behavior, making them easier to classify with higher confidence.

In essence, the inter-class similarities or differences play a significant role in determining the computational resources needed by the $\mu$Classifier. When designing a context-aware system, careful consideration should be given to the grouping of classes, taking into account the inherent characteristics of the data to optimize performance and resource utilization.

% For example, we could contemplate several $\mu$Classifier designs. One approach, based on temporal co-occurrence, might be to simply load a $\mu$Classifier for the three most recently observed classes. On the other hand, a more meticulous design could involve selecting the three classes that yield the best performance based on certain criteria or metrics. The crux here lies in discerning whether there is a substantial performance difference between these options. We start by analyzing and comparing the efficacy of these designs to provide insights into the optimization of context-aware neural network models.

\subsection{Similarity metric}

% How can we capture this intuition in a metric? Such a metric is necessary to quickly determine which $\mu Classifiers$ to select and what configuration to use to train it.

To capture this intuition, we define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities would also share a similar $\mu$Classifier configuration. 

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

We note that the above metric was chosen after consideration of several alternate measures of similarity. We show empirical results comparing these metrics in \S\ref{}.

\subsection{Similarity as proxy for compressibility} 

We now look at whether the similarity metric that we have defined captures the essential resource-accuracy tradeoffs in grouping classes into a $\mu Classifier$. 

Figure~\ref{heatmap} shows that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to the similarity among classes (darker $\implies$ higher accuracy). X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (constructed by varying model size and image resolutions) sorted from least to most compute complexity. We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models.}
    \label{heatmap}
\end{figure}

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.}
    \label{fig:kNN-training}
\end{figure}


==> Backup/Jun29/EValuation.tex <==
\section{Evaluation}
We first describe the experiment settings in \S~\ref{sec:settings}, and then evaluate the end-to-end system over three datasets and on real platforms  in \S~\ref{sec:end-to-end} and the components of \myname{} in \S~\ref{sec:predictor}-\ref{sec:selector}. 
We further perform ablation studies on context change frequency and scalability of the system in \S~\ref{sec:ablation} and implement a case study using camera trap application in \S\ref{sec:case-study} 



\subsection{Experiment Settings}
\label{sec:settings}

\begin{comment}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resolution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\end{comment}

\mypara{Dataset:}
\label{dataset}
We use three datasets. 
Our primary dataset is Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}, which has temporal data captured by trail cameras with real-world context changes. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images, each time in a sequence of three. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two snapshot projects, Enonkishu \cite{Camera_trap_enonkishu} and Camdeboo \cite{Camera_trap_camdeboo}, were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species were picked from the Snapshot Camdeboo dataset (both from cameras in the African savannah) to get a total of ten species. %The dataset has labels over 3-frame image sequences (i.e. the label would be for a species even if it is present in one of the frames), which leads to erroneous labels for several individual frames. Hence, accuracy is lower across all methods for this dataset.

Since there is a lack of labeled temporal datasets, we also evaluate on two other image datasets, STL-10 \cite{STL10}, and Places365 \cite{PLACES365}, from which we synthesize temporal sequences.
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 
% 
PLACES365 is intended for visual understanding tasks such as scene context, object recognition, and action prediction. 
% It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 40 scene categories, each with 1200 samples with a size of 256$\times$256. Most of our results are shown for 20 scene categories but we evaluate scalability of \myname{} for 40 classes.


% Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10 species classes + 1 empty class to be close to the real-world setting. As mentioned, Camera Trap images form a sequence of 3 frames and the labels in each sequence are the same. However, sometimes one or more frames in the sequence do not show any species in the scene as they have left the scene. Hence, those frames are wrongly labeled as that species. It leads to non-accurate labels which lower the accuracy of the classification task.}

Since the space of $\mu$Classifier configurations is very large, we take a deeper dive into 3-class $\mu$Classifiers. This represents an extreme point with $\mu$Classifiers with highest compressibility but also requires the most switching between contexts. 
So, it helps us evaluate the upper limits of how a nimble context-aware system can be designed with $\mu$Classifiers. 
%By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. %Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

% \mypara{Inter-class similarity metric:}
% The configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
% We used the feature extractor of ResNet-50 to extract the embedding of images from a class and average the embeddings into a single vector to be used for computing the inter-class similarities. 


% \mypara{The configuration space of $\mu$Classifiers:}
% The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
% We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
% We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that besides the EfficientNet-B0 we get a total of four feature extractor architectures.  
% %The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The range of image resolutions is considered 100-320, 58-96, and 130-256 for Camera Trap, STL-10, and PLACES datasets respectively. For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
% A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
% The two heads use two Fully Connected layers. Feature extractors are fine-tuned once on all classes, and then frozen during the training of the two heads of $\mu$Classifiers.

\mypara{KNN-based configuration predictor:}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that besides the EfficientNet-B0 we get a total of four feature extractor architectures.  
%The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The range of image resolutions is considered 100-320, 58-96, and 130-256 for Camera Trap, STL-10, and PLACES datasets respectively. For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
The two heads use two Fully Connected layers. Feature extractors are fine-tuned once on all classes, and then frozen during the training of the two heads of $\mu$Classifiers.

To calculate the context representation of every 3-class combination, 
We used the feature extractor of ResNet-50 to extract the embedding of images from a class and average the embeddings into a single vector to be used for computing inter-class similarity metric. We then calculate context representation as Eq.~\ref{eq:rep_vector}.


To build the training data for the configuration predictor, we applied similarity-directed sampling (detailed in \S\ref{sec:knn}) to use only 5\% of the 3-class combinations when we have 40 classes in total, 7\% of the combinations for 30-classes, 17\% of combinations for 20-classes, and 33\% combinations for 10 classes.
% 500 3-class combination samples from 9880 combinations ($C^{40}_3$) in the PLACES (40 class) dataset, 
% 300 out of 4060 combinations ($C^{30}_3$) for the PLACES (30 class), 
% 200 out of 1140 combinations ($C^{20}_3$) for the PLACES (20 class), 
% and 40 out of 120 combinations ($C^{10}_3$) for the STL-10, Camera Trap, and PLACES (10 class) datasets. 
For each sampled 3-class combination, we train $\mu$Classifiers with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 
The thresholds are 93$\%$, 97$\%$, and 92$\%$ for STL-10, PLACES, and Camera Trap datasets respectively.

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
KNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority, it considers 4 nearest neighbors and so on until a majority is achieved.


\mypara{Context-aware switching:} 
As discussed in \S\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect the context change. 
It is trained to output a value close to 0 for the target classes of the $\mu$Classifier and a value around 1 for other classes. 
We used $0.5$ for all three datasets.
Once context change is detected, we execute an all-class model (ResNet-50 for in the cloud offload cases and uses EfficientNet-B0 in the on-device case) to identify which new class occurs in the scene. All-class models are pre-trained on ImageNet and fine-tuned on the target dataset.

\mypara{Implementation:}
% \mypara{IoT processors:} 
We implement the \myname{} pipeline on three different IoT devices --- Raspberry Pi 4B, Raspberry Pi Zero W, and GAP8. We generate \textbf{TensorFlow Lite} models using the default optimization and int-8 quantization to reduce the model size and execution latency. On all the platforms, we profile the execution latency of models of different configurations on different datasets.
% 
For profiling on Raspberry Pi 4B and Zero W, we utilize the \textbf{TVM} framework \cite{TVM} to tune the operator implementations to reduce the execution latency for the Arm Cores. 
% 
For profiling on GAP8, we use the GAP8 tool chain \cite{URL:GAP8_tool} to transform the \textbf{TensorFlow Lite} models into C code by fusing the operations. 
% 
% \mypara{Training:} 
An NVIDIA Tesla M40 24GB GPU was used for training models and as the edge-cloud in some of our experiments. 
% 
% \mypara{Open source code:} 
If accepted, we will make our code on all the above platforms openly available.

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.

\subsection{End-to-End Evaluation}
\label{sec:end-to-end}





\begin{table*}[t]
% \scalebox{0.55}{
\footnotesize 
\tabcolsep=0.2cm 
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES20}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) \\
%   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) \\ 
  \midrule
All-Class Model & 82.0\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 92.1\% & 107.9 (1.0$\times$)& 124.5 (1.0$\times$)& 90.5\% & 521.1 (1.0$\times$)& 1162.1 (1.0$\times$) \\
All-Class-Early Exit & 81.0\% & 450.0 (1.9$\times$) & 916.6 (2.0$\times$) & 91.9\% & 100.1 (1.1$\times$)& 108.9 (1.1$\times$)& 90.1\% & 417.2 (1.2$\times$)& 883.2 (1.3$\times$)\\
All-Class-Pruned & 76.2\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 84.3\% & 89.0 (1.2$\times$)& 95.5 (1.3$\times$)& 84.9\% & 377.7 (1.4$\times$)& 587.1 (2.0$\times$)\\
FAST \cite{FAST} & 82.9\% & 801.6 (1.0$\times$) & 1730.4 (1.0$\times$)& 92.5\% & 108.9 (1.0$\times$)& 124.4 (1.0$\times$)& 91.0\% & 501.6 (1.0$\times$)& 1091.7 (1.0$\times$)\\
PALLEON \cite{palleon} & 83.8\% & 767.3 (1.1$\times$) & 1656.5 (1.1$\times$) & 92.4\% & 103.8 (1.0$\times$)& 118.1 (1.0$\times$)& 92.2\% & 483.7 (1.0$\times$)& 1051.2 (1.1$\times$)\\
\myname{} (Highest FLOPs) & 91.4\% & 842.6 (1.0$\times$) & 1854.7 (1.0$\times$) & 95.9\% & 120.7 (0.9$\times$)& 137.6 (0.9$\times$)& 96.8\% & 534.4 (1.0$\times$)& 1168.4 (1.0$\times$)\\
\myname{} (Oracle) & 88.8\% & 227.8 (2.3$\times$) & 355.4 (5.1$\times$)& 93.8\% & 90.6 (1.2$\times$)& 96.2 (1.3$\times$)& 95.7\% & 292.6 (1.8$\times$)& 511.6 (2.3$\times$)\\
\myname{} & 88.5\% & 229.1 (3.6$\times$) & 382.0 (4.8$\times$)& 93.5\% & 88.9 (1.2$\times$)& 94.1 (1.3$\times$)& 95.2\% & 291.0 (1.8$\times$)& 512.4 (2.2$\times$)\\
\bottomrule 
\end{tabular}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context changes every 30 frames on average. Note that Speedup values are rounded.}
\label{End-to-end-online}
\vspace{-0.2in}
\end{table*}


This section looks at an edge-cloud assisted system (the unattended setting is examined in \S~\ref{sec:selector}).
To evaluate the end-to-end performance of \myname{}, we need datasets that have context changes. The Camera Trap dataset provides us with a real-world temporal flow with context changes but other datasets are not temporal. 
Hence, we sequence test sets from the Places and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. 

Specifically, we find that the context interval is 30 frames on average (context changes in every 30 frames) for the Camera Trap dataset when considering 3-class $\mu$Classifiers. We use this to synthesize a test set with context interval of 30 frames for the PLACES and STL-10 datasets and use this in our evaluation unless noted differently.
To generate a test set with temporal flow, we randomly construct a sequence of 3-class combinations, where every two consecutive combinations show a context change of a single class. To match the context interval of 30 frames, we persist the current context for 30 frames by picking random samples from the current context. 
In \S~\ref{sec:ablation}, we further study the effects of different context change rate in the performance of \myname{}.




We compare the classification accuracy and overall latency of \myname{} against the following baselines: 
(a) \textbf{FAST} \cite{FAST}, a context aware approach which assumes the class skews are known offline and trains compact models for each class skew. During inference it detects the class skew using a window-based detector and loads the corresponding model, (b) \textbf{PALLEON} \cite{palleon}, a state-of-the-art video processing framework which applies a bayesian filter to adapt the model to the context. The bayesian filter is determined by applying an all-class model on a window of frames.
(c) \textbf{All-Class Model}, which uses the well-trained EfficientNet-B0 with all the classes and full image resolution. 
(d) \textbf{All-Class-Early Exit}, which is the early exit variant (exit heads in stages 4 and 6)  of the All-Class Model.
(e) \textbf{All-Class-Pruned}, where we apply 30$\%$ pruning rate to the all-class model. We choose 30\% since it gives the best accuracy and efficiency trade-offs. 
(f) \myname{} \textbf{(Highest FLOPs)}, which uses the $\mu$Classifier that has same classes as \myname{} predicts but uses full image resolution and no pruning (and hence computationally the most expensive).
(g) \myname{} \textbf{(Oracle)} i.e. the $\mu$Classifier that meets the target accuracy threshold with minimum FLOPs (which would be selected by an omniscient scheme rather than the kNN-based method we use). 
We note that training the Oracle is not scalable --- it takes a total of 120, 40, and 300 hours longer than our approach for the Camera Trap, STL-10 and PLACES20 respectively.


Table~\ref{End-to-end-online} shows the end-to-end results on two devices. The IoT device communicates via WiFi with data rate of $10$ Mbps. 
The reported latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices. We assumed no $\mu$Classifiers are cached on the device which is the \emph{worst-case scenario} as it requires more transmission and increases the overall latency. We report average latencies over the test set. 


Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 
When compared to All-Class Model, 
\myname{} has comparable or higher accuracy (6.5\% higher for the Camera Trap dataset) but offers substantial computational gains (latency speedup of $1.2-3.6\times$ for the Pi0 and $1.3-4.8\times$ for the GAP8). 
When compared to Highest FLOPs $\mu$Classifier, \myname{} has $1.6-2.9\%$ less accuracy but similar speedup as above.
\myname{}'s performance is also very close to the Oracle $\mu$Classifier. 

\myname{} outperforms two other context-agnostic baselines, All-Class-Early Exit, and All-Class-Pruned, in terms of both accuracy and latency due to the leverage of context awareness to improve efficiency. 
Compared to two existing context-aware approaches FAST~\cite{FAST} and PALLEON~\cite{palleon}, \myname{} has $1-5.6\%$ and $1.1-4.7\%$ higher accuracy respectively with higher speedups. FAST and PALLEON needs to execute all-class model for n (more than 10) frames after detecting a context change to determine the class distribution of the new context. Thus, they provide speedups only if the context change is very sparse. 
% Hence, before they can determine the class distribution of the current context, context changes and they need to repeat the execution of all-class model. 
For this reason, they could not provide a speedup over 1.1$\times$ which is significantly lower than \myname{}.


% Overall, We can achieve marginally higher accuracy (0.4\%) than Random selection as well, but the main advantage is in the selection of low-cost $\mu$Classifiers. Results follow a similar trend for the GAP8.

% Table \ref{local_end-to-end} shows that the accuracy increases as we store more $\mu$Classifiers on the device. Also, only 40 $\mu$Classifiers are needed to be stored on the device to achieve the same accuracy as the All-Class EfficientNet (Table \ref{End-to-end-online}) while we still gain 3$\times$ speedup.

% On the Raspberry Pi Zero-W platform, the latency slightly increases by selecting more $\mu$Classifiers. The reason is that the computation cost of the selected $\mu$Classifiers slightly increase as we expand the number of picked $\mu$Classifiers. For instance, it is expected that any other $\mu$Classifier have a higher computation cost than the chosen 20 $\mu$Classifiers as the greedy selector aims to pick the lightest $\mu$Classifiers. Although storing a high number of $\mu$Classifiers helps the device to lower the number of execution of the all-class model, it doesn't necessarily lead to lower latency in comparison to storing a small number of $\mu$Classifiers. It is due to the fact that the computation cost of the selected $\mu$Classifiers dominates the latency. In case we employ a more complex model like ResNet50 as the all-class model on the device, its computation cost may dominate the computation cost of the $\mu$Classifiers.


% \mypara{Case study: Trail camera} We implemented an end-to-end use case of \myname{} inference pipeline for detecting animals observed by a trail camera for the Raspberry Pi Zero W. This is a common use-case for low-power IoT platforms which wakeup upon detecting that there is movement in the scene. The video in \cite{} shows an example where we use the Camera Trap datasets \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} as input and locally store 40 $\mu$Classifiers for switching.

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}








% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}


% \subsection{Case study: Trail camera} 

% We briefly provide some end-to-end memory benchmarks from an end-to-end implementation. In order to better visualize how the \myname{} pipeline works, we built a demo on the Raspberry Pi 4B running at $1$ GHz. The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows a working end-to-end system.

% In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 
% We resize the captured images into $4$ different sizes: $100$, $160$, $240$, $320$ depending on configuration parameters and use the corresponding feature extractors and $\mu$Classifiers to generate the classification results and regression results. 

% For the regression results, we use a threshold of $0.6$ to trigger the context change. When the regression results are smaller than $0.6$, we consider the current context might not be appropriate anymore and trigger the full model to do the inference again. The full model is latency-heavy on the Raspberry Pi 4B which will cost more than $600$ ms. The all-class model uses the image of the size $320$ as input and will generate the classification results of $11$ classes. Based on the classification results, we will find the most proper context. We find the new combinations of 3-class in a First-In-First-Out(\textbf{FIFO}) manner by removing the oldest classes and adding the latest predicted classes. If the new combination has no valid $\mu$Classifiers, we will iteratively remove the second and third oldest classes instead of the first one. If there is no valid combination using the heuristic, we will randomly sample one valid combination containing the predicted class. 

% When the regression results are larger than the threshold, we will remain on the current context and accept the predicted $3$-class results. Overall, we find out that we could achieve $82\%$ accuracy and $16\%$ rate of triggering the all-class models.

\subsection{Performance of Config Predictor}
\label{sec:predictor}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}

We now look at the performance of the $\mu$Classifier \textit{Configuration Predictor}. 
We vary the target accuracy threshold from the lowest to the highest of all the trained $\mu$Classifiers to show how the threshold affects the performance of the configuration predictor. 
A lower target accuracy will result in lighter $\mu$Classifiers and thus less FLOPs. 



\begin{figure}[h]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.24\textwidth]{figures/camera_k_nn_performance.png}}}%
    % \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % % \qquad
    \subfloat[\centering PLACES\label{fig:Places_roc}]{{\includegraphics[width=.24\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance of configuration predictor with different accuracy thresholds. The orange curve aligns well with the oracle, indicating that the kNN together with the inter-class similarity metric works well in selecting the best configuration. }
\label{knn_performance}
\end{figure}

Figure~\ref{knn_performance} shows how different target accuracy thresholds affect the classification accuracy and the computation costs for our methods and baselines. We omit the result on the STL-10 dataset for limited space. 
% We sweep over target accuracy thresholds for the curves but the dotted horizontal line shows a specific choice of target accuracy that we use in the rest of this paper (chosen as described in \S\ref{experiment_setting}). 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   
% 
Overall, we see that \myname{} can cover a wide trade-off region between accuracy and computational cost --- accuracies vary by 3.5-8.8\% and compute by 3.9$\times$ to 13$\times$. Across the range, the accuracy is nearly as good as the \myname{} (Oracle), indicating that \textit{the kNN together with the inter-class similarity metric works well in selecting the best configuration. }
In contrast, All-Class Model (red star) and \myname{} (Highest FLOPs) (green star) are point solutions. 
Note that, \myname{} (Highest FLOPs) outperforms the accuracy of the All-Class Model by a large margin even though both models have the same FLOPs. The accuracy benefits comes from the fact that \myname{} narrows down a prediction task to contexts, echoing the observations in \S~\ref{sec:motivations}.  

% Although All-Class-Pruned and All-Class-Early-Exit can result in accuracy-efficiency trade-offs, the models achieve less accuracy given the same FLOPs budget. We note that the comparison favors All-Class-Pruned and All-Class-Early-Exit because pruning and early exits can also be applied to the $\mu$Classifier on \myname{}, as demonstrated in Section~\ref{sec:motivations}.
% \HG{after the data is updated, might update the description to be more quantitative.}


% We compare these models against a specific instance of \myname{}, i.e. the point where the dotted line intersects the \myname{} curve (orange) based on the threshold we choose. 
% This configuration of \myname{} is 0.8-10\% more accurate than All-Class EfficientNet and requires $53\%$ to $75\%$ less computation to hit the target accuracy. 
% When comparing against \myname{} (Highest FLOPs), we see that \myname{} achieves 53-75\% computation savings while sacrificing 1.5-4.3\% classification accuracy. 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

% We now compare \myname{} against {all-class EfficientNet} (red star). \myname{} is between 5.1\% -- 12.3\% more accurate and requires 53\% to $74.79\%$ less computation to hit the target accuracy (horizontal dotted line).

% When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
% For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_vs_sim_eval}]{{\includegraphics[width=.24\textwidth]{figures/Accuracy_Vs_Similarity.png}}}%
    \subfloat[\centering \label{fig:comp_gain_Vs_Similarity}]{{\includegraphics[width=.235\textwidth]{figures/comp_gain_Vs_Similarity.png}}}%
    \caption{(a) The accuracy of a representative configuration correlates well with the inter-class similarity. 
    (b) The computational complexity of the predicted $\mu$Classifiers correlates well with the inter-class similarity. 
    % We see that both accuracy and computation savings (over All-Class Model) correlates well with our proposed inter-class similarity metric, indicating that the similarity metric closely mirrors the actual difficulty level of contexts. 
    Similarity is normalized to [0, 1] in both figures.}
    \vspace{-0.2in}
% \label{}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.25\textwidth]{figures/Accuracy_Vs_Similarity.png}
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
%     \label{acc_vs_sim_eval}
% \end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/comp_gain_Vs_Similarity.png}
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
%     \label{speedup_vs_sim_eval}
% \end{figure}
% \HG{since the configuration predictor is fundamentally a classification problem. Should we report the classification accuracy as well? } \M{Accuracy of kNN won't be impressive as it is not necessarily good on predicting the exact config, most of the time it predicts a configuration which is computationally and accuracy wise close to the ground truth}

\mypara{Effectiveness of the inter-class similarity metric:}
The good predictive performance of the configuration predictor results from the effectiveness of the inter-class similarity metric in capturing difficulty level of contexts. 

% We now examine the effectiveness of the proposed inter-class similarity metric. 

Figure~\ref{fig:acc_vs_sim_eval} illustrates how the accuracy of a representative $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
% 
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.86-0.97$), indicating that \textit{our similarity metric closely mirrors the difficulty level of 3-class combinations.  }

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure~\ref{fig:comp_gain_Vs_Similarity} looks at this relation from another performance dimension --- computation savings. 
% The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-class similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class Model/\myname{} (Highest FLOPs) and the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the similarity-aware kNN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{figure}[h]
    \centering
\includegraphics[width=0.4\textwidth]{figures/diff_sim_metric.png}
    \caption{Accuracy difference of predicted $\mu$Cs by kNN from oracle $\mu$Cs using different similarity metrics (Oracle-Predicted)}
    \label{fig:Diff_Sim_Metric}
    \vspace{-0.1in}
\end{figure}

\mypara{Comparison with other similarity metrics:}
We also investigate alternative similarity metrics and context representations including (1) confusion matrix-based similarity and (2) maximum and minimum of pair-wise similarities in a combination. 
For computing the pair-wise similarity using confusion matrix, the number of samples that two classes are misclassified as another are summed and normalized as the percentage by the total number of those two classes.
Figure~\ref{fig:Diff_Sim_Metric} shows the comparison using the Camera Trap dataset. Each bar reflects the averaged accuracy difference between predicted $\mu$Classifiers and oracle $\mu$Classifiers over all 3-class combinations for each similarity metric. We see KNN using our similarity metric (mean,std) provides more accurate predictions in comparison to confusion matrix-based similarity metric over all three datasets. 
%KNN with our inter-class similarity metric but using maximum and minimum as context representations has a poor performance on Camera Trap dataset as the accuracy of its predictions are on average 2.5\% lower than the oracle.






\subsection{Perf. of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
% An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. 
A false positive (FP) that wrongly predicts a context change would introduce additional cost whereas a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot detect the context change. 
To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.


\begin{table}[htb]
\footnotesize 
\tabcolsep=0.05cm
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
$\mu$C+regression (ours) & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
$\mu$C+maximum prob~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\  
Oracle $\mu$C+regression & 13.11\% & 13.26\% & 13.83\% & 11.15\% & 8.57\% & 7.64\% \\
Highest FLOPs $\mu$C+regression & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\ 
\bottomrule
\end{tabular}
% }
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\vspace{-0.2in}
\end{table}


Table~\ref{fpfnt} compares the context-change detection performance of \myname{} (``$\mu$C + regression'') against baselines: 
(a) the same $\mu$Classifier as \myname{} but with a different approach for context change detection based on maximum probability \cite{maxsoft1}.
(b) the \myname{} (Oracle) $\mu$Classifier with regression head (``Oracle $\mu$C + regression''). 
(c) the \myname{} (Highest FLOPs) with regression head (``Highest FLOPs $\mu$C + regression'') as a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.

\myname{}'s use of a regression head is much more accurate compared to the baseline that uses the maximum probability. 
The FP and FN rates of our approach are $10-20\%$ lower than the baseline. 
\myname{} is quite close to the Oracle $\mu$Classifer as well. 
There is a gap in performance between \myname{} and \myname{} \textbf{(Highest FLOPs)} (2-4\% for Camera Trap and PLACES, and 6-7\% for STL-10) but this is to be expected since we are operating with a lower target accuracy, and have considerable computational gains.
These values can be further lowered by increasing the $Acc_{thr}$ explained in \S\ref{sec:budget} as it directly affects the predicted configuration and therefore FP and FN rates. 

\begin{table}[t]
\begin{tabular}{@{}l|lcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{5}{c}{Context Interval} \\
 & 10 & 15 & 20 & 30 & 60\\ \midrule
Accuracy Gain & 3.7\%& 4.3\%& 4.4\%& 4.7\%& 5.2\% \\
SpeedUp &2.13$\times$& 2.16$\times$& 2.21$\times$& 2.26$\times$& 2.28$\times$\\ 
\bottomrule
\end{tabular}
\caption{\myname{} accuracy gain and speedup for the GAP8 with different number of context interval in comparison to All-Class Model on PLACES dataset.}
\label{diff_context}
\vspace{-0.2in}
\end{table}


\begin{table}[t]
\begin{tabular}{@{}l|lcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c}{Number of Classes} \\
 & 10 & 20 & 30 & 40 \\ \midrule
Accuracy Gain & 4.4\%& 4.7\%& 4.3\%& 4.6\% \\
SpeedUp &2.33$\times$& 2.26$\times$& 2.18$\times$& 2.10$\times$\\ 
\bottomrule
\end{tabular}
\caption{Effect of scaling the number of covered classes on \myname{} performance (PLACES dataset). Accuracy gain and speedup are reported.}
\label{scalability}
\vspace{-0.2in}
\end{table}

% \begin{table*}[t]
% %\scalebox{1}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% & \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c|}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8\\ 
%   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}
%     &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c}{(ms)}\\ 
%   \midrule
% Greedy Selection & 80.92\% & 266.76 & - & 81.55\% & 267.41 & - & 81.65\% & 288.84 & - & 81.97\% & 305.16 & -\\
% Random Selection & 81.30\% & 352.60 & - & 81.22\% & 369.33 & - & 81.31\% & 357.06 & - & 81.53\% & 369.34 & - \\

% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}
% \caption{End-To-End performance of Local inference; $3\%$ Context change rate}
% \label{local_end-to-end}
% \end{table*}


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_local}]{{\includegraphics[width=.235\textwidth]{figures/acc_local.png}}}%    
    \subfloat[\centering \label{fig:late_local}]{{\includegraphics[width=.24\textwidth]{figures/late_local.png}}}%
    \caption{End-to-End performance of local inference setting using Greedy $\mu$C selector and Top-K most frequent contex ($\mu$C) selector. (a) Classification accuracy and (b) Latency (on Rasp. Pi0; GAP8 results are similar) for different number of stored $\mu$C}
    \vspace{-0.2in}
% \label{}
\end{figure}

\subsection{Perf. of Greedy Selector} 
\label{sec:selector}
This section evaluates the performance of local inference. This scenario assumes communication/cloud is not available and the IoT have to rely on a set of $\mu$Classifiers. As a result, For switching between $\mu$Classifiers, the all-class model should be deployed on the device and we choose All-Class EfficientNet for this purpose (ResNet-50 is heavy for target processors). However, The main difference is the use of a greedy selection method that selects $\mu$classifiers that achieve coverage over all classes of interest while also having high accuracy and low FLOPs. 

We compare our greedy selection method against Top-K most frequent $\mu$Classifiers (contexts). The later scheme assumes we have prior information about the distribution of contexts. Both schemes aim to decrease the computation overhead but with different approach. Greedy selector tries pick the most efficient $\mu$Classifiers (context) and finally in its second stage, it makes sure the target accuracy of threshold is met by chosen $\mu$Classifiers. On the other hand, Top-K selector tries to pick the most frequent contexts and store the corresponding $\mu$Classifiers in order to minimize triggering the All-Class Model which impose high computation cost. We show results for the Camera Trap dataset as this dataset have temporal flow (30 frames context interval).

Figure~\ref{fig:late_local} shows the end-to-end latency with different numbers (K) of stored $\mu$Classifiers (averages over 20 runs are reported). We see that on the Raspberry Pi Zero W platform, we have 1.28$\times$ -- 1.42$\times$ speedup over Top-K scheme when the number of stored $\mu$Classifiers increases from 10 to 50 (trend on the GAP8 is similar). Results show that the greedy selection of $\mu$Classifiers (context) is more effective than reducing the cost of triggering all-class model even on such a short context interval dataset. 

Figure~\ref{fig:acc_local} shows the end-to-end accuracy with respect to the different numbers of $\mu$Classifiers (picked by the Greedy selector) on the device. Even with only 10 $\mu$Classifiers i.e. 8.3\% of all $C^{10}_3$ 3-class subsets, we see that the accuracy drop is only 0.3\% but we have 3$\times$ speedup in latency.  




\subsection{Ablation Study}
\label{sec:ablation}
\mypara{Effect of context change rate:}
We also evaluated how our end-to-end results change as the interval between context changes varies from every 60 frames to 10 frames on the GAP8 platform and the PLACES dataset. Table \ref{diff_context} shows that \myname{} maintains its advantage even with higher context change rates i.e. shorter context intervals. The speedup decreases slightly from 2.28$\times$ to 2.13$\times$ and accuracy gain decreases from 5.2$\%$ to 3.7$\%$ as the interval becomes smaller but \myname{} is still considerably better.

\mypara{Scalability:}
We now look at the scalability of \myname{} with increasing number of classes. Generally, the performance of any approach drops as the number of classes increases. More classes make the classification task more complex. Table \ref{scalability} shows how \myname{} end-to-end performance changes relative to the all-class model as the reference. We see \myname{}'s accuracy gain over the All-Class Model remains the same which shows \myname{} maintains its advantage in terms of accuracy as the classification task scales up to more classes. Speedup drops slightly from 2.3$\times$ to 2.1$\times$ since the accuracy of the all-class model decreases with increasing number of classes and this leads to more context switches which increases overhead. We expect this gap can be narrowed by using a more powerful all-class model.


% The reason behind this negligible drop is that the accuracy all-class model on the cloud side decreases with the increase of number of classes and whenever the IoT detects the context change, the cloud all-class model may not be able to predict the correct class and provides a wrong $\mu$Classifier, and finally it dictates to more transmission overhead. A more powerful all-class model on the cloud can solve the issue. 

% Figure \ref{diff_context_change} shows how the end-to-end results change on the Raspberry Pi Zero W as the context change rates increase from 3\% to 9\%. The latency slowly increases from 88.9 to 100.6 and 297 to 316.4 milliseconds for the STL-10 and PLACES365 datasets respectively. Also, accuracy slightly decreases from 93.6 to 92.7 and 96 to 94.9 for the STL-10 and PLACES365 datasets respectively. Overall, \myname{} keeps its advantage in terms of accuracy and latency even with higher context change rates.

% On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

% When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less accuracy but $2.6\times$ speedup, and c) For the STL-10 dataset, 
% \M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}


\subsection{Case study: Trail camera}
\label{sec:case-study}
We also provide an end-to-end implementation of a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time on the Raspberry Pi 4B. A video\footnote{\url{https://anonymous.4open.science/r/ZIGZAG-F7E0/README.md}} is provided to show a working end-to-end system.

In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint of the models is $28$ MB and that of the feature extractors and all-class model is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 


==> Backup/June20/CAse.tex <==
\section{Case for Context-aware $\mu$Classifiers}
\label{case_context}
In this section, we make the case for \myname{} by comparing two designs for squeezing classifiers on IoT devices ---  the canonical method of training and compressing an \textit{all-class model} and our approach of using a \textit{context-aware $\mu$Classifier} and switching between them when the context changes.
% , and also trained to detect changes in context. 
% If a context change event is detected, then a new $\mu$Classifier that is relevant to the new context is loaded. 
% We show that there is a significant performance gap between these two approaches, and this argues for a deeper dive into the design space of switchable $\mu$Classifiers.

\mypara{Observation 1: Using fewer classes has significant performance benefits.} Intuitively, if a classifier has fewer classes than another, it should be more accurate given the same resources. But how much is this gain in accuracy?

% The first question that we ask is whether this gap is significant enough to argue for a $\mu$Classifier based design.

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Fewer classes is better\label{fig:accuracy_vs_classes}]{{\includegraphics[width=.32\textwidth]{figures/Acc_vs_Classes.png}}}%
    \subfloat[\centering Pruning does not reduce gap (STL-10) \label{fig:accuracy_vs_size}]{{\includegraphics[width=.335\textwidth]{figures/STL_All_Config_V3.png}}}%
    % \qquad
    \subfloat[\centering Early exit does not reduce gap \label{fig:early_exit accuracy_vs_size}]{{\includegraphics[width=.32\textwidth]{figures/Early_Exit_Acc_Vs_Classes.png}}}%
    \caption{Context-aware $\mu$Classifiers can provide substantial performance advantages. (a)  shows that accuracy drop is substantial as \#classes increases; (b) shows that model compression expands this gap further and (c) shows a similar trend for early-exit models.}
\label{knn_performance}
\end{figure*}

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/Acc_vs_Classes.png}
%     \caption{Accuracy drops as number of classes increases}
%     \label{fig:accuracy_vs_classes}
% \end{figure}


To answer this, we look at the accuracy of the EfficientNet-B0 on different subsets of classes from STL-10 \cite{STL10} and Camera Trap dataset~\cite{Camera_trap_enonkishu,Camera_trap_camdeboo} (See \S\ref{experiment_setting} for details on the datasets).
Figure~\ref{fig:accuracy_vs_classes} shows the average accuracy across all 3-class subsets of the 10 classes, the 4-class subsets, and so on till all 10 classes. 
Post-training dynamic range quantization~\cite{dynamicq} is applied to all models. 

We see that accuracy drops steadily as the number of classes increases: the overall drop is by about 5\% and 13\% for STL-10 and Camera Trap respectively when we go from 3 classes to 10 classes. 
This is quite a substantial gap in performance and makes the case for a $\mu$Classifier-based design for increased efficiency.

\mypara{Observation 2: Model compression cannot reduce this gap.} 
In Figure~\ref{fig:accuracy_vs_classes}, we used EfficientNet-B0 with quantization but did not apply other techniques that are available for optimizing deep learning models for embedded MCUs (e.g. weight sparsification, filter pruning, and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand,cheng2017survey}). We now ask whether these techniques can bridge the performance gap between $\mu$Classifiers and the all-class model.

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.42\textwidth]{figures/STL_All_Config_V3.png}
%     \caption{Gap between all-class and $\mu$Classifiers increases as models are pruned more.}
%     \label{fig:accuracy_vs_size}
% \end{figure}

Figure~\ref{fig:accuracy_vs_size} shows the performance gap between 10-class and 3-class EfficientNet after model pruning and quantization on the STL-10 dataset. We apply filter pruning~\cite{str_p1} which reduces the number of filters in each layer based on $\ell_1$ norm. The accuracy of each orange point that represents a 3-class model is computed by averaging the accuracy of all 3-class subsets. 
We see that the performance gap between the $\mu$Classifier and all-class classifier increases as resources reduce (5\% at 148 MFLOPs to 11.5\% at 70 MFLOPs). 
% Another way to describe performance is that the $\mu$Classifier has the same accuracy as the all-class model at less than half the computational resources. 
Thus, model optimization techniques cannot bridge the gap between all-class and $\mu$Classifiers.

\mypara{Observation 3: The benefits hold for early exit models.} 
Another approach to reduce the computational requirements of executing models on IoT devices is to use early exit, where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers~\cite{teerapittayanon2016branchynet, kaya2019shallow, fleet2023}.
We now ask whether a $\mu$Classifier outperforms all-class models with the early exit capability.  

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/Early_Exit_Acc_Vs_Classes.png}
%     \caption{Gap between all-class and $\mu$Classifiers is significant even for early-exit models.}
%     \label{fig:early_exit accuracy_vs_size}
% \end{figure}

Figure~\ref{fig:early_exit accuracy_vs_size} shows the average accuracy across all 3-class subsets of 10 classes, 4-class subsets, and so on till all 10 classes after applying quantization and adding two early exit branches (stages 4 and 6) to the EfficientNet-B0. We can see that accuracy drops with increase in the number of covered classes and the gap between 3-class and all-class models is 5\% and 12\% for STL-10 and Camera Trap datasets respectively. Thus, the performance advantages of $\mu$Classifiers remain even if we augment the model with early exits.

\begin{comment}
\mypara{Is switching $\mu$Classifiers expensive?} 
So far, we have shown that there is significant performance benefits to using $\mu$Classifiers. The main cost of such an approach, however, is switching overhead to transition to a new model every time the current context changes. Thus, if the current context changes very frequently, the overhead of switching between $\mu$Classifiers can be significant and diminish performance.

However, in many static deployments, there is significant temporal stability and context change is not frequent. 

To illustrate, we look at how frequently the set of classes changes in the case of a trail camera or backyard camera. We use a large trail camera trap dataset \cite{} from Africa for this analysis. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. For Figure ~\ref{fig:CDF_Temporal}, we used the entire Enonkishu dataset \cite{} comprising 38 species.

Figure~\ref{fig:CDF_Temporal} shows the distribution of the number of captured unique species in a whole day by a camera. As we can see, less than 6 species show up on most days.

% \mypara{Limits of alternate approaches:} 

% There are many methods exist to reduce the computational cost of executing classifiers of IoT devices. We argue that each of these have their limitations when scaled down to small processors/resources, and it is generally beneficial to have classifiers with fewer classes.


% There are a number of existing approaches for optimizing deep learning models for embedded MCUs  \cite{cheng2017survey}. These include model compression techniques such as weight quantization, weight sparsification, compact filters and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand}. 

% There are also early exit methods where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers \cite{teerapittayanon2016branchynet, kaya2019shallow,Fleet-Mobicom23}. But all these approaches improve in accuracy and performance if fewer classes are used. 

% \begin{itemize}
% \item \emph{Graph: Accuracy vs Size.} Show that a 10 or 20 class classifier will lose accuracy quickly if squeezed below some threshold size for either method (under some resource constraints in terms of number of layers/parameters)

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/Acc_vs_Model_Size.png}
%     \caption{Accuracy Drops as the model gets smaller (Places Dataset)}
%     \label{fig:accuracy_vs_model_size}
% \end{figure}


% \item Fewer classes is better. Classifiers with fewer classes is better from performance perspective.
% \end{itemize}


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/contx_c_dist_V2.png}
    \caption{Number of unique classes per day - Camera Trap Dataset (Enonkishu).}
    \label{fig:CDF_Temporal}
\end{figure}

% \mypara{Our approach:} To summarize, we have shown that context-aware $\mu$Classifiers consume less resources and can offer \textbf{higher accuracy} in resource-constrained settings. We also see that there is typically temporal consistency in many real-world environments and context change may not be very frequent for static deployments. Thus, the overhead of switching can also potentially be kept low.

% But for the technique to work, we need to answer a few questions. First, how 
\end{comment}

==> Backup/June20/Design.tex <==
\section{Configuration Prediction}
\label{sec:configuration-prediction}
% The key premise in our work is that given a total of $N$ classes, a classifier that works on only a subset of these $N$ classes can afford to be more computationally efficient compared to the classifier that works on the entire set of $N$ classes since classification tasks with fewer classes is significantly easier. 

The goal of the configuration selector is to identify the best configuration of the $\mu$Classifier for an arbitrary subset of classes. 
We note that the ``best configuration'' is defined based on application needs, i.e.  the available resources and accuracy tolerance for the application. 
For example, when resources are a priority (e.g. highly constrained IoT devices), then there may be more tolerance for lower accuracy. 
In the rest of the paper, we refer to the best configuration as the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$ (as defined for the application). 

A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions: (1) \textit{What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? }, and (2) \textit{How to quickly identify the most efficient yet accurate $\mu$Classifier, given any subset of classes?}

% \begin{enumerate}
%     \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
%     \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
% \end{enumerate}


\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. 
While there are a number of techniques that can be used to compress machine learning models, we specifically look for configuration parameters that provide large dynamic range of resource-accuracy tradeoffs for $\mu$Classifiers.

We find that two methods are particularly effective for configuring $\mu$Classifiers --- image resolution and filter pruning. Varying the resolution of the image that we provide as input to the $\mu$Classifier is particularly effective because a) the computation complexity of a feature extractor decreases quadratically as resolution (height and width) decreases, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. Filter pruning with different sparsity ratios to control the computation complexity of the feature extractor is also effective. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

% In this work, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset).
%  can be augmented with other secondary techniques such as filter pruning and quantization for further expanding the configuration space.

% Thus, our overall configuration space is as follows. 
% In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
% In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and pruning level scales down better as compute decreases compared to varying only the pruning level. Each point shows the average accuracy across all 3-class subsets of 10 classes.  We see that varying both resolution and pruning level provides us configurations with lower computation costs while accuracy remains in a reasonable range. Pruning performs poorly in the low FLOPs regime since it requires very high pruning levels which leads to very low accuracies.

\begin{figure}[h]
    \includegraphics[width=0.4\textwidth]{figures/res_size_vs_size_V3.png}
    \caption{Configuring resolution and model size (by varying the pruning level) provides us a large dynamic range in resource-accuracy tradeoffs for configuring $\mu$Classifiers. (Camera Trap dataset is used.)}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.



\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely configuration (i.e., resolution and model sizes) without needing to train a huge number of them. 
% A $\mu$Classifier can be made computation-efficient by compressing the model via filter pruning and reducing the resolution of input images. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ $\mu$Classifiers to evaluate in order to identify the best one for an arbitrary subset of classes. 
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of $N$ classes (i.e., an \textit{m-class combination}), we will need to train a total of $C^{N}_m \times R \times S$ models to find the best $\mu$Classifier for every $m$-class combination, which can be prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to the similarity among classes (darker $\implies$ higher accuracy). X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolutions) sorted from least to most compute complexity. We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS \cite{NAS1,NAS2}). 
% However, this method doesn't address the problem due to two fundamental limitations. 
% First, 
although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of $\mu$Classifiers on a given subset of classes, it still needs to examine $C^N_{m}$ number of $m$ class combinations, each of which incurs significant training overhead.
% Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. 
Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities would also share a similar $\mu$Classifier configuration. 

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?} 
Figure~\ref{heatmap} shows that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.}
    \label{fig:kNN-training}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}
Given that inter-class similarity accurately tracks resource-accuracy trade-offs of a $\mu$Classifier, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


% \mypara{Similarity-directed sampling.} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration of the remaining combinations accurately. This is critical to ensure the performance of kNN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a \textbf{similarity-directed sampling} scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the kNN.
Compared to random sampling, our empirical evaluation on three datasets demonstrates that similarity-directed sampling can reduce 25-66\% of samples while getting similar prediction accuracy.  



% \mypara{Input for kNN training.} The input to train the kNN comprises the vector representation (Eq.~\ref{eq:rep_vector}) for the chosen m-class subsets and their best $\mu$Classifier configuration. We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 
% \DG{We need a figure to show this stage}


% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}

\section{Budget-limited $\mu$C selection}
% \HG{we do not have an evaluation section corresponding to the classifier selection component} 
So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for an $m$-class combination. 
However, we may not be able to train and/or store all $m$-class subsets. This raises another question:
\textit{How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes?}
% \begin{enumerate}
%     \item How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes.
% \end{enumerate}


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to cover all classes that can possibly occur in a scene, and achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of covering as many classes as possible is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifier should work in any possible context. 

The problem can be re-phrased as a combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is minimized while each model meets a target accuracy threshold and the collection meets some class coverage requirement. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{salkin1975knapsack}. 
We next elaborate on our greedy algorithm to approximate the optimal solution. 

% \M{Our solution has a different objective in comparison to the stated problem. The Problem says we want to maximize accuracy s.t a budget limit. But our approach aims to minimize computation s.t that the accuracy over a threshold. Do you agree?}
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training of the $\mu$Classifiers.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
If this is the case, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. Since the selection is based on kNN prediction, we again need to go through the process of training the newly selected model to check if the accuracy requirement ($Acc_{thr}$) is satisfied.
% In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
% As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If so, the replacement happens; otherwise, the process repeats and the next lightest $\mu$Classifier will be selected and trained. 
% and checked until the replacement happens. 
% Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
This process continues until the $Acc_{thr}$ threshold is met. 
In our experience, kNN has high accuracy, hence the number of times a $\mu$Classifier in the selected set needs to be replaced is very low.

\mypara{Optimizing storage requirements:} 
Since $\mu$Classifiers that operate on the same model size (same pruning level) share the same model weights, we can further reduce storage requirements by storing one feature extractor per model size, and then only storing the classification and context change detection heads for each chosen $\mu$Classifier. 

% only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

% \subsection{Local and Edge-cloud} 

% We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

% \mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

% The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
% Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

% During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

% On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

% \mypara{Edge-cloud assisted IoT devices.} 
% Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
% The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

% Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
% The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change:} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computationally intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the $\mu$Classifier as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching:} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. Once this is determined, we use a simple technique where the last $p$ predictions made by the pipeline are observed and the farthest predicted class among the previous set of classes is substituted by the new ones. 

As described in \S\ref{sec:overview}, the \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/June20/DesignOverview.tex <==
\section{Design Overview}
\label{des_over}

While context-aware $\mu$Classifiers consume \emph{less resources} and offer \emph{higher accuracy} in resource-constrained settings, instantiating such a system in practice presents three challenges. 

\subsection{Challenges}
\label{challenge}
\mypara{Challenge 1: Minimizing training overhead.}
The first challenge is reducing overhead for training a huge number of $\mu$Classifiers. 
For example, if there are 20 classes and we consider 3-class $\mu$classifiers, there are $C^{20}_3 = 1140$ $\mu$Classifers. Furthermore, each 3-class combination will need to be optimized by model compression for which we need to determine the best configuration (e.g. quantization, pruning, resolution, etc). 
% This configuration space is quite large and requires us to train models with different choices per 3-class combination to determine the $\mu$Classifier that offers the best accuracy and computation tradeoff. 
If we consider 100 configurations per $\mu$Classifier, then 114K models need to be trained. 
% When the search space is larger, for example, 100 classes in ImageNet \cite{}, this increases to 16 million 3-class models.

\mypara{Challenge 2: Detecting context switch.} 
A second key challenge is designing an accurate detector that can precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. Since context change detection lies on the critical path of every prediction, the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 


\mypara{Challenge 3: Addressing storage constraints.}
% The large number of $\mu$Classifiers raises not just a training challenge but also a storage challenge.
An IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. 
If the IoT device is connected to an edge-cloud, it may be possible to train a $\mu$Classifier \emph{on-demand} and download the learned weights during run-time. 
But this incurs high communication overhead and only works for devices connected to an edge-cloud. 
Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead.

\subsection{\myname{} Overview}
\label{sec:overview}
% We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}. 

% \mypara{\myname{} contributions:} Our work has three major contributions. First, we develop a similarity-aware model configuration predictor to reduce training overhead. 
% The core building block for our method is a \emph{similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
% We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

% Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
% This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the rate to invoke the heavyweight classifier.

% Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
% Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

\myname{} comprises three main components.
During the training phase, the \textit{Configuration Predictor} leverages the ``similarity'' between classes and a kNN model to efficiently identify the suitable configuration of the $\mu$Classifier for each subset of classes. 
The \textit{Budget-limited $\mu$Classifier Selector} selects a smaller subset of $\mu$Classifiers to train and store on device from 
% among the set of $C^N_m$ combinations 
among all possible candidates
to achieve high coverage, high accuracy, and low computational costs while meeting the storage requirements. 
These steps happen offline and are shown in Figure~\ref{fig:offline}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/offline.png}
    \caption{Similarity-based configuration prediction and budget-limited $\mu$Classifier selection}
    \label{fig:offline}
\end{figure}

\begin{figure*}[t!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_v6.png}
    \caption{Context-Aware Switching in the proposed \myname{} architecture. (CCD: Context change detection, FE: Feature extractor)}
    \label{framework_all}
\end{figure*}

At run-time, \textit{context-aware switching} occurs in two steps.
To detect context changes, we augment the \emph{$\mu$Classifier} with an additional lightweight \textit{Context Change Detector} head. 
The \textit{Context Change Detector} head rapidly detects if the input frame is a new class without determining which is the new class. 
If context change is detected, \myname{} executes the \textit{all-class model}, a heavyweight classification module, that determines which classes are present in the scene. 
If a new class is detected, it triggers a ``model switch'' to load a new context-specific $\mu$Classifier. Figure~\ref{framework_all} illustrates switching at run-time.

\mypara{\myname{} in practice.} \myname{} can be instantiated both for local and cloud-assisted IoT deployment. 

When the IoT device is operating autonomously, we pre-load a subset of $\mu$Classifiers selected by the budget-limited $\mu$Classifier selection process on the device prior to deployment. During inference, the choice of the all-class model to run for context change detection depends on available resources. 
On low-end IoT platforms (e.g. with MCU), the all-class model also needs to be resource-constrained and hence a lightweight model like EfficientNet can be used. 
On heterogeneous multi-core processors (e.g. NXP's i.MX \cite{URL:iMX}), a more computationally heavy model like ResNet \cite{resnet-50} can be used to leverage the more powerful cores.

When an IoT device is operating with edge-cloud support, it locally executes the $\mu$Classifier.  
It transmits images to the edge-cloud when a context change is detected. 
The edge-cloud uses a powerful model like ResNet-50 to determine whether a new class needs to be added to the $\mu$Classifier. 
It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. 
The parameters of the trained model are then downloaded to the IoT device. 
To reduce the frequency with which model parameters need to be downloaded via a wireless link, a smaller set of  $\mu$Classifiers selected via the budget-limited $\mu$Classifier selection procedure can be cached on the IoT device.

We now describe these components in more detail.




% \paragraph{Configuration Selector} 
% This component determines the optimal architecture configuration of a \textit{$\mu$Classifier} to achieve both high computation efficiency and task accuracy for a arbitrary subset of classes. 
% It leverages a k-NN model that takes as input a vector representation for a subset of classes, and predict its appropriate \textit{$\mu$Classifier} configuration.
% % We represent a subset of classes as the mean and standard deviation of pair-wise class similarities, which captures how difficult it is to achieve high accuracy for the subset.
% Since not all \textit{$\mu$Classifiers} can be stored on a device, the configuration selector also determines the set of \textit{$\mu$Classifiers} that need to be loaded on device to optimize on-device efficiency.
%  % leverages a greedy approach to select a set of \textit{$\mu$Classifiers} that can fit on device and achieve target task accuracy and the lowest computation cost. \HG{note that I put the selection of subset of mini-classifier here.}



% % We considered several levels of image size downsampling and model size to create a configuration space. Unimportant filters in convolutional layers are pruned to compress the model. 

% % The output vector of the oracle's feature extractor is considered to represent a class and the similarity between two classes is measured using the cosine distance of their vectors. statistics such as mean and std are extracted from pair-wise similarities of a set of classes. Since all possible pair-wise similarities only need to be computed once and k-NN inference is quite fast, the runtime overhead of predicting a configuration is negligible. For training the k-NN we sample a few sets of classes from different levels of hardness/similarity. To make a dataset, we extract the mentioned statistics as the input and label each set of classes with a configuration based on predefined criteria.

% \paragraph{$\mu$Classifier Constructor} 
% This module materializes a well-trained $\mu$Classifier based on the selected configuration by the k-NN. 
% A $\mu$Classifier has a feature extractor, one class label classification head, and a context change detection head. 
% The $\mu$Classifier constructor initializes the feature extractor of the  $\mu$Classifier using parameters that are trained on all classes of the dataset, and trains only the classification and detection heads using the subset of classes. 
% Freezing the feature extractor has two benefits. (1) It makes the training process faster since the computation of the heads are much more lightweight compared to that of the feature extractor. (2) $\mu$Classifiers with the same configuration can share the same feature extractor, reducing space of storing $\mu$Classifiers on device.   


% % The feature extractor of the $\mu$Classifier is previously fine-tuned on all classes of the dataset and will be initialized with these weights. 
% % The feature extractor is kept frozen during training of the classification and context change detector heads. The training process is quite fast as the major part of the $\mu$Classifier is frozen. 
% % The classification and context change detector heads are quantized and then transmitted to the IoT alongside the feature extractor ID. The feature extractor ID notifies the IoT which of the pre-stored feature extractors should be loaded on the IoT.

% \paragraph{$\mu$Classifier-based Predictor}
% This module executes $\mu$Classifiers on device to predict the label of an input image and detect whether a context change happens. 
% If a context change is detected, the input image will be sent to another module \textit{new class detector} to further identify which new class appears.
% In case a new class appear, the predictor will load another $\mu$Classifier that covers the new class and the other recently appeared classes to make predictions.  


 
 
% % This part of the RASCAM architecture is responsible for detecting the new context which is essentially any class other than the current target classes. On the IoT side, there is a convolutional network called $\mu$Classifier with two output heads. One head does the classification task and the other decides whether the context has changed in the current frame or not. 

% % The context change detector is a regressor and it is trained to output a number close to 1 whenever the context changes and a number close to 0 in case the current frame contains an object from the current target classes. Its architecture is shown in Figure \ref{framework1}.

% \paragraph{New Class Detector} 
% This module executes a model that is trained on all classes to identify the class of an input image. 
% We refer to the model as a \textit{all-class model}.  
% If network is available, the module can be placed on the cloud: whenever a context change is detected by the $\mu$Classifier, the image will be compressed and transmitted to the cloud so that the module can execute the all-class model to predict the class label. 
% The class label will be sent back to the device for the device to make the decision on switching $\mu$Classifiers. 
% If the module is placed on the device due to the lack of network connections, it loads the all-class model from storage and executes it locally. 

% The oracle is a powerful model that covers all classes in the dataset. It is fed with the frame as the input and predicts its label. If the predicted class is not in the covered set of classes by the current $\mu$Classifier, the process of preparing a new $\mu$Classifier will be started by the micro-classifier configuration selector module.


% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/framework_iot_v2.png}
%     \caption{IoT node framework}
%     \label{framework1}
% \end{figure}




% Next, we explain the three key components in more detail. 

==> Backup/June20/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant activity in recent years in optimizing deep learning methods for low-power embedded systems and IoT devices (e.g. \cite{lai2018enable, warden2019tinyml,mazumder2021survey}). 
%  vlin2021memory
% While there is great diversity in the computational capabilities (e.g. low-power microcontrollers, neural architectures and heterogeneous multi-core processors) and communication capabilities (e.g. BLE and WiFi) of these devices, they share the constraint that they are heavily resource constrained. 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.

% \mypara{Squeezing deep learning models on IoT platforms.} 
Prior approaches to squeeze deep learning models fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. 
% Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. 
%Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 
% 
The second category is partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud~\cite{kang2017neurosurgeon,teerapittayanon2017distributed,choi2018deep, cohen2020lightweight, huang2020clio, itahara2021packet}
% 
The third category is early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations include model compression, partitioning, and early-exit.}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference and its challenges:} 
We argue that one dimension that has not been explored in prior efforts is \emph{context-aware inference}. 
Context awareness improves efficiency because it can reduce the \emph{number of classes} that need to be classified to those relevant to the current context. 
Fewer classes lead to a simpler classification problem which has better accuracy with a resource-constrained model.

% We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. 

In many applications, context can remain static for long periods making context-aware inference particularly effective. 
For example, a trail camera may be seeing the same set of animals, and a doorbell camera is likely to see the same types of vehicles and individuals. 
When compute and memory are scarce, it can make a big difference whether the classifier needs to classify between all classes or just the classes relevant to the current context. We refer to the classifier that has all classes as \textit{all-class model} and the context-aware classifier that has a subset of classes as \textit{$\mu$Classifier}. 

% We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a subset of the overall set of classes, making it more resource-efficient and accurate.

% This paradigm shift necessitates a change in a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

While a context-aware $\mu$Classifier can be more efficient, its design raises three key challenges. 
The first is that we need to minimize training overhead given the large number of $\mu$Classifiers. 
For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class $\mu$Classifiers and $C^{20}_4$ (4845) four-class $\mu$Classifiers that are possible. 
In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. %It is impractical to pre-train and optimize a huge number of $\mu$Classifers.
%As we show later, the optimal parameters depend greatly upon the specific set of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to detect context change so that we can switch to the appropriate $\mu$Classifier for the new context when an entity that is not in the class set of the current $\mu$Classifier enters the scene. In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier.

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the lowest computation while meeting the desired accuracy, coverage across classes of interest, and not exceeding available storage. 

\mypara{The \myname{} approach:} We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}.\footnote{\myname{} connotes the back-and-forth nature of switching between $\mu$Classifiers depending on context.}

Our work has three major contributions. First, we develop a similarity-aware kNN-based model configuration predictor to reduce training overhead. 
The core building block for our method is an \emph{inter-class similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the frequency of invoking the heavyweight classifier.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

% In this paper, we present a novel solution that addresses these problems. 
% %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
% First, we define a inter-class similarity metric that captures the similarity of classes and the hardness of distinguishing them.
% A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
% %The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
% Second, we add a regression head to the $\mu$Classifier as the second output head to detect context changes. 
% Since the classification and regression heads share a feature extractor, the overhead for context change detection is negligible. 
% %The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.
% Third, we present a budget-limited $\mu$Classifier selector that selects the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
%     \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
%     \label{fig:our-approach}
% \end{figure}

We implement \myname{} by modifying EfficientNet-B0 \cite{efficientnet} and conduct extensive evaluation across three datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}) and multiple IoT processors (Risc-V(GAP8) \cite{URL:GAP8} and low-end ARM 11 \cite{URL:Arm11} to high-end Cortex-A77 \cite{URL:Cortex-A77}). We show that:
\begin{itemize}
    \item \myname{} can provide up to 13$\times$ reduction in computational cost while outperforming all-class EfficientNet-B0 across a wide range of desired accuracy thresholds. 
    \item Our inter-class similarity metric captures the hardness of a set of classes in a $\mu$Classifier very well (0.86-0.97 Pearson's coefficient between classification accuracy and our metric).
    \item \myname{}'s context change detector has 10-20\% fewer false positives and false negatives than an alternate lightweight detector that uses similar FLOPs. It has only  3-7\% higher false positives and false negatives than a heavyweight detector that uses 2-4$\times$ more FLOPs. 
    \item End-to-end results on the Raspberry Pi Zero W and GAP8 IoT processors show that \myname{} can achieve 1.2$\times$ -- 4.4$\times$ speed-up and up to $5\%$ gain in accuracy compared to all-class EfficientNet. We also show that our greedy algorithm that selects a subset of $\mu$Classifiers to balance accuracy, FLOPs, and coverage under storage constraints has up to 1.4$\times$ speed-up compared to a solely coverage-focused method.
    
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Mar11/Evaluation.tex <==




\section{Evaluation}
This section evaluates how \myname{} addresses the three challenges in Section \ref{case_context}. 
We first describe the datasets, the baselines, and evaluation metrics, and then evaluate the components of the system over datasets and real platforms. 
We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Experiment Settings}

\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resulution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\mypara{Dataset:}
\label{dataset}
We use three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and Camera Trap \cite{}. \HG{fill in}  
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 


Places365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 


Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two cameras were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset (both from cameras in the African savvanah). Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10+1 classes to be close to the real-world setting. 

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_size}) but also requires the most switching between contexts. 
So, it helps us understand how a nimble system can be designed with $\mu$Classifiers. 
By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.



\mypara{The configuration space of $\mu$Classifiers.}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both model size and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning and get a total of four feature extractor configurations.  
The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The considered image resolutions for each dataset are provided in Table~\ref{tab:expt-settings}.  
These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (detecting context change). 
The two heads use two Fully Connected layers.
$\mu$Classifiers are fine-tuned on the target dataset before they are deployed on devices. 

\mypara{Inter-class similarity metric.}
The Configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of the all-class model ResNet-50 to extract embedding of images from a class and average the embedding into a single vector as that class' inter-class similarity representation. 


\mypara{KNN-based configuration selection.}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in Section~\ref{sec:knn}) to get 200, 40, and 40 number of 3-class combination samples from 1140, 120, and 120 in total for the three datasets PLACES, STL-10, and Camera Trap respectively. 
For each sampled 3-class combination, we train $\mu$Classifier with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of the best and the worst accuracy of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. \HG{check if it makes sense} 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved for a configuration.


\mypara{Context-aware switching.} 
As discussed in section~\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect context change. 
It is trained to output a value close to 0 for the target classes (no context change) of the $\mu$Classifier and a value around 1 for other classes (context change). 
We used $0.5$ as the decision boundary. 

Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50~\cite{resnet-50} for its high classification accuracy in case the IoT device is using a heterogeneous multi-core process or if the all-class model execution can be offloaded to the cloud and uses EfficientNet-B0~\cite{efficientnet} otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on our three target datasets.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance for different thresholds \M{Updated}}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}


This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of the all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in smaller $\mu$Classifiers and thus less FLOPs.  



We compared the classification accuracy and computation cost of the predicted configuration (\textbf{Predicted $\mu$Classifier}) with the following baselines: 
\begin{itemize}
    \item \textbf{All-Class EfficientNet}: This uses the well-trained EfficientNet-B0 with all the classes and full image resolution, even though only three classes are of interests in a scene.  
    
    \item \textbf{3-Class EfficientNet}: We replace the classification head in all-class EfficientNet with a 3-class classification head and fine-tune the model on each 3-class combination of the target dataset. Since the model uses the same feature extractor as the all-class EfficientNet, the computation costs (in FLOPS) remains the same. 
    
    \item \textbf{Oracle $\mu$Classifier}: For a 3-class combination, we get the oracle by enumerating and training $\mu$Classifier with all possible configurations and picking the one that meets a target accuracy threshold. 
    Note that this brute force search needs to train a total of XX, XX, and XX 3-class $\mu$Classifier for the three datasets XX, XX, and XX respectively. It takes a total of XX hours, XX-XX longer than our approach.  \HG{fill in}
\end{itemize}


Figure~\ref{} shows how different target accuracy threshold affects the classification accuracy and the computation costs for our methods and baselines. 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   


We first compare \myname{}'s configuration predictor (orange curve) against the Oracle (blue curve. We see that the accuracy is nearly the same regardless of the target accuracy threshold, while our method has significantly lower training cost.

can predict the configuration of the $\mu$Classifiers (the orange curve) close enough to the oracle (the blue curve) but with much less training costs, regardless of the target accuracy threshold. The accuracy gap between \myname{} and the oracle $\mu$Classifiers under the same compute budget was very small on the three datasets.
For the STL-10 dataset, the accuracy gap between the \myname{} predicted model and the best $\mu$Classifier configuration was as small as -$0.35\%$ while the computation cost was almost equal. 
The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset, however, our predicted configurations save $10.7\%$ in computation cost. 
These results show the k-NN together with the inter-class similarity metric works well in selecting the configurations. \HG{if figure updated, consider update the above numbers as well} 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

Compared to {all-class EfficientNet}, our predicted $\mu$Classifiers have  high accuracy gains and computation savings for all three datasets. 
For the Camera Trap dataset, Our approach is $9\%$ more accurate than the all-class EfficientNet while while we save $86.87\%$ computation. 
Although the accuracy gain on STL-10 was not noticable, we could still gain over $62.37\%$ computation saving.

Compared to {3-Class EfficientNet}, our method achieves a significant amount of computation savings by sacrificing some classification accuracy. 
For instance, if we choose 3-Class EfficientNet (full resolution) for all combinations the $3.36\%$ accuracy gain comes with a cost of $6.61\times$ more computation overhead in comparison to our predicted configuration for the Camera Trap dataset. 


\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.904$)\label{fig:CameraTrap_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Acc_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.974$) \label{fig:STL_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Acc_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.857$)\label{fig:Places_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Acc_Vs_Similarity_V2.png}}}%
    \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes}
\label{acc_vs_sim_eval}
\end{figure*}

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.934$)\label{fig:CameraTrap_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_SpeedUp_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.973$) \label{fig:STL_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Speedup_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.81$)\label{fig:Places_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Speedup_Vs_Similarity_V2.png}}}%
    \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
\label{speedup_vs_sim_eval}
\end{figure*}

\mypara{Effectiveness of the inter-class similarity metric} We further examine the effectiveness of the proposed inter-class similarity metrics in quantifying the difficulty level of differentiating a set of classes. 
Recall that our underlying assumption in configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold; two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. 
In other words, we assumed the difficulty level can be quantified by our proposed inter-class similarity metric. 


Figure~\ref{acc_vs_sim_eval} illustrates how the accuracy of an all-class EfficientNet on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For a clear demonstration, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
We observed that the higher the inter-class similarity is, the lower the classification accuracy it has. The Pearson correlation between the inter-class similarity metric and the classification accuracy is as high as $0.857-0.974$, indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure \ref{speedup_vs_sim_eval} further illustrates how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to 3-Class EfficientNet (full resolution) while the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the k-NN works well in selecting light configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
 Predicted $\mu$Classifier+maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\ \hline 
Predicted $\mu$Classifier+regression head & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
Oracle $\mu$Classifier +regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
3-class EfficientNet (full res)+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. A false positive (FP) that wrongly predicts a context change, would introduce  computation costs if the all-class model is executed on device or communication costs if the all-class model is offloaded to the edge-cloud. On the other hand, a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot recognize the new class that occurs in the scene. 

To evaluate the performance of the regression head, we simulate context changes and calculate FP and FN rates as follows. 
\HG{fill in how do you simulate a context change here; how do you get the FP and FN?}
% Since 3-Class EfficientNet with the full resolution is the most complex $\mu$Classifier, it is included in the table. 
% For each combination of 3 classes in the test set, a $\mu$Classifier was constructed based on the predicted configuration by the k-NN, and its FN and FP rates were calculated. 
% The mean of the FN and FP rates over all combinations in the test was reported in the table. 


Table~\ref{fpfnt} compares the FP and FN rates for our method that uses a regression head with an alternative solution that uses the maximum probability~\cite{}. Overall, using regression head is much more accurate compared to the baseline that uses the maximum probablility. The FP and FN rates of our approach is $20\%$ lower than the baseline.

Table~\ref{fpfnt} further reports the results of using the regression head on our predicted $\mu$Classifier, the oracle $\mu$Classifier, and the 3-class EfficientNet with full resolution. The goal is to show how the choice of $\mu$Classifier would affect the performance of the regression head, 
Note that 3-Class EfficientNet + regression head would provide a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.  
Predicted $\mu$Classifier does increase the FP and FN rates to a small extend compared to the lower bound. However, the gap between our predicted $\mu$Classifiers and the lower bound for both metrics are in the range of $2.3$ to $4.6\%$ for the Camera Trap and PLACES365 datasets, much smaller than the gap between using regression head v.s. using maximum probability. 
These values can be further lowered by increasing the $Accuracy_{thr}$ explained in Section \ref{sec4.4.3} as it directly affects the predicted configuration and therefore FP and FN rates.


\subsection{Online End-To-End Results}

To evaluate the end-to-end performance of the framework, we need to have a sequenced test set providing a specific context change rate to mimic the temporal flow of the context change in the real world. 
If we consider m-class combinations, the context changes whenever a frame represents a class different from the last m distinct classes. 
The context can be represented by an m-class combination and whenever the context changes a new m-class combination represents the current context. For instance, in the 3-class combination setting, let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is:

\begin{equation}
    n=\lceil{CCR\times |TS|}\rceil
\end{equation}

We randomly construct a sequence of $n$ m-class combinations, where every two consecutive combinations show a context change. In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantee n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  



 \begin{algorithm}
        \caption{Generating a sequence of contexts}
        \label{Alg3}
\begin{flushleft}
        \textbf{INPUT} 
        \\$TS$: Original test set)
        \\$CCR$: Context change rate
        \\$S$: List of all m-class combinations\\     
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State $n = \lceil{CCR\times |TS|}\rceil$
            \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
            \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
            \While{$|C|\neq n$}
            \State $New_C = random\_choice(S)$ \Comment{New context candidate}
            \If {$|New_C\cap Curr_C|==m-1$}
               \State $C=C\cup New_C$
               \State $Curr_C=New_C$
            \EndIf
            \EndWhile
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: A sequence of $n$ contexts  
\end{flushleft}           
    \end{algorithm}


    

\begin{table*}[h]
\scalebox{0.7}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
\label{End-to-end1}
\end{table*}


\begin{table*}[h]
\scalebox{0.5}{
\begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
\toprule
Methods & \multicolumn{5}{c|}{Camera Trap - ResNet-50} & \multicolumn{5}{c|}{STL-10 - ResNet-50} & \multicolumn{5}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) \\ \midrule
Our Approach & 82.98\% & 14.93\% & 6.43\% & 216.78 & 72.57 & 93.64\% & 17.53\% & 6.45\% & 77.81 & 30.02 & 96.01\% & 13.71\% & 5.95\% & 263.28 & 90.40 \\
Oracle $\mu$Classifier & 83.21\% & 14.98\% & 6.23\% & 216.67 & 71.88 & 94.00\% & 16.43\% & 6.13\% & 79.75 & 30.53 & 96.39\% & 13.28\% & 6.03\% & 286.12 & 98.48\\
3-class EfficientNet (full res) & 86.03\% & 11.36\% & 6.88\% & 822.56 & 264.29 & 96.06\% & 10.93\% & 5.93\% & 107.38 & 41.73 & 97.36\% & 10.06\% & 5.78\% & 520.33 & 179.72\\
All-Class EfficientNet (full res) & 83.00\% & 0.00\% & 0.00\% & 833.40 & 264.29 & 92.13\% & 0.00\% & 0.00\% & 107.88 & 41.77 & 90.95\% & 0.00\% & 0.00\% & 521.12 & 180.01 \\

\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}






\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
  &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
\label{End-to-end2}
\end{table*}



\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{5 $\mu$Cs} & \multicolumn{3}{c|}{15 $\mu$Cs}  & \multicolumn{3}{c}{30 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms)\\ \midrule
Greedy & 82.41\% & 272.58 & 88.35 & - & -\% & - & -\% & - & - \\
Random $\mu$Classifier & 82.36\% & 337.74 & 110.89 & - & -\% & - & -\% & -& - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{Local-Switching; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}

==> Backup/Mar11/Introduction.tex <==
% \newpage 
\section{Introduction}

There has been significant interest in recent years in bringing advances in deep learning to embedded systems running on microcontrollers and other specialized low-power accelerators that are common in IoT devices \cite{vlin2021memory,warden2019tinyml,mazumder2021survey,lai2018enabling}. These platforms are highly resource constrained since they need to operate at very low energy budgets (typically a few milliwatts on average), to ensure that they can run for weeks or months on battery power.

A wide range of approaches have been proposed to squeeze deep learning models onto resource-constrained devices including pruning, quantization, knowledge distillation, early exits and others (summarized in Figure~\ref{fig:alternatives}). For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input  during inference by executing different sub-networks. 

% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/alternatives.png}
    \caption{Prior approaches for addressing IoT resource limitations either squeeze larger models or partition large models across IoT devices and a more powerful remote device. \DG{Needs to be re-drawn - this is just a sketch}\HG{remove compression and sparsification when redraw since sparsification belongs to pruning; both pruning and quantization belongs to compression}}
    \label{fig:alternatives}
\end{figure}

But one dimension that has not been exploited in prior work is adapting the \emph{number of classes} that need to be classified based on the current context. The assumption in all prior work is that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time. 

We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. For example, a backyard camera may be primarily observing a dog or child playing for a certain period of time. In other words, the current context may have only a subset of classes of interest. When compute and memory are scarce, it can make a big difference whether the classifier needs to classify between 10 classes or three classes. We refer to a context-aware classifer as a $\mu$Classifier since it can focus on a few of the overall set of classes that relevant to the current context, making it more resource-efficient and accurate.

While a context-aware $\mu$Classifier can be more efficient, its design raises two key challenges. \HG{need to revise this later to match with the design section}
The first is that there are many possible subsets of classes that can occur in a given context. 
For example, even with only 20 classes, there are $C_{20}^3$ (1140) three-class micro-classifiers and $C_{20}^4$ (4845) four-class micro-classifiers that are possible. 
Further complicating the process, each of these $\mu$Classifiers will need to use model compression techniques to optimize its size. As we show later, the optimal parameters depend greatly upon the choice of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. 
These $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Thus, it is clearly impractical to pre-train, optimize and store a huge number of $\mu$Classifers.

The second challenge is that we need a robust method to determine context change so that we can switch to the appropriate $\mu$Classifier when the context changes, for example, when an entity that is not in the current $\mu$classifier set enters the scene. 
In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier.

In this paper, we present a novel solution that addresses these problems. Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 

In order to detect the context change, a regression head is attached to $\mu$Classifiers as the second output head. Since the classification and regression heads share a feature extractor, the added overhead by the context change detector is negligible. The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.


In the classification task, we observed a direct relationship between the similarity of classes and the hardness of distinguishing them for the classifier. 
In order to quantify the similarity between two classes, the cosine distance of their embedding from a feature extractor is considered. 
A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
As IoT devices are limited in resources, only a portion ($n$) of $\mu$Classifiers can be stored on the device. 
A greedy algorithm is implemented to select the lightest n $\mu$Classifier covering all classes in the dataset.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
    \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
    \label{fig:our-approach}
\end{figure}


% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Mar12/Evaluation.tex <==




\section{Evaluation}
This section evaluates how \myname{} addresses the three challenges in Section \ref{case_context}. 
We first describe the datasets, the baselines, and evaluation metrics, and then evaluate the components of the system over datasets and real platforms. 
We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Experiment Settings}
\label{experiment_setting}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resulution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\mypara{Dataset:}
\label{dataset}
We use three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and Camera Trap \cite{}. \HG{fill in}  
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 


Places365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 


Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two cameras were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset (both from cameras in the African savvanah). Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10+1 classes to be close to the real-world setting. 

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_size}) but also requires the most switching between contexts. 
So, it helps us understand how a nimble system can be designed with $\mu$Classifiers. 
By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.



\mypara{The configuration space of $\mu$Classifiers.}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both model size and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning and get a total of four feature extractor configurations.  
The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The considered image resolutions for each dataset are provided in Table~\ref{tab:expt-settings}.  
These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (detecting context change). 
The two heads use two Fully Connected layers.
$\mu$Classifiers are fine-tuned on the target dataset before they are deployed on devices. 

\mypara{Inter-class similarity metric.}
The Configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of the all-class model ResNet-50 to extract embedding of images from a class and average the embedding into a single vector as that class' inter-class similarity representation. 


\mypara{KNN-based configuration selection.}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in Section~\ref{sec:knn}) to get 200, 40, and 40 number of 3-class combination samples from 1140, 120, and 120 in total for the three datasets PLACES, STL-10, and Camera Trap respectively. 
For each sampled 3-class combination, we train $\mu$Classifier with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved for a configuration.


\mypara{Context-aware switching.} 
As discussed in section~\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect context change. 
It is trained to output a value close to 0 for the target classes (no context change) of the $\mu$Classifier and a value around 1 for other classes (context change). 
We used $0.5$ as the decision boundary. 

Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50~\cite{resnet-50} for its high classification accuracy in case the IoT device is using a heterogeneous multi-core process or if the all-class model execution can be offloaded to the cloud and uses EfficientNet-B0~\cite{efficientnet} otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on our three target datasets.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance for different thresholds}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}


This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of the all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in smaller $\mu$Classifiers and thus less FLOPs.  



We compared the classification accuracy and computation cost of the predicted configuration (\textbf{Predicted $\mu$Classifier}) with the following baselines: 
\begin{itemize}
    \item \textbf{All-Class EfficientNet}: This uses the well-trained EfficientNet-B0 with all the classes and full image resolution, even though only three classes are of interests in a scene.  
    
    \item \textbf{3-Class EfficientNet}: We replace the classification head in all-class EfficientNet with a 3-class classification head and fine-tune the model on each 3-class combination of the target dataset. Since the model uses the same feature extractor as the all-class EfficientNet, the computation costs (in FLOPs) remains the same. 
    
    \item \textbf{Oracle $\mu$Classifier}: For a 3-class combination, we get the oracle by enumerating and training $\mu$Classifier with all possible configurations and picking the one that meets a target accuracy threshold. 
    Note that this brute force search needs to train a total of 1920, 1920, and 18240 3-class $\mu$Classifier for the three datasets STL-10, Camera Trap, and PLACES365 respectively. It takes a total of XX hours, XX-XX longer than our approach.  \HG{fill in}
\end{itemize}


Figure~\ref{knn_performance} shows how different target accuracy threshold affects the classification accuracy and the computation costs for our methods and baselines. 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   


We first compare \myname{}'s configuration predictor (orange curve) against the Oracle (blue curve). We see that the accuracy is nearly the same regardless of the target accuracy threshold, despite significantly lower training cost. 
For the STL-10 dataset, the accuracy gap between the \myname{} predicted model and the best $\mu$Classifier configuration was as small as -$0.35\%$ while the computation cost was almost equal. 
With almost the same computation cost, The biggest gap in accuracy with $-0.95\%$ is for the Camera Trap dataset. 
These results show the k-NN together with the inter-class similarity metric works well in selecting the configurations.


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

We now compare \myname{} against {all-class EfficientNet}. We see that \myname{}-predicted $\mu$Classifiers has high accuracy gain and computation savings across all three datasets. 
For the Camera Trap dataset, Our approach is $9.3\%$ more accurate than all-class EfficientNet while we save $74.79\%$ in computation. 
For the STL-10 dataset, the accuracy gain is close to $1\%$ but we obtain over $53\%$ in computation savings.

When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.904$)\label{fig:CameraTrap_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Acc_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.974$) \label{fig:STL_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Acc_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.857$)\label{fig:Places_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Acc_Vs_Similarity_V2.png}}}%
    \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes}
\label{acc_vs_sim_eval}
\end{figure*}

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.87$)\label{fig:CameraTrap_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_SpeedUp_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.94$) \label{fig:STL_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Speedup_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.87$)\label{fig:Places_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Speedup_Vs_Similarity_V2.png}}}%
    \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
\label{speedup_vs_sim_eval}
\end{figure*}

\mypara{Effectiveness of the inter-class similarity metric.} We now examine the effectiveness of the proposed inter-class similarity metrics in quantifying the difficulty level of differentiating a set of classes. 
Recall that our underlying assumption in the configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold. Thus, two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. We now ask whether this is indeed the case i.e. can the difficulty level can be quantified by our proposed inter-class similarity metric? 

Figure~\ref{acc_vs_sim_eval} illustrates how the accuracy of a fixed $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.857-0.974$), indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure \ref{speedup_vs_sim_eval} looks at this relation from another performance dimension --- computation gain. The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class/3-Class EfficientNet (full resolution) while the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the simularity-aware k-NN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
 Predicted $\mu$Classifier+maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\ \hline 
Predicted $\mu$Classifier+regression head & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
Oracle $\mu$Classifier +regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
3-class EfficientNet (full res)+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. A false positive (FP) that wrongly predicts a context change, would introduce  computation costs if the all-class model is executed on device or communication costs if the all-class model is offloaded to the edge-cloud. On the other hand, a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot recognize the new class that occurs in the scene. 

To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.
% Since 3-Class EfficientNet with the full resolution is the most complex $\mu$Classifier, it is included in the table. 
% For each combination of 3 classes in the test set, a $\mu$Classifier was constructed based on the predicted configuration by the k-NN, and its FN and FP rates were calculated. 
% The mean of the FN and FP rates over all combinations in the test was reported in the table. 


Table~\ref{fpfnt} compares the FP and FN rates for our method that uses a regression head with a baseline proposed in prior work that uses the maximum probability~\cite{maxsoft1}. Overall, using a regression head is much more accurate compared to the baseline that uses the maximum probablility. The FP and FN rates of our approach are $10-20\%$ lower than the baseline.

Table~\ref{fpfnt} further reports the results of using the regression head on our predicted $\mu$Classifier, the oracle $\mu$Classifier, and the 3-class EfficientNet with full resolution. The goal is to show how the choice of $\mu$Classifier would affect the performance of the regression head, 
Note that 3-Class EfficientNet + regression head would provide a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.  
The predicted $\mu$Classifier does increase the FP and FN rates to a small extent compared to the lower bound. However, the gap between our predicted $\mu$Classifiers and the lower bound for both metrics are in the range of $2.3$ to $4.2\%$ for the Camera Trap and PLACES365 datasets, much smaller than the gap between using regression head v.s. using maximum probability. 
These values can be further lowered by increasing the $Acc_{thr}$ explained in Section \ref{sec4.4.3} as it directly affects the predicted configuration and therefore FP and FN rates.


\subsection{End-To-End Results}

In order to evaluate the end-to-end performance of the framework, we need to have a sequenced test set providing a specific context change rate to mimic the temporal flow of the context change in the real world. 
If we consider m-class combinations, the context changes whenever a frame represents a class different from the last m distinct classes. 
The context can be represented by an m-class combination and whenever the context changes a new m-class combination represents the current context. For instance, in the 3-class combination setting, let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is:

\begin{equation}
    n=\lceil{CCR\times |TS|}\rceil
\end{equation}

We randomly construct a sequence of $n$ m-class combinations, where every two consecutive combinations show a context change. In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantees n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  

In the 3-class combination setting the context change rate is $3\%$ for the Camera Trap dataset. As this dataset has a temporal flow and it shows a real-world use case for \myname{}, its intrinsic context change rate is considered for evaluating all three datasets unless noted differently.



 \begin{algorithm}
        \caption{Generating a sequence of contexts}
        \label{Alg3}
\begin{flushleft}
        \textbf{INPUT} 
        \\$TS$: Original test set)
        \\$CCR$: Context change rate
        \\$S$: List of all m-class combinations\\     
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State $n = \lceil{CCR\times |TS|}\rceil$
            \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
            \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
            \While{$|C|\neq n$}
            \State $New_C = random\_choice(S)$ \Comment{New context candidate}
            \If {$|New_C\cap Curr_C|==m-1$}
               \State $C=C\cup New_C$
               \State $Curr_C=New_C$
            \EndIf
            \EndWhile
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: A sequence of $n$ contexts  
\end{flushleft}           
    \end{algorithm}

\mypara{Edge-Cloud Assisted:}
This section evaluates the end-to-end results in case communication is available. Since the framework forms a loop and components affect each other's performance, it is important to evaluate the end-to-end performance of the system. As mentioned in Section \ref{experiment_setting}, in case the communication is available, the all-class model is ResNet-50. The data rate for the transmission is considered $10$ Mbps.

In the section, latencies show the average value over the test set. The latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices.

Table \ref{End-to-end-online} shows the end-to-end results on two devices. Overall, our approach has the advantage in terms of accuracy and especially the latency over the baselines. For the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup compared to all-class EfficientNet on Raspberry Pi Zero-W. Although we didn't gain accuracy for the Camera Trap dataset, still our approach is over $3.5\times$ faster than the all-class EfficientNet on Raspberry Pi Zero-W. For the PLACES365 dataset, the 3-class EfficientNet (full resolution) is slightly more accurate than our approach but it comes with a cost of $100\%$ more latency. For the Camera Trap, 3-class EfficientNet gains $3\%$, though it sacrifices the latency by being $2.6\times$ slower than our approach. \M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}
    

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}


\begin{table*}[h]
\scalebox{0.45}{
\begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
\toprule
Methods & \multicolumn{5}{c|}{Camera Trap - ResNet-50} & \multicolumn{5}{c|}{STL-10 - ResNet-50} & \multicolumn{5}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers (ms)} & \multicolumn{1}{l|}{$\mu$C Switches (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers (ms)} & \multicolumn{1}{l|}{$\mu$C Switches (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers (ms)} & \multicolumn{1}{l|}{$\mu$C Switches (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) \\ \midrule
Our Approach & 82.98\% & 8.00 & 10.28 & 216.78 & 72.57 & 93.64\% & 0.74 & 10.32 & 77.81 & 30.02 & 96.01\% & 2.32 & 9.52 & 263.28 & 90.40 \\
Oracle $\mu$Classifier & 83.21\% & 8.02 & 9.96 & 216.67 & 71.88 & 94.00\% & 0.69 & 9.80 & 79.75 & 30.53 & 96.39\% & 2.24 & 9.64 & 286.12 & 98.48\\
3-class EfficientNet (full res) & 86.03\% & 6.08 & 14.58 & 822.56 & 264.29 & 96.06\% & 0.46 & 12.57 & 107.38 & 41.73 & 97.36\% & 1.70 & 12.25 & 520.33 & 179.72\\
All-Class EfficientNet (full res) & 83.00\% & 0.00 & 0.00 & 833.40 & 264.29 & 92.13\% & 0.00 & 0.00 & 107.88 & 41.77 & 90.95\% & 0.00 & 0.00 & 521.12 & 180.01 \\

\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}






% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}



\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{5 $\mu$Cs} & \multicolumn{3}{c|}{15 $\mu$Cs}  & \multicolumn{3}{c}{30 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms)\\ \midrule
Greedy & 82.41\% & 272.58 & 88.35 & - & -\% & - & -\% & - & - \\
Random $\mu$Classifier & 82.36\% & 337.74 & 110.89 & - & -\% & - & -\% & -& - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{Local-Switching; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}

==> Backup/Mar12/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant interest in recent years in bringing advances in deep learning to low-power embedded systems running on microcontrollers and other specialized low-power accelerators that are common in IoT devices \cite{vlin2021memory,warden2019tinyml,mazumder2021survey,lai2018enabling}. These platforms are highly resource constrained since they need to operate at very low energy budgets (typically a few milliwatts on average), to ensure that they can run for weeks or months on battery power.

Prior approaches to optimize deep learning models on resource-constrained devices fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first category is approaches to shrink the model via pruning, quantization, and knowledge distillation. For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. %Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 

The second category of approaches is early exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently.

The third line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. 

% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/alternatives.png}
    \caption{Prior approaches for addressing IoT resource limitations either squeeze larger models or partition large models across IoT devices and a more powerful remote device. \DG{Needs to be re-drawn - this is just a sketch}\HG{remove compression and sparsification when redraw since sparsification belongs to pruning; both pruning and quantization belongs to compression}}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference.} One approach that has not been explored in prior efforts is \emph{context-aware inference}. Context awareness can improve efficiency because it can shrink the \emph{number of classes} that need to be classified to be those relevant to the current context. This allows us to change a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. For example, a backyard camera may be primarily observing a dog or child playing for a certain period of time. In other words, the current context may have only a subset of classes of interest. When compute and memory are scarce, it can make a big difference whether the classifier needs to classify between 10 classes or three classes. We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a few of the overall set of classes that relevant to the current context, making it more resource-efficient and accurate.

While a context-aware $\mu$Classifier can be more efficient, its design raises three key challenges. 

The first is that we need to minimize training overhead. This can be large because there are many possible subsets of classes that can occur in a given context. 
For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class micro-classifiers and $C^{20}_4$ (4845) four-class micro-classifiers that are possible. In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression. As we show later, the optimal parameters depend greatly upon the choice of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to determine context change so that we can switch to the appropriate $\mu$Classifier when the context changes, for example, when an entity that is not in the current $\mu$classifier set enters the scene. 
In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the best accuracy and coverage across classes of interest while not exceeding available storage.

\mypara{The \myname{} approach.} In this paper, we present a novel solution that addresses these problems. %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
In the classification task, we observed a direct relationship between the similarity of classes and the hardness of distinguishing them for the classifier. 
In order to quantify the similarity between two classes, the cosine distance of their embedding from a feature extractor is considered. 
A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
In order to detect the context change, a regression head is attached to $\mu$Classifiers as the second output head. Since the classification and regression heads share a feature extractor, the added overhead by the context change detector is negligible. The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.

As IoT devices are limited in resources, only a portion ($n$) of $\mu$Classifiers can be stored on the device. 
We present a greedy algorithm to select the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
    \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
    \label{fig:our-approach}
\end{figure}

We evaluate \myname{} extensively across the range of three datasets and multiple IoT processors, and show that \DG{Text below is from FLEET - can you edit with numbers from this paper}: 
\begin{itemize}
    \item Compared to local execution, \myname{} can achieve 2.3$\times$ -- 4.7$\times$ speed-up in latency and 2.1$\times$ -- 4.4$\times$ saving in energy. Compared to Edge-cloud Model Partitioning, \myname{} achieves 1.2$\times$ -- 3.3$\times$ speed-up in latency and 1.8$\times$ -- 2.6$\times$ reduction in energy. Compared with JPEG-compressed data offload, \myname{} achieves 1.7$\times$ -- 6.1$\times$ speed-up in latency and 1.6$\times$ -- 4.4$\times$ energy savings.
    \item Overall, \myname{} can achieve 1.2$\times$--4.0$\times$ reduction in latency when compared with the best of all local and remote execution baselines; \myname{} also achieves 1.2$\times$-- 2.5$\times$ saving in energy consumption. 
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    \item \myname{} outperforms baselines on a range of IoT processors (from low end Cortex-M33 \cite{URL:Cortex-M33} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A77 \cite{URL:Cortex-A77}), across different datasets (ImageNet-100, TinyImageNet and CIFAR-100), and different models (MobileNetV3, ResNet34 and InceptionV3).
    \item \myname{} is robust to packet losses and can operate seamlessly without requiring knowledge of underlying duty-cycling parameters while providing substantial latency speed-up. 
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Mar14/Case.tex <==
\section{Case for Context-aware $\mu$Classifiers}
\label{case_context}

In this section, we compare two design points in the space of classifiers for IoT devices. 
The first is the canonical method of training a model across all classes that are relevant to the IoT node, and optimizing the model with a variety of model compression and early exit based methods. 
We refer to the model as an \textit{all-class model}.
The second is our proposed class of methods that use a context-aware $\mu$Classifier that is trained only for a small set of classes that are relevant to the current context.
% , and also trained to detect changes in context. 
% If a context change event is detected, then a new $\mu$Classifier that is relevant to the new context is loaded. 
We show that there is a significant performance gap between these two approaches, and this argues for a deeper dive into the design space of switchable $\mu$Classifiers.

\mypara{Observation 1: Using fewer classes brings significant performance benefits.} Intuitively, if a classifier has fewer classes than another, it should be more accurate given the same resources. The first question that we ask is whether this gap is significant enough to argue for a $\mu$Classifier based design.


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/Acc_vs_Classes.png}
    \caption{Accuracy Drops as the classifier coverage increases}
    \label{fig:accuracy_vs_classes}
\end{figure}


To understand this, we look at the accuracy of the EfficientNet~\cite{tan2019efficientnet} for different subsets of classes from the STL-10 Dataset~\cite{STL10} and the Camera Trap dataset~\cite{} (See Section~\ref{experiment_setting} for details on the datasets). \HG{add citations for the two datasets since it is the first time the two datasets are mentioned}
Figure~\ref{fig:accuracy_vs_classes} shows the average accuracy across all 3-class subsets of the 10 classes, the 4-class subsets, and so on till 10-class subsets. 
The dynamic range post-training quantization~\cite{dynamicq} is applied to all models. We see that the accuracy drops steadily as the number of classes increases: the overall drop is by about 5\% and XX\% for STL-10 and Camera Trap respectively when we go from 3 classes to 10 classes. 
This is quite a substantial gap in performance and demonstrates that $\mu$Classifiers are more favorable than a all-class model when only a subset of classes are active.  

\mypara{Observation 2: Model compression cannot reduce this gap.} 
In the previous results, we used EfficientNet (with quantization) but did not apply a host of other techniques that are available for optimizing deep learning models for embedded MCUs~\cite{cheng2017survey}. 
This includes model compression techniques such as weight quantization, weight sparsification, filter pruning and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand}. 
We now ask whether these techniques can bridge the performance gap between $\mu$Classifiers and all-class models.

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/STL_All_Config_V3.png}
    \caption{Accuracy Drops when models get pruned. All models were quantized.}
    \label{fig:accuracy_vs_size}
\end{figure}

Figure~\ref{fig:accuracy_vs_size} shows the performance gap between 10-class and 3-class EfficientNet after model pruning and quantization on the STL-10 dataset. We applied filter pruning~\cite{str_p1} which reduces the number of filters in each layer based on $\ell_1$ norms. The accuracy of each orange point that represents a 3-class model is computed by averaging across all 3-class subsets. 
We see that the performance gap between the $\mu$Classifier and all-class classifier increases as resources reduce. 
The accuracy gap increases from about 5\% at 148Mflops to roughly 11.5\% at 70 Mflops. 
Another way to describe performance is that the $\mu$Classifier has the same accuracy as the all-class model at less than half the computational resources. 
Thus, the gap between the methods remains the same or increases as model optimization techniques are applied.


\mypara{Observation 3: The benefits hold for early exit models.} 
Another approach to reduce the computational requirements of executing models on IoT devices is to use early exit, where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers~\cite{teerapittayanon2016branchynet, kaya2019shallow,Fleet-Mobicom23}. 
We now ask whether a $\mu$Classifier outperforms all-class models with early exit capability.  

Figure~\ref{} compares the...\DG{Mohammad, please add a graph or table that compares early exit vs micro-classifer for different number of classes.\M{will be added by end of tuesday}}


\begin{comment}
\mypara{Is switching $\mu$Classifiers expensive?} 
So far, we have shown that there is significant performance benefits to using $\mu$Classifiers. The main cost of such an approach, however, is switching overhead to transition to a new model every time the current context changes. Thus, if the current context changes very frequently, the overhead of switching between $\mu$Classifiers can be significant and diminish performance.

However, in many static deployments, there is significant temporal stability and context change is not frequent. 

To illustrate, we look at how frequently the set of classes changes in the case of a trail camera or backyard camera. We use a large trail camera trap dataset \cite{} from Africa for this analysis. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. For Figure ~\ref{fig:CDF_Temporal}, we used the entire Enonkishu dataset \cite{} comprising 38 species.

Figure~\ref{fig:CDF_Temporal} shows the distribution of the number of captured unique species in a whole day by a camera. As we can see, less than 6 species show up on most days.

% \mypara{Limits of alternate approaches:} 

% There are many methods exist to reduce the computational cost of executing classifiers of IoT devices. We argue that each of these have their limitations when scaled down to small processors/resources, and it is generally beneficial to have classifiers with fewer classes.


% There are a number of existing approaches for optimizing deep learning models for embedded MCUs  \cite{cheng2017survey}. These include model compression techniques such as weight quantization, weight sparsification, compact filters and others \cite{he2018amc,liu2019metapruning,bhattacharya2016sparsification,lai2018cmsis,yao2018fastdeepiot,lane2015deepear,liu2018demand}. 

% There are also early exit methods where the model only executes until it is sufficiently confident about the result and can exit without having to run the remaining layers \cite{teerapittayanon2016branchynet, kaya2019shallow,Fleet-Mobicom23}. But all these approaches improve in accuracy and performance if fewer classes are used. 

% \begin{itemize}
% \item \emph{Graph: Accuracy vs Size.} Show that a 10 or 20 class classifier will lose accuracy quickly if squeezed below some threshold size for either method (under some resource constraints in terms of number of layers/parameters)

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/Acc_vs_Model_Size.png}
%     \caption{Accuracy Drops as the model gets smaller (Places Dataset)}
%     \label{fig:accuracy_vs_model_size}
% \end{figure}


% \item Fewer classes is better. Classifiers with fewer classes is better from performance perspective.
% \end{itemize}


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/contx_c_dist_V2.png}
    \caption{Number of unique classes per day - Camera Trap Dataset (Enonkishu).}
    \label{fig:CDF_Temporal}
\end{figure}

% \mypara{Our approach:} To summarize, we have shown that context-aware $\mu$Classifiers consume less resources and can offer \textbf{higher accuracy} in resource-constrained settings. We also see that there is typically temporal consistency in many real-world environments and context change may not be very frequent for static deployments. Thus, the overhead of switching can also potentially be kept low.

% But for the technique to work, we need to answer a few questions. First, how 
\end{comment}

==> Backup/Mar14/Design.tex <==
\section{Configuration Prediction}

% The key premise in our work is that given a total of $N$ classes, a classifier that works on only a subset of these $N$ classes can afford to be more computationally efficient compared to the classifier that works on the entire set of $N$ classes since classification tasks with fewer classes is significantly easier. 
We refer to the classifier that has $N$ classes as \textit{all-class model} while the classifier that has a subset of N classes as \textit{$\mu$Classifier}. 
The goal of configuration selector is to identify the best configuration of the $\mu$Classifier for an arbitrary subset of classes. 
We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 


A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor.  

This raises two questions. 
\begin{enumerate}
    \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
    \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
\end{enumerate}

\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. 
There are a number of techniques that can be used to shrink machine learning models including quantization, pruning, and others. 
However, $\mu$Classifiers are much more restricted than a typical 100 or 10-class classifier, implying new opportunities in exploiting accuracy and resource trade-offs. 
Hence we need to re-evaluate which methods provide sufficient dynamic range of configurations to optimize $\mu$Classifiers for IoT devices. 

We find that two methods are particularly effective for configuring $\mu$Classifiers. 
The primary one is the image resolution dimension i.e. we vary the resolution of the image that we provide as input to the $\mu$Classifier. 
This is because a) the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. 
This can be augmented with other secondary techniques such as filter pruning and quantization for further expanding the configuration space.

Thus, our overall configuration space is as follows. 
In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). 
We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient $\mu$Classifier compares to varying only model sizes. 
We see that if we only vary model sizes, we can vary the $\mu$Classifier compute requirements by roughly 2$\times$ and accuracy by roughly 5\% but if we vary both resolution and model size, this increases to a more significant performance regime of 5$\times$ in compute and 11\% in accuracy.
\HG{The conclusion doesn't really hold. Because you can always prune the model even more to achieve even lower FLOPS. It is hard to believe that filter pruning reaches a hard limit of 2X FLOPS reduction. In an extreme cases, you can always prune every layer to until there is only one filter left or all the filters are gone (the layer is removed). I think the point we want to make here is that, varying both resolution and model sizes together, we are able to find models that achieve similar accuracy but with much less FLOPS.}


\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/res_size_vs_size.png}
    \caption{Configuring resolution and model size provides us much larger dynamic range in resource-accuracy tradeoffs than only using model size. In this plot, we show results for the STL-10 dataset when we use four resolutions (58 to 96) and four pruning levels ($0\%$ to $40\%$). Resolution + model size provides us a configuration space of 5$\times$ in compute and 11\% in accuracy whereas only model size provides us a configuration space of 2$\times$ in compute and 5\% in accuracy.}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely configuration (i.e., resolution and model sizes) without needing to train a huge number of them. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of $\mu$Classifier to evaluate in order to identify the best one for an arbitrary subset of classes. 
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., an \textit{m-class combination}), we will need to train a total of $C_N^m \times R \times S$ models to find the $\mu$Classifier for every $m$-class combination, which is prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are not similar, a low model complexity suffices (performance is similar to more complex models) and when classes are similar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS). 
However, this method doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of $\mu$Classifiers on a given subset of classes, it still needs to examine $C_N^m$ number of $m$ class combinations, each of which incurs significant training overhead.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. 
Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities, they would also share a similar $\mu$Classifier configuration. 
We first define the similarity metric and show how it provides us with a simple method for determining the best configuration.

\mypara{Similarity of $m$-class combinations.} 
We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?} 
Figure~\ref{heatmap} show that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset which has a total of 10 classes. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (x-axis). 
The y-axis shows the model complexity of $\mu$Classifiers measured by FLOPS. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPS for a 3-class combination (darker is higher accuracy). 

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/knn_train.png}
    \caption{To train the kNN, we (a) use similarity-directed sampling to select a subset of classes, (b) determine the inter-class similarity and the best configuration for the subset, and (c) construct the kNN based on this data.}
    \label{fig:kNN-training}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}
Given that inter-class similarity accurately tracks resource-accuracy tradeoffs of a $\mu$Classifier, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the k-NN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


\mypara{Similarity-directed sampling.} The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration accurately. This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a similarity-directed sampling scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the k-NN.
\HG{we need some results to show the similarity-directed sampling is better than random sampling. Otherwise, we can remove this paragraph.}\M{We already have a table (it's commented out) that can be turned into a graph as well.}

% \mypara{Input for kNN training.} The input to train the kNN comprises the vector representation (Eq.~\ref{eq:rep_vector}) for the chosen m-class subsets and their best $\mu$Classifier configuration. We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 
% \DG{We need a figure to show this stage}


% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}

\section{Budget-limited $\mu$C selection}

So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for a a $m$-class combination. 
However, we may not be able to train and/or store all $m$-class subsets. This raises another question:
\begin{enumerate}
    \item How should we quickly identify which subsets should be chosen from among the $C^N_m$ $m$-class subsets of all $N$ classes.
\end{enumerate}

We look at how to choose the m-class subsets and how this can be useful for IoT deployments with and without edge-cloud support.


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to (1) cover all classes that can possibly occur in a scene, and (2) achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of the first condition is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifiers can work in any possible context. 

The problem can be re-phrased as an combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and a resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is no larger than the budget, the total accuracy is as high as possible, and all classes are covered. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{}. 
We next elaborate our greedy algorithm to approximate the optimal solution. 
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. 
In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If it is met,  the replacement happens; otherwise, the next lightest $\mu$Classifier will be trained and checked until the replacement happens. 
Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
If not, this process continues until the threshold is met. 
By experience, only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

\subsection{Local and Edge-cloud} 

We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

\mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

\mypara{Edge-cloud assisted IoT devices.} 
Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change.} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computation intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching.} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by a \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier.

As shown in Figure~\ref{}, the \emph{all-class} model can be either executed locally or at the network edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. Besides its indirect contribution to accuracy by determining the current context, the all-class model directly affects the accuracy as the IoT should rely on the prediction of the all-class model for the out-of-context frames.

One additional minutiae is the question of which classes should be replaced from the current set of classes in a $\mu$classifier if a new class is detected. We use a simple technique where the last $p$ predictions made by the IoT device are observed and the farthest predicted class among the previous set of classes is substituted by the new one. 
If the IoT device is operating autonomously without an edge-cloud, we will switch to a $\mu$Classifier that covers both the new class and the most of recent classes. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}

 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}


%  \begin{algorithm}
%         \caption{AccuComp}
%         \label{Alg2}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$C$: Output of the GreeComp Algorithm
%         \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
%         \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
%         \\$A$: Accuracy of each $\mu$Cs in $S$ (ordered according to the sorted $F$)
%         \\$N$: Total number of classes in the Dataset
%         \\$Acc_{thr}$: Desired threshold accuracy
%         \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $Acc_{Avg}=Avg\_Acc(C)$ \Comment{Average of accuracy over C}
%             \While{$Acc_{Avg}<Acc_{thr}$}
%             \State $l=Min\_Acc(C, A)$ \Comment{$\mu C$ with the lowest accuracy in C}
%             \State $acc_{low}=A[l]$
%             \State $C_{temp}=C$
%             \For{$i=1$ to $|S|$}
%             \If{$S[i] \notin C$ \& $A[i]>acc_{low}$}
%             \State del $l$ from $C$
%             \State add $S[i]$ to $C$
%             \If{$CVRG(C)==N$}
%             \State break
%             \Else
%             \State $C=C_{temp}$
%             \EndIf
%             \EndIf
%             \EndFor
%             \State $Acc_{Avg}=Avg\_Acc(C)$
%             \EndWhile     
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}
 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Mar14/Eval.tex <==




\section{Evaluation}
This section evaluates how \myname{} addresses the three challenges in Section \ref{case_context}. 
We first describe the datasets, the baselines, and evaluation metrics, and then evaluate the components of the system over datasets and real platforms. 
We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Experiment Settings}
\label{experiment_setting}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resulution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\mypara{Dataset:}
\label{dataset}
We use three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and Camera Trap \cite{}. \HG{fill in}  
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 


Places365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 


Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two cameras were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset (both from cameras in the African savvanah). Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10+1 classes to be close to the real-world setting. 

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_size}) but also requires the most switching between contexts. 
So, it helps us understand how a nimble system can be designed with $\mu$Classifiers. 
By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.



\mypara{The configuration space of $\mu$Classifiers.}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both model size and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning and get a total of four feature extractor configurations.  
The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The considered image resolutions for each dataset are provided in Table~\ref{tab:expt-settings}.  
These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (detecting context change). 
The two heads use two Fully Connected layers.
$\mu$Classifiers are fine-tuned on the target dataset before they are deployed on devices. 

\mypara{Inter-class similarity metric.}
The Configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of the all-class model ResNet-50 to extract embedding of images from a class and average the embedding into a single vector as that class' inter-class similarity representation. 


\mypara{KNN-based configuration selection.}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in Section~\ref{sec:knn}) to get 200, 40, and 40 number of 3-class combination samples from 1140, 120, and 120 in total for the three datasets PLACES, STL-10, and Camera Trap respectively. 
For each sampled 3-class combination, we train $\mu$Classifier with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved for a configuration.


\mypara{Context-aware switching.} 
As discussed in section~\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect context change. 
It is trained to output a value close to 0 for the target classes (no context change) of the $\mu$Classifier and a value around 1 for other classes (context change). 
We used $0.5$ as the decision boundary. 

Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50~\cite{resnet-50} for its high classification accuracy in case the IoT device is using a heterogeneous multi-core process or if the all-class model execution can be offloaded to the cloud and uses EfficientNet-B0~\cite{efficientnet} otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on our three target datasets.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance for different thresholds}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}


This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of the all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in smaller $\mu$Classifiers and thus less FLOPs.  



We compared the classification accuracy and computation cost of the predicted configuration (\textbf{Predicted $\mu$Classifier}) with the following baselines: 
\begin{itemize}
    \item \textbf{All-Class EfficientNet}: This uses the well-trained EfficientNet-B0 with all the classes and full image resolution, even though only three classes are of interests in a scene.  
    
    \item \textbf{3-Class EfficientNet}: We replace the classification head in all-class EfficientNet with a 3-class classification head and fine-tune the model on each 3-class combination of the target dataset. Since the model uses the same feature extractor as the all-class EfficientNet, the computation costs (in FLOPs) remains the same. 
    
    \item \textbf{Oracle $\mu$Classifier}: For a 3-class combination, we get the oracle by enumerating and training $\mu$Classifier with all possible configurations and picking the one that meets a target accuracy threshold. 
    Note that this brute force search needs to train a total of 1920, 1920, and 18240 3-class $\mu$Classifier for the three datasets STL-10, Camera Trap, and PLACES365 respectively. It takes a total of XX hours, XX-XX longer than our approach.  \HG{fill in}
\end{itemize}


Figure~\ref{knn_performance} shows how different target accuracy threshold affects the classification accuracy and the computation costs for our methods and baselines. 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   


We first compare \myname{}'s configuration predictor (orange curve) against the Oracle (blue curve). We see that the accuracy is nearly the same regardless of the target accuracy threshold, despite significantly lower training cost. 
For the STL-10 dataset, the accuracy gap between the \myname{} predicted model and the best $\mu$Classifier configuration was as small as -$0.35\%$ while the computation cost was almost equal. 
With almost the same computation cost, The biggest gap in accuracy with $-0.95\%$ is for the Camera Trap dataset. 
These results show the k-NN together with the inter-class similarity metric works well in selecting the configurations.


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

We now compare \myname{} against {all-class EfficientNet}. We see that \myname{}-predicted $\mu$Classifiers has high accuracy gain and computation savings across all three datasets. 
For the Camera Trap dataset, Our approach is $9.3\%$ more accurate than all-class EfficientNet while we save $74.79\%$ in computation. 
For the STL-10 dataset, the accuracy gain is close to $1\%$ but we obtain over $53\%$ in computation savings.

When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


% \begin{figure*}[t]%
%     \centering
%     \subfloat[\centering Camera Trap ($r=-0.904$)\label{fig:CameraTrap_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Acc_Vs_Similarity_V2.png}}}%
%     \subfloat[\centering STL-10 ($r=-0.974$) \label{fig:STL_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Acc_Vs_Similarity_V2.png}}}%
%     % \qquad
%     \subfloat[\centering PLACES365 ($r=-0.857$)\label{fig:Places_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Acc_Vs_Similarity_V2.png}}}%
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes}
% \label{acc_vs_sim_eval}
% \end{figure*}

\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/Accuracy_Vs_Similarity.png}
    \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
    \label{acc_vs_sim_eval}
\end{figure}

\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/comp_gain_Vs_Similarity.png}
    \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
    \label{speedup_vs_sim_eval}
\end{figure}

% \begin{figure*}[t]%
%     \centering
%     \subfloat[\centering Camera Trap ($r=-0.87$)\label{fig:CameraTrap_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_SpeedUp_Vs_Similarity_V2.png}}}%
%     \subfloat[\centering STL-10 ($r=-0.94$) \label{fig:STL_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Speedup_Vs_Similarity_V2.png}}}%
%     % \qquad
%     \subfloat[\centering PLACES365 ($r=-0.87$)\label{fig:Places_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Speedup_Vs_Similarity_V2.png}}}%
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
% \label{speedup_vs_sim_eval}
% \end{figure*}

\mypara{Effectiveness of the inter-class similarity metric.} We now examine the effectiveness of the proposed inter-class similarity metrics in quantifying the difficulty level of differentiating a set of classes. 
Recall that our underlying assumption in the configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold. Thus, two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. We now ask whether this is indeed the case i.e. can the difficulty level can be quantified by our proposed inter-class similarity metric? 

Figure~\ref{acc_vs_sim_eval} illustrates how the accuracy of a fixed $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.857-0.974$), indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure \ref{speedup_vs_sim_eval} looks at this relation from another performance dimension --- computation gain. The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class/3-Class EfficientNet (full resolution) while the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the simularity-aware k-NN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
 Predicted $\mu$Classifier+maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\ \hline 
Predicted $\mu$Classifier+regression head & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
Oracle $\mu$Classifier +regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
3-class EfficientNet (full res)+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. A false positive (FP) that wrongly predicts a context change, would introduce  computation costs if the all-class model is executed on device or communication costs if the all-class model is offloaded to the edge-cloud. On the other hand, a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot recognize the new class that occurs in the scene. 

To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.
% Since 3-Class EfficientNet with the full resolution is the most complex $\mu$Classifier, it is included in the table. 
% For each combination of 3 classes in the test set, a $\mu$Classifier was constructed based on the predicted configuration by the k-NN, and its FN and FP rates were calculated. 
% The mean of the FN and FP rates over all combinations in the test was reported in the table. 


Table~\ref{fpfnt} compares the FP and FN rates for our method that uses a regression head with a baseline proposed in prior work that uses the maximum probability~\cite{maxsoft1}. Overall, using a regression head is much more accurate compared to the baseline that uses the maximum probablility. The FP and FN rates of our approach are $10-20\%$ lower than the baseline.

Table~\ref{fpfnt} further reports the results of using the regression head on our predicted $\mu$Classifier, the oracle $\mu$Classifier, and the 3-class EfficientNet with full resolution. The goal is to show how the choice of $\mu$Classifier would affect the performance of the regression head, 
Note that 3-Class EfficientNet + regression head would provide a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.  
The predicted $\mu$Classifier does increase the FP and FN rates to a small extent compared to the lower bound. However, the gap between our predicted $\mu$Classifiers and the lower bound for both metrics are in the range of $2.3$ to $4.2\%$ for the Camera Trap and PLACES365 datasets, much smaller than the gap between using regression head v.s. using maximum probability. 
These values can be further lowered by increasing the $Acc_{thr}$ explained in Section \ref{sec4.4.3} as it directly affects the predicted configuration and therefore FP and FN rates.


\subsection{End-To-End Results}

In order to evaluate the end-to-end performance of \myname{}, we need to evaluate on a dataset that has context change and over a real embedded platform. The Camera Trap dataset provides us with a real-world temporal flow with context changes but other datasets and not temporal. We sequence test sets from the Places and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. We describe this below.

If we consider $m$-class combinations, the context changes whenever a frame represents a class different from the last $m$ distinct classes. 
Consider the case when $m=3$ i.e. 3-class combinations. Let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is:

\begin{equation}
    n=\lceil{CCR\times |TS|}\rceil
\end{equation}

We find that the context change rate is $3\%$ for the Camera Trap dataset when considering 3-class $\mu$Classifiers. We use this to synthesize a test set with 3\% context change for the PLACES and STL-10 datasets and use this in our evaluation unless noted differently.

To generate a test set with temporal flow, we randomly construct a sequence of $n$ m-class combinations, where every two consecutive combinations show a context change of a single class. To match the frequency of context changes to 3\%, we persist the current context for appropriate time by picking random samples from the current context. 

% In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantees n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  

% In the 3-class combination setting the context change rate is $3\%$ for the Camera Trap dataset. As this dataset has a temporal flow and it shows a real-world use case for \myname{}, its intrinsic context change rate is considered for evaluating all three datasets unless noted differently.



%  \begin{algorithm}
%         \caption{Generating a sequence of contexts}
%         \label{Alg3}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$TS$: Original test set)
%         \\$CCR$: Context change rate
%         \\$S$: List of all m-class combinations\\     
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $n = \lceil{CCR\times |TS|}\rceil$
%             \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
%             \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
%             \While{$|C|\neq n$}
%             \State $New_C = random\_choice(S)$ \Comment{New context candidate}
%             \If {$|New_C\cap Curr_C|==m-1$}
%               \State $C=C\cup New_C$
%               \State $Curr_C=New_C$
%             \EndIf
%             \EndWhile
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: A sequence of $n$ contexts  
% \end{flushleft}           
%     \end{algorithm}

\mypara{Edge-Cloud Assisted Inference.} We look at performance in an edge-cloud assisted system that uses an all-class model is ResNet-50 with WiFi data rate of $10$ Mbps for communication with edge-cloud. The latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices. Also, we assumed no $\mu$Classifiers are stored on the device which is the worst-case scenario as it requires more transmission and incereases the overall latency. The latencies that we report are the average value over the test set. 

Table \ref{End-to-end-online} shows the end-to-end results on two devices. Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 

On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less latency but $2.6\times$ speedup. c) For the STL-10 dataset, 
\M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}

\mypara{Local inference.} 
This section evaluates the performance of local inference in case there is no communication. Also, the performance of \textit{Greedy $\mu$Classifier Selector} is analyzed.

Table \ref{local_end-to-end} shows the end-to-end results with different numbers of stored $\mu$Classifiers on two devices. Overall, the \textit{Greedy $\mu$Classifier Selection} was effective in picking low-cost $\mu$Classifiers to lower the inference latency. This experiment was repeated 20 times and the average accuracy and latency were reported.

On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to the random selection of $\mu$Classifiers: a) we achieved 1.32$\times$ -- 1.38$\times$ when 20 -- 60 $\mu$Classifiers are stored on the device. Our approach provided the same accuracy when we picked 20 and 50 $\mu$Classifiers while we could gain up to 0.33$\%$ accuracy if 40 or 60 $\mu$Classifiers are supposed to be stored on the device.

\mypara{Local inference (prototype).} 

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}


\begin{table*}[h]
\scalebox{0.55}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Methods & \multicolumn{4}{c|}{Camera Trap - ResNet-50} & \multicolumn{4}{c|}{STL-10 - ResNet-50} & \multicolumn{4}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency-Comm (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency-Comm (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency-Comm (ms)} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) \\ \midrule
Our Approach & 82.48\% & 18.28 & 216.78 & 72.57 & 93.64\% & 11.06 & 77.81 & 30.02 & 96.01\% & 11.84 & 263.28 & 90.40 \\
Oracle $\mu$Classifier & 82.71\% & 17.98 & 216.67 & 71.88 & 94.00\% & 10.49 & 79.75 & 30.53 & 96.39\% & 11.88 & 286.12 & 98.48\\
3-class EfficientNet (full res) & 85.53\% & 20.66 & 822.56 & 264.29 & 96.06\% & 13.03 & 107.38 & 41.73 & 97.36\% & 13.95 & 520.33 & 179.72\\
All-Class EfficientNet (full res) & 81.62\% & 0.00 & 833.40 & 264.29 & 92.13\% & 0.00 & 107.88 & 41.77 & 90.95\% & 0.00 & 521.12 & 180.01 \\

\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}






% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}



\begin{table*}[h]
\scalebox{0.6}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Latency-Pi0 (ms)} & Latency-GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Latency-Pi0 (ms)} & Latency-GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Latency-Pi0 (ms)} & Latency-GAP8 (ms)\\ \midrule
Greedy Selection (Ours) & 80.92\% & 288.84 & - & 81.55\% & 267.41 & - & 81.65\% & 265.76 & - & 81.92\% & 264.12 & -\\
Random Selection & 81.00\% & 381.33 & - & 81.22\% & 369.33 & - & 81.60\% & 357.06 & - & 81.67\% & 351.58 & - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of Local inference; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}

==> Backup/Mar14/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant interest in recent years in bringing advances in deep learning to low-power embedded systems and IoT devices. This includes a plethora of computational architectures including low-power microcontrollers, ultra-low power neural accelerators, and heterogeneous multi-core processors that pair low-power and high-power compute elements \cite{vlin2021memory,warden2019tinyml,mazumder2021survey, lai2018enable}. While there is great diversity in the computational architecture, a common constraint across all such systems is that they tend to be highly resource constrained since they need to operate at very low energy budgets (typically a few milliwatts on average), to ensure that they can run for weeks or months on battery power.

\mypara{Squeezing deep learning models on embedded platforms.}
The diversity in low-power processors has led to a diverse range of methods for squeezing deep learning models on such devices. Prior approaches fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first is approaches to shrink the model via pruning, quantization, and knowledge distillation. For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. %Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 

The second category is early exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently.

The third category is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. 

% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations either squeeze larger models or partition large models across IoT devices and a more powerful remote device.}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference.} We argue that one dimension that has not been explored in prior efforts is \emph{context-aware inference}. Context awareness can improve efficiency because it can shrink the \emph{number of classes} that need to be classified to be those relevant to the current context. Fewer classes leads to a simpler classification problem which in turn leads to better accuracy with a resource-constrained model.

% We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. 

In many applications, context can remain static for long periods making context-aware inference particularly effective. For example, a trail camera may be seeing the same set of animals; a doorbell camera is likely to see the same types of vehicles and individuals; and a backyard camera may be primarily observing a dog or child playing for a certain period of time. In other words, the current context may have only a subset of classes of interest. When compute and memory are scarce, it can make a big difference whether the classifier needs to classify between 50 classes or three classes. We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a few of the overall set of classes that relevant to the current context, making it more resource-efficient and accurate.

% This paradigm shift necessitates a change in a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

While a context-aware $\mu$Classifier can be more efficient, its design raises three key challenges. 

The first is that we need to minimize training overhead. This can be large because there are many possible subsets of classes that can occur in a given context. 
For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class micro-classifiers and $C^{20}_4$ (4845) four-class micro-classifiers that are possible. In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression. As we show later, the optimal parameters depend greatly upon the choice of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to determine context change so that we can switch to the appropriate $\mu$Classifier when the context changes, for example, when an entity that is not in the current $\mu$classifier set enters the scene. 
In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the best accuracy and coverage across classes of interest while not exceeding available storage.

\mypara{The \myname{} approach.} In this paper, we present a novel solution that addresses these problems. %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
In the classification task, we observed a direct relationship between the similarity of classes and the hardness of distinguishing them for the classifier. 
In order to quantify the similarity between two classes, the cosine distance of their embedding from a feature extractor is considered. 
A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
In order to detect the context change, a regression head is attached to $\mu$Classifiers as the second output head. Since the classification and regression heads share a feature extractor, the added overhead by the context change detector is negligible. The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.

As IoT devices are limited in resources, only a portion ($n$) of $\mu$Classifiers can be stored on the device. 
We present a greedy algorithm to select the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
%     \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
%     \label{fig:our-approach}
% \end{figure}

We evaluate \myname{} extensively across the range of three datasets and multiple IoT processors, and show that \DG{Text below is from FLEET - can you edit with numbers from this paper}: 
\begin{itemize}
    \item In the edge-cloud assisted setting, Compared to the model that covers all classes in the dataset, \myname{} can achieve 1.2$\times$ -- 3.5$\times$ speed-up in latency and up to $5\%$ gain in accuracy. Compared to most accurate baseline, \myname{} achieves 1.3$\times$ -- 3.6$\times$ speed-up while it sacrifies 1.3$\%$ -- 3$\%$ accuracy.
    
    \item In the local switching setting, \M{will be completed after getting the results}
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
    \item \myname{} is robust to packet losses and can operate seamlessly without requiring knowledge of underlying duty-cycling parameters while providing substantial latency speed-up.\M{we may say that our approach works even for higher context change rate}
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Mar15/Design.tex <==
\section{Configuration Prediction}
\label{sec:configuration-prediction}
% The key premise in our work is that given a total of $N$ classes, a classifier that works on only a subset of these $N$ classes can afford to be more computationally efficient compared to the classifier that works on the entire set of $N$ classes since classification tasks with fewer classes is significantly easier. 

The goal of configuration selector is to identify the best configuration of the $\mu$Classifier for an arbitrary subset of classes. 
We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. 
For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 
In the rest of the paper, we refer to best configuration as the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$. 

A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions. 
\begin{enumerate}
    \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
    \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
\end{enumerate}

\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. 
While there are a number of techniques that can be used to compress machine learning models (e.g. quantization, pruning, and others), $\mu$Classifiers are much more restricted in the number of classes, necessitating a re-evaluation of the best configuration parameters to optimize $\mu$Classifiers for IoT devices.

We find that two methods are particularly effective for configuring $\mu$Classifiers. 
The primary one is the image resolution dimension i.e. we vary the resolution of the image that we provide as input to the $\mu$Classifier. 
This is because a) the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. In this work, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). 
The second one is filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

%  can be augmented with other secondary techniques such as filter pruning and quantization for further expanding the configuration space.

% Thus, our overall configuration space is as follows. 
% In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
% In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient $\mu$Classifier compares to varying only model sizes. 
We see that if we only vary model sizes, we can vary the $\mu$Classifier compute requirements by roughly 2$\times$ and accuracy by roughly 5\% but if we vary both resolution and model size, this increases to a more significant performance regime of 5$\times$ in compute and 11\% in accuracy.
\HG{The conclusion doesn't really hold. Because you can always prune the model even more to achieve even lower FLOPS. It is hard to believe that filter pruning reaches a hard limit of 2X FLOPS reduction. In an extreme cases, you can always prune every layer to until there is only one filter left or all the filters are gone (the layer is removed). I think the point we want to make here is that, varying both resolution and model sizes together, we are able to find models that achieve similar accuracy but with much less FLOPS.}


\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/res_size_vs_size.png}
    \caption{Configuring resolution and model size provides us much larger dynamic range in resource-accuracy tradeoffs than only using model size. In this plot, we show results for the STL-10 dataset when we use four resolutions (58 to 96) and four pruning levels ($0\%$ to $40\%$). Resolution + model size provides us a configuration space of 5$\times$ in compute and 11\% in accuracy whereas only model size provides us a configuration space of 2$\times$ in compute and 5\% in accuracy.}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely configuration (i.e., resolution and model sizes) without needing to train a huge number of them. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of $\mu$Classifier to evaluate in order to identify the best one for an arbitrary subset of classes. 
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., an \textit{m-class combination}), we will need to train a total of $C_N^m \times R \times S$ models to find the $\mu$Classifier for every $m$-class combination, which is prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are not similar, a low model complexity suffices (performance is similar to more complex models) and when classes are similar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS). 
However, this method doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of $\mu$Classifiers on a given subset of classes, it still needs to examine $C_N^m$ number of $m$ class combinations, each of which incurs significant training overhead.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. 
Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities, they would also share a similar $\mu$Classifier configuration. 
We first define the similarity metric and show how it provides us with a simple method for determining the best configuration.

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?} 
Figure~\ref{heatmap} show that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset which has a total of 10 classes. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (x-axis). 
The y-axis shows the model complexity of $\mu$Classifiers measured by FLOPS. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPS for a 3-class combination (darker is higher accuracy). 

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/knn_train.png}
    \caption{To train the kNN, we (a) use similarity-directed sampling to select a subset of classes, (b) determine the inter-class similarity and the best configuration for the subset, and (c) construct the kNN based on this data.}
    \label{fig:kNN-training}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}
Given that inter-class similarity accurately tracks resource-accuracy tradeoffs of a $\mu$Classifier, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the k-NN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


% \mypara{Similarity-directed sampling.} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration accurately. This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a \textbf{similarity-directed sampling} scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the k-NN.
Compared to random sampling, our empirical evaluation demonstrates that similarity-directed sampling can reduce XX-XX\% of samples while getting similar prediction accuracy. 
\HG{fill in: no need to show the table; just statistics should be fine} 
% \HG{we need some results to show the similarity-directed sampling is better than random sampling. Otherwise, we can remove this paragraph.}\M{We already have a table (it's commented out) that can be turned into a graph as well.}

% \mypara{Input for kNN training.} The input to train the kNN comprises the vector representation (Eq.~\ref{eq:rep_vector}) for the chosen m-class subsets and their best $\mu$Classifier configuration. We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 
% \DG{We need a figure to show this stage}


% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}

\section{Budget-limited $\mu$C selection}
% \HG{we do not have an evaluation section corresponding to the classifier selection component} 
So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for a a $m$-class combination. 
However, we may not be able to train and/or store all $m$-class subsets. This raises another question:
\begin{enumerate}
    \item How should we quickly identify which subsets should be chosen from among the $C^N_m$ $m$-class subsets of all $N$ classes.
\end{enumerate}

We look at how to choose the m-class subsets and how this can be useful for IoT deployments with and without edge-cloud support.


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to (1) cover all classes that can possibly occur in a scene, and (2) achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of the first condition is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifiers can work in any possible context. 

The problem can be re-phrased as an combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and a resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is no larger than the budget, the total accuracy is as high as possible, and all classes are covered. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{}. 
We next elaborate our greedy algorithm to approximate the optimal solution. 
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. 
In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If it is met,  the replacement happens; otherwise, the next lightest $\mu$Classifier will be trained and checked until the replacement happens. 
Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
If not, this process continues until the threshold is met. 
By experience, only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

\subsection{Local and Edge-cloud} 

We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

\mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

\mypara{Edge-cloud assisted IoT devices.} 
Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change.} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computation intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching.} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by a \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier.

As shown in Figure~\ref{framework_all}, the \emph{all-class} model can be either executed locally or at the network edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. Besides its indirect contribution to accuracy by determining the current context, the all-class model directly affects the accuracy as the IoT should rely on the prediction of the all-class model for the out-of-context frames.

One additional minutiae is the question of which classes should be replaced from the current set of classes in a $\mu$classifier if a new class is detected. We use a simple technique where the last $p$ predictions made by the IoT device are observed and the farthest predicted class among the previous set of classes is substituted by the new one. 
If the IoT device is operating autonomously without an edge-cloud, we will switch to a $\mu$Classifier that covers both the new class and the most of recent classes. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Mar15/Eval.tex <==
\section{Evaluation}
This section evaluates how \myname{} addresses the three challenges in Section \ref{case_context}. 
We first describe the experiment settings, and then evaluate the components of the system over datasets and real platforms. 
% We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Experiment Settings}
\label{experiment_setting}

\begin{comment}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resolution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\end{comment}

\mypara{Dataset:}
\label{dataset}
We use three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}.
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 

Places365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 

Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two cameras were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset (both from cameras in the African savvanah) to get a total of ten species. Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10 species classes + 1 empty class to be close to the real-world setting. 

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation i.e. each $\mu$Classifier has 3 places, objects or species depending on the dataset. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_size}) but also requires the most switching between contexts. 
So, it helps us evaluate the upper limits of how a nimble context-aware system can be designed with $\mu$Classifiers. 
By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. %Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

\mypara{The configuration space of $\mu$Classifiers.}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both model size and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning and get a total of four feature extractor configurations.  
The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The image resolutions that we consider for each dataset are provided in Table~\ref{tab:expt-settings}. \HG{since we remove the table, need to explain the resolutions here} 
These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
The two heads use two Fully Connected layers.
$\mu$Classifiers are fine-tuned on the target dataset before they are deployed on device. 

\mypara{Inter-class similarity metric.}
The Configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of the all-class model ResNet-50 to extract embedding of images from a class and average the embedding into a single vector as that class' inter-class similarity representation. 


\mypara{KNN-based configuration selection.}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in Section~\ref{sec:knn}) to get 200 3-class combination samples from 1140 combinations ($C^{20}_3$) in the PLACES365 dataset, and 40 out of 120 combinations ($C^{10}_3$) for the STL-10 and Camera Trap datasets. 
For each sampled 3-class combination, we train $\mu$Classifier with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved for a configuration.


\mypara{Context-aware switching.} 
As discussed in section~\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect context change. 
It is trained to output a value close to 0 for the target classes (no context change) of the $\mu$Classifier and a value around 1 for other classes (context change). 
We used $0.5$ as the decision boundary. 

Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50~\cite{resnet-50} for its high classification accuracy if higher resources are available (e.g. cloud offload or heterogeneous multi-core processor) and uses EfficientNet-B0~\cite{efficientnet} otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on our three target datasets.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance of Configuration Prediction with different accuracy thresholds.}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}

This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of the all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in smaller $\mu$Classifiers and thus less FLOPs. 

We compared the classification accuracy and computation cost of the predicted configuration (\textbf{Predicted $\mu$Classifier}) with the following baselines: 
\begin{itemize}
    \item \textbf{All-Class EfficientNet}: This uses the well-trained EfficientNet-B0 with all the classes and full image resolution, even though only three classes are of interest given the current context.  
    
    \item \textbf{3-Class EfficientNet}: We replace the classification head in all-class EfficientNet with a 3-class classification head and fine-tune the model on each 3-class combination of the target dataset. Since the model uses the same feature extractor as the all-class EfficientNet, the computation costs (in FLOPs) is the same as the above model but accuracy is higher.
    
    \item \textbf{Oracle $\mu$Classifier}: The Oracle $\mu$Classifier is the one that meets the target accuracy threshold with minimum FLOPs. For each 3-class combination, we get the oracle by enumerating and training $\mu$Classifier with all possible configurations and picking the best one. 
    Note that this brute force search needs to train a total of 18240 ($C^{20}_3$ combinations $\times 16$ configurations), 1920 ($C^{10}_3 \times 16$) and 1920 ($C^{10}_3 \times 16$) 3-class $\mu$Classifiers for the three datasets PLACES365, STL-10, and Camera Trap respectively. It takes a total of XX hours, XX-XX longer than our approach.  \HG{fill in} \DG{this needs to be highlighted as a result where you show how much you improve training time. this is one of the challenges, so we need a corresponding result.}
\end{itemize}

Figure~\ref{knn_performance} shows how different target accuracy threshold affects the classification accuracy and the computation costs for our methods and baselines. We sweep over target accuracy thresholds for the curves but the dotted horizontal line shows a specific choice of target accuracy that we use in the rest of this paper (chosen as described in \S\ref{experiment_setting}). 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   

We see that \myname{} (the orange curve) can cover a wide trade-off region between accuracy and computational cost --- accuracies vary by 3-6\% and compute by 3.5$\times$ to 10$\times$. Across this range, the accuracy is nearly as good as the Oracle (blue curve) which shows that the k-NN together with the inter-class similarity metric works well in selecting the best configuration. 

In contrast, All-Class EfficientNet (red star) and 3-class EfficientNet (green star) are point solutions. We compare these models against a specific instance of \myname{} i.e. the point where the dotted line intersects the Predicted $\mu$Classifier curve based on the threshold we choose. 
This configuration of \myname{} is XXX\% -- XXX\% more accurate than All-Class EfficientNet and requires $53\%$ to $74.79\%$ less computation to hit the target accuracy. 
When comparing against {3-Class EfficientNet}, we see that \myname{} achieves XXX-XXX\%  computation savings while sacrificing XXX-XXX\% classification accuracy. 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

% We now compare \myname{} against {all-class EfficientNet} (red star). \myname{} is between 5.1\% -- 12.3\% more accurate and requires 53\% to $74.79\%$ less computation to hit the target accuracy (horizontal dotted line).

% When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
% For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_vs_sim_eval}]{{\includegraphics[width=.23\textwidth]{figures/Accuracy_Vs_Similarity.png}}}%
    \subfloat[\centering \label{fig:comp_gain_Vs_Similarity}]{{\includegraphics[width=.24\textwidth]{figures/comp_gain_Vs_Similarity.png}}}%
    \caption{(a) The accuracy of a fixed model \HG{what is this fixed model? a 3-class full resolution efficientnet?}\M{One random configuration} drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes. (b) Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets. Similarity is normalized to [0, 1] in both figures.}
% \label{}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.25\textwidth]{figures/Accuracy_Vs_Similarity.png}
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
%     \label{acc_vs_sim_eval}
% \end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/comp_gain_Vs_Similarity.png}
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
%     \label{speedup_vs_sim_eval}
% \end{figure}

\mypara{Effectiveness of the inter-class similarity metric.} We now examine the effectiveness of the proposed inter-class similarity metrics in quantifying the difficulty level of differentiating a set of classes. 
Recall that our underlying assumption in the configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold. Thus, two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. We now ask whether this is indeed the case i.e. can the difficulty level can be quantified by our proposed inter-class similarity metric? 

Figure~\ref{fig:acc_vs_sim_eval} illustrates how the accuracy of a fixed $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.857-0.974$), indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure~\ref{fig:comp_gain_Vs_Similarity} looks at this relation from another performance dimension --- computation gain. The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class/3-Class EfficientNet (full resolution) and the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the similarity-aware k-NN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
Predicted $\mu$Classifier+regression head (\myname{}) & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
Predicted $\mu$Classifier+maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\  
Oracle $\mu$Classifier +regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
3-class EfficientNet (full res)+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\ \hline

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. A false positive (FP) that wrongly predicts a context change, would introduce additional computation costs if the all-class model is executed on device or communication costs if offloaded to the edge-cloud. On the other hand, a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot recognize the new class that occurs in the scene. 

To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.

Table~\ref{fpfnt} compares the context-change detection performance of \myname{} against several baselines: a) the same $\mu$Classifier as \myname{} but with a different approach for change detection based on max probability \cite{maxsoft1}, b) the Oracle $\mu$Classifier with regression head and c) a 3-Class EfficientNet (full res.) with regression head as a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.

\myname{}'s use of a regression head is much more accurate compared to the baseline that uses the maximum probablility. The FP and FN rates of our approach are $10-20\%$ lower than the baseline. \myname{} is quite close to the Oracle $\mu$Classifer as well. There is a gap in performance between \myname{} and the 3-class EfficientNet (2-4\% for Camera Trap and PLACES365, and 6-7\% for STL-10) but this is to be expected since we are operating with a lower accuracy target, and have considerable computational gains.
These values can be further lowered by increasing the $Acc_{thr}$ explained in Section \ref{sec:configuration-prediction} as it directly affects the predicted configuration and therefore FP and FN rates. 



\subsection{End-To-End Results}
\label{sec:end-to-end}


In order to evaluate the end-to-end performance of \myname{}, we need to evaluate on a dataset that has context change and over a real embedded platform. The Camera Trap dataset provides us with a real-world temporal flow with context changes but other datasets are not temporal. We sequence test sets from the Places and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. Specifically, we find that the context change rate is $3\%$ for the Camera Trap dataset when considering 3-class $\mu$Classifiers. We use this to synthesize a test set with 3\% context change for the PLACES365 and STL-10 datasets and use this in our evaluation unless noted differently.

% If we consider $m$-class combinations, the context changes whenever a frame represents a class different from the last $m$ distinct classes. 
% Consider the case when $m=3$ i.e. 3-class combinations. Let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

% Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is $n=\lceil{CCR\times |TS|}\rceil$.


To generate a test set with temporal flow, we randomly construct a sequence of $n$ 3-class combinations, where every two consecutive combinations show a context change of a single class. To match the frequency of context changes to 3\%, we persist the current context for appropriate time by picking random samples from the current context. 

% In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantees n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  

% In the 3-class combination setting the context change rate is $3\%$ for the Camera Trap dataset. As this dataset has a temporal flow and it shows a real-world use case for \myname{}, its intrinsic context change rate is considered for evaluating all three datasets unless noted differently.



%  \begin{algorithm}
%         \caption{Generating a sequence of contexts}
%         \label{Alg3}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$TS$: Original test set)
%         \\$CCR$: Context change rate
%         \\$S$: List of all m-class combinations\\     
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $n = \lceil{CCR\times |TS|}\rceil$
%             \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
%             \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
%             \While{$|C|\neq n$}
%             \State $New_C = random\_choice(S)$ \Comment{New context candidate}
%             \If {$|New_C\cap Curr_C|==m-1$}
%               \State $C=C\cup New_C$
%               \State $Curr_C=New_C$
%             \EndIf
%             \EndWhile
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: A sequence of $n$ contexts  
% \end{flushleft}           
%     \end{algorithm}

\mypara{Edge-Cloud Assisted Inference.} First, we look at an edge-cloud assisted system that uses ResNet-50 as the all-class model in the cloud to predict the label of the new context. The IoT communicates via WiFi with data rate of $10$ Mbps. The reported latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices. Also, we assumed no $\mu$Classifiers are stored on the device which is the worst-case scenario as it requires more transmission and increases the overall latency. We report average latencies over the test set. 

Table \ref{End-to-end-online} shows the end-to-end results on two devices. Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 

On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less latency but $2.6\times$ speedup, and c) For the STL-10 dataset, 
\M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}

\mypara{Local inference.} 
This section evaluates the performance of local inference in case there is no communication. Also, the performance of \textit{Greedy $\mu$Classifier Selector} is analyzed. EfficientNet is used as the all-class model for predicting the label of the new context.

Table \ref{local_end-to-end} shows the end-to-end results with different numbers of stored $\mu$Classifiers on two devices. This experiment was repeated 20 times and the average accuracy and latency were reported. Overall, the \textit{Greedy $\mu$Classifier Selection} was effective in picking low-cost $\mu$Classifiers to lower the inference latency.

On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to the random selection of $\mu$Classifiers: a) we achieved 1.21$\times$ -- 1.38$\times$ speedup when 20 -- 60 $\mu$Classifiers are stored on the device and b) Greedy selected $\mu$Classifiers could also gain up to 0.44$\%$ accuracy.

Table \ref{local_end-to-end} shows that the accuracy increases as we store more $\mu$Classifiers on the device. Also, only 40 $\mu$Classifiers are needed to be stored on the device to achieve the same accuracy as the All-Class EfficientNet (Table \ref{End-to-end-online}) while we still gain 3$\times$ speedup.

On the Raspberry Pi Zero-W platform, the latency slightly increases by selecting more $\mu$Classifiers. The reason is that the computation cost of the selected $\mu$Classifiers slightly increase as we expand the number of picked $\mu$Classifiers. For instance, it is expected that any other $\mu$Classifier have a higher computation cost than the chosen 20 $\mu$Classifiers as the greedy selector aims to pick the lightest $\mu$Classifiers. Although storing a high number of $\mu$Classifiers helps the device to lower the number of execution of the all-class model, it doesn't necessarily lead to lower latency in comparison to storing a small number of $\mu$Classifiers. It is due to the fact that the computation cost of the selected $\mu$Classifiers dominates the latency. In case we employ a more complex model like ResNet50 as the all-class model on the device, its computation cost may dominate the computation cost of the $\mu$Classifiers.


\mypara{Local inference (prototype).} 

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}


\begin{table*}[h]
% \scalebox{0.55}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Methods & \multicolumn{4}{c|}{Camera Trap - ResNet-50} & \multicolumn{4}{c|}{STL-10 - ResNet-50} & \multicolumn{4}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Comm} & \multicolumn{1}{c|}{Pi0} & Pi4 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Comm} & \multicolumn{1}{c|}{Pi0} & Pi4 &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Comm} & \multicolumn{1}{c|}{Pi0} & Pi4 \\
  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{} & 
  \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)} & (ms) \\ \midrule
Our Approach & 82.5\% & 18.3 & 216.8 & 72.6 & 93.6\% & 11.1 & 77.8 & 30 & 96\% & 11.8 & 263.3 & 90.4 \\
Oracle $\mu$Classifier & 82.7\% & 18 & 216.7 & 71.9 & 94\% & 10.5 & 79.8 & 30.5 & 96.4\% & 11.9 & 286.1 & 98.5\\
3-class EfficientNet (full res) & 85.5\% & 20.7 & 822.6 & 264.3 & 96.1\% & 13 & 107.4 & 41.7 & 97.4\% & 14 & 520.3 & 179.7\\
All-Class EfficientNet (full res) & 81.6\% & 0.0 & 833.4 & 264.3 & 92.1\% & 0.0 & 107.9 & 41.8 & 91\% & 0.0 & 521.1 & 180 \\
\midrule
\end{tabular}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}






% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}



\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8\\ 
  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}
    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c}{(ms)}\\ 
  \midrule
Greedy Selection (\myname{}) & 80.92\% & 266.76 & - & 81.55\% & 267.41 & - & 81.65\% & 288.84 & - & 81.97\% & 305.16 & -\\
Random Selection & 81.30\% & 352.60 & - & 81.22\% & 369.33 & - & 81.31\% & 357.06 & - & 81.53\% & 369.34 & - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of Local inference; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}



==> Backup/Mar15/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant activity in recent years in optimizing deep learning methods for low-power embedded systems and IoT devices \cite{lai2018enable, warden2019tinyml,mazumder2021survey}. 
%  vlin2021memory
% While there is great diversity in the computational capabilities (e.g. low-power microcontrollers, neural architectures and heterogeneous multi-core processors) and communication capabilities (e.g. BLE and WiFi) of these devices, they share the constraint that they are heavily resource constrained. 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.

% \mypara{Squeezing deep learning models on IoT platforms.} 
Prior approaches to squeeze deep learning models fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. 
% Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. 
%Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 
% 
The second category is partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud~\cite{huang2020clio}. 
% 
The third category is early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations either squeeze larger models or partition large models across IoT devices and a more powerful remote device.}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference and its challenges.} 
We argue that one dimension that has not been explored in prior efforts is \emph{context-aware inference}. 
Context awareness improves efficiency because it can reduce the \emph{number of classes} that need to be classified to those relevant to the current context. 
Fewer classes leads to a simpler classification problem which has better accuracy with a resource-constrained model.

% We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. 

In many applications, context can remain static for long periods making context-aware inference particularly effective. 
For example, a trail camera may be seeing the same set of animals, and a doorbell camera is likely to see the same types of vehicles and individuals. 
When compute and memory are scarce, it can make a big difference whether the classifier needs to classify between all classes or just the classes relevant to the current context.
We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a subset of the overall set of classes, making it more resource-efficient and accurate.

% This paradigm shift necessitates a change in a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

While a context-aware $\mu$Classifier can be more efficient, its design raises three key challenges. 
The first is that we need to minimize training overhead given the large number of $\mu$Classifiers. 
For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class $\mu$Classifiers and $C^{20}_4$ (4845) four-class $\mu$Classifiers that are possible. 
In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. 
%As we show later, the optimal parameters depend greatly upon the specific set of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to determine context change so that we can switch to the appropriate $\mu$Classifier when the context changes, for example, when an entity that is not in the current $\mu$classifier set enters the scene. 
In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the best accuracy and coverage across classes of interest while not exceeding available storage.

\mypara{The \myname{} approach.} We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}. 

\mypara{\myname{} contributions:} In this paper, we present a novel solution that addresses these problems. Our work has three major contributions. First, we develop a similarity-aware model configuration predictor to reduce training overhead. 
The core building block for our method is a \emph{similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the rate to invoke the heavyweight classifier.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

% In this paper, we present a novel solution that addresses these problems. 
% %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
% First, we define a inter-class similarity metric that captures the similarity of classes and the hardness of distinguishing them.
% A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
% %The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
% Second, we add a regression head to the $\mu$Classifier as the second output head to detect context changes. 
% Since the classification and regression heads share a feature extractor, the overhead for context change detection is negligible. 
% %The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.
% Third, we present a budget-limited $\mu$Classifier selector that selects the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
%     \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
%     \label{fig:our-approach}
% \end{figure}

We implement \myname{} by modifying EfficientNet and extensively evaluate across three datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}) and multiple IoT processors (low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}). We show that:
\begin{itemize}
    \item By tuning the desired accuracy threshold, \myname{} can provide up to 10$\times$ reduction in computational cost while outperforming EfficientNet across this entire range.
    \item Our inter-class similarity metric captures the hardness of a $\mu$Classifier very well (0.857-0.974 Pearson's coefficient between classification accuracy and our metric).
    \item \myname{} has good accuracy in context change detection, and matches an oracle method while outperforming other methods. \HG{this is a little vague}
    \item End-to-end results show that \myname{} can achieve 1.2$\times$ -- 3.5$\times$ speed-up and up to $5\%$ gain in accuracy in edge-cloud assisted settings, and XXX in the local setting.
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Mar16/Evatex.tex <==
\section{Evaluation}
This section evaluates how \myname{} addresses the three challenges in Section \ref{case_context}. 
We first describe the experiment settings, and then evaluate the components of the system over datasets and real platforms. 
% We show that \myname{} achieves high accuracy and frame rate for scenarios with low frequency context changes on low-resource processors.

\subsection{Experiment Settings}
\label{experiment_setting}

\begin{comment}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resolution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\end{comment}

\mypara{Dataset:}
\label{dataset}
We use three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}.
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 

Places365 is designed based on principles of human visual cognition and can be used for visual understanding tasks such as scene context, object recognition, and action prediction. 
It consists of 365 scene categories and the labels represent the entry-level of an environment. 
We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. 
From those 900 samples, 600 images were selected as the train set and the rest as the test set. 

Camera Trap images captured by trail cameras provide a real-world application of the methods in this paper. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. 
As a result, Camera Trap images from two cameras were fused to make a 10+1 classes train and test set. 
Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset (both from cameras in the African savvanah) to get a total of ten species. Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10 species classes + 1 empty class to be close to the real-world setting. 

Since the space of $\mu$Classifier possibilities is quite large, we focus on 3-class $\mu$Classifiers in our evaluation i.e. each $\mu$Classifier has 3 places, objects or species depending on the dataset. 
This represents the option with the highest accuracy on most datasets (as shown in Figure~\ref{fig:accuracy_vs_size}) but also requires the most switching between contexts. 
So, it helps us evaluate the upper limits of how a nimble context-aware system can be designed with $\mu$Classifiers. 
By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. %Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

\mypara{The configuration space of $\mu$Classifiers.}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that besides the EfficientNet-B0 we get a total of four feature extractor architectures.  
%The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The range of image resolutions is considered 58-96, 130-256, and 100-320 for STL-10, PLACES365, and Camera Trap datasets respectively. For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
The two heads use two Fully Connected layers.
$\mu$Classifiers are fine-tuned on the target dataset before they are deployed on device. 

\mypara{Inter-class similarity metric.}
The Configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
We used the feature extractor of the all-class model ResNet-50 to extract embedding of images from a class and average the embedding into a single vector as that class' inter-class similarity representation. 


\mypara{KNN-based configuration selection.}
The configuration predictor requires a set of training data which consists of a subset of 3-class combinations, their interclass-similarity vector and the best $\mu$Classifier parameters for the combination. 
To build the training data, we applied similarity-directed sampling (detailed in Section~\ref{sec:knn}) to get 200 3-class combination samples from 1140 combinations ($C^{20}_3$) in the PLACES365 dataset, and 40 out of 120 combinations ($C^{10}_3$) for the STL-10 and Camera Trap datasets. 
For each sampled 3-class combination, we train $\mu$Classifier with all 16 configurations to select the most efficient one that achieves a target accuracy. 
The target accuracy threshold for selecting the best $\mu$Classifier given a 3-class combination is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier parameters for the remaining 3-class combinations. 
kNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers 4 nearest neighbors and so on until a majority is achieved for a configuration.


\mypara{Context-aware switching.} 
As discussed in section~\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect context change. 
It is trained to output a value close to 0 for the target classes (no context change) of the $\mu$Classifier and a value around 1 for other classes (context change). 
We used $0.5$ as the decision boundary. 

Once context change is detected, this module executes an all-class model to identify which new class occur in the scene. The all-class model uses ResNet-50~\cite{resnet-50} for its high classification accuracy if higher resources are available (e.g. cloud offload or heterogeneous multi-core processor) and uses EfficientNet-B0~\cite{efficientnet} otherwise. All-class models are also pre-trained on ImageNet and fine-tuned on our three target datasets.

 

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.




\subsection{Performance of Configuration Prediction}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance of Configuration Prediction with different accuracy thresholds.}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}

This section reports the performance of the $\mu$Classifier \textit{Configuration Predictor}, whose goal is to predict the best configuration of $\mu$Classifier for any given 3-class combination. 
In this experiment, we varied the target accuracy threshold from the lowest to the highest of the all the trained $\mu$Classifiers in order to show how the threshold affects the performance of the configuration predictor. A lower target accuracy will result in smaller $\mu$Classifiers and thus less FLOPs. 

We compared the classification accuracy and computation cost of the predicted configuration (\textbf{Predicted $\mu$Classifier}) against the following baselines: (a) \textbf{All-Class EfficientNet}, which uses the well-trained EfficientNet-B0 with all the classes and full image resolution, (b) \textbf{Highest FLOPs $\mu$Classifier}, which uses the same $\mu$Classifier as \myname{} predicts but with full image resolution and no pruning (and hence computationally more expensive), and (c) \textbf{Oracle $\mu$Classifier} i.e. the $\mu$Classifier that meets the target accuracy threshold with minimum FLOPs (which would be selected by an omniscient scheme rather than the kNN-based method we use). It takes a total of 40, 120, 300 hours longer than our approach for the STL-10, Camera Trap, and PLACES365 respectively.

Figure~\ref{knn_performance} shows how different target accuracy threshold affects the classification accuracy and the computation costs for our methods and baselines. We sweep over target accuracy thresholds for the curves but the dotted horizontal line shows a specific choice of target accuracy that we use in the rest of this paper (chosen as described in \S\ref{experiment_setting}). 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.   

We see that \myname{} (the orange curve) can cover a wide trade-off region between accuracy and computational cost --- accuracies vary by 3-6\% and compute by 3.5$\times$ to 10$\times$. Across this range, the accuracy is nearly as good as the Oracle (blue curve) which shows that the k-NN together with the inter-class similarity metric works well in selecting the best configuration. 

In contrast, All-Class EfficientNet (red star) and 3-class EfficientNet (green star) are point solutions. We compare these models against a specific instance of \myname{} i.e. the point where the dotted line intersects the Predicted $\mu$Classifier curve based on the threshold we choose. 
This configuration of \myname{} is \DG{XXX\% -- XXX\%} more accurate than All-Class EfficientNet and requires $53\%$ to $74.79\%$ less computation to hit the target accuracy. 
When comparing against {3-Class EfficientNet}, we see that \myname{} achieves \DG{XXX-XXX\%}  computation savings while sacrificing \DG{XXX-XXX\%} classification accuracy. 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

% We now compare \myname{} against {all-class EfficientNet} (red star). \myname{} is between 5.1\% -- 12.3\% more accurate and requires 53\% to $74.79\%$ less computation to hit the target accuracy (horizontal dotted line).

% When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
% For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_vs_sim_eval}]{{\includegraphics[width=.23\textwidth]{figures/Accuracy_Vs_Similarity.png}}}%
    \subfloat[\centering \label{fig:comp_gain_Vs_Similarity}]{{\includegraphics[width=.24\textwidth]{figures/comp_gain_Vs_Similarity.png}}}%
    \caption{(a) The accuracy of a fixed model \HG{what is this fixed model? a 3-class full resolution efficientnet?}\M{One random configuration} drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes. (b) Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets. Similarity is normalized to [0, 1] in both figures.}
% \label{}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.25\textwidth]{figures/Accuracy_Vs_Similarity.png}
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
%     \label{acc_vs_sim_eval}
% \end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/comp_gain_Vs_Similarity.png}
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
%     \label{speedup_vs_sim_eval}
% \end{figure}

\mypara{Effectiveness of the inter-class similarity metric.} We now examine the effectiveness of the proposed inter-class similarity metrics in quantifying the difficulty level of differentiating a set of classes. 
% Recall that our underlying assumption in the configuration predictor is that, as a set of classes gets harder to distinguish, a more complex model is required to maintain accuracy over a specific threshold. Thus, two sets of classes with similar difficulty level would use similar configurations for their $\mu$Classifier. We now ask whether this is indeed the case i.e. can the difficulty level can be quantified by our proposed inter-class similarity metric? 

Figure~\ref{fig:acc_vs_sim_eval} illustrates how the accuracy of a fixed $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.857-0.974$), indicating that our similarity metric closely mirrors the difficulty level of 3-class combinations.  

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure~\ref{fig:comp_gain_Vs_Similarity} looks at this relation from another performance dimension --- computation gain. The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to All-Class/3-Class EfficientNet (full resolution) and the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the similarity-aware k-NN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.8in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
Predicted $\mu$Classifier+regression head (\myname{}) & 12.84\% & 12.75\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
Predicted $\mu$Classifier +maximum probability ~\cite{maxsoft1} & 23.21\% &25.84\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\  
Oracle $\mu$Classifier +regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
Highest FLOPs $\mu$Classifier+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\ \hline

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}



\subsection{Performance of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. 
% An accurate context change detection is important since, once the model predicts a context change, the heavyweight all-class model will need to be executed to identify the new class. 
A false positive (FP) that wrongly predicts a context change, would introduce additional cost whereas a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot detect the context change. 
To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.

Table~\ref{fpfnt} compares the context-change detection performance of \myname{} against several baselines: a) the same $\mu$Classifier as \myname{} but with a different approach for change detection based on max probability \cite{maxsoft1}, b) the Oracle $\mu$Classifier with regression head and c) a 3-Class EfficientNet (full res.) with regression head as a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.

\myname{}'s use of a regression head is much more accurate compared to the baseline that uses the maximum probablility. The FP and FN rates of our approach are $10-20\%$ lower than the baseline. \myname{} is quite close to the Oracle $\mu$Classifer as well. There is a gap in performance between \myname{} and the 3-class EfficientNet (2-4\% for Camera Trap and PLACES365, and 6-7\% for STL-10) but this is to be expected since we are operating with a lower accuracy target, and have considerable computational gains.
These values can be further lowered by increasing the $Acc_{thr}$ explained in Section \ref{sec:configuration-prediction} as it directly affects the predicted configuration and therefore FP and FN rates. 

\begin{table*}[t]
% \scalebox{0.55}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{Camera Trap - ResNet-50} & \multicolumn{3}{c|}{STL-10 - ResNet-50} & \multicolumn{3}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 \\
  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) \\ \midrule
Our Approach & 82.5\% & 235.1 & - & 93.6\% & 88.9 & - & 96.0\% & 291.0 & - \\
Oracle $\mu$Classifier & 82.7\% & 234.7 & - & 94\% & 90.3 & - & 96.4\% & 298.0 & -\\
3-class EfficientNet (full res) & 85.5\% & 843.3 & - & 96.1\% & 120.4 & - & 97.4\% & 534.3 & -\\
All-Class EfficientNet (full res) & 81.6\% & 833.4 & - & 92.1\% & 107.9 & - & 91.0\% & 521.1 & - \\
\midrule
\end{tabular}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}

\begin{figure}[h]
    \includegraphics[width=0.4\textwidth]{figures/diff_context_change.png}
    \caption{\myname{} performance with different context change rate in Edge-Cloud assisted setting. The blue curves show the end-to-end latency for PLACES365 and STL-10 datasets. The red curves show the accuracy for the two mentioned datasets.} 
    \label{diff_context_change}
\end{figure}

\begin{table*}[t]
%\scalebox{1}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c|}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8\\ 
  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}
    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c}{(ms)}\\ 
  \midrule
Greedy Selection & 80.92\% & 266.76 & - & 81.55\% & 267.41 & - & 81.65\% & 288.84 & - & 81.97\% & 305.16 & -\\
Random Selection & 81.30\% & 352.60 & - & 81.22\% & 369.33 & - & 81.31\% & 357.06 & - & 81.53\% & 369.34 & - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}
\caption{End-To-End performance of Local inference; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}

\subsection{End-To-End Results}
\label{sec:end-to-end}


In order to evaluate the end-to-end performance of \myname{}, we need to evaluate on a dataset that has context change and over a real embedded platform. The Camera Trap dataset provides us with a real-world temporal flow with context changes but other datasets are not temporal. We sequence test sets from the Places and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. Specifically, we find that the context change rate is $3\%$ for the Camera Trap dataset when considering 3-class $\mu$Classifiers. We use this to synthesize a test set with 3\% context change for the PLACES365 and STL-10 datasets and use this in our evaluation unless noted differently.

% If we consider $m$-class combinations, the context changes whenever a frame represents a class different from the last $m$ distinct classes. 
% Consider the case when $m=3$ i.e. 3-class combinations. Let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

% Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is $n=\lceil{CCR\times |TS|}\rceil$.


To generate a test set with temporal flow, we randomly construct a sequence of $n$ 3-class combinations, where every two consecutive combinations show a context change of a single class. To match the frequency of context changes to 3\%, we persist the current context for appropriate time by picking random samples from the current context. 

% In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantees n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  

% In the 3-class combination setting the context change rate is $3\%$ for the Camera Trap dataset. As this dataset has a temporal flow and it shows a real-world use case for \myname{}, its intrinsic context change rate is considered for evaluating all three datasets unless noted differently.



%  \begin{algorithm}
%         \caption{Generating a sequence of contexts}
%         \label{Alg3}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$TS$: Original test set)
%         \\$CCR$: Context change rate
%         \\$S$: List of all m-class combinations\\     
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $n = \lceil{CCR\times |TS|}\rceil$
%             \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
%             \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
%             \While{$|C|\neq n$}
%             \State $New_C = random\_choice(S)$ \Comment{New context candidate}
%             \If {$|New_C\cap Curr_C|==m-1$}
%               \State $C=C\cup New_C$
%               \State $Curr_C=New_C$
%             \EndIf
%             \EndWhile
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: A sequence of $n$ contexts  
% \end{flushleft}           
%     \end{algorithm}

\mypara{Edge-Cloud Assisted Inference.} First, we look at an edge-cloud assisted system that uses ResNet-50 as the all-class model in the cloud to predict the label of the new context. The IoT communicates via WiFi with data rate of $10$ Mbps. The reported latencies include the inference on the device, transmission of the triggered frames to the cloud, and  transmission of the classification and regression heads to devices. We assumed no $\mu$Classifiers are cached on the device which is the \emph{worst-case scenario} as it requires more transmission and increases the overall latency. We report average latencies over the test set. 

Table \ref{End-to-end-online} shows the end-to-end results on two devices. We describe results for the Raspberry Pi Zero W (results for GAP8 are similar). When compared to All-class EfficientNet, \myname{} has comparable or higher accuracy (5\% higher for the PLACES 365 dataset) but offers substantial computational gains (latency speedup of $1.2-3.5\times$). When compared to 3-class EfficientNet (the most complex $\mu$Classifier), \myname{} has $1.4-3\%$ less accuracy but $2-2.6\times$ speedup. Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 

Figure \ref{diff_context_change} shows how the end-to-end results change on the Raspberry Pi Zero W as the context change rates increase from 3\% to 9\%. The latency slowly increases from 88.9 to 100.6 and 297 to 316.4 milliseconds for the STL-10 and PLACES365 datasets respectively. Also, accuracy slightly decreases from 93.6 to 92.7 and 96 to 94.9 for the STL-10 and PLACES365 datasets respectively. Overall, \myname{} keeps its advantage in terms of accuracy and latency even with higher context change rates.

Figure \ref{diff_context_change} shows how the end-to-end results change on the Raspberry Pi Zero W as the context change rates increase from 3\% to 9\%. The latency slowly increases from 88.9 to 100.6 and 297 to 316.4 milliseconds for the STL-10 and PLACES365 datasets respectively. Also, accuracy slightly decreases from 93.6 to 92.7 and 96 to 94.9 for the STL-10 and PLACES365 datasets respectively. Overall, \myname{} keeps its advantage in terms of accuracy and latency even with higher context change rates.

% On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

% When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less accuracy but $2.6\times$ speedup, and c) For the STL-10 dataset, 
% \M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}

\mypara{Local inference.} 
This section evaluates the performance of local inference when the full-class model (EfficientNet) is executed on the local device. 

Table \ref{local_end-to-end} shows the end-to-end results with different numbers of stored $\mu$Classifiers on two platforms. This experiment was repeated 20 times and the average accuracy and latency were reported. 

Overall, the \textit{Greedy $\mu$Classifier Selection} was effective in picking low-cost $\mu$Classifiers to lower the inference latency.

On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to the random selection of $\mu$Classifiers: a) we achieved 1.21$\times$ -- 1.38$\times$ speedup when 20 -- 60 $\mu$Classifiers are stored on the device and b) Greedy selected $\mu$Classifiers could also gain up to 0.44$\%$ accuracy.

Table \ref{local_end-to-end} shows that the accuracy increases as we store more $\mu$Classifiers on the device. Also, only 40 $\mu$Classifiers are needed to be stored on the device to achieve the same accuracy as the All-Class EfficientNet (Table \ref{End-to-end-online}) while we still gain 3$\times$ speedup.

On the Raspberry Pi Zero-W platform, the latency slightly increases by selecting more $\mu$Classifiers. The reason is that the computation cost of the selected $\mu$Classifiers slightly increase as we expand the number of picked $\mu$Classifiers. For instance, it is expected that any other $\mu$Classifier have a higher computation cost than the chosen 20 $\mu$Classifiers as the greedy selector aims to pick the lightest $\mu$Classifiers. Although storing a high number of $\mu$Classifiers helps the device to lower the number of execution of the all-class model, it doesn't necessarily lead to lower latency in comparison to storing a small number of $\mu$Classifiers. It is due to the fact that the computation cost of the selected $\mu$Classifiers dominates the latency. In case we employ a more complex model like ResNet50 as the all-class model on the device, its computation cost may dominate the computation cost of the $\mu$Classifiers.


\mypara{Local inference (prototype).} 

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}








% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}






==> Backup/Mar16/Implementation.tex <==

\section{Implementation}
We tested \myname{} on several IoT accelerators and processors using three datasets. The implementation details are described below.

\subsection{Compiling Models to IoT devices:}
We implement the \myname{} pipeline on the different IoT devices including Raspberry Pi 4B, Raspberry Pi Zero W and GAP8. For the different models on the different datasets, we generate the \textbf{TensorFlow Lite} models using the default optimization and int-8 quantization to reduce the model size and the execution latency. For the profiling on raspberry Pi 4B and Zero W, we utilize the \textbf{TVM} framework to tune the operation orders to reduce the execution latency for the Arm Cores. For the profiling on GAP8, we use the gap8 tool chain to transform the \textbf{TensorFlow Lite} models into C code by fusing the operations. On all the platforms, we profile the execution latency of the models of the different configurations on the different datasets.
\mypara{Demo:}In order to better visualize how \myname{} pipeline works, we built a demo on the Raspberry Pi 4B running at $1$ GHz. The link to the demo is. The application demo is a wild-life camera that could be deployed in the wild to capture the images of the wilds and classify the different animals on the images. 

Due to the fact that Raspberry Pi has enough memory($4$GB), we could store $60$ $\mu$Classifiers and the different feature extractors. The total memory footprint to store the weights of $60$ $u$Classifiers is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images on Camera Trap dataset to visualize the demo. We also tested that using the images captured from the camera connected to the Raspberry Pi 4B is working. Given the current context($\mu$Classifiers), we resize the captured images into $4$ different sizes: $100$, $160$, $240$, $320$ and use the corresponding feature extractors and $\mu$Classifiers to generate the classification results and regression results. 

For the regression results, we use a threshold of $0.6$ to trigger the context change. When the regression results are smaller than $0.6$, we consider the current context might not be appropriate anymore and trigger the full model to do the inference again. The full model is latency-heavy on the Raspberry Pi 4B which will cost more than $600$ ms. The all-class model uses the image of the size $320$ as input and will generate the classification results of $11$ classes. Based on the classification results, we will find the most proper context. We find the new combinations of 3-class in a First-In-First-Out(\textbf{FIFO}) manner by removing the oldest classes and adding the latest predicted classes. If the new combination has no valid $\mu$Classifiers, we will iteratively remove the second and third oldest classes instead of the first one. If there is no valid combination using the heuristic, we will randomly sample one valid combination containing the predicted class. 

When the regression results are larger than the threshold, we will remain on the current context and accept the predicted $3$-class results. Overall, we find out that we could achieve $82\%$ accuracy and $16\%$ rate of triggering the all-class models.

==> Backup/Mar5/Design.tex <==
\section{Configuration Selector}
Given a total of N classes, the classifier that works on only a subset of these N classes can afford to be more computation efficient compared to the classifier that works on the N classes since the classification tasks with less classes could be easier. 
We refer to the classifier that has N classes as \textit{full-class model} while the classifier that has a subset of N classes as \textit{partial-class model}. 
$\mu$Classifiers are the most efficient partial-class models that achieve a target task accuracy on the subset of classes. 

The goal of configuration selector is to identify the architecture configuration of a $\mu$Classifiers for an arbitrary subset of classes as well as the best set of $\mu$Classifiers to be loaded on device. 
We elaborate on how configuration selectors achieves the two goals. 

\subsection{Predicting $\mu$Classifiers Configurations}

A naive way of constructing a partial-class model is to simply replace the classification head that addresses N classes with the one that addresses the target subset of classes. However, the resulting partial-class model provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head.  
To maximize computation efficiency, we need to use a more lightweight feature extractor for the partial-class model.  
This naturally raises two questions. 
\begin{enumerate}
    \item What is the configuration space of the partial-class models? 
    \item How to quickly identify the most efficient yet accurate partial-class model as the $\mu$Classifier, given a subset of classes? 
\end{enumerate}

\subsubsection{Multi-Dimension--based Configuration Space} 
To address the first question, we consider two dimensions for controlling partial-class models' computational complexity: the image resolution and the model size.
In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
We consider the image resolution dimension because the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings.  
We utilized post-training quantization to further lower the inference runtime and reduce the model size.


Figure \ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient partial-class models compares to varying only model sizes. \HG{in the figure, we need to also show what is the baseline accuracy. Expectation: with only varying model size, the accuracy is always higher than the baseline accuracy; however, by varying both resolution and the model size, we are able to have smallest FLOPs while still meeting the accuracy target. }

\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/res_size_vs_size.png}
    \caption{Resolution beside model size for the search space provides more options and flexibility in comparison to model size. Four resolutions ranging from 58 to 96 and four model sizes ranging from ... to ... are used for this plot. Blue hollow dots represent four model sizes with a fixed resolution (96). Accuracies are calculated on the STL-10 dataset.}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsubsection{k-NN--based Configuration Predictor}
\label{k-nn}
To address the second question, the configuration selector needs to efficiently search the configuration space of partial-class models. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of partial-class models to evaluate in order to identify the $\mu$Classifier for an arbitrary subset of classes, which can be time-consuming. 

Furthermore, there is no single configuration that can fit all possible class combination well.  
Figure~\ref{} illustrates problem. 
We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
\HG{fill in the figure and the number; fill in the figure.}
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., a \textit{m class combination}), we will need to train a total of $C_N^m \times R \times S$ partial-class models to find the $\mu$Classifiers for every $m$ class combination, which is prohibitively expensive.

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from high to low similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are similar, a low model complexity model suffices (performance is similar to more complex models) and when when classes are dissimilar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.}
    \label{heatmap}
\end{figure}
 
Neural Architecture Search (NAS) doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of partial-class models on a given subset of classes, it still requires to examine $C_N^m$ number of $m$ class combinations, each incurring a time-consuming training process.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture.  

Our basic idea to address the problem is to use a k-NN--based predictor. 
Each training data point for the k-NN is a pair of a m-class combination and its ground truth $\mu$Classifier configuration. 
During inference, the k-NN takes any $m$ out of $N$ classes as input and predict its $\mu$Classifier 
 configuration based on the ground truth $\mu$Classifier configuration of the $k$ most similar $m$ class combinations in the training dataset. 
We next discuss how we represent m class combinations to encode inter-combination similarity and how we construct an effective training dataset for the k-NN. 


\paragraph{Representation of  m class combinations} 
The design principle of the representation is that two m class combination that share similar representations would also like to share the similar $\mu$Classifier configuration. 
We design the vector representation of a m class combination based on statistics of \textit{inter-class similarities}--that is, the similarities among the m classes. 
The rationale is that, if the m classes are more similar to each other, the classification task addressing the m classes is more difficult and thus requires classifiers with higher computation complexity; 
if two m class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all N classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of a m class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of a m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C.
\end{equation}


% The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. 
% To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. 
% The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

\paragraph{Construction of the k-NN training dataset} 
The training dataset of the k-NN are representations of m class combinations and their corresponding ground truth $\mu$Classfier configurations. 
The challenge lies in how to sample the training data points, where each point corresponds to a m class combination. 
On the one hand, we want the samples to have a good coverage of the spectrum ranging from the easiest m-class combinations to the hardest ones. 
This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible. It is because, for each sample, we need to train all possible partial-class models to identify its ground truth $\mu$Classifer that is the most efficient while meeting a target accuracy. 
The training costs grow linearly with the number of samples we selected. 

\HG{I didn't revise this paragraph yet. This paragraph should elaborate on our similarity-directed sampling scheme; and also justify that it is better than random sampling. The table's data might be better to visualize using a graph instead of the table.} \M{Not sure if we should present the similarity-directed sampling as it is not noticeably better than random sampling, See Table \ref{sampling}}
To sample efficiently, we propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. 
The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
\begin{table}[h]
\begin{tabular}{@{}l|ccc@{}}
\toprule
Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
  &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
\midrule
20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
\bottomrule
\end{tabular}
\caption{\HG{change this table to figure}}
\label{sampling}
\end{table}



\subsection{Selecting $\mu$Classifiers} 
A device could have limited memory and storage space and thus cannot afford to keep all $\mu$Classifiers locally.  
The second goal of the Configuration Selector is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the full-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the full-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

A $\mu$Classifer may be computationally cheaper than the other, but on the other hand, it may have a higher False Positive Rate (FPR). This higher false positive rate triggers the full-class model more often and increases the overall latency. Also, the False Negative Rate (FNR) decreases the latency by mistakenly not triggering the full-class model. In order to consider the effect of the FPR and FNR we computed the expected FLOPS for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is below:

\begin{equation}
  \label{exp_comp}
  \begin{aligned}[b]
   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
 \end{aligned}
\end{equation}

In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPS of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPS of the full-class model. $F_i$ calculates the expected value of computation for an image if $\mu Classifier_{i}$ is deployed on the device.

We implemented the algorithm named GreeComp to heuristically select the lightest set of $\mu Classifiers$. The algorithm starts by initializing the set C with n random $\mu$Classifiers that cover N classes of the dataset. Then, it iteratively identifies the $\mu Classifier$ with the highest expected FLOPS in set C and replaces it with the lightest available $\mu Classifier$ that maintains the coverage of N for the updated set C. This process continues until the average of expected FLOPS over set C doesn't decrease in comparison to the previous iteration.

As mentioned in Section \ref{k-nn}, k-NN is trained to predict the lightest partial-class model meeting a target accuracy. However, It is not a perfect predictor and some predicted $\mu Classifiers$ may not meet the target accuracy. To make sure that the selected m-class combinations, on average meet the target accuracy, the AccuComp algorithm can be applied to the output of the GreeComp. AccuComp picks the $\mu Classifier$ with the lowest task accuracy in set C and replaces it with the lightest available $\mu Classifier$ with a higher task accuracy maintaining the coverage of N. AccuComp continues this until the average accuracy of $\mu Classifiers$ in set C reaches the $Acc_{thr}$.

 \begin{algorithm}
        \caption{GreeComp}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
        \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
        \\$N$: Total number of classes in the Dataset
        \\$n$: Number of desired $\mu$Cs
        \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State  Initialize $C$ with $n$ distinct random $\mu$Cs s.t $CVRG(C)==N$
            \State Initialize $New_F=0$ and $Old_F=1$
            \While{$New_F<Old_F$}
            \State $Old_F=Avg\_Comp(C)$ \Comment{Average of FLOPS over C}
            \State $m=Max\_Comp(C, F)$ \Comment{$\mu C$ with the highest FLOPS in C}
            \State $idx=Index(F(m))$
            \State $C_{temp}=C$
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C$}
            \State del $m$ from $C$
            \State add $S[i]$ to $C$
            \If{$CVRG(C)==N$}
            \State break
            \Else
            \State $C=C_{temp}$
            \EndIf
            \EndIf
            \EndFor
            \State $New_F=Avg\_Comp(C)$
            \EndWhile    
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}


 \begin{algorithm}
        \caption{AccuComp}
        \label{Alg2}
\begin{flushleft}
        \textbf{INPUT} 
        \\$C$: Output of the GreeComp Algorithm
        \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
        \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
        \\$A$: Accuracy of each $\mu$Cs in $S$ (ordered according to the sorted $F$)
        \\$N$: Total number of classes in the Dataset
        \\$Acc_{thr}$: Desired threshold accuracy
        \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State $Acc_{Avg}=Avg\_Acc(C)$ \Comment{Average of accuracy over C}
            \While{$Acc_{Avg}<Acc_{thr}$}
            \State $l=Min\_Acc(C, A)$ \Comment{$\mu C$ with the lowest accuracy in C}
            \State $acc_{low}=A[l]$
            \State $C_{temp}=C$
            \For{$i=1$ to $|S|$}
            \If{$S[i] \notin C$ \& $A[i]>acc_{low}$}
            \State del $l$ from $C$
            \State add $S[i]$ to $C$
            \If{$CVRG(C)==N$}
            \State break
            \Else
            \State $C=C_{temp}$
            \EndIf
            \EndIf
            \EndFor
            \State $Acc_{Avg}=Avg\_Acc(C)$
            \EndWhile     
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}


\section{$\mu$Classifier-based Predictor}
\label{context_change}
This component assumes a set of $\mu$Classifiers are already loaded on a device. 
The predictor executes the same $\mu$Classifier to make  predictions for input image frames that falling into the same context--that is, the expected class label of the input image frames should be one of the classes in the $\mu$Classifier. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
The key challenge in designing an accurate predictor is to precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast. 


Detecting context changes for a $\mu$Classifier is essentially to detect out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. Although many approaches have been proposed for uncertain estimation, most of them are computation intensive and thus cannot be applied in our real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. However, it doesn't have a satisfying performance in our work as the false positive an false negative rates are high. 

In this work, we introduced a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor is supposed to output a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes (new context). Classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
In case the regression head detects a new context, that frame will be sent to the \textit{New Class Detector} for further analysis.


Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. We set $\theta=0.5$ by default.

% \subsection{New Class Detector}
% Whenever the cloud receives a frame, it is fed to a huge model which covers all possible classes to detect the label of the possible new context. The oracle is supposed to have a reasonably high accuracy over the full set of classes. In case the predicted label is a member of new context classes, the covered classes by the $\mu$Classifier should be updated and the new $\mu$Classifier configuration should be selected. But the question is which class should be removed from the previous set of target classes? The last P predictions made by the IoT are observed and the least contributing class among the previous set of classes will be substituted by the new one. The new target classes are sent to the Micro-Classifier Configuration Selector. In contrast, if the predicted label by the oracle is among the current target classes, the IoT does not need to be updated with a new $\mu$Classifier.



==> Backup/Mar6/Design-old.tex <==
\section{Design Overview}
\label{des_over}
The RaSC consists of four modules.  
\textit{Configuration Selector} and \textit{$\mu$Classifier Constructor} efficiently identify the suitable configuration of the \textit{$\mu$Classifiers} for each subset of classes and materialize them offline. 
\textit{$\mu$Classifier-based predictor} and  \textit{New Class Detector} executes and enables seamlessly switches between \textit{$\mu$Classifiers} to produce accurate predictions on a device on-the-fly. 
Figure~\ref{framework_all} illustrates the four modules and their interactions in the RaSC pipeline. 


\paragraph{Configuration Selector} 
This component determines the optimal architecture configuration of a \textit{$\mu$Classifier} to achieve both high computation efficiency and task accuracy for a arbitrary subset of classes. 
It leverages a k-NN model that takes as input a vector representation for a subset of classes, and predict its appropriate \textit{$\mu$Classifier} configuration.
% We represent a subset of classes as the mean and standard deviation of pair-wise class similarities, which captures how difficult it is to achieve high accuracy for the subset.
Since not all \textit{$\mu$Classifiers} can be stored on a device, the configuration selector also determines the set of \textit{$\mu$Classifiers} that need to be loaded on device to optimize on-device efficiency.
 % leverages a greedy approach to select a set of \textit{$\mu$Classifiers} that can fit on device and achieve target task accuracy and the lowest computation cost. \HG{note that I put the selection of subset of mini-classifier here.}



% We considered several levels of image size downsampling and model size to create a configuration space. Unimportant filters in convolutional layers are pruned to compress the model. 

% The output vector of the oracle's feature extractor is considered to represent a class and the similarity between two classes is measured using the cosine distance of their vectors. statistics such as mean and std are extracted from pair-wise similarities of a set of classes. Since all possible pair-wise similarities only need to be computed once and k-NN inference is quite fast, the runtime overhead of predicting a configuration is negligible. For training the k-NN we sample a few sets of classes from different levels of hardness/similarity. To make a dataset, we extract the mentioned statistics as the input and label each set of classes with a configuration based on predefined criteria.

\paragraph{$\mu$Classifier Constructor} 
This module materializes a well-trained $\mu$Classifier based on the selected configuration by the k-NN. 
A $\mu$Classifier has a feature extractor, one class label classification head, and a context change detection head. 
The $\mu$Classifier constructor initializes the feature extractor of the  $\mu$Classifier using parameters that are trained on all classes of the dataset, and trains only the classification and detection heads using the subset of classes. 
Freezing the feature extractor has two benefits. (1) It makes the training process faster since the computation of the heads are much more lightweight compared to that of the feature extractor. (2) $\mu$Classifiers with the same configuration can share the same feature extractor, reducing space of storing $\mu$Classifiers on device.   


% The feature extractor of the $\mu$Classifier is previously fine-tuned on all classes of the dataset and will be initialized with these weights. 
% The feature extractor is kept frozen during training of the classification and context change detector heads. The training process is quite fast as the major part of the $\mu$Classifier is frozen. 
% The classification and context change detector heads are quantized and then transmitted to the IoT alongside the feature extractor ID. The feature extractor ID notifies the IoT which of the pre-stored feature extractors should be loaded on the IoT.

\paragraph{$\mu$Classifier-based Predictor}
This module executes $\mu$Classifiers on device to predict the label of an input image and detect whether a context change happens. 
If a context change is detected, the input image will be sent to another module \textit{new class detector} to further identify which new class appears.
In case a new class appear, the predictor will load another $\mu$Classifier that covers the new class and the other recently appeared classes to make predictions.  


 
 
% This part of the RASCAM architecture is responsible for detecting the new context which is essentially any class other than the current target classes. On the IoT side, there is a convolutional network called $\mu$Classifier with two output heads. One head does the classification task and the other decides whether the context has changed in the current frame or not. 

% The context change detector is a regressor and it is trained to output a number close to 1 whenever the context changes and a number close to 0 in case the current frame contains an object from the current target classes. Its architecture is shown in Figure \ref{framework1}.

\paragraph{New Class Detector} 
This module executes a model that is trained on all classes to identify the class of an input image. 
We refer to the model as a \textit{full-class model}.  
If network is available, the module can be placed on the cloud: whenever a context change is detected by the $\mu$Classifier, the image will be compressed and transmitted to the cloud so that the module can execute the full-class model to predict the class label. 
The class label will be sent back to the device for the device to make the decision on switching $\mu$Classifiers. 
If the module is placed on the device due to the lack of network connections, it loads the full-class model from storage and executes it locally. 

% The oracle is a powerful model that covers all classes in the dataset. It is fed with the frame as the input and predicts its label. If the predicted class is not in the covered set of classes by the current $\mu$Classifier, the process of preparing a new $\mu$Classifier will be started by the micro-classifier configuration selector module.


% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/framework_iot_v2.png}
%     \caption{IoT node framework}
%     \label{framework1}
% \end{figure}

\begin{figure*}[h!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_all_v2.png}
    \caption{The RASCAM architecture. \HG{need to redraw the figure to match with the text}}
    \label{framework_all}
\end{figure*}

Next, we explain the two key components \textit{Configuration Selector} and \textit{$\mu$Classifier-based Predictor} in more detail. 

\section{Configuration Selector}
Given a total of N classes, the classifier that works on only a subset of these N classes can afford to be more computation efficient compared to the classifier that works on the N classes since the classification tasks with less classes could be easier. 
We refer to the classifier that has N classes as \textit{full-class model} while the classifier that has a subset of N classes as \textit{partial-class model}. 
$\mu$Classifiers are the most efficient partial-class models that achieve a target task accuracy on the subset of classes. 

The goal of configuration selector is to identify the architecture configuration of a $\mu$Classifiers for an arbitrary subset of classes as well as the best set of $\mu$Classifiers to be loaded on device. 
We elaborate on how configuration selectors achieves the two goals. 

\subsection{Predicting $\mu$Classifiers Configurations}

A naive way of constructing a partial-class model is to simply replace the classification head that addresses N classes with the one that addresses the target subset of classes. However, the resulting partial-class model provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head.  
To maximize computation efficiency, we need to use a more lightweight feature extractor for the partial-class model.  
This naturally raises two questions. 
\begin{enumerate}
    \item What is the configuration space of the partial-class models? 
    \item How to quickly identify the most efficient yet accurate partial-class model as the $\mu$Classifier, given a subset of classes? 
\end{enumerate}

\subsubsection{Multi-Dimension--based Configuration Space} 
To address the first question, we consider two dimensions for controlling partial-class models' computational complexity: the image resolution and the model size.
In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
We consider the image resolution dimension because the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings.  
We utilized post-training quantization to further lower the inference runtime and reduce the model size.


Figure \ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient partial-class models compares to varying only model sizes. \HG{in the figure, we need to also show what is the baseline accuracy. Expectation: with only varying model size, the accuracy is always higher than the baseline accuracy; however, by varying both resolution and the model size, we are able to have smallest FLOPs while still meeting the accuracy target. }

\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/res_size_vs_size.png}
    \caption{Resolution beside model size for the search space provides more options and flexibility in comparison to model size. Four resolutions ranging from 58 to 96 and four model sizes ranging from ... to ... are used for this plot. Blue hollow dots represent four model sizes with a fixed resolution (96). Accuracies are calculated on the STL-10 dataset. \DG{Mohammad, I'm tired of seeing this figure here. Please make it more final/polished. No lines between points. Use large point markers for both (say round and star points). Then have a line like you show in figure 4 to illustrate the dynamic range you can achieve with the two methods i.e. 10x in Flops and 10\% in accuracy for res + model size and 2x in Flops and 4\% in accuracy when you vary only model size. Can you fix asap. thanks.}}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsubsection{k-NN--based Configuration Predictor}
\label{k-nn}
To address the second question, the configuration selector needs to efficiently search the configuration space of partial-class models. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of partial-class models to evaluate in order to identify the $\mu$Classifier for an arbitrary subset of classes, which can be time-consuming. 

Furthermore, there is no single configuration that can fit all possible class combination well.  
Figure~\ref{} illustrates problem. 
We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
\HG{fill in the figure and the number; fill in the figure.}
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., a \textit{m class combination}), we will need to train a total of $C_N^m \times R \times S$ partial-class models to find the $\mu$Classifiers for every $m$ class combination, which is prohibitively expensive.

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from high to low similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are similar, a low model complexity model suffices (performance is similar to more complex models) and when when classes are dissimilar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.\DG{X-axis label should be ``3-class combinations sorted by similarity''; instead of numbers 1..30 on x-axis, replace by ``high similarty'' on the left, ``medium similarity'' and ``low similarity'' on the right. Similarly, Y-axis label should be: ``Models sorted by compute complexity'' and high on top, medium middle and low on bottom (or you can use actual flops on y-axis..that might be better possibly - try both)...make sure the y-axis legends are vertical so it doesn't take too much space.}}
    \label{heatmap}
\end{figure}
 
Neural Architecture Search (NAS) doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of partial-class models on a given subset of classes, it still requires to examine $C_N^m$ number of $m$ class combinations, each incurring a time-consuming training process.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture.  

Our basic idea to address the problem is to use a k-NN--based predictor. 
Each training data point for the k-NN is a pair of a m-class combination and its ground truth $\mu$Classifier configuration. 
During inference, the k-NN takes any $m$ out of $N$ classes as input and predict its $\mu$Classifier 
 configuration based on the ground truth $\mu$Classifier configuration of the $k$ most similar $m$ class combinations in the training dataset. 
We next discuss how we represent m class combinations to encode inter-combination similarity and how we construct an effective training dataset for the k-NN. 


\paragraph{Representation of  m class combinations} 
The design principle of the representation is that two m class combination that share similar representations would also like to share the similar $\mu$Classifier configuration. 
We design the vector representation of a m class combination based on statistics of \textit{inter-class similarities}--that is, the similarities among the m classes. 
The rationale is that, if the m classes are more similar to each other, the classification task addressing the m classes is more difficult and thus requires classifiers with higher computation complexity; 
if two m class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all N classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of a m class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of a m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C.
\end{equation}


% The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. 
% To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. 
% The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

\paragraph{Construction of the k-NN training dataset} 
The training dataset of the k-NN are representations of m class combinations and their corresponding ground truth $\mu$Classfier configurations. 
The challenge lies in how to sample the training data points, where each point corresponds to a m class combination. 
On the one hand, we want the samples to have a good coverage of the spectrum ranging from the easiest m-class combinations to the hardest ones. 
This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible. It is because, for each sample, we need to train all possible partial-class models to identify its ground truth $\mu$Classifer that is the most efficient while meeting a target accuracy. 
The training costs grow linearly with the number of samples we selected. 

\HG{I didn't revise this paragraph yet. This paragraph should elaborate on our similarity-directed sampling scheme; and also justify that it is better than random sampling. The table's data might be better to visualize using a graph instead of the table.} \M{Not sure if we should present the similarity-directed sampling as it is not noticeably better than random sampling, See Table \ref{sampling}}
To sample efficiently, we propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. 
The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
\begin{table}[h]
\begin{tabular}{@{}l|ccc@{}}
\toprule
Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
  &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
\midrule
20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
\bottomrule
\end{tabular}
\caption{\HG{change this table to figure}}
\label{sampling}
\end{table}



\subsection{Selecting $\mu$Classifiers} 
A device could have limited memory and storage space and thus cannot afford to keep all $\mu$Classifiers locally.  
The second goal of the Configuration Selector is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the full-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the full-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

A $\mu$Classifer may be computationally cheaper than the other, but on the other hand, it may have a higher False Positive Rate (FPR). This higher false positive rate triggers the full-class model more often and increases the overall latency. Also, the False Negative Rate (FNR) decreases the latency by mistakenly not triggering the full-class model. In order to consider the effect of the FPR and FNR we computed the expected FLOPS for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is below:

\begin{equation}
  \label{exp_comp}
  \begin{aligned}[b]
   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
 \end{aligned}
\end{equation}

In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPS of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPS of the full-class model. $F_i$ calculates the expected value of computation for an image if $\mu Classifier_{i}$ is deployed on the device.

We implemented the algorithm named GreeComp to heuristically select the lightest set of $\mu Classifiers$. The algorithm starts by initializing the set C with n random $\mu$Classifiers that cover N classes of the dataset. Then, it iteratively identifies the $\mu Classifier$ with the highest expected FLOPS in set C and replaces it with the lightest available $\mu Classifier$ that maintains the coverage of N for the updated set C. This process continues until the average of expected FLOPS over set C doesn't decrease in comparison to the previous iteration.

As mentioned in Section \ref{k-nn}, k-NN is trained to predict the lightest partial-class model meeting a target accuracy. However, It is not a perfect predictor and some predicted $\mu Classifiers$ may not meet the target accuracy. To make sure that the selected m-class combinations, on average meet the target accuracy, the AccuComp algorithm can be applied to the output of the GreeComp. AccuComp picks the $\mu Classifier$ with the lowest task accuracy in set C and replaces it with the lightest available $\mu Classifier$ with a higher task accuracy maintaining the coverage of N. AccuComp continues this until the average accuracy of $\mu Classifiers$ in set C reaches the $Acc_{thr}$.

 \begin{algorithm}
        \caption{GreeComp}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
        \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
        \\$N$: Total number of classes in the Dataset
        \\$n$: Number of desired $\mu$Cs
        \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State  Initialize $C$ with $n$ distinct random $\mu$Cs s.t $CVRG(C)==N$
            \State Initialize $New_F=0$ and $Old_F=1$
            \While{$New_F<Old_F$}
            \State $Old_F=Avg\_Comp(C)$ \Comment{Average of FLOPS over C}
            \State $m=Max\_Comp(C, F)$ \Comment{$\mu C$ with the highest FLOPS in C}
            \State $idx=Index(F(m))$
            \State $C_{temp}=C$
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C$}
            \State del $m$ from $C$
            \State add $S[i]$ to $C$
            \If{$CVRG(C)==N$}
            \State break
            \Else
            \State $C=C_{temp}$
            \EndIf
            \EndIf
            \EndFor
            \State $New_F=Avg\_Comp(C)$
            \EndWhile    
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}


 \begin{algorithm}
        \caption{AccuComp}
        \label{Alg2}
\begin{flushleft}
        \textbf{INPUT} 
        \\$C$: Output of the GreeComp Algorithm
        \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
        \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
        \\$A$: Accuracy of each $\mu$Cs in $S$ (ordered according to the sorted $F$)
        \\$N$: Total number of classes in the Dataset
        \\$Acc_{thr}$: Desired threshold accuracy
        \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State $Acc_{Avg}=Avg\_Acc(C)$ \Comment{Average of accuracy over C}
            \While{$Acc_{Avg}<Acc_{thr}$}
            \State $l=Min\_Acc(C, A)$ \Comment{$\mu C$ with the lowest accuracy in C}
            \State $acc_{low}=A[l]$
            \State $C_{temp}=C$
            \For{$i=1$ to $|S|$}
            \If{$S[i] \notin C$ \& $A[i]>acc_{low}$}
            \State del $l$ from $C$
            \State add $S[i]$ to $C$
            \If{$CVRG(C)==N$}
            \State break
            \Else
            \State $C=C_{temp}$
            \EndIf
            \EndIf
            \EndFor
            \State $Acc_{Avg}=Avg\_Acc(C)$
            \EndWhile     
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}


\section{$\mu$Classifier-based Predictor}
\label{context_change}
This component assumes a set of $\mu$Classifiers are already loaded on a device. 
The predictor executes the same $\mu$Classifier to make  predictions for input image frames that falling into the same context--that is, the expected class label of the input image frames should be one of the classes in the $\mu$Classifier. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
The key challenge in designing an accurate predictor is to precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast. 


Detecting context changes for a $\mu$Classifier is essentially to detect out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. Although many approaches have been proposed for uncertain estimation, most of them are computation intensive and thus cannot be applied in our real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. However, it doesn't have a satisfying performance in our work as the false positive an false negative rates are high. 

In this work, we introduced a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor is supposed to output a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes (new context). Classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
In case the regression head detects a new context, that frame will be sent to the \textit{New Class Detector} for further analysis.


Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. We set $\theta=0.5$ by default.

% \subsection{New Class Detector}
% Whenever the cloud receives a frame, it is fed to a huge model which covers all possible classes to detect the label of the possible new context. The oracle is supposed to have a reasonably high accuracy over the full set of classes. In case the predicted label is a member of new context classes, the covered classes by the $\mu$Classifier should be updated and the new $\mu$Classifier configuration should be selected. But the question is which class should be removed from the previous set of target classes? The last P predictions made by the IoT are observed and the least contributing class among the previous set of classes will be substituted by the new one. The new target classes are sent to the Micro-Classifier Configuration Selector. In contrast, if the predicted label by the oracle is among the current target classes, the IoT does not need to be updated with a new $\mu$Classifier.



==> Backup/Mar6/Design.tex <==
\section{Configuration Controller}

The key premise in our work is that given a total of N classes, a classifier that works on only a subset of these N classes can afford to be more computationally efficient compared to the classifier that works on the entire set of N classes since the classification tasks with less classes is significantly easier. 
We refer to the classifier that has N classes as \textit{full-class model} while the classifier that has a subset of N classes as \textit{partial-class model}. 

The goal of configuration selector is to identify the architecture configuration of the most efficient partial-class model i.e. $\mu$Classifier that can achieve a target task accuracy for an arbitrary subset of classes. We elaborate on how configuration selectors achieves this goal.

% \subsection{Predicting $\mu$Classifiers Configurations}

A naive way of constructing a partial-class model is to simply replace the \emph{full-class} model's classification head that targets N classes with a head that targets the desired subset of classes in the $\mu$Classifier. However, the resulting partial-class model provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, if we want to achieve computational savings from a $\mu$Classifier, we need to use a more lightweight feature extractor for the partial-class model.  

This naturally raises two questions. 
\begin{enumerate}
    \item What parameters should we tune to have a large resource-accuracy configuration space of the partial-class models? 
    \item How to quickly identify the most efficient yet accurate partial-class model as the $\mu$Classifier, given a subset of classes?
\end{enumerate}

\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. There are a number of techniques that can be used to shrink machine learning models including quantization, pruning, sparsification, and others. However, we find that these are not sufficient by themselves since they do not provide a sufficiently large dynamic range of configurations to optimize $\mu$Classifiers for IoT devices. 

Hence, we also add the image resolution dimension i.e. we vary the resolution of the image that we provide as input to the $\mu$Classifier. This is because a) the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes.

Thus, our overall configuration space is as follows. In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure \ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient partial-class models compares to varying only model sizes. We see that if we only vary model size, we can vary the $\mu$Classifier compute requirements by roughly 2$\times$ and accuracy by roughly 5\% but if we vary both resolution and model size, this increases to a more significant performance regime of 5$\times$ in compute and 11\% in accuracy.

\HG{in the figure, we need to also show what is the baseline accuracy. Expectation: with only varying model size, the accuracy is always higher than the baseline accuracy; however, by varying both resolution and the model size, we are able to have smallest FLOPs while still meeting the accuracy target. }

\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/res_size_vs_size.png}
    \caption{Resolution beside model size for the search space provides more options and flexibility in comparison to model size. Four resolutions ranging from 58 to 96 and four model sizes ranging from ... to ... are used for this plot. Blue hollow dots represent four model sizes with a fixed resolution (96). Accuracies are calculated on the STL-10 dataset.}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely parameters for the best configuration without needing to train a huge number of partial-class models. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of partial-class models to evaluate in order to identify the $\mu$Classifier for an arbitrary subset of classes. Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., a \textit{m class combination}), we will need to train a total of $C_N^m \times R \times S$ partial-class models to find the $\mu$Classifiers for every $m$ class combination, which is prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are not similar, a low model complexity model suffices (performance is similar to more complex models) and when when classes are similar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS); however, this method doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of partial-class models on a given subset of classes, it still needs to examine $C_N^m$ number of $m$ class combinations, each of which incurs significant training overhead.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities, they would also share a similar $\mu$Classifier configuration. We first define the similarity metric and show how it provides us with a simple method for determining the best configuration.

\mypara{Similarity of $m$-class combinations.} 
We design the vector ``similarity'' representation of a $m$ class partial-class model based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the m classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity; 
if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of a $m$ class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of a m class combination $C$, where $|C|=m$, is:
\begin{equation}
    \label{rep_vector}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C.
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?}Figure~\ref{heatmap} show that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different combinations of three classes from the  STL-10 image classification dataset which has a total of 10 classes. We sort these combinations in terms of their mean similarity (Eq \ref{rep_vector}) from low to high (x-axis). The y-axis shows the accuracy (darker is higher accuracy). 

When inter-class similarity is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when inter-class similarity is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.

Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.

% The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. 
% To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. 
% The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

\subsection{kNN-based configuration selection}

Given that inter-class similarity accurately tracks resource-accuracy tradeoffs of a partial-class model, we can use a kNN-based predictor to predict which configuration parameters to choose for a given combination of classes. 

% Each training data point for the k-NN is a pair of a m-class combination and its ground truth $\mu$Classifier configuration. 
% During inference, the k-NN takes any $m$ out of $N$ classes as input and predicts its $\mu$Classifier 
%  configuration based on the ground truth $\mu$Classifier configuration of the $k$ most similar $m$ class combinations in the training dataset. 
% We next discuss how we represent m class combinations to encode inter-combination similarity and how we construct an effective training dataset for the k-NN. 


The k-NN takes as input the vector representation of the desired $m$ class combination and predicts the configuration that is most efficient for the combination.

The challenge lies in how to train the kNN in a resource-efficient manner. On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration accurately. This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible partial-class models to identify the $\mu$classifier configuration that is the most efficient while meeting a target accuracy. Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. We then cluster them into three groups of similarity (bottom third, middle third, and top third percentiles). We then sample randomly from each cluster to gather enough data samples for training the k-NN. 

\DG{We need a figure to show this stage}

% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}


\section{Context-aware Switching}
\label{context_change}
% This component assumes a set of $\mu$Classifiers are already loaded on a device. 

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast. 

% The predictor executes the same $\mu$Classifier to make  predictions for input image frames that falling into the same context--that is, the expected class label of the input image frames should be one of the classes in the $\mu$Classifier. 

\mypara{Detecting context change.} The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. Although many approaches have been proposed for uncertainty estimation, most of them are computation intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. We set $\theta=0.5$ by default.

\mypara{Classifier switching.} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by a \emph{full-class} model that determines which are the classes that need to be included in the new $\mu$classifier.

As shown in Figure~\ref{}, the \emph{full-class} model can be either executed locally or at the network edge cloud depending on connectivity. Executing the full-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. Besides its indirect contribution to accuracy by determining the current context, the full-class model directly affects the accuracy as the Iot should rely on the prediction of the full-class model for the out-of-context frames.

One additional minutiae is the question of which classes should be replaced from the current set of classes in a $\mu$classifier if a new class is detected. We use a simple technique where the last $p$ predictions made by the IoT device are observed and the farthest predicted class among the previous set of classes is substituted by the new one. 

\section{Budget-limited $\mu$C selection} 

We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the full-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the full-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{full-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

\begin{equation}
  \label{exp_comp}
  \begin{aligned}[b]
   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
 \end{aligned}
\end{equation}

In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the full-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

\DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

\mypara{Greedy $\mu$classifier selection.} 
Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
%         \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
%         \\$N$: Total number of classes in the Dataset
%         \\$n$: Number of desired $\mu$Cs
%         \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State  Initialize $C$ with $n$ distinct random $\mu$Cs s.t $CVRG(C)==N$
%             \State Initialize $New_F=0$ and $Old_F=1$
%             \While{$New_F<Old_F$}
%             \State $Old_F=Avg\_Comp(C)$ \Comment{Average of FLOPS over C}
%             \State $m=Max\_Comp(C, F)$ \Comment{$\mu C$ with the highest FLOPS in C}
%             \State $idx=Index(F(m))$
%             \State $C_{temp}=C$
%             \For{$i=1$ to $idx$}
%             \If{$S[i] \notin C$}
%             \State del $m$ from $C$
%             \State add $S[i]$ to $C$
%             \If{$CVRG(C)==N$}
%             \State break
%             \Else
%             \State $C=C_{temp}$
%             \EndIf
%             \EndIf
%             \EndFor
%             \State $New_F=Avg\_Comp(C)$
%             \EndWhile    
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


%  \begin{algorithm}
%         \caption{AccuComp}
%         \label{Alg2}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$C$: Output of the GreeComp Algorithm
%         \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
%         \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
%         \\$A$: Accuracy of each $\mu$Cs in $S$ (ordered according to the sorted $F$)
%         \\$N$: Total number of classes in the Dataset
%         \\$Acc_{thr}$: Desired threshold accuracy
%         \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $Acc_{Avg}=Avg\_Acc(C)$ \Comment{Average of accuracy over C}
%             \While{$Acc_{Avg}<Acc_{thr}$}
%             \State $l=Min\_Acc(C, A)$ \Comment{$\mu C$ with the lowest accuracy in C}
%             \State $acc_{low}=A[l]$
%             \State $C_{temp}=C$
%             \For{$i=1$ to $|S|$}
%             \If{$S[i] \notin C$ \& $A[i]>acc_{low}$}
%             \State del $l$ from $C$
%             \State add $S[i]$ to $C$
%             \If{$CVRG(C)==N$}
%             \State break
%             \Else
%             \State $C=C_{temp}$
%             \EndIf
%             \EndIf
%             \EndFor
%             \State $Acc_{Avg}=Avg\_Acc(C)$
%             \EndWhile     
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}
 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Mar6/Design2.tex <==
\section{Configuration Prediction}

The key premise in our work is that given a total of $N$ classes, a classifier that works on only a subset of these $N$ classes can afford to be more computationally efficient compared to the classifier that works on the entire set of $N$ classes since classification tasks with fewer classes is significantly easier. 
We refer to the classifier that has $N$ classes as \textit{full-class model} while the classifier that has a subset of N classes as \textit{partial-class model}. 

The goal of configuration selector is to identify the architecture configuration of the most efficient partial-class model i.e. $\mu$Classifier that can achieve a target task accuracy for an arbitrary subset of classes. 

% \subsection{Predicting $\mu$Classifiers Configurations}

A naive way of constructing a partial-class model is to simply replace the \emph{full-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes in the $\mu$Classifier. However, the resulting partial-class model provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, if we want to achieve computational savings from a $\mu$Classifier, we need to use a more lightweight feature extractor for the partial-class model.  

This naturally raises two questions. 
\begin{enumerate}
    \item What parameters should we tune to have a large resource-accuracy configuration space of partial-class models? 
    \item How to quickly identify the most efficient yet accurate partial-class model as the $\mu$Classifier, given a subset of classes?
\end{enumerate}

\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. There are a number of techniques that can be used to shrink machine learning models including quantization, pruning or sparsification, and others. However, $\mu$Classifiers are much more restricted than a typical 100 or 10-class classifier, hence we need to re-evaluate which methods provide sufficient dynamic range of configurations to optimize $\mu$Classifiers for IoT devices. 

We find that two methods are particularly effective for configuring $\mu$Classifiers. The primary one is the image resolution dimension i.e. we vary the resolution of the image that we provide as input to the $\mu$Classifier. This is because a) the computation complexity of a feature extractor decreases quadratically as the resolution (both height and width) of images decreases, leading to a significant amount of computation savings, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. This can be augmented with other secondary techniques such as filter pruning and quantization for further expanding the configuration space.

Thus, our overall configuration space is as follows. In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure \ref{res_size_vs_size} shows that varying both image resolution and the model size allows much more efficient partial-class models compares to varying only model sizes. We see that if we only vary model size, we can vary the $\mu$Classifier compute requirements by roughly 2$\times$ and accuracy by roughly 5\% but if we vary both resolution and model size, this increases to a more significant performance regime of 5$\times$ in compute and 11\% in accuracy.

% \HG{in the figure, we need to also show what is the baseline accuracy. Expectation: with only varying model size, the accuracy is always higher than the baseline accuracy; however, by varying both resolution and the model size, we are able to have smallest FLOPs while still meeting the accuracy target. }

\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/res_size_vs_size.png}
    \caption{Configuring resolution and model size provides us much larger dynamic range in resource-accuracy tradeoffs than only using model size. In this plot, we show results for the STL-10 dataset when we use four resolutions (58 to 96) and four model sizes (XXX to XXX). Resolution + model size provides us a configuration space of 5$\times$ in compute and 11\% in accuracy whereas only model size provides us a configuration space of 2$\times$ in compute and 5\% in accuracy.}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely parameters for the best configuration without needing to train a huge number of partial-class models. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ amount of partial-class models to evaluate in order to identify the $\mu$Classifier for an arbitrary subset of classes. Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of N classes (i.e., a \textit{m class combination}), we will need to train a total of $C_N^m \times R \times S$ partial-class models to find the $\mu$Classifiers for every $m$ class combination, which is prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to similarity among classes. X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolution) sorted from least to most compute complexity. We see that when classes are not similar, a low model complexity model suffices (performance is similar to more complex models) and when when classes are similar, there is a significant performance drop if a low complexity model is chosen. Thus, the choice of $\mu$Classifier complexity depends greatly on the similarity among classes.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS); however, this method doesn't address the problem due to two fundamental limitations. 
First, although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of partial-class models on a given subset of classes, it still needs to examine $C_N^m$ number of $m$ class combinations, each of which incurs significant training overhead.
Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities, they would also share a similar $\mu$Classifier configuration. We first define the similarity metric and show how it provides us with a simple method for determining the best configuration.

\mypara{Similarity of $m$-class combinations.} 
We design the vector ``similarity'' representation of a $m$ class partial-class model based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the m classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity; 
if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of a $m$ class combination is the mean and standard deviation of similarities among all the two class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of a m class combination $C$, where $|C|=m$, is:
\begin{equation}
    \label{rep_vector}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C.
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?} 
Figure~\ref{heatmap} show that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset which has a total of 10 classes. We sort these combinations in terms of their mean similarity (Eq \ref{rep_vector}) from low to high (x-axis). The y-axis shows the accuracy (darker is higher accuracy). 

When inter-class similarity is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when inter-class similarity is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.

Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.

% The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. 
% To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. 
% The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

\subsection{kNN-based configuration selection}

Given that inter-class similarity accurately tracks resource-accuracy tradeoffs of a partial-class model, we can use a kNN-based predictor to predict which configuration parameters to choose for a given combination of classes. 

As shown in Figure~\ref{}, the k-NN takes as input the vector representation of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 

% Each training data point for the k-NN is a pair of a m-class combination and its ground truth $\mu$Classifier configuration. 
% During inference, the k-NN takes any $m$ out of $N$ classes as input and predicts its $\mu$Classifier 
%  configuration based on the ground truth $\mu$Classifier configuration of the $k$ most similar $m$ class combinations in the training dataset. 
% We next discuss how we represent m class combinations to encode inter-combination similarity and how we construct an effective training dataset for the k-NN. 

\mypara{Similarity-directed sampling.} The challenge lies in how to train the kNN in a resource-efficient manner. On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration accurately. This is critical to ensure performance of k-NN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible partial-class models to identify the $\mu$classifier configuration that is the most efficient while meeting a target accuracy. Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. We then cluster them into three groups of similarity (bottom third, middle third, and top third percentiles). We then sample randomly from each cluster to gather enough data samples for training the k-NN. \DG{why not four groups - quartiles is easier to state (not crucial)}

\mypara{Input for kNN training.} The input to train the kNN comprises the inter-class similarity vector for the chosen m-class subset, and the most efficient configuration corresponding to the m classes. We note that the ``most efficient configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 

\DG{We need a figure to show this stage}

% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}

\section{Optimizing training costs}

Once we have constructed the kNN, the configuration controller can be used to optimize the training costs in different ways. In the basic case we considered above, we use it only to determine the configuration parameters for a desired $m$-class model. However, the question of which m-class subsets to choose from among the entire set of $N$ classes has not yet been addressed. We look at how to choose the m-class subsets and how this can be useful for IoT deployments with and without edge-cloud support.
 
\subsection{Budget-limited $\mu$C selection} 

% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the full-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the full-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{full-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

\begin{equation}
  \label{exp_comp}
  \begin{aligned}[b]
  &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
  &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
 \end{aligned}
\end{equation}

In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the full-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

\DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

\mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. 
Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$). 

Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method uses the kNN to identify the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration. Note that this selection procedure is done solely with the predictions from the kNN and does not involve training.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy, FPR and FNR. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and uses the kNN to predict a replacement i.e. the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. This model is now trained and the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

\subsection{Local and Edge-cloud} 

We now look at how the kNN and budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments. We look at two deployment scenarios (shown in Figure~\ref{}). 

\mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on-board the device prior to deployment. The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, we need to use the budget-limited $\mu$Classifier selection process to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

\mypara{Edge-cloud assisted IoT devices.} The second scenario is when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are downloaded to the IoT device.

Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decid which models to cache at the IoT device given its resource limitations.

\section{Context-aware Switching}
\label{context_change}
% This component assumes a set of $\mu$Classifiers are already loaded on a device. 

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast. 

% The predictor executes the same $\mu$Classifier to make  predictions for input image frames that falling into the same context--that is, the expected class label of the input image frames should be one of the classes in the $\mu$Classifier. 

\mypara{Detecting context change.} The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. Although many approaches have been proposed for uncertainty estimation, most of them are computation intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the partial-class models as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. We set $\theta=0.5$ by default.

\mypara{Classifier switching.} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by a \emph{full-class} model that determines which are the classes that need to be included in the new $\mu$classifier.

As shown in Figure~\ref{}, the \emph{full-class} model can be either executed locally or at the network edge cloud depending on connectivity. Executing the full-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. Besides its indirect contribution to accuracy by determining the current context, the full-class model directly affects the accuracy as the Iot should rely on the prediction of the full-class model for the out-of-context frames.

One additional minutiae is the question of which classes should be replaced from the current set of classes in a $\mu$classifier if a new class is detected. We use a simple technique where the last $p$ predictions made by the IoT device are observed and the farthest predicted class among the previous set of classes is substituted by the new one. 

\section{Budget-limited $\mu$C selection} 

We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the full-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the full-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{full-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

\begin{equation}
  \label{exp_comp}
  \begin{aligned}[b]
  &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
  &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
 \end{aligned}
\end{equation}

In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the full-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

\DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

\mypara{Greedy $\mu$classifier selection.} 
Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
%         \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
%         \\$N$: Total number of classes in the Dataset
%         \\$n$: Number of desired $\mu$Cs
%         \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State  Initialize $C$ with $n$ distinct random $\mu$Cs s.t $CVRG(C)==N$
%             \State Initialize $New_F=0$ and $Old_F=1$
%             \While{$New_F<Old_F$}
%             \State $Old_F=Avg\_Comp(C)$ \Comment{Average of FLOPS over C}
%             \State $m=Max\_Comp(C, F)$ \Comment{$\mu C$ with the highest FLOPS in C}
%             \State $idx=Index(F(m))$
%             \State $C_{temp}=C$
%             \For{$i=1$ to $idx$}
%             \If{$S[i] \notin C$}
%             \State del $m$ from $C$
%             \State add $S[i]$ to $C$
%             \If{$CVRG(C)==N$}
%             \State break
%             \Else
%             \State $C=C_{temp}$
%             \EndIf
%             \EndIf
%             \EndFor
%             \State $New_F=Avg\_Comp(C)$
%             \EndWhile    
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


%  \begin{algorithm}
%         \caption{AccuComp}
%         \label{Alg2}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$C$: Output of the GreeComp Algorithm
%         \\$S$: All $m$-class combinations (ordered according to the sorted $F$)
%         \\$F$: Expected computation/FLOPS of each $\mu$Cs in $S$ (Sorted)
%         \\$A$: Accuracy of each $\mu$Cs in $S$ (ordered according to the sorted $F$)
%         \\$N$: Total number of classes in the Dataset
%         \\$Acc_{thr}$: Desired threshold accuracy
%         \\$CVRG()$: It returns the coverage of a set of $\mu$Cs\\      
%         \textbf{Procedure}
% \end{flushleft}
%         \begin{algorithmic}
%             \State $Acc_{Avg}=Avg\_Acc(C)$ \Comment{Average of accuracy over C}
%             \While{$Acc_{Avg}<Acc_{thr}$}
%             \State $l=Min\_Acc(C, A)$ \Comment{$\mu C$ with the lowest accuracy in C}
%             \State $acc_{low}=A[l]$
%             \State $C_{temp}=C$
%             \For{$i=1$ to $|S|$}
%             \If{$S[i] \notin C$ \& $A[i]>acc_{low}$}
%             \State del $l$ from $C$
%             \State add $S[i]$ to $C$
%             \If{$CVRG(C)==N$}
%             \State break
%             \Else
%             \State $C=C_{temp}$
%             \EndIf
%             \EndIf
%             \EndFor
%             \State $Acc_{Avg}=Avg\_Acc(C)$
%             \EndWhile     
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}
 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Mar6/DesignOverview.tex <==
\section{Design Overview}
\label{des_over}

While context-aware $\mu$Classifiers consume \emph{less resources} and offer \emph{higher accuracy} in resource-constrained settings, instantiating such a system in practice requires us to track context changes and switch rapidly between $\mu$Classifers. This presents three challenges that we tackle in this paper.

\subsection{Practical Challenges}

\mypara{Challenge 1: Minimizing training overhead.} The first challenge is reducing training overhead for training a huge number of $\mu$Classifiers. For example, if there are 20 classes and we are considering 3-class $\mu$classifiers, them there are $C_{20}^3 = 1140$ $\mu$Classifers. Furthermore, each 3-class combination will need to be optimized by model compression for which we need to determine the best parameters (e.g. quantization, sparsification, etc). This requires us to train models with different parameter choices per 3-class combination to determine the $\mu$Classifier that offers the best accuracy vs computation tradeoff. If we consider 10 configurations per $\mu$Classifier, then 11400 models need to be trained. When the search space is larger, for example, 1000 classes in ImageNet \cite{}, then this increases to 166 million 3-class models which is clearly impractical.

\mypara{Challenge 2: Detecting context switch.} A second key challenge is designing an accurate predictor is to precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. Since context change detection lies on the critical path of every prediction, the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 

\mypara{Challenge 3: Addressing storage constraints.}
The large number of $\mu$Classifiers raises not just a training challenge but also a storage challenge.
An IoT device has limited storage and thus cannot afford to keep all $\mu$Classifiers locally. If the IoT device is connected to an edge cloud, it may be possible to train a $\mu$Classifier \emph{on-demand} and download the learned weights during run-time. But this incurs high communication overhead and only works for devices connected to an edge-cloud. Thus, the third challenge is to select an optimal subset of $\mu$Classifiers to load on a device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in detecting the classes and (3) low computational overhead for each $\mu$Classifier.

\subsection{\myname{} Overview}

We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}. 

\mypara{\myname{} contributions:} Our work has three major contributions. First, we develop a similarity-aware model configuration predictor to reduce training overhead. The core building block for our method is a \emph{similarity} metric to estimate the difficulty of classifying the set of classes in each $\mu$Classifer. We show that this metric is highly correlated with the choice of configuration parameters for the model, hence it allows us to rapidly and cheaply estimate the best configuration for each classifier.

Second, we split context change prediction into two parts -- a lightweight context change detector that executes as a separate head attached to the classifier, and a more heavyweight context predictor that executes as a regular classifier. This separation allows us to execute context change detection rapidly and with minimal overhead.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. Our approach leverages the above-mentioned similarity metric to reduce the search space to determine the bag of $\mu$Classifers to store on-device.

\mypara{Components:} \myname{} comprises three main components as shown in Figure~\ref{framework_all}. During the training phase, the \textit{Configuration Controller} leverages the ``simularity'' between classes to efficiently identify the suitable configuration of the $\mu$Classifier for each subset of classes. The $\mu$Classifier is a two-head model that has the class detection as one of the heads and a lightweight \textit{Context Change Detector} as the other head. 

At run-time, the \textit{Context Change Detector} rapidly detects if there is a new class in the scene without determining which is the new class. The \textit{New Class Detector} is a heavyweight classification module that executes to determine which classes are present in the scene. If a new class is detected, it triggers a ``model switch'' to load a more context-specific $\mu$Classifier.

% \paragraph{Configuration Selector} 
% This component determines the optimal architecture configuration of a \textit{$\mu$Classifier} to achieve both high computation efficiency and task accuracy for a arbitrary subset of classes. 
% It leverages a k-NN model that takes as input a vector representation for a subset of classes, and predict its appropriate \textit{$\mu$Classifier} configuration.
% % We represent a subset of classes as the mean and standard deviation of pair-wise class similarities, which captures how difficult it is to achieve high accuracy for the subset.
% Since not all \textit{$\mu$Classifiers} can be stored on a device, the configuration selector also determines the set of \textit{$\mu$Classifiers} that need to be loaded on device to optimize on-device efficiency.
%  % leverages a greedy approach to select a set of \textit{$\mu$Classifiers} that can fit on device and achieve target task accuracy and the lowest computation cost. \HG{note that I put the selection of subset of mini-classifier here.}



% % We considered several levels of image size downsampling and model size to create a configuration space. Unimportant filters in convolutional layers are pruned to compress the model. 

% % The output vector of the oracle's feature extractor is considered to represent a class and the similarity between two classes is measured using the cosine distance of their vectors. statistics such as mean and std are extracted from pair-wise similarities of a set of classes. Since all possible pair-wise similarities only need to be computed once and k-NN inference is quite fast, the runtime overhead of predicting a configuration is negligible. For training the k-NN we sample a few sets of classes from different levels of hardness/similarity. To make a dataset, we extract the mentioned statistics as the input and label each set of classes with a configuration based on predefined criteria.

% \paragraph{$\mu$Classifier Constructor} 
% This module materializes a well-trained $\mu$Classifier based on the selected configuration by the k-NN. 
% A $\mu$Classifier has a feature extractor, one class label classification head, and a context change detection head. 
% The $\mu$Classifier constructor initializes the feature extractor of the  $\mu$Classifier using parameters that are trained on all classes of the dataset, and trains only the classification and detection heads using the subset of classes. 
% Freezing the feature extractor has two benefits. (1) It makes the training process faster since the computation of the heads are much more lightweight compared to that of the feature extractor. (2) $\mu$Classifiers with the same configuration can share the same feature extractor, reducing space of storing $\mu$Classifiers on device.   


% % The feature extractor of the $\mu$Classifier is previously fine-tuned on all classes of the dataset and will be initialized with these weights. 
% % The feature extractor is kept frozen during training of the classification and context change detector heads. The training process is quite fast as the major part of the $\mu$Classifier is frozen. 
% % The classification and context change detector heads are quantized and then transmitted to the IoT alongside the feature extractor ID. The feature extractor ID notifies the IoT which of the pre-stored feature extractors should be loaded on the IoT.

% \paragraph{$\mu$Classifier-based Predictor}
% This module executes $\mu$Classifiers on device to predict the label of an input image and detect whether a context change happens. 
% If a context change is detected, the input image will be sent to another module \textit{new class detector} to further identify which new class appears.
% In case a new class appear, the predictor will load another $\mu$Classifier that covers the new class and the other recently appeared classes to make predictions.  


 
 
% % This part of the RASCAM architecture is responsible for detecting the new context which is essentially any class other than the current target classes. On the IoT side, there is a convolutional network called $\mu$Classifier with two output heads. One head does the classification task and the other decides whether the context has changed in the current frame or not. 

% % The context change detector is a regressor and it is trained to output a number close to 1 whenever the context changes and a number close to 0 in case the current frame contains an object from the current target classes. Its architecture is shown in Figure \ref{framework1}.

% \paragraph{New Class Detector} 
% This module executes a model that is trained on all classes to identify the class of an input image. 
% We refer to the model as a \textit{full-class model}.  
% If network is available, the module can be placed on the cloud: whenever a context change is detected by the $\mu$Classifier, the image will be compressed and transmitted to the cloud so that the module can execute the full-class model to predict the class label. 
% The class label will be sent back to the device for the device to make the decision on switching $\mu$Classifiers. 
% If the module is placed on the device due to the lack of network connections, it loads the full-class model from storage and executes it locally. 

% The oracle is a powerful model that covers all classes in the dataset. It is fed with the frame as the input and predicts its label. If the predicted class is not in the covered set of classes by the current $\mu$Classifier, the process of preparing a new $\mu$Classifier will be started by the micro-classifier configuration selector module.


% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/framework_iot_v2.png}
%     \caption{IoT node framework}
%     \label{framework1}
% \end{figure}

\begin{figure*}[h!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_all_v5.png}
    \caption{The \myname{} architecture; Local Switching. \DG{still too much whitespace and takes more space than we have...fonts need work but it looks generally good.}}
    \label{framework_all}
\end{figure*}

Next, we explain the two key components \textit{Configuration Selector} and \textit{$\mu$Classifier-based Predictor} in more detail. 


==> Backup/Mar6/Evaluation.tex <==


\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.904$)\label{fig:CameraTrap_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Acc_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.974$) \label{fig:STL_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Acc_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.857$)\label{fig:Places_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Acc_Vs_Similarity_V2.png}}}%
    \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes}
\label{acc_vs_sim_eval}
\end{figure*}

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.934$)\label{fig:CameraTrap_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_SpeedUp_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL-10 ($r=-0.973$) \label{fig:STL_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Speedup_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES365 ($r=-0.81$)\label{fig:Places_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Speedup_Vs_Similarity_V2.png}}}%
    \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
\label{speedup_vs_sim_eval}
\end{figure*}


\section{Evaluation}
This section evaluates how \textbf{ZAG} addresses the two challenges in Section \ref{case_context}: how to decide the appropriate configuration for a micro-classifier for an arbitrary subset of classes and how to reliably detect context change to switch between $\mu$Classifiers. We first define datasets, then evaluate our proposed context change detector, $\mu$Classifier configuration selector, and the end-to-end performance. We show that RaSC achieves high accuracy and frame rate for rare context-change scenarios on low-resource processors.

\subsection{Experiment Settings}

\HG{This subsection is not only about dataset, but also on the explaination of baselines, evaluation metrics (or the metrics we care about), etc.} 

\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resulution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\mypara{Dataset:}
\label{dataset}
We evaluate using three datasets, STL-10 \cite{STL10}, Places365 \cite{PLACES365}, and the Camera Trap dataset. STL-10 is an image recognition dataset inspired by CIFAR-10 \cite{CIFAR10} consisting of RGB images with a size of 96$\times$96. The dataset contains 10 classes, each with 1300 labeled images. Places365 is designed based on principles of human visual cognition that can be used for visual understanding tasks such as scene context, object recognition, and action prediction. It consists of 365 scene categories and the labels represent the entry-level of an environment. We chose 20 scene categories, each with 900 samples with a size of 256$\times$256. From those 900 samples, 600 images were selected as the train set and the rest as the test set. Camera Trap images captured by trail cameras provide a rare-context-change scenario in the real world. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images. Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. The empty class makes up a large part of these datasets and only a few of the classes have enough samples for both train and test sets. As a result, two Camera Trap datasets were fused to make a 10+1 classes train and test set. Eight species with more than 270 samples were chosen from the Snapshot Enonkishu dataset and two other species are picked from the Snapshot Camdeboo dataset. Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the train set was determined to be class-balanced, the test set follows the distribution of 10+1 classes to be close to the real-world setting.

In the rest of the paper, $\mu$Classifiers do the classification on combinations of 3 classes for STL-10 and Places365. For the Camera dataset, $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

\mypara{kNN as the configuration selector:}
kNN predicts the parameters of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority for a configuration, it considers the 4 nearest neighbors and so on until a majority is achieved for a configuration.

\mypara{DNN Models:}
We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. ResNet-50 is a potent network capable of fulfilling the mentioned requirement. This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. EfficientNet-B0 was initialized with ImageNet weights. 

\mypara{Similarity Measurement:}
The full-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.

\mypara{Configurations Details:}
Configurations are determined by two variables, model size and the resolution of the input frame. The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT. All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.


\mypara{Test Set Generation for End-To-End Evaluation:}
To evaluate the end-to-end performance of the framework we need to have a sequenced test set providing a specific context change rate to mimic the temporal flow of the context change in the real world. If we consider m-class combinations, the context changes whenever a frame represents a class different from the last m distinct classes. The context can be represented by an m-class combination and whenever the context changes a new m-class combination represents the current context. For instance, in the 3-class combination setting, let the current context be $\{s_1, s_2, s_3\}$. Assuming the next frame represents class $s_4$ the context changes and one among $s_1$, $s_2$, and $s_3$ should be replaced by $s_4$.

Let $CCR$ and $TS$ be the context change rate and original test set respectively. The number of frames resulting in a context change is:

\begin{equation}
    n=\lceil{CCR\times |TS|}\rceil
\end{equation}

We randomly construct a sequence of $n$ m-class combinations, where every two consecutive combinations show a context change. In other words, the intersection of every two consecutive m-class combinations is a set with a size of $m-1$. This sequence of n m-class combinations guarantee n context changes. Considering which combinations include a class, we divide samples of that class equally among those combinations. By this, the test set is reordered to have exactly $n$ context changes.  



 \begin{algorithm}
        \caption{Generating a sequence of contexts}
        \label{Alg3}
\begin{flushleft}
        \textbf{INPUT} 
        \\$TS$: Original test set)
        \\$CCR$: Context change rate
        \\$S$: List of all m-class combinations\\     
        \textbf{Procedure}
\end{flushleft}
        \begin{algorithmic}
            \State $n = \lceil{CCR\times |TS|}\rceil$
            \State $C = [(s_1, s_2, ..., s_m)]$ \Comment{Initialize $C$ with a random m-class combination from $S$}
            \State $Curr_C = (s_1, s_2, ..., s_m)$ \Comment{Current context}
            \While{$|C|\neq n$}
            \State $New_C = random\_choice(S)$ \Comment{New context candidate}
            \If {$|New_C\cap Curr_C|==m-1$}
               \State $C=C\cup New_C$
               \State $Curr_C=New_C$
            \EndIf
            \EndWhile
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: A sequence of $n$ contexts  
\end{flushleft}           
    \end{algorithm}

\subsection{Configuration Selector Performance}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.32\textwidth]{figures/camera_k_nn_performance.png}}}%
    \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % \qquad
    \subfloat[\centering PLACES365\label{fig:Places_roc}]{{\includegraphics[width=.32\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance for different thresholds}
\label{knn_performance}
\end{figure*}

% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}


In this section, our goal is to evaluate the performance of the $\mu$Classifier \textit{Configuration Selector}. we compared the accuracy and computation cost of the predicted configuration versus the oracle (label) , 3-Class EfficientNet with full resolution, and full-class EfficientNet with full resolution. For each combination of 3 classes in the test set, The accuracy and FLOPS of the used model was calculated and finally, the mean over the test set was used for the comparison. The computation saving was calculated in comparison to full-class EfficientNet with full resolution. the Table \ref{kmeans_perf} shows the comparison results. We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

We see our approach outperforms full-class EfficientNet (full resolution) with a high accuracy gain and computation saving for all three datasets. For the Camera Trap dataset, Our approach is $9\%$ more accurate than the full-class EfficientNet while while we save $86.87\%$ computation. Although the accuracy gain on STL-10 was not noticable, we could still gain over $62.37\%$ computation saving.

Although the accuracy gap between the predicted configurations and 3-Class EfficientNet (full resolution) is rather big, the computation efficiency is sacrificed. For instance, if we choose 3-Class EfficientNet (full resolution) for all combinations the $3.36\%$ accuracy gain comes with a cost of $6.61\times$ more computation overhead in comparison to our predicted configuration for the Camera Trap dataset. 

As mentioned before, the k-NN is supposed to select a configuration resulting in the most efficient partial-class model for a set of classes based on statistics of pair-wise similarities. As a set of classes gets harder to distinguish a more complex model is required to maintain accuracy over a specific threshold. We assumed the mentioned level of hardness can be quantified by a similarity metric. The results in table \ref{kmeans_perf} explain the effectiveness of the similarity-based k-NN configuration selector. Figures \ref{acc_vs_sim_eval} and \ref{speedup_vs_sim_eval} completely validate the precision of the similarity metric 

Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure \ref{speedup_vs_sim_eval} validates the functionality of our similarity metric and subsequently the k-NN configuration selector. The same procedure of grouping combinations into six bins and averaging from Figure \ref{acc_vs_sim_eval}is applied here. The Y-axis shows the computation saving of the predicted configurations versus 3-Class EfficientNet (full resolution) while the X-axis is the in-combination similarity. We see the computation saving drops as the similarity increases considering a more powerful model should be utilized to hit the threshold accuracy. It also shows the k-NN functions correctly by selecting light configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{table*}[ht]
\begin{tabular}{@{}p{2.5in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
Predicted $\mu$Classifier+regression head & 12.66\% & 13.13\% & 13.53\% & 11.09\% & 8.91\% & 8.18\% \\
Oracle $\mu$Classifier (Label)+regression head & 13.11\% & 13.26\% & 13.836\% & 11.15\% & 8.57\% & 7.64\% \\
3-class EfficientNet (full res)+regression head & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\

\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs baselines}
\label{fpfnt}
\end{table*}


\begin{table*}[ht]
\begin{tabular}{@{}p{2.7in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES365} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
Predicted $\mu$Classifier+regression head & 12.66\% & 13.13\% & 13.53\% & 11.09\% & 8.91\% & 8.18\% \\
Predicted $\mu$Classifier+maximum probability ~\cite{maxsoft1} & 23.42\% &24.94\% & 33.16\% & 31.70\% & 19.49\% & 18.29\% \\


\midrule
\end{tabular}
\caption{False Positive and False Negative rates of our approach vs Related Works using predicted $\mu$Classifiers by the k-NN}
\label{fpfn_baseline_other}
\end{table*}

\subsection{$\mu$Classifier-based Predictor Performance}
This section is devoted to the evaluation of the \textit{$\mu$Classifier-based Predictor} module. As discussed in section \ref{context_change}, a regression head is attached to the IoT $\mu$Classifier as the second output head. It is trained to output a value close to 0 for the target classes (negative) of the $\mu$Classifier and a value around 1 for other classes (positive). We considered $0.5$ as the decision boundary. 

In Table \ref{fpfnt} we presented the FP and FN rates for our predicted $\mu$Classifiers, the oracle $\mu$Classifiers (label), and 3-Class EfficientNet with full resolution. Since 3-Class EfficientNet with the full resolution is the most complex $\mu$Classifier, it is included in the table. For each combination of 3 classes in the test set, a $\mu$Classifier was constructed based on the predicted configuration by the k-NN, and its FN and FP rates were calculated. The mean of the FN and FP rates over all combinations in the test was reported in the table. Table \ref{fpfnt} shows our approach has an acceptable FN and FP rate and it is not far from 3-Class EfficientNet with the full resolution that provides the lower bound for FN and FP among all configurations. Specifically, the gap between our $\mu$Classifiers and the lower bound for both metrics are in the range of $2.3$ to $4.6\%$ for the Camera Trap and PLACES365 datasets which is reasonable though this range was expanded to around $7\%$ for the STL-10 dataset. These values can be lowered by increasing the $Accuracy_{thr}$ explained in Section \ref{sec4.4.3} as it directly affects the predicted configuration and therefore FP and FN rates.

Table \ref{fpfnt} also shows that the performance of the predicted $\mu$Classifiers is very close to models with the label configuration in terms of context change detection. Our approach had lower FP and FN rates in comparison to the oracle $\mu$Classifier on the Camera Trap and STL-10 datasets. Overall, the gap is at most $0.5\%$ for both metrics. This comparison also proves that the k-NN is acting very accurately in predicting the configuration.

As it was mentioned in Section \ref{context_change}, Maximum Softmax Probability \cite{maxsoft1} is an alternative for our regression-based context-change detection. It is very cheap in terms of the computation as it utilizes the softmax probability of the predicted class for detecting the out-of-distribution frames. We considered the Maximum Softmax Probability approach instead of the regression head for the predicted $\mu$Classifier. Table \ref{fpfn_baseline_other} shows the FP and FN rates of the Maximum Softmax Probability approach is much higher than ours. For example, the FP and FN rates of our approach is $20\%$ lower than the other approach.

\subsection{Online End-To-End Results}

\begin{table*}[h]
\scalebox{0.7}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
\label{End-to-end1}
\end{table*}


\begin{table*}[h]
\scalebox{0.5}{
\begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
\toprule
Methods & \multicolumn{5}{c|}{Camera Trap - ResNet-50} & \multicolumn{5}{c|}{STL-10 - ResNet-50} & \multicolumn{5}{c}{PLACES365 - ResNet-50}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & \multicolumn{1}{l|}{Latency-Pi0 (ms)} & Latency-Pi4 (ms) \\ \midrule
Our Approach & 82.98\% & 14.93\% & 6.43\% & 216.78 & 72.57 & 93.64\% & 17.53\% & 6.45\% & 77.81 & 30.02 & 96.01\% & 13.71\% & 5.95\% & 263.28 & 90.40 \\
Oracle $\mu$Classifier & 83.21\% & 14.98\% & 6.23\% & 216.67 & 71.88 & 94.00\% & 16.43\% & 6.13\% & 79.75 & 30.53 & 96.39\% & 13.28\% & 6.03\% & 286.12 & 98.48\\
3-class EfficientNet (full res) & 86.03\% & 11.36\% & 6.88\% & 822.56 & 264.29 & 96.06\% & 10.93\% & 5.93\% & 107.38 & 41.73 & 97.36\% & 10.06\% & 5.78\% & 520.33 & 179.72\\
All-Class EfficientNet (full res) & 83.00\% & 0.00\% & 0.00\% & 833.40 & 264.29 & 92.13\% & 0.00\% & 0.00\% & 107.88 & 41.77 & 90.95\% & 0.00\% & 0.00\% & 521.12 & 180.01 \\

\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context Change rate is $3\%$}
\label{End-to-end-online}
\end{table*}






\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
  &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
\label{End-to-end2}
\end{table*}



\begin{table*}[h]
\scalebox{0.8}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
& \multicolumn{3}{c|}{5 $\mu$Cs} & \multicolumn{3}{c|}{15 $\mu$Cs}  & \multicolumn{3}{c}{30 $\mu$Cs} \\
  &\multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms) & \multicolumn{1}{c|}{Acc} & Latency-Pi0 (ms) & Latency-Pi4 (ms)\\ \midrule
Greedy & 82.41\% & 272.58 & 88.35 & - & -\% & - & -\% & - & - \\
Random $\mu$Classifier & 82.36\% & 337.74 & 110.89 & - & -\% & - & -\% & -& - \\

%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}}
\caption{Local-Switching; $3\%$ Context change rate}
\label{local_end-to-end}
\end{table*}

==> Backup/Nov28/Design.tex <==
\section{Configuration Predictor}
\label{sec:similarity}

\myname{} needs to train a resource-efficient $\mu$Classifier for every possible context. 
As the optimal $\mu$Classifier configuration for different contexts varies, the core challenge lies in how to quickly determine the optimal configuration of the $\mu$Classifier given a context.  

To see why the optimal $\mu$Classifier configuration varies across contexts, consider classifying animals captured by a trail camera. 
When a context consists of animals with similar features, textures, or behaviors, the $\mu$Classifier faces a more challenging task in distinguishing between them. 
For instance, if the three classes represent a deer, an elk, and a moose, the classifier has to contend with the fact that all three animals have somewhat similar body shapes, sizes, and features. Consequently, the model may need to employ more computational resources to scrutinize subtle distinctions and achieve a comparable level of accuracy.
% In contrast, if the context is composed of animals that are markedly disparate in features, they are more easily distinguishable, and the $\mu$Classifier can make decisions with less computational effort. For example, consider a group comprising a deer, a rabbit, and a raccoon. These animals are drastically different in size, appearance, and behavior, making them easier to classify with higher confidence.
In essence, the inter-class similarities or differences play a significant role in determining the computational resources needed by the $\mu$Classifier. 



To address the challenge, our idea is to design an ``inter-class similarity'' metric that captures the similarity between the set of classes in a $\mu$Classifier, which in turn correlates with how much computational resources (i.e., the configuration) the model requires.
Based on the metric, we design a lightweight kNN-based configuration selector to identify the best configuration of the $\mu$Classifier without requiring training all configurations. 
The configuration selector can be queried to output the best configuration i.e. the one that achieves the lowest resource demands while meeting a target accuracy for a set of classes (i.e., a context).
We next present the proposed inter-class similarity metric, and then elaborate on the design of the kNN-based configuration predictor. 



% Indeed, we show that selection of classes within a $\mu$Classifier is of paramount importance, as different groups of three classes can exhibit different levels of compressibility when subjected to various model compression techniques such as pruning, quantization, or early exiting. \DG{correct?} \M{True} 

% Intuitively, the manner in which inter-class similarity and resource needs relate can be understood by considering the inherent characteristics of the classes in question. Imagine that the classes are representative of different animals that might be captured by a trail camera. When the classes consist of animals with similar features, textures, or behaviors, the classifier faces a more challenging task in distinguishing between them. For instance, if the three classes represent a deer, an elk, and a moose, the classifier has to contend with the fact that all three animals have somewhat similar body shapes, sizes, and features. Consequently, the model may need to employ more computational resources to scrutinize subtle distinctions and achieve a comparable level of accuracy.

% In contrast, if the classes are composed of animals that are markedly disparate in features, they are more easily distinguishable, and the classifier can make decisions with less computational effort. For example, consider a group comprising a deer, a rabbit and a racoon. These animals are drastically different in size, appearance, and behavior, making them easier to classify with higher confidence.

% In essence, the inter-class similarities or differences play a significant role in determining the computational resources needed by the $\mu$Classifier. When designing a context-aware system, careful consideration should be given to the grouping of classes, taking into account the inherent characteristics of the data to optimize performance and resource utilization.

% For example, we could contemplate several $\mu$Classifier designs. One approach, based on temporal co-occurrence, might be to simply load a $\mu$Classifier for the three most recently observed classes. On the other hand, a more meticulous design could involve selecting the three classes that yield the best performance based on certain criteria or metrics. The crux here lies in discerning whether there is a substantial performance difference between these options. We start by analyzing and comparing the efficacy of these designs to provide insights into the optimization of context-aware neural network models.

\subsection{Inter-Class Similarity Metric}

Given a set of classes, the inter-class similarity metric is a set of real numbers, each representing a \textit{pairwise class similarity}.
Two sets of classes that have similar statistics of inter-class similarities would share a similar $\mu$Classifier configuration. 
We use the statistics of inter-class similarities to represent a context, called \textit{context representation}. 
% \HG{The definition of inter-class similarity is pretty weak; now it represents a set of numbers; But in Figure 5, we use the mean of inter-class similarities. it is a little messy with all the definitions.}

\mypara{Pairwise Class Similarity:}
To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we get its embedding from a feature extractor that is trained on all classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
The similarity between two classes is calculated as the Cosine Similarity between their class representations. 

\mypara{Context Representation:} The vector representation of a set of classes  (i.e., a context) is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an $m$ class combination $C$ ($|C|=m$), is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

We note that the above class similarity and context representation were chosen after consideration of several alternate measures of similarity. 
We show empirical results comparing these metrics in \S\ref{sec:predictor}. 

% \HG{here, we have two dimensions to verify. 1) why choose the current pairwise class similarity; e.g., class similarity can also based on confusion matrix. 2) why chose the current context representation based on the pairwise class similarities? e.g., context representation can also be just using mean value, or using median or max value. }

% \mypara{Similarity as proxy for compressibility} 

% We now look at whether the similarity metric that we have defined captures the essential resource-accuracy tradeoffs in grouping classes into a $\mu Classifier$. 

Figure~\ref{heatmap} shows that the mean value of the inter-class similarity metric generally tracks the difficulty level of a context. 
 We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq. \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 
Overall, \textit{the higher the mean value of the inter-class similarity metric is, the more difficult the context is and thus the less accuracy achieved by $\mu$Classifiers with the same configuration (i.e., same FLOPS). }
The figure indicates that our proposed inter-class similarity metric correlates well with the computational efforts required by a context. 


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Model complexity versus the proposed inter-class similarity metric among classes (darker is higher accuracy). 
    We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models.}
    \label{heatmap}
\end{figure}

% When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% % 
% Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its context representation.}
    \label{fig:kNN-training}
    \vspace{-0.1in}
\end{figure}


\subsection{KNN-based Configuration Predictor}
\label{sec:knn}

The inter-class similarity metric allows us to develop a simple kNN-based approach to estimate the optimal configuration for a $\mu$Classifier. 
Building the kNN-based configuration predictor requires a configuration space for $\mu$Classifiers, and a set of training data points that consist of context representations and their corresponding optimal configurations.  
We next explain the configuration space and the similarity-directed sampling to build an effective training set. 
We then elaborate how the configuration predictor can be quried to predict the optimal $\mu$Classifier for any given context. 
 
% As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 
% % We first discuss the selection of configuration space,  the construction of training data points, and the query of the KNN-based predictor. 
% \HG{need to revise the above paragraph}


% The core challenge during the process of training $\mu$Classifiers is determining the most likely configuration without needing to train a huge number of models. 

% Our idea is to design a lightweight configuration selector that can identify the best configuration of the $\mu$Classifier without requiring so many models to be trained. The configuration selector can be queried to output best configuration i.e. the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$ for a set of classes to be included in the $\mu$Classifier.

% A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
% However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions: (1) \textit{What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? }, and (2) \textit{How to quickly identify the most efficient yet accurate $\mu$Classifier, given any subset of classes?}

% \begin{enumerate}
%     \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
%     \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
% \end{enumerate}

\mypara{Configuration Space:}
While in principle the configuration space can include any model compression methods and parameters, for practical reasons, we restrict ourselves to a few parameters to make training tractable. We therefore restrict our focus to configuration parameters that provide the large dynamic range of resource-accuracy tradeoffs for $\mu$Classifiers.
% 
We find that two methods are particularly effective for configuring $\mu$Classifiers --- changing the input image resolution and the number of filters via filter pruning. 
% Varying the resolution of the image that we provide as the input to the $\mu$Classifier is particularly effective because a) the computation complexity of the $\mu$Classifier decreases quadratically as resolution (height and width) decreases, and b) lower resolution inputs are often sufficient when the $\mu$Classifier is separating more dissimilar classes. Filter pruning with different sparsity ratios to control the computation complexity of the $\mu$Classifier is also effective. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

% Figure~\ref{res_size_vs_size} shows that varying both image resolution and pruning level scales down better as compute decreases compared to varying only the pruning level. Each point shows the average accuracy across all 3-class subsets of 10 classes.  We see that varying both resolution and pruning level provides us configurations with lower computation costs while accuracy remains in a reasonable range. Pruning performs poorly in the low FLOPs regime since it requires very high pruning levels which leads to very low accuracies.

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/res_size_vs_size_V3.png}
%     \caption{Configuring resolution and model size (by varying the pruning level) provides us a large dynamic range in resource-accuracy tradeoffs for configuring $\mu$Classifiers. (Camera Trap dataset is used.)}
%     \label{res_size_vs_size}
% \end{figure}

% \subsubsection{kNN-based configuration selection}
% \label{sec:knn}
% We now have two pieces of the puzzle: a) an effective inter-class similarity metric that accurately tracks resource-accuracy trade-offs of a $\mu$Classifier, and b) a narrower parameter space of resolution and model size as the two parameters that we tune. Given these, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
% As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/kNN-training.pdf}
%     \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.\DG{We need somethign that shows both how the kNN is constructed and how it is queried. There is a lot of confusion about the kNN and we need to clarify.}}
%     \label{fig:kNN-training}
% \end{figure*}

\mypara{Similarity-directed sampling:} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want samples to have good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration of the remaining combinations accurately. 
% This is critical to ensure the performance of kNN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers (configurations) to identify the best one. 
% Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a {similarity-directed sampling} scheme that samples at different levels of hardness among all possible subsets of classes. 
Figure \ref{fig:kNN-training} illustrates the training of kNN.
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the kNN. 
% 
Compared to random sampling, our empirical evaluation on five datasets shows that our sampling scheme can reduce up to 95\% of samples while getting similar prediction accuracy.  

 
\mypara{Querying the kNN:} 
Once the kNN is constructed, it can be queried at run-time to predict the optimal $\mu$Classifier for the current context. 
The mean and std of inter-class similarities of the classes in the context are used to determine the closest configuration parameters in the kNN as the predicted optimal $\mu$Classifier configuration.
Feature extractors of $\mu$Classifiers are frozen during training to save storage overhead on device and also training time on the cloud. 

% This predicted model can be trained on the cloud and downloaded to an IoT device. 
% If the same context re-appears, the IoT device can just use the cached model and this does not need to be re-trained. 
% Feature extractors of $\mu$Classifiers are frozen during training. Hence, only fully connected layers are trained and downloaded to the IoT device. 

% Since the feature extractors are fixed, they can be stored on the IoT during installation to reduce runtime communication overhead. \HG{Here might be the reason why the reviewers ask us on the storage overhead.. the baselines store only the full-class model; but we need to store all the possible configurations of feature extractors. How much more storage do we need in our approach vs. the full-class model?} 

We note that an alternate approach to using a kNN-based configuration predictor is to use Neural Architecture Search (NAS \cite{NAS1,NAS2}). 
Our method is considerably lighter weight since given a context we can cheaply determine which configuration parameters to use via the kNN.

\section{Context-aware Switching}
\label{context_change}

Another essential part of making our system work is precisely detecting the context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
% 
It poses two challenges. 
The first challenge is to robustly and rapidly detect context changes. 
A context change occurs when an input frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast. 
% 
The second challenge is to determine the appropriate $\mu$Classifier to switch to after the new class is identified.  Switching to a $\mu$Classifier with less number of classes can reduce the inference cost per input frame as the $\mu$Classifier can be more lightweight. However, it could introduce more frequent context switches and thus runtime overhead in the future. 
% 
We next explain the proposed context change adaptation pipeline and the hybrid context switching policy that address the two challenges. 

\subsection{Context Change Adaptation Pipeline}
% \HG{This subsection corresponds to the 2nd contribution: enabling on-the-fly context switching using a two-step approach. 1st step to detect change and 2nd step is to detect new class.}

We design an efficient context change adaptation pipeline by splitting the process into two parts – a lightweight \textit{context change detector} that executes on each image
as a separate head attached to each $\mu$Classifer, and a more
heavyweight \textit{context predictor} that executes a regular all-
class classifier to identify the new class. This separation
allows us to invoke the heavyweight classifier sparingly thereby reducing the computational cost.

\mypara{Context change detector:}
% The first step in context-aware switching is detecting when the current context has changed. 
Its goal is to detect when the current context has changed. 
The problem is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computationally intensive and thus cannot be applied in a real-time scenario (see \S\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context-change detector. 
Specifically, a regression head is added to the $\mu$Classifier as the second output head along with the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. 
Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Context predictor:}
After a context change is confirmed by the context change detector, the next step is to identify the new class. This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. 
% 
The \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching.


\subsection{Hybrid Context Switching Policy} 
\label{sec:switch-policy}
After a new class is identified, the challenge in determining to which $\mu$Classifier to switch is to effectively balance the tradeoff between using $\mu$Classifiers with a larger number
of classes to reduce future context switches and using  $\mu$Classifiers with a small number of classes to reduce inference latency per input frame. 
 
Our core insights to address the challenge are two-folds. First, the right balance depends on the deployment environment: A device that encounters much more active classes than another device is likely to prefer $\mu$Classifiers with more classes to avoid higher context switch overheads.  
This requires us to introduce some configuration parameter that can be easily tuned based on the targeted deployment environment to determine how the $\mu$Classifiers are switched. 

Second, we also note that the computational benefits of $\mu$Classifiers drops dramatically as the number of classes in them increases.  
Figure~\ref{fig:comp_save_muc_size} illustrates the phenomenon using the PLACES20 dataset, which consists of a total of 20 classes from PLACES365 ~\cite{PLACES365}. 
% We set a predetermined accuracy threshold which remains the same for all of $m$-class $\mu$Classifier. 
For each combination of $m$ classes, we select the most efficient configuration that meets a pre-defined accuracy threshold. Then we calculate an average of the computation savings compared to the full-class model for all possible combinations of $m$ classes. 
% This average serves as the representative metric for each $m$.
As the number of classes in a $\mu$Classifier goes beyond ten, the $\mu$Classifier brings no computation savings compared to the full-class model.
This motivates us to prioritize $\mu$Classifiers with a small number of classes (e.g., 2 to 5) to captalize on the computation savings from context-aware inference. 
% and also make no or, if necessary, only incremental change in the number of classes in the new $\mu$Classifier to be used. 

\begin{figure}[h]
\includegraphics[width=0.35\textwidth]{figures/compute_save_size_muc.png}
    \caption{Computation saving of m-class $\mu$Classifiers for different m.}
    \label{fig:comp_save_muc_size}
\end{figure}

% Based on the two insights, we develop a context switch policy that determine how the $\mu$Classifers are switched based on a single tuning knob.  
% The policy is \textit{hybrid} because a $k$-class $\mu$Classier can be switched to a $m$-class $\mu$Classier, where $m \in \{k-1, k, k+1\}$ to allow no or incremental changes in the number of active classes considered in the new context.

Based on the two insights, we develop a context switch policy that allows a single tunable know to control how the $\mu$Classifers are switched based on the deployment environment.  
The policy is \textit{hybrid} because a $\mu$Classier can be switched to another $\mu$Classier with a different number of classes. 
 Our policy works as follows.   
\HG{the following paragraph on model switching policy needs to be made more clear. Will work on it this afternoon}
A kNN is already trained for each $m \in \{2, 3, 4\}$ with a predetermined accuracy threshold and it is assumed that each kNN provides a configuration that hits the threshold accuracy. 
The m-class context which has the lightest configuration is considered and the corresponding model will be deployed on the device. If more than one context share a same configuration, the biggest m will be picked to reduce future context switches and transmission overhead. 



Our evaluation in section \ref{sec:ablation} shows that the proposed hybrid context switching policy can achieve near 2$\times$ speedups on GAP8 when the active classes changes as fast as one class changes in every 4 input frames.



% \HG{this subsection should corresponds to the 3rd contribution: balancing context switching costs and performance gains via simple yet effective switching policies.}
% The second step is switching from the current $\mu$classifier to the one appropriate to the new context. 
% For this, we need to first determine what are the new class(es). This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. We then use a simple technique where the last $p$ predictions made by the pipeline are observed and the farthest predicted class among the previous set of classes is substituted by the new ones. 
% 
% The \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching.

% \HG{D1. Although the paper started with an exciting design space about the micro-classifiers and their configurations, the
% number of classes for the micro-classifiers is fixed throughout the design and the evaluations. It would be very interesting
% to investigate the tradeoffs between four 3-classifers and three 4-classifers. SOLUTION: add switching policy}

% \HG{the paper focuses on the smallest 3-class context and 2 out of 3 datasets used simulated temporal context change
% patterns. SOLUTION: show that with more classes in a micro-classifier, the benefits of context-aware decrease. There is a balance between using a micro-classifier with larger number of classes to reduce context swithes vs. with a small number of classes to reduce inference latency; This motivates our hybrid model switching policy}

% \HG{It'd be also
% interesting to see the performance tradeoffs for microC configured with different context lengths (3, 4, 5, etc). SOLUTION: we could explicitly point out the tradeoffs between using micro-classifiers with more classes vs. with less classes. add a figure: x-axis is the \#classs in the micro-classifier, y-axis: switching cost and the inference cost. }

% \subsection{Optimizations for Local Only Support}
% \HG{this subsection describe how we do model caching on device to support local only mode; and how to minimize storage overhead. These optimizations are relatively trival. We put them here together to complete the overall pipeline.}

We future explain two optimizations to efficiently implement the context switching policy in both cloud-assisted and unattended operation modes. 

\mypara{Caching $\mu$Classifiers:}
In the cloud-assisted mode, after a device downloads the $\mu$Classifier for a new context, it will cache the  $\mu$Classifier on device to avoid model training for the same context. 
If the cache is full due to device storage constraints, the least frequently used model will be replaced. 
Model caching reduces the overhead of cloud-side model training and the device-cloud communitation at runtime. 

In the unattended mode, a set of $\mu$Classifiers will be pre-installed on the device before deployment. 
The context switching policy will switch between only the pre-installed $\mu$Classifiers. 
We select the $\mu$Classifiers that are most frequently used based on an input trace collected from the IoT device deployed in a targeted environment. 


% So far, we have assumed the availability of cloud assistance but \myname{} can also operate in autonomous settings where connectivity is too limited to download new models. This is often true for IoT deployments where low-power radios like BLE or LoRa are used since bandwidth is too low to download all a few megabytes of model weights.
% 
% For this discussion, we assume that the IoT camera is deployed in a new environment without prior knowledge of what classes temporally co-occur, so we need to identify the best subset of $\mu$Classifiers to cache on-device. This is often the case for first-time camera deployments (e.g. trail cams). \HG{fix the description; describe how caching as an optimization is done to support fully on-device mode.}




\begin{comment}
\section{Budget-limited $\mu$C selection}
\label{sec:budget}

So far, we have assumed the availability of cloud assistance but \myname{} can also operate in autonomous settings where connectivity is too limited to download new models. This is often true for IoT deployments where low-power radios like BLE or LoRa are used since bandwidth is too low to download all a few megabytes of model weights.

For this discussion, we assume that the IoT camera is deployed in a new environment without prior knowledge of what classes temporally co-occur, so we need to identify the best subset of $\mu$Classifiers to cache on-device. This is often the case for first-time camera deployments (e.g. trail cams).

% This raises another question:
% \textit{How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes?}
% \begin{enumerate}
%     \item How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes.
% \end{enumerate}

Our strategy is to store a subset of $\mu$Classifiers on-device such that we have (1) coverage across the classes that occur in the scene, (2) high accuracy in recognizing the classes and (3) low computational overhead. 
% The best set of $\mu$Classifiers to store on a device should be able to cover all classes that can possibly occur in a scene, and achieve the highest classification accuracy and computation efficiency than any other sets. 
% The rationale of covering as many classes as possible is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifier should work in any possible context. 
% 
The problem can be re-phrased as a combinatorial optimization problem: given a set of $\mu$Classifiers, each with a classification accuracy and resource consumption, determine which $\mu$Classifiers to include in the collection so that the total resource consumption is minimized while each model meets a target accuracy threshold and the collection meets some class coverage requirement. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{salkin1975knapsack}. 
We next elaborate on our greedy algorithm to approximate the optimal solution. 

% \M{Our solution has a different objective in comparison to the stated problem. The Problem says we want to maximize accuracy s.t a budget limit. But our approach aims to minimize computation s.t that the accuracy over a threshold. Do you agree?}
 

% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

\mypara{Greedy $\mu$classifier selection:}
Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
% If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage i.e. the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training of the $\mu$Classifiers.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
If this is the case, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. Since the selection is based on kNN prediction, we again need to go through the process of training the newly selected model to check if the accuracy requirement ($Acc_{thr}$) is satisfied.
% In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
% As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If so, the replacement happens; otherwise, the process repeats and the next lightest $\mu$Classifier will be selected and trained. 
% and checked until the replacement happens. 
% Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
This process continues until the $Acc_{thr}$ threshold is met. 
In our experience, the kNN has high accuracy, hence the number of times a $\mu$Classifier in the selected set needs to be replaced is very low.
\end{comment}

\mypara{Optimizing storage requirements:} 
$\mu$Classifiers that operate on the same model size share the same model weights as their feature extractors are frozen during training. We can reduce storage requirements by storing one feature extractor per model size, and then only storing the classification and context change detection heads for each chosen $\mu$Classifier. 

Specifically, in the cloud-assisted mode, a device stores all the unique sized feature extractors, one classification and context change detection head for the current context, and if storage allowed, additional classification and context change detection heads from previous contexts. 
In the unattended mode (i.e., without cloud availability), a device stores all the unique sized feature extractors, a full-class model for context predictor, and, subject to storage capacity, classification, and context change detection heads from chosen contexts based on the trace of the training data. 
These contexts are the most frequent when we apply the hybrid context-switching policy on the training set.
We show in \S~\ref{sec:case-study} that the total amount of storage required for 60 $\mu$Classifiers are only 46 MBs. 

% Here we assume the device is not capable of training the classification and context change detection heads. Consequently, it becomes necessary to pre-store these modules for frequently encountered contexts, limited only by the device's available storage capacity. This approach ensures that the device is equipped to handle common contexts efficiently, despite its training limitations.\HG{is it true? if so, we need to justify why the extra storage overhead is OK. We can remove this paragraph to save space; but we need  to report the storage overhead in eval.} \M{Fixed}

% \HG{D7. It is a bit confusing which efficiency metric the paper focuses on. It seems that storage or memory on the IoT devices
% is not a constraint. For example, the feature extractor of the all-class model is stored on the IoT devices. And the all-class
% model may also be executed on the IoT devices. SOLUTION: clarify that local storage is a constraint. Where do we expect the full-class model to execute?}


% \HG{D4. It seems that the solution assumes incremental changes in the context. The classifier-switch is triggered on a perclass
% basis, and it relies on the all-class model to detect each changed class. For example, if the current 10 classes
% change to another 10 classes, then the solution needs to run the all-class model 10 times and train 10 models, each
% differs in 1 class, to eventually switch to the right 10-classifier. SOLUTION: report that our solution can still achieve speedups in high context swithing rate. A side question is what is the largest context switching rate that our algorithm can support? 
% \M{Table 3 is updated (3Mb/s). I included Both Pi0 and GAP8. Pi0 is better if we want to show when our algorithm stops providing speedup. On the other hand GAP8 shows better numbers. Although if we decrease the transmission bandwidth, we can claim that context interval 5 is where our algorithm stops providing speedup. Decreasing the context interval to 2 or 3 reverse the trend of number of frame triggering and Model switch. Instead of increasing, frame trigger and model switching decreases for context interval 2 or 3.}}

% only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

% \subsection{Local and Edge-cloud} 

% We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

% \mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

% The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
% Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

% During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

% On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

% \mypara{Edge-cloud assisted IoT devices.} 
% Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
% The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

% Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
% The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Backup/Nov28/DesignOverview.tex <==
\section{\myname{} Design Overview}
\label{des_over}

We build on these observations to design a context-aware inference pipeline \myname{}, which executes context-aware $\mu$Classifiers for a prediction task and dynamically switches between $\mu$Classifiers to handle context changes. 

% \subsection{Challenges}
% \label{challenge}
 

% \mypara{Challenge 1: Identifying resource-efficient $\mu$Classifers for every possible context.}
% The first challenge is to identify the most resource-efficient $\mu$Classifers for every possible context that reaches a target accuracy. 
% The total number of contexts grows exponentially with the total number of classes. 
% For example, if there are 40 classes and we consider 3-class $\mu$classifiers, there are $C^{40}_3 = 9880$ $\mu$Classifers. 
% And what's worse, the optimal configurations of the $\mu$Classifer depends on the difficulty level of the context.  
% A context whose classes have similar patterns or features would be harder to recognize and need to use a $\mu$Classifier that has higher model capacity.  
% If we consider 10 configurations per $\mu$Classifier, then nearly 100K models need to be trained to identify the optimal $\mu$Classifers for all possible contexts. 


% \mypara{Challenge 2: Detecting context switch.} 
% The second key challenge is designing an accurate detector that can precisely detect context change and, once detected, rapidly switch to the right $\mu$Classifier for the new context. 
% Since context change detection lies on the critical path of every prediction, 
% the detector needs to be very fast since it cannot add significant additional computation overhead to the $\mu$Classifier. 

% \mypara{Challenge 3: Robustness to connectivity.}
% The third key challenge is operating in different communication regimes. For example, when connectivity is strong, we can train new $\mu Classifiers$ on-demand in the cloud and download the learned weights during run-time when a new context arises. But when cloud-assistance is unavailable or bandwidth too limited, then a subset of $\mu$Classifiers need to be pre-trained and stored locally in the limited IoT storage.

\begin{figure*}[t!!!]
    \centering
    \includegraphics[width=1\textwidth]{figures/framework_v7.png}
    \caption{Context-Aware Switching in \myname{}. In case the communication or cloud is not available, the framework relies on cached/stored $\mu$Classifiers. (CCD: Context change detection, FE: Feature extractor)}
    \label{framework_all}
\end{figure*}


% \subsection{\myname{} Overview}
% \label{sec:overview}



 
\myname{} has two main components.
The first component, \textit{Configuration Predictor}, identifies the suitable configuration of the $\mu$Classifier for each context, i.e., a subset of classes (called active classes), without any training costs.  
It represent a context based on an \textit{inter-class similarity} metric, which estimates the difficulty in classifying the active classes in a context. 
The metric allows a simple k-nearest neighbor approach to rapidly predict the optimal configuration of a $\mu$Classifier without training every possible configuration. 

 
The second component, \textit{context-aware switching}, enables the device to seamlessly switch between $\mu$Classifiers based on context changes. 
It occurs in two steps. 
To detect context changes, we augment $\mu$Classifiers with a lightweight \textit{Context Change Detector} head. 
The first step executes the \textit{Context Change Detector} head to rapidly detect if the input frame is a new class without determining which is the new class. 
If context change is detected, the second step executes the \textit{all-class model}, a heavyweight classification module, that determines which classes are present in the scene. 
If a new class is detected, it triggers a ``model switch'' to load a new $\mu$Classifier based on the context switching policy. 
Figure~\ref{framework_all} illustrates switching at run-time.

% The last component \textit{Budget-limited $\mu$Classifier Selector} selects a smaller subset of $\mu$Classifiers to train and store on device from among all possible candidates. 
% It allows devices to switch between $\mu$Classifiers locally during run-time when cloud assistance is unavailable.  

\mypara{Usage scenarios:} \myname{} supports cloud-assisted and unattended operation. When cloud assistance is available, context-aware switching detects changes in context and requests a $\mu$Classifier for the new context. \myname{} cloud executes the Configuration Predictor to rapidly identify the suitable configuration of the $\mu$Classifier, then trains the model on-demand and sends the model to the device to handle the new context. The new model can be cached on-device and the next time the same context occurs, the cached model can be used as shown in Figure~\ref{framework_all}.
For unattended operation i.e. no cloud availability, \myname{} relies on locally stored $\mu$Classifiers. 
% At installation time, the \textit{Budget-limited $\mu$Classifier Selector} and Configuration Predictor are used to select the optimal set of  $\mu$Classifiers to store on the device such that context-aware switching can happen locally. 
% Figure~\ref{fig:offline} illustrates the two steps. 
% 
In variable connectivity settings, a combination of cloud-assisted and unattended operation is also possible. We now describe the two components in more detail.



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/offline.png}
%     \caption{Similarity-based configuration prediction and budget-limited $\mu$Classifier selection}
%     \label{fig:offline}
% \end{figure}





==> Backup/Nov28/Evaluation.tex <==
\section{Evaluation}
We first describe the experiment settings in \S~\ref{sec:settings}, and then evaluate the end-to-end system over three datasets and on real platforms  in \S~\ref{sec:end-to-end} and the components of \myname{} in \S~\ref{sec:predictor}-\ref{sec:selector}. 
We further perform ablation studies on context change frequency and scalability of the system in \S~\ref{sec:ablation} and implement a camera trap application in \S\ref{sec:case-study} 
% \HG{update this paragraph to match with the new eval section if necessary}



\subsection{Experiment Settings}
\label{sec:settings}

\begin{comment}
\begin{table*}[htbp]
\begin{tabular}{@{}llllllll@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Feature\\ Extractor\end{tabular} & Resolution & \#Class & \#Comb & \begin{tabular}[c]{@{}l@{}}\#Context\\ Change\\ Detector\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cloud\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}Conf\\ Selector\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\myname{}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}6/8/13\\ /Full\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}320/240/160/100 (\textbf{CT})\\ 256/200/160/130 (\textbf{P365})\\ 96/72/64/58 (\textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}16\\ Conf\end{tabular}} & \multirow{2}{*}{ResNet-50} & k-NN \\ \cmidrule(r){1-1} \cmidrule(l){8-8} 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\myname{}\\ (Oracle)\end{tabular}} &  &  &  &  &  &  & \begin{tabular}[c]{@{}l@{}}Dictionary\\ (optimal)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (3-class)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}3+1 (\textbf{CT})\\ 3 (\textbf{P365}, \textbf{STL})\end{tabular} & \begin{tabular}[c]{@{}l@{}}120 (\textbf{CT})\\ 200 (\textbf{P365}, \textbf{STL})\end{tabular} & 1 & ResNet-50 & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Full)\end{tabular}} & Full & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}EfficientNet\\ (Early-Exit)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\end{tabular} & Full & \begin{tabular}[c]{@{}l@{}}11 (\textbf{CT})\\ 20 (\textbf{P365})\\ 10 (\textbf{STL})\end{tabular} & No & No & No & No \\ \bottomrule
\end{tabular}
\label{tab:expt-settings}
\caption{Experiment settings of different baselines and methods. The only difference between \myname{} with Oracle-mode is the different method in Configuration Selector  discussed in Sec~{}. Our approach has 16 configurations by leveraging 4 different layers and 4 different resolutions for better efficiency. Dataset Abbreviation: CT - Camera Trap, P365 - Places 365, STL - STL-10.}
\end{table*}

\end{comment}

\mypara{Dataset:}
\label{dataset}
We use five datasets. Three datasets come from the Camera Trap applications called Enonkishu \cite{Camera_trap_enonkishu}, Camdeboo \cite{Camera_trap_camdeboo}, and Serengeti (season 4) \cite{Camera_trap_serengeti}. 
We refer to them together as Camera Trap datasets. 
They have temporal data captured by trail cameras with real-world context changes. Trail cameras make use of an infrared motion detector and time-lapse modes to capture images, each time in a sequence of three. 
The Camera Trap datasets normally include a lot of species plus an empty class whose images show a scene with no species in it. 
Not all species have enough samples for both train and test sets. Hence we considered the most frequent species plus the empty class for the classification task. The number of considered classes were 9, 11, and 18 for Enonkishu, Camdeboo, and Serengeti respectively. 
% Since the images captured by the trail cameras are of high resolution, we have resized them to a uniform dimension of 320×320 pixels. This resizing facilitates processing by devices with limited resources, ensuring that these images can be efficiently handled on less powerful hardware. 

We also evaluate on two other image datasets, STL-10 \cite{STL10}, and PLACES365 \cite{PLACES365}, from which we synthesize temporal sequences.
STL-10 is an image recognition dataset 
consisting of RGB images with a size of 96$\times$96. 
The dataset contains 10 classes, each with 1300 labeled images. 
% 
PLACES365 is intended for visual understanding tasks such as scene context, object recognition, and action prediction.  
We chose 100 scene categories, each with 1200 samples with a size of 256$\times$256. 
Most of our results are shown for 20 scene categories (called PLACE20) but we evaluate the scalability of \myname{} for 100 classes.



% Furthermore, samples of the empty class from both datasets were added to the mentioned set. While the training set was class-balanced, the test set follows the distribution of 10 species classes + 1 empty class to be close to the real-world setting. As mentioned, Camera Trap images form a sequence of 3 frames and the labels in each sequence are the same. However, sometimes one or more frames in the sequence do not show any species in the scene as they have left the scene. Hence, those frames are wrongly labeled as that species. It leads to non-accurate labels which lower the accuracy of the classification task.}

% Since the space of $\mu$Classifier configurations is very large, we take a deeper dive into 3-class $\mu$Classifiers. This represents an extreme point with $\mu$Classifiers with the highest compressibility but also requires the most switching between contexts. 
% So, it helps us evaluate the upper limits of how a nimble context-aware system can be designed with $\mu$Classifiers.

%By changing the number of classes, different accuracy vs switching overhead costs can be achieved in practice. %Hence, we focus on 3-class $\mu$Classifiers for the STL-10 and Places365 datasets; for the Camera dataset, the empty class is quite frequent when there are no animals in the scene, hence we add an empty class to the three animal classes (but still refer to this as a 3-class $\mu$Classifier).

% $\mu$Classifiers are considered to do the classification task on combinations of 4 (3+1) classes while one of them is fixed (empty class) and the other 3 are variables. For simplicity, we also refer to them as the classifier of 3 classes.

% \mypara{Inter-class similarity metric:}
% The configuration predictor needs class representations to calculate the inter-class similarity vector of a 3-class combination (Eq.~\ref{eq:rep_vector}). 
% We used the feature extractor of ResNet-50 to extract the embedding of images from a class and average the embeddings into a single vector to be used for computing the inter-class similarities. 


% \mypara{The configuration space of $\mu$Classifiers:}
% The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
% We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
% We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that besides the EfficientNet-B0 we get a total of four feature extractor architectures.  
% %The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The range of image resolutions is considered 100-320, 58-96, and 130-256 for Camera Trap, STL-10, and PLACES datasets respectively. For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.
% A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
% The two heads use two Fully Connected layers. Feature extractors are fine-tuned once on all classes, and then frozen during the training of the two heads of $\mu$Classifiers.

\mypara{KNN-based configuration predictor:}
The $\mu$Classifier is based on the feature extractor of EfficientNet-B0~\cite{efficientnet} pre-trained on ImageNet. 
We vary both the pruning level and the resolution of input frames to get different configurations of the feature extractor.  
We applied three levels of $\ell1$ pruning, 10\%, 30\%, and 40\%, so that including the EfficientNet-B0, we have a total of four unique-sized feature extractors.  
%The model sizes are 16.6, 14.1, 8.4, and 6.8 MB and, after quantization, these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
The range of image resolutions is considered 100--320, 58--96, and 130--256 for Camera Trap, STL-10, and PLACES datasets respectively. 
% For each dataset, four image resolutions were to yield different levels of computation complexity while keeping the accuracy of the models reasonable. 
Overall, the size of the configuration space is 16.
A $\mu$Classifier consists of one of the four feature extractors and two heads, one for classification and one for regression (to detect context change). 
The two heads use two Fully Connected layers. 
Feature extractors are fine-tuned once on all classes, and then frozen during the training of the two heads of $\mu$Classifiers.

% To calculate the context representation of every 3-class combination, 


To build the training data for the configuration predictor, we applied similarity-directed sampling (detailed in \S\ref{sec:knn}) on m-class combinations.
% when we have 40 classes in total, 7\% of the combinations for 30-classes, 17\% of combinations for 20-classes, and 33\% combinations for 10 classes.
% 500 3-class combination samples from 9880 combinations ($C^{40}_3$) in the PLACES (40 class) dataset, 
% 300 out of 4060 combinations ($C^{30}_3$) for the PLACES (30 class), 
% 200 out of 1140 combinations ($C^{20}_3$) for the PLACES (20 class), 
% and 40 out of 120 combinations ($C^{10}_3$) for the STL-10, Camera Trap, and PLACES (10 class) datasets. 
For each sampled $m$-class combination, we train $\mu$Classifiers with all 16 configurations to select the most efficient one that achieves a target accuracy (i.e., the optimal $\mu$Classifier configuration). 
We further use the feature extractor of ResNet-50 to extract the embedding of images from a class and average the embeddings into a single vector to compute context representation as Eq.~\ref{eq:rep_vector}.
The pairs of context representation for the sampled $m$-class combinations and the optimal $\mu$Classifier configuration for the context are the training dataset of the KNN. 

% The target accuracy threshold for selecting the best $\mu$Classifier is set to be the median of all the trained $\mu$Classifiers to balance computation efficiency and accuracy, unless noted differently. 
% The thresholds are 93$\%$, 97$\%$, and 92$\%$ for STL-10, PLACES, and Camera Trap datasets respectively.

To balance computation efficiency and accuracy, the target accuracy threshold for selecting the best $\mu$Classifier is set to be around 94$\%$, 87$\%$, 92$\%$, 92$\%$, and 97$\%$ for Enonkishu, Camdeboo, Serengeti, STL-10, and PLACES20 datasets respectively, unless noted differently. 

After collecting the training data, we use the KNN to predict the best $\mu$Classifier configuration for the remaining $m$-class combinations. 
KNN predicts the configuration of a $\mu$Classifier based on the majority vote. It starts with 3 nearest neighbors and if there is no majority, it considers 4 nearest neighbors and so on until a majority is achieved.


\mypara{Context-aware switching:} 
As discussed in \S\ref{context_change}, a regression head is attached to a $\mu$Classifier to detect the context change. 
% It is trained to output a value close to 0 for the target classes of the $\mu$Classifier and a value around 1 for other classes. 
% We used $0.5$ as the decision boundary for all three datasets.
Once context change is detected, we execute an all-class model (ResNet-50 for the edge-cloud assisted setting and EfficientNet-B0 for unattended op.) to identify which new class occurs in the scene. 
All-class models are pre-trained on ImageNet and fine-tuned on the target dataset.

\mypara{Implementation:}
We implement the \myname{} pipeline on three different IoT devices --- Raspberry Pi 4B, Raspberry Pi Zero W, and GAP8. 
We generate \textbf{TensorFlow Lite} models using the default optimization and int-8 quantization to reduce the model size and execution latency. On all the platforms, we profile the execution latency of models of different configurations on different datasets.
% 
For profiling on Raspberry Pi 4B and Zero W, we utilize the \textbf{TVM} framework \cite{TVM} to tune the operator implementations to reduce the execution latency for the Arm Cores. 
% 
For profiling on GAP8, we use the GAP8 tool chain \cite{URL:GAP8_tool} to transform the \textbf{TensorFlow Lite} models into C code by fusing the operations. 
% 
% \mypara{Training:} 
An NVIDIA Tesla M40 24GB GPU was used for training models and as the edge-cloud in some of our experiments. 
% 
% \mypara{Open source code:} 
If accepted, we will make our code on all the above platforms openly available.

% \mypara{Configurations Details:}
% Configurations are determined by two variables, model size and the resolution of the input frame. 
% The feature extractor of the base model is EfficientNet-B0 with ImageNet weights. 
% We applied different levels of $\ell1$ pruning to construct 3 other feature extractors. 
% According to Section \ref{des_over}, these feature extractors are once fine-tuned on the target dataset and stored on the cloud and the IoT.
% All four feature extractors share the same architecture for classification and regression head and these output heads consist of two Fully Connected layers. The model sizes are 16.6, 14.1, 8.4, and 6.8 MB although after quantization these values decrease to 4.8, 4.1, 2.6, and 2.1 MB respectively. 
% The image size mentioned for each dataset in Section \ref{dataset} was downsampled with 3 different steps to expand the configuration space. 
% The considered image sizes for each dataset are provided in Table \ref{ressize}. These values were chosen to yield different levels of computation complexity while keeping the accuracy of the models reasonable. Overall, the size of the configuration space is 16.



% We used ResNet-50 \cite{resnet-50} as the feature extractor of the \textit{New Class Detector} in case the network is available. 
% The \textit{New Class Detector} model should be very accurate as its job is to predict the label of the transmitted frame and this label affects the used $\mu$Classifier on the IoT. 
% ResNet-50 is a potent network capable of fulfilling the mentioned requirement. 
% This model was initialized with ImageNet weights and fine-tuned on each dataset. If this module is placed on the device, EfficientNet-B0 \cite{efficientnet} is considered as the feature extractor of the \textit{New Class Detector} model. 
% EfficientNet-B0 obtained state-of-the-art performance of ImageNet while it is very lightweight. EfficientNet-B0 was also selected as the foundation of the partial-class models. 
% EfficientNet-B0 was initialized with ImageNet weights. 

% \mypara{Similarity Measurement:}
% The all-class model with ResNet-50 as the feature extractor, mentioned in \textbf{DNN Models} is employed for extracting the embedding for each class. These embedding vectors were used for computing the inter-class similarity.

\subsection{End-to-End Evaluation}
\label{sec:end-to-end}



% \begin{table*}[ht]
% % \scalebox{0.55}{
% \footnotesize 
% \tabcolsep=0.2cm 
% \scalebox{0.7}{\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{Enonkishu} & \multicolumn{3}{c|}{Camdeboo} & \multicolumn{3}{c|}{Serengeti} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES20}\\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) \\
% %   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) \\ 
%   \midrule
% All-Class Model & 89.1\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 65.6\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 74.6\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 92.1\% & 107.9 (1.0$\times$)& 124.5 (1.0$\times$)& 90.5\% & 521.1 (1.0$\times$)& 1162.1 (1.0$\times$) \\
% All-Class-Early Exit & 84.6\% & 494.3 (1.7$\times$) & 926.2 (2.0$\times$) & 66.0\% & 728.9 (1.1$\times$) & 1591.3 (1.2$\times$) & 68.7\% & 549.2 (1.5$\times$) & 1247.6 (1.5$\times$) & 91.9\% & 100.1 (1.1$\times$)& 108.9 (1.1$\times$)& 90.1\% & 417.2 (1.2$\times$)& 883.2 (1.3$\times$)\\
% All-Class-Pruned & 81.4\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 57.7\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 69.6\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 84.3\% & 89.0 (1.2$\times$)& 95.5 (1.3$\times$)& 84.9\% & 377.7 (1.4$\times$)& 587.1 (2.0$\times$)\\
% FAST \cite{FAST} & 90.1\% & 799.3 (1.0$\times$) & 1768.7 (1.0$\times$) & 64.9\% & 799.7 (1.0$\times$) & 1792.8 (1.0$\times$) & 74.8\% & 810.7 (1.0$\times$) & 1801.4 (1.0$\times$)& 92.5\% & 108.9 (1.0$\times$)& 124.4 (1.0$\times$)& 91.0\% & 501.6 (1.0$\times$)& 1091.7 (1.0$\times$)\\
% PALLEON \cite{palleon} & 90.7\% & 772.4 (1.1$\times$) & 1681.5 (1.1$\times$) & 65.7\% & 791.9 (1.0$\times$) & 1774.0 (1.0$\times$) & 74.8\% & 822.5 (1.0$\times$) & 1836.0 (1.0$\times$) & 92.4\% & 103.8 (1.0$\times$)& 118.1 (1.0$\times$)& 92.2\% & 483.7 (1.0$\times$)& 1051.2 (1.1$\times$)\\
% % \myname{} (Highest FLOPs) & 91.4\% & 842.6 (1.0$\times$) & 1854.7 (1.0$\times$) & 95.9\% & 120.7 (0.9$\times$)& 137.6 (0.9$\times$)& 96.8\% & 534.4 (1.0$\times$)& 1168.4 (1.0$\times$)\\
% % \myname{} (Oracle) & 88.8\% & 227.8 (2.3$\times$) & 355.4 (5.1$\times$)& 93.8\% & 90.6 (1.2$\times$)& 96.2 (1.3$\times$)& 95.7\% & 292.6 (1.8$\times$)& 511.6 (2.3$\times$)\\
% \myname{} & 92.2\% & 236.9 (3.5$\times$) & 365.4 (5.0$\times$) & 65.5\% & 518.5 (1.6$\times$) & 933.7 (2.0$\times$) & 73.8\% & 393.1 (2.1$\times$) & 657.6 (2.8$\times$)& 94.4\% & 117.5 (0.9$\times$)& 118.2 (1.0$\times$)& 95.9\% & 266.2 (2.0$\times$)& 412.5 (2.8$\times$)\\
% \bottomrule 
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on three datasets; Context changes every 30 frames on average. Note that Speedup values are rounded.}
% \label{End-to-end-online}
% \vspace{-0.2in}
% \end{table*}




% \begin{table*}[ht]
% % \scalebox{0.55}{
% \footnotesize 
% \tabcolsep=0.2cm 
% \scalebox{0.87}{\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{Enonkishu} & \multicolumn{3}{c|}{Camdeboo} & \multicolumn{3}{c|}{Serengeti} & \multicolumn{3}{c}{PLACES20}\\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 (ms) \\
% %   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{(ms)} & (ms) &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & (ms) \\ 
%   \midrule
% All-Class Model & 89.1\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 65.6\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 74.6\% & 833.4 (1.0$\times$) & 1844.0 (1.0$\times$) & 90.5\% & 521.1 (1.0$\times$)& 1162.1 (1.0$\times$) \\
% All-Class-Early Exit & 84.6\% & 494.3 (1.7$\times$) & 926.2 (2.0$\times$) & 65.5\% & 728.9 (1.1$\times$) & 1591.3 (1.2$\times$) & 68.7\% & 549.2 (1.5$\times$) & 1247.6 (1.5$\times$) & 90.1\% & 417.2 (1.2$\times$)& 883.2 (1.3$\times$)\\
% All-Class-Pruned & 81.4\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 57.7\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 69.6\% & 676.6 (1.2$\times$) & 1092.1 (1.7$\times$) & 84.9\% & 377.7 (1.4$\times$)& 587.1 (2.0$\times$)\\
% FAST \cite{FAST} & 90.1\% & 799.3 (1.0$\times$) & 1768.7 (1.0$\times$) & 64.9\% & 799.7 (1.0$\times$) & 1792.8 (1.0$\times$) & 74.0\% & 810.7 (1.0$\times$) & 1801.4 (1.0$\times$)& 91.0\% & 501.6 (1.0$\times$)& 1091.7 (1.0$\times$)\\
% PALLEON \cite{palleon} & 90.7\% & 772.4 (1.1$\times$) & 1681.5 (1.1$\times$) & 65.7\% & 791.9 (1.0$\times$) & 1774.0 (1.0$\times$) & 74.1\% & 822.5 (1.0$\times$) & 1836.0 (1.0$\times$) & 92.2\% & 483.7 (1.0$\times$)& 1051.2 (1.1$\times$)\\
% % \myname{} (Highest FLOPs) & 91.4\% & 842.6 (1.0$\times$) & 1854.7 (1.0$\times$) & 95.9\% & 120.7 (0.9$\times$)& 137.6 (0.9$\times$)& 96.8\% & 534.4 (1.0$\times$)& 1168.4 (1.0$\times$)\\
% % \myname{} (Oracle) & 88.8\% & 227.8 (2.3$\times$) & 355.4 (5.1$\times$)& 93.8\% & 90.6 (1.2$\times$)& 96.2 (1.3$\times$)& 95.7\% & 292.6 (1.8$\times$)& 511.6 (2.3$\times$)\\
% \myname{} & 92.2\% & 236.9 (3.5$\times$) & 365.4 (5.0$\times$) & 65.5\% & 518.5 (1.6$\times$) & 933.7 (2.0$\times$) & 73.8\% & 393.1 (2.1$\times$) & 657.6 (2.8$\times$)& 95.9\% & 266.2 (2.0$\times$)& 412.5 (2.8$\times$)\\
% \bottomrule 
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on three datasets; Context changes every 30 frames on average. Note that Speedup values are rounded. Due to space constraints, results for STL-10 are not included.}
% \label{End-to-end-online}
% \vspace{-0.2in}
% \end{table*}



\begin{table*}[ht]
% \scalebox{0.55}{
\small 
\tabcolsep=0.2cm 
\scalebox{1.0}{\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{Enonkishu} & \multicolumn{3}{c|}{Camdeboo} & \multicolumn{3}{c|}{Serengeti} & \multicolumn{3}{c}{PLACES20}\\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 \\
  \midrule
All-Class Model & 89.1\% & 1.0$\times$ & 1.0$\times$ & 65.6\% & 1.0$\times$ & 1.0$\times$ & 74.6\% & 1.0$\times$ & 1.0$\times$ & 90.5\% & 1.0$\times$& 1.0$\times$ \\
All-Class-Early Exit & 84.6\% & 1.7$\times$ & 2.0$\times$ & 65.5\% & 1.1$\times$ & 1.2$\times$ & 68.7\% & 1.5$\times$ & 1.5$\times$ & 90.1\% & 1.2$\times$& 1.3$\times$\\
All-Class-Pruned & 81.4\% & 1.2$\times$ & 1.7$\times$ & 57.7\% & 1.2$\times$ & 1.7$\times$ & 69.6\% & 1.2$\times$ & 1.7$\times$ & 84.9\% & 1.4$\times$& 2.0$\times$\\
FAST \cite{FAST} & 90.1\% & 1.1$\times$ & 1.2$\times$ & 64.9\% & 1.0$\times$ & 1.0$\times$ & 74.0\% & 1.0$\times$ & 1.0$\times$& 91.0\% & 1.0$\times$& 1.0$\times$\\
PALLEON \cite{palleon} & 90.7\% & 1.2$\times$ & 1.3$\times$ & 65.7\% & 1.0$\times$ & 1.0$\times$ & 74.1\% & 1.0$\times$ & 1.0$\times$ & 92.2\% & 1.0$\times$& 1.1$\times$\\\hline
\myname{} & \textbf{92.2\%} & \textbf{3.5$\times$} & \textbf{5.0$\times$} & \textbf{65.5\%} & \textbf{1.6$\times$} & \textbf{2.0$\times$} & \textbf{73.8\%} & \textbf{2.1$\times$} & \textbf{2.8$\times$} & \textbf{95.9\%} & \textbf{2.0$\times$} & \textbf{2.8$\times$}\\
\bottomrule 
\end{tabular}}
\caption{End-To-End performance of our approach vs baselines on three datasets; Context changes every 30 frames on average. Note that Speedup values are rounded. The gains improve if wireless data rates are higher (we use 3Mbps) or if cachine is used (we assume no caching of the $\mu$Classifier heads). Due to space constraints, results for STL-10 are not included but they follow similar trends.}
\label{End-to-end-online}
\vspace{-0.2in}
\end{table*}





% \HG{Although, the paper claims it is compatible with model compression, a direct comparison is not provided. The authors
% state that the classifier can be used with model compression, however, its effect on accuracy compared to the full model
% needs to be validated. \\SOLUTION: clarify the baselines we compared with; emphasize that we indeed compare with model compression approaches  such as early exit and pruning}
% \HG{is it necessary to add another approach: computation completely offload to cloud? \M{It is going to have a very low latency with the considered bandwidth (3Mb/s). So it may be better not to mention it.}}
This section looks at an edge-cloud assisted system (the unattended setting is examined in \S~\ref{sec:selector}).
To evaluate the end-to-end performance of \myname{}, we need datasets that have context changes. The three Camera Trap datasets provide us with a real-world temporal flow with context changes but other datasets are not temporal. 
Hence, we sequence test sets from the PLACES and STL-10 datasets to mimic the temporal flow of the Camera Trap to create a temporal sequence with which to evaluate our methods. 
% 
Specifically, we find that the context interval is 30 frames on average (context changes in every 30 frames) for the Camera Trap dataset. 
We thus synthesize a test set with the context interval of 30 frames for the PLACES and STL-10 datasets and use this in our evaluation unless noted differently.
In \S~\ref{sec:ablation}, we further study the effects of different context change rates in the performance of \myname{}.


%%%%%% I Commented the description below as the details on how you synthesize the sequence relies on a 3-class combination... it can cause some concerns on how about other number of class combinations. 
%%%%%%%
% To generate a test set with temporal flow, we randomly construct a sequence of 3-class combinations, where every two consecutive combinations show a context change of a single class. To match the context interval of 30 frames, we persist the current context for 30 frames by picking random samples from the current context. 





We compare the classification accuracy and overall latency of \myname{} against the following baselines: 
(a) \textbf{FAST} \cite{FAST}, a context-aware approach that assumes the class skews are known offline. During inference it detects the class skew using a window-based detector and train a specialized classifier (Fully Connected layers), 
(b) \textbf{PALLEON} \cite{palleon}, a state-of-the-art video processing framework that applies a Bayesian filter to adapt the model to the context. 
The Bayesian filter is determined by applying an all-class model on a window of frames.
(c) \textbf{All-Class Model}, which uses the well-trained EfficientNet-B0 with all the classes and full image resolution. 
(d) \textbf{All-Class-Early Exit}, which is the early exit variant (exit heads in stages 4 and 6)  of the All-Class Model.
(e) \textbf{All-Class-Pruned}, where we apply 30$\%$ pruning rate to the all-class model. We choose 30\% since it gives the best accuracy and efficiency trade-offs. 
% (f) \myname{} \textbf{(Highest FLOPs)}, which uses the $\mu$Classifier that has the same classes as \myname{} predicts but uses full image resolution and no pruning (and hence computationally the most expensive).
% (g) \myname{} \textbf{(Oracle)} i.e. the $\mu$Classifier that meets the target accuracy threshold with minimum FLOPs (which would be selected by an omniscient scheme rather than the kNN-based method we use). 
% We note that training the Oracle is not scalable --- for example, on one GPU, it takes 300 hours longer than our approach for 20 classes and 2400 hours longer for 40 classes in the PLACES dataset.

% it takes a total of 120, 40, and 300 hours longer than our approach for the Camera Trap, STL-10 and PLACES20 respectively.


Table~\ref{End-to-end-online} shows the end-to-end results on two devices. 
The IoT device communicates at a data rate of $3$ Mbps (typical LTE speed).
The reported latencies include the time spent on the inference on the device, transmission of the triggered frames to the cloud, and transmission of the classification and regression heads to the device. 
We assumed no $\mu$Classifiers are cached on the device which is the \emph{worst-case scenario} as it requires more transmission and increases the overall latency. We can achieve higher speedup if caching is utilized. We averaged latencies over the test set and computed the speedup relative to All-Class model.


Overall, our approach has the advantage in terms of accuracy and particularly in latency over baselines. 
When compared to All-Class Model, 
\myname{} has comparable or higher accuracy (up to 5.4\% higher) and also offers substantial computational gains (latency speedup of $1.6 - 3.5 \times$ for the Pi0 and $2.0 - 5.0 \times$ for the GAP8).
% When compared to Highest FLOPs $\mu$Classifier, \myname{} has $1.6-2.9\%$ less accuracy but similar speedup as above.
% \myname{}'s performance is also very close to the Oracle $\mu$Classifier. 
% 
\myname{} outperforms two other context-agnostic baselines, All-Class-Early Exit, and All-Class-Pruned, in terms of both accuracy and latency due to the leverage of context awareness to improve efficiency. 


Compared to the context-aware approaches FAST \cite{FAST} and PALLEON \cite{palleon}, \myname{} demonstrates comparable accuracy or an improvement of up to $4.9\%$ and 3.7$\%$ respectively, while also delivering highers speedups. FAST and PALLEON need to execute the all-class model for n (more than 10) frames to determine the class skew. Thus, they provide speedups only if the context change is very sparse. 
% Hence, before they can determine the class distribution of the current context, context changes and they need to repeat the execution of all-class model. 
For this reason, they could not provide a speedup higher than 1.1$\times$ which is significantly lower than \myname{}.


% Table \ref{local_end-to-end} shows that the accuracy increases as we store more $\mu$Classifiers on the device. Also, only 40 $\mu$Classifiers are needed to be stored on the device to achieve the same accuracy as the All-Class EfficientNet (Table \ref{End-to-end-online}) while we still gain 3$\times$ speedup.

% On the Raspberry Pi Zero-W platform, the latency slightly increases by selecting more $\mu$Classifiers. The reason is that the computation cost of the selected $\mu$Classifiers slightly increase as we expand the number of picked $\mu$Classifiers. For instance, it is expected that any other $\mu$Classifier have a higher computation cost than the chosen 20 $\mu$Classifiers as the greedy selector aims to pick the lightest $\mu$Classifiers. Although storing a high number of $\mu$Classifiers helps the device to lower the number of execution of the all-class model, it doesn't necessarily lead to lower latency in comparison to storing a small number of $\mu$Classifiers. It is due to the fact that the computation cost of the selected $\mu$Classifiers dominates the latency. In case we employ a more complex model like ResNet50 as the all-class model on the device, its computation cost may dominate the computation cost of the $\mu$Classifiers.


% \mypara{Case study: Trail camera} We implemented an end-to-end use case of \myname{} inference pipeline for detecting animals observed by a trail camera for the Raspberry Pi Zero W. This is a common use-case for low-power IoT platforms which wakeup upon detecting that there is movement in the scene. The video in \cite{} shows an example where we use the Camera Trap datasets \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} as input and locally store 40 $\mu$Classifiers for switching.

% \begin{table*}[h]
% \scalebox{0.7}{
% \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
% \toprule
% Methods & \multicolumn{4}{c|}{6$\%$ Context Change} & \multicolumn{4}{c|}{4$\%$ Context Change} & \multicolumn{4}{c}{2$\%$ Context Change} \\
%   &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Frame Triggers} & \multicolumn{1}{l|}{$\mu$C Switches} & Flops (M)\\ \midrule
% Our Approach & 93.00\% & 18.70\% & 7.70\% & 39.04 & 92.66\% & 17.86\% & 6.20\% & 37.86 & 92.66\% & 13.20\% & 3.86\% & 44.35 \\
% Oracle $\mu$Classifier & 93.13\% & 19.43\% & 7.73\% & 33.23 & 93.83\% & 17.86\% & 5.60\% & 34.81 & 92.83\% & 14.53\% & 3.63\% & 40.43 \\
% 3-class EfficientNet (full res)  & 96.13\% & 12.16\% & 7.6\% & 74 & 96.30\% & 10.9\% & 5.63\% & 74 & 95.63\% & 7.66\% & 3.66\% & 74 \\
% All-Class EfficientNet (full res)  & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 & 91.43\% & 0.00\% & 0.00\% & 74 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the STL-10 dataset}
% \label{End-to-end1}
% \end{table*}








% \begin{table*}[h]
% \scalebox{0.8}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% Methods & \multicolumn{3}{c|}{100$\%$ Oracle} & \multicolumn{3}{c|}{95$\%$ Oracle} & \multicolumn{3}{c|}{90$\%$ Oracle}  & \multicolumn{3}{c}{ResNet-50 Oracle} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M) & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{\#Switches} & Flops (M)\\ \midrule
% Our Approach & 92.25\% & 68 & 245.99 & 91.62\% & 82 & 236.20 & 89.37\% & 113 & 219.10 & 83.54\% & 116 & 246.85 \\
% Oracle $\mu$Classifier & 91.95\% & 62 & 195.46 & 91.58\% & 80 & 217.53 & 90.29\% & 111 & 232.06 & 83.20\% & 120 & 214.98 \\
% 3-class EfficientNet (full res) & 93.79\% & 68 & 900 & 92.41\% & 86 & 900 & 92.45\% & 92 & 900 & 84.83\% & 128 & 900 \\
% All-Class EfficientNet (full res) & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900 & 83.00\% & \textendash & 900  & 83.00\% & \textendash & 900 \\
% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}}
% \caption{End-To-End performance of our approach vs baselines on the Camera Trap dataset; $3\%$ context change}
% \label{End-to-end2}
% \end{table*}


% \subsection{Case study: Trail camera} 

% We briefly provide some end-to-end memory benchmarks from an end-to-end implementation. In order to better visualize how the \myname{} pipeline works, we built a demo on the Raspberry Pi 4B running at $1$ GHz. The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows a working end-to-end system.

% In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 
% We resize the captured images into $4$ different sizes: $100$, $160$, $240$, $320$ depending on configuration parameters and use the corresponding feature extractors and $\mu$Classifiers to generate the classification results and regression results. 

% For the regression results, we use a threshold of $0.6$ to trigger the context change. When the regression results are smaller than $0.6$, we consider the current context might not be appropriate anymore and trigger the full model to do the inference again. The full model is latency-heavy on the Raspberry Pi 4B which will cost more than $600$ ms. The all-class model uses the image of the size $320$ as input and will generate the classification results of $11$ classes. Based on the classification results, we will find the most proper context. We find the new combinations of 3-class in a First-In-First-Out(\textbf{FIFO}) manner by removing the oldest classes and adding the latest predicted classes. If the new combination has no valid $\mu$Classifiers, we will iteratively remove the second and third oldest classes instead of the first one. If there is no valid combination using the heuristic, we will randomly sample one valid combination containing the predicted class. 

% When the regression results are larger than the threshold, we will remain on the current context and accept the predicted $3$-class results. Overall, we find out that we could achieve $82\%$ accuracy and $16\%$ rate of triggering the all-class models.

\subsection{Performance of Config Predictor}
\label{sec:predictor}

% \begin{table}
%   \caption{The used resolutions for constructing the configuration space}
%   \label{ressize}
%   \begin{tabular}{l|l}
%     \toprule
%     \textbf{Dataset}&\textbf{Resolution}\\
%     \midrule
%     \textbf{PLACES365} & $256\times256$, $200\times200$, $160\times160$, $130\times130$ \\
%     \textbf{Camera Trap} & $320\times320$, $240\times240$, $160\times160$, $100\times100$ \\
%     \textbf{STL-10} & $96\times96$, $72\times72$, $64\times64$, $58\times58$ \\    
%   \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[ht]
% \scalebox{0.75}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL-10} & \multicolumn{3}{c}{PLACES365} \\
%  & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c|}{Computation Saving} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{FLOPS (M)} & \multicolumn{1}{c}{Computation Saving} \\ \midrule
% Our Approach (Predicted $\mu$Classifier) & 91.99\% & 118.12 & 86.87\% & 93.17\% & 27.84 & 62.37\% & 96.33\% & 129.19 & 75.15\% \\  
% Oracle $\mu$Classifier (Label) & 93.07\% & 214.43 & 76.17\% & 93.52\% & 29.46 & 60.18\% & 97.22\% & 162.13 & 68.82\% \\
% 3-class EfficientNet (full res) &  95.35\% & 900.00 & 0.00\% & 97.32\% & 74.00 & 0.00\% & 98.05\% & 520.00 & 0.00\% \\
% All-class EfficientNet (full res) & 83.00\% & 900.00 & 0.00\% & 92.13\% & 74.00 & 0.00\% & 90.95\% & 520.00 & 0.00\% \\
% % vs. All-class Early Exit (full res) & 81.12 & 423.57 & 52.93\% & 91.59\% & 38.80 & 47.55\% & - & - & - \\
% \midrule
% Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
% \midrule
% \end{tabular}}
% \caption{The performance gain/loss of our predicted configurations versus different baselines}
% \label{kmeans_perf}
% \end{table*}

We now look at the performance of the $\mu$Classifier \textit{Configuration Predictor}. 
We vary the target accuracy threshold from the lowest to the highest of all the trained $\mu$Classifiers to show how the threshold affects the performance of the configuration predictor. 
A lower target accuracy will result in lighter $\mu$Classifiers and thus less FLOPs. 



\begin{figure}[h]%
    \centering
    \subfloat[\centering Camera Trap\label{fig:CameraTrap_roc}]{{\includegraphics[width=.24\textwidth]{figures/camera_k_nn_performance.png}}}%
    % \subfloat[\centering STL-10 \label{fig:STL_roc}]{{\includegraphics[width=.32\textwidth]{figures/stl_k_nn_performance.png}}}%
    % % \qquad
    \subfloat[\centering PLACES\label{fig:Places_roc}]{{\includegraphics[width=.24\textwidth]{figures/places_k_nn_performance.png}}}%
    \caption{Performance of configuration predictor with different accuracy thresholds. The orange curve aligns well with the oracle, indicating that the kNN together with the inter-class similarity metric works well in selecting the best configuration. \HG{replace the name ``Camera Trap'' with one of the camera trap datasets, e.g., Enonkishu? }}
\label{knn_performance}
\end{figure}

Figure~\ref{knn_performance} shows how different target accuracy thresholds affect the classification accuracy and the computation cost for our method and baselines. 
We compare the \myname{}'s configuration predictor (noted as \textbf{\myname{} $\mu$C} in the figure) with three baselines: 
(a) \myname{} \textbf{(Oracle) $\mu$C} i.e. the $\mu$Classifier that meets the target accuracy threshold with minimum FLOPs (which would be selected by an omniscient scheme rather than the kNN-based method we use). 
We note that training the Oracle is not scalable --- for example, on one GPU, it takes 300 hours longer than our approach for 20 classes and 2400 hours longer for 40 classes in the PLACES dataset.
(b) \myname{} \textbf{(Highest FLOPs) $\mu$C}, which uses the $\mu$Classifier that has the same classes as \myname{} predicts but uses full image resolution and no pruning (and hence computationally the most expensive).
(c) \textbf{All-Class Model}, which uses the well-trained EfficientNet-B0 with all
the classes and full image resolution.
We omit the result on the other datasets for limited space. 
Both the classification accuracy and FLOPs are averaged over $\mu$Classifiers for all 3-class combinations.  


Overall, we see that \myname{} can cover a wide trade-off region between accuracy and computational cost --- accuracies vary by 3.5-6\% and compute by 6.5$\times$ to 13$\times$. 
Across the range, the accuracy is nearly as good as the \myname{} (Oracle), indicating that \textit{the kNN together with the inter-class similarity metric works well in selecting the best configuration. }
In contrast, All-Class Model (red star) and \myname{} (Highest FLOPs) (green star) are point solutions. 
Note that, \myname{} (Highest FLOPs) outperforms the accuracy of the All-Class Model by a large margin even though both models have the same FLOPs. The accuracy benefits come from the fact that \myname{} narrows down a prediction task to contexts, echoing the observations in \S~\ref{sec:motivations}.  

% Although All-Class-Pruned and All-Class-Early-Exit can result in accuracy-efficiency trade-offs, the models achieve less accuracy given the same FLOPs budget. We note that the comparison favors All-Class-Pruned and All-Class-Early-Exit because pruning and early exits can also be applied to the $\mu$Classifier on \myname{}, as demonstrated in Section~\ref{sec:motivations}.
% \HG{after the data is updated, might update the description to be more quantitative.}


% We compare these models against a specific instance of \myname{}, i.e. the point where the dotted line intersects the \myname{} curve (orange) based on the threshold we choose. 
% This configuration of \myname{} is 0.8-10\% more accurate than All-Class EfficientNet and requires $53\%$ to $75\%$ less computation to hit the target accuracy. 
% When comparing against \myname{} (Highest FLOPs), we see that \myname{} achieves 53-75\% computation savings while sacrificing 1.5-4.3\% classification accuracy. 


% old text %
% We see the k-NN has done a good job in predicting the configuration for the $\mu$Classifiers as the accuracy gap with the oracle $\mu$Classifiers was very small on the three datasets. 
% For the STL-10 dataset, the accuracy gap between k-NN predicted models and labels was as small as -$0.35\%$ while the computation cost was relatively equal. 
% The biggest gap in accuracy with $-1.08\%$ is for the Camera Trap dataset while our predicted configurations save $10.7\%$ more computation on average. 
% These results show the k-NN works well in selecting the configurations which means the similarity metric as the basis of the k-NN input is very accurate.

% We now compare \myname{} against {all-class EfficientNet} (red star). \myname{} is between 5.1\% -- 12.3\% more accurate and requires 53\% to $74.79\%$ less computation to hit the target accuracy (horizontal dotted line).

% When comparing against {3-Class EfficientNet}, we see that \myname{} achieves significant  computation savings while sacrificing a small amount of classification accuracy. 
% For instance, in the case of the Camera Trap dataset, \myname{} has $3.03\%$ lower accuracy than 3-Class EfficientNet (full resolution) but also $3\times$ less computation overhead.


\begin{figure}[t]%
    \centering
    \subfloat[\centering \label{fig:acc_vs_sim_eval}]{{\includegraphics[width=.24\textwidth]{figures/Accuracy_Vs_Similarity.png}}}%
    \subfloat[\centering \label{fig:comp_gain_Vs_Similarity}]{{\includegraphics[width=.235\textwidth]{figures/comp_gain_Vs_Similarity.png}}}%
    \caption{(a) The accuracy of a representative configuration correlates well with the inter-class similarity. 
    (b) The computational complexity of the predicted $\mu$Classifiers correlates well with the inter-class similarity. 
    % We see that both accuracy and computation savings (over All-Class Model) correlates well with our proposed inter-class similarity metric, indicating that the similarity metric closely mirrors the actual difficulty level of contexts. 
    Similarity is normalized to [0, 1] in both figures.\HG{if we decided to remove the STL-10 benchmark, we should remove STL-10 from the figure. Again, for the camera trap, we need to be specific on which camera trap dataset we are using. Another solution is to clarify the camera trap specifically refers to Enonkishu for example in the caption.}}
    \vspace{-0.2in}
% \label{}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.25\textwidth]{figures/Accuracy_Vs_Similarity.png}
%     \caption{The accuracy of a fixed model drops with the increase of the combination's similarity. Our inter-class similarity metric closely mirrors the actual difficulty level of combinations of 3 classes\M{I had to normalize their similarity values to show them in a single figure as their similarity ranges are very different. But for the camera trap dataset in figure 11, the curve doesn't look good since the y-axis range is big}}
%     \label{acc_vs_sim_eval}
% \end{figure}

% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{figures/comp_gain_Vs_Similarity.png}
%     \caption{Computation gain of our approach against full resolution 3-class or All-Class EfficientNet. Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets} 
%     \label{speedup_vs_sim_eval}
% \end{figure}
% \HG{since the configuration predictor is fundamentally a classification problem. Should we report the classification accuracy as well? } \M{Accuracy of kNN won't be impressive as it is not necessarily good on predicting the exact config, most of the time it predicts a configuration which is computationally and accuracy wise close to the ground truth}

\mypara{Effectiveness of the inter-class similarity metric:}
The good predictive performance of the configuration predictor results from the effectiveness of the inter-class similarity metric in capturing the difficulty level of contexts. 

% We now examine the effectiveness of the proposed inter-class similarity metric. 

Figure~\ref{fig:acc_vs_sim_eval} illustrates how the accuracy of a representative $\mu$Classifier on each 3-class combination correlates with the inter-class similarity averaged over the 3 classes. 
For the graph, all 3-class combinations were binned into six clusters based on the inter-class similarity metric and the accuracy and similarity values are averaged in each cluster.
% 
We observed that there is a clear inverse relation between inter-class similarity and classification accuracy. The Pearson correlation between the inter-class similarity metric and the classification accuracy is extremely high ($0.86-0.97$), indicating that \textit{our similarity metric closely mirrors the difficulty level of 3-class combinations.  }

% Figure \ref{acc_vs_sim_eval} shows our similarity metric reflects the hardness level of the classification task on combinations of three classes. 
% The mean of pair-wise similarities is calculated for each combination of three classes and the classification accuracy is computed using a fixed model. 
% For a clear demonstration, the mentioned combinations were binned into six clusters and the accuracy and similarity values are averaged in each cluster. As it is shown in this figure, the accuracy drops with the increase in the similarity. The Pearson correlation coefficient is close to -0.9 for all three datasets which validates the functionality of our similarity metric.

Figure~\ref{fig:comp_gain_Vs_Similarity} looks at this relation from another performance dimension --- computation savings. 
% The figure shows how the computational complexity of the predicted $\mu$Classifiers correlates with the inter-class similarity of 3 classes for all 3-class combinations.   
The same procedure of grouping 3-class combinations into six bins is applied here.  
The Y-axis shows the computation saving of the predicted configurations compared to the All-Class Model/\myname{} (Highest FLOPs) and the X-axis is the inter-class similarity. 
We see the computation saving drops as the similarity increases since a more powerful model should be used to meet the target accuracy threshold. 
It also shows that the similarity-aware kNN works well in selecting lightweight configurations for low similarity combinations and more powerful configurations for harder cases.

\begin{figure}[h]
    \centering
\includegraphics[width=0.4\textwidth]{figures/diff_sim_metric.png}
    \caption{Accuracy difference of predicted $\mu$Cs by kNN from oracle $\mu$Cs using different similarity metrics (Oracle-Predicted).  \HG{need to fix Camera Trap label.}}
    \label{fig:Diff_Sim_Metric}
    \vspace{-0.1in}
\end{figure}

\mypara{Comparison with other similarity metrics:}
We also investigate alternative similarity metrics and context representations including (1) confusion matrix-based similarity and (2) maximum and minimum of pair-wise similarities in a combination. 
For computing the pair-wise similarity using the confusion matrix, the number of samples that two classes are misclassified as another are summed and normalized as the percentage by the total number of those two classes.
Figure~\ref{fig:Diff_Sim_Metric} shows the comparison using all three datasets. Each bar reflects the accuracy difference between predicted $\mu$Classifiers and oracle $\mu$Classifiers averaged over all 3-class combinations for each similarity metric. We see kNN using our similarity metric (mean,std) provides more accurate predictions in comparison to the confusion matrix-based similarity metric over all three datasets. 
%KNN with our inter-class similarity metric but using maximum and minimum as context representations has a poor performance on Camera Trap dataset as the accuracy of its predictions are on average 2.5\% lower than the oracle.






\subsection{Perf. of Context-Aware Switching}
\label{sec:switching} 

This section evaluates the performance of the \textit{context-aware switching} module. We first evaluate the performance of the regression-based context change detector and then the hybrid context switching policy. 

\mypara{Effectiveness of the context change detector:}
A false positive (FP) that wrongly predicts a context change would introduce additional cost whereas a false negative (FN) will cause accuracy degradation since the $\mu$Classifier cannot detect the context change. 
To evaluate the performance of the regression head, we test the $\mu$Classifier corresponding to a 3-class combination with the test samples of 3 classes to calculate the FP rate. In order to compute the FN rate, we test the mentioned $\mu$Classifier with samples of all out-of-context classes. For each approach, the reported FP and FN rates are averaged over all combinations.


\begin{table}[htb]
\footnotesize 
\tabcolsep=0.05cm
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Enonkishu} & \multicolumn{2}{c|}{STL-10} & \multicolumn{2}{c}{PLACES} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
$\mu$C+regression (ours) & 3.88\% & 13.61\% & 13.58\% & 10.91\% & 8.91\% & 8.18\% \\
$\mu$C+maximum prob~\cite{maxsoft1} & 16.96\% & 22.89\% & 31.44\% & 33.25\% & 19.49\% & 18.29\% \\  
Oracle $\mu$C+regression & 4.01\% & 13.73\% & 13.83\% & 11.15\% & 8.57\% & 7.64\% \\
% Highest FLOPs $\mu$C+regression & 9.57\% & 8.52\%  & 6.11\% & 4.42\%  & 5.20\% & 5.81\%  \\ 
\bottomrule
\end{tabular}
% }
\caption{False Positive and False Negative rates of our approach vs baselines. The ratio of FP and FN can be tuned by changing the context change detection threshold.}
\label{fpfnt}
\vspace{-0.2in}
\end{table}


Table~\ref{fpfnt} compares the context-change detection performance of \myname{} (``$\mu$C + regression'') against baselines: 
(a) the same $\mu$Classifier as \myname{} but with a different approach for context change detection based on maximum softmax probability \cite{maxsoft1}.
(b) the \myname{} (Oracle) $\mu$Classifier with regression head (``Oracle $\mu$C + regression''). 
% (c) the \myname{} (Highest FLOPs) with regression head (``Highest FLOPs $\mu$C + regression'') as a lower-bound on the FP and FN rates since it uses the most computation expensive feature extractor.
% 
\myname{} is much more accurate at context change detection compared to the baseline that uses the maximum softmax probability. 
The FP and FN rates of our approach are $10-20\%$ lower than the baseline. 
\myname{} is quite close to the Oracle $\mu$Classifer as well. 
% There is a gap in performance between \myname{} and \myname{} \textbf{(Highest FLOPs)} (2-4\% for Camera Trap and PLACES, and 6-7\% for STL-10) but this is to be expected since we are operating with a lower target accuracy, and have considerable computational gains.
We note that the FP and FN rates can be lowered by increasing the accuracy threshold explained in \S\ref{sec:settings} or by using larger $\mu$Classifiers (e.g. 4 or 5-class) which would incur fewer context switches.



% \begin{table}[t]
% \tabcolsep=0.07cm
% \begin{tabular}{@{}l|lccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{7}{c}{Number of Classes} \\
%  & 10 & 20 & 30 & 40 & 60 & 70 & 100 \\ \midrule
% Accuracy Gain& 4.4\%& 4.7\%& 4.3\%& 4.6\% & 5.3$\%$ & 5.6$\%$ & 6.5$\%$ \\
% SpeedUp (GAP8)&2.33$\times$& 2.26$\times$& 2.18$\times$& 2.10$\times$ & 1.96$\times$& 1.86$\times$ & 1.63$\times$\\ 
% $SD_{sampling}$ ratio& 50.0$\%$& 17.5$\%$& 10.0$\%$& 7.5$\%$ & 6.0$\%$ & 5.0$\%$ & 5.0$\%$\\ 
% \bottomrule
% \end{tabular}
% \caption{Effect of scaling the number of covered classes on \myname{}'s performance (PLACES dataset). $SD_{sampling}$ is the ratio os used $\mu$Cs for training the kNN.}
% \label{scalability}
% \vspace{-0.2in}
% \end{table}

% \begin{table*}[t]
% %\scalebox{1}{
% \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
% \toprule
% & \multicolumn{3}{c|}{20 $\mu$Cs} & \multicolumn{3}{c|}{40 $\mu$Cs}  & \multicolumn{3}{c|}{50 $\mu$Cs} & \multicolumn{3}{c}{60 $\mu$Cs} \\
%   &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0 (ms)} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8 & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Pi0} & GAP8\\ 
%   &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}    &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}
%     &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(ms)}  &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c}{(ms)}\\ 
%   \midrule
% Greedy Selection & 80.92\% & 266.76 & - & 81.55\% & 267.41 & - & 81.65\% & 288.84 & - & 81.97\% & 305.16 & -\\
% Random Selection & 81.30\% & 352.60 & - & 81.22\% & 369.33 & - & 81.31\% & 357.06 & - & 81.53\% & 369.34 & - \\

% %10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
% \midrule
% \end{tabular}
% \caption{End-To-End performance of Local inference; $3\%$ Context change rate}
% \label{local_end-to-end}
% \end{table*}


% \begin{figure}[t]%
%     \centering
%     \subfloat[\centering \label{fig:acc_local}]{{\includegraphics[width=.235\textwidth]{figures/acc_local.png}}}%    
%     \subfloat[\centering \label{fig:late_local}]{{\includegraphics[width=.24\textwidth]{figures/late_local.png}}}%
%     \caption{End-to-End performance of local inference setting using Greedy $\mu$C selector and Top-K most frequent contex ($\mu$C) selector. (a) Classification accuracy and (b) Latency (on Rasp. Pi0; GAP8 results are similar) for different number of stored $\mu$C \HG{This figures need to be replaced with results (table or figures) that demonstrate how our local only version \myname{} still outperform baselines}}
%     \vspace{-0.2in}
% % \label{}
% \end{figure}



\mypara{Effectivenss of the hybrid context switching policy:}
In order to justify the effectiveness of the utilized hybrid context switching scheme, we compared it to fixed-class switching policies. Same as \S\ref{sec:end-to-end}, the hybrid policy let the IoT device switch between 2-class, 3-class, and 4-class contexts. We compare it against policies which only allows switching between 2-class or 3-class  or 4-class contexts. Table \ref{hybrid_perf} shows the accuracy and overall speedup for Serengeti dataset. Generally 3-class and 4-class context switching policies can achieve higher accuracy as they trigger the all-class model less than 2-class or hybrid policies. All-class models are less accurate and overusing them can negatively affect the end-to-end performance. On the other hand, as it was shown in Figure \ref{fig:comp_save_muc_size}, utilizing m-class $\mu$Classifier with higher m leads to higher model inference latency. Since the dominant factor in the overall latency is the inference of the deployed model, 3-class and 4-class policies have lower overall speedup. For instance, \myname{} (Hybrid) achieves 73.8$\%$ accuracy and 2.8$\times$ speedup while the 4-class policy provides 1.1$\%$ accuracy gain at the cost of near no speedup. Overall, \myname{} (Hybrid) outperforms all fixed-class policies in terms of speedup while it achieves a reasonable accuracy. 

% \begin{table}[t]
% \scalebox{0.93}{\begin{tabular}{@{}l|cc|cc@{}}
% \toprule
% Methods & \multicolumn{2}{c|}{Enonkishu} & \multicolumn{2}{c}{Serengeti}\\
%   &\multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{c|}{Pi0 (ms)} &\multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c}{Pi0 (ms)} \\
%   \midrule
% \myname{} (Hybrid) & 92.2\% & 3.5$\times$ & 73.8\% & 2.1$\times$\\
% \myname{} (2-Class) & 91.5\% & 3.9$\times$ & 72.8\% & 1.4$\times$\\ 
% \myname{} (3-Class) & 93.9\% & 1.4$\times$ & 74.1\% & 1.3$\times$\\  
% \myname{} (4-Class) & 93.9\% & 1.0$\times$ & 74.9\% & 1.0$\times$\\
% \bottomrule
% \end{tabular}}
% \caption{Comparison between the hybrid switching policy versus fixed-class switching}
% \label{hybrid_perf}
% \vspace{-0.2in}
% \end{table}



\begin{table}[t]
\scalebox{0.88}{\begin{tabular}{@{}l|ccc@{}}
\toprule
Methods & \multicolumn{3}{c}{Serengeti}\\
  &\multicolumn{1}{l|}{Accuracy} & \multicolumn{1}{c|}{SpeedUp (Pi0)} & \multicolumn{1}{c}{SpeedUp (GAP8)} \\
  \midrule
\myname{} (Hybrid) & 73.8\% & 2.1$\times$ & 2.8$\times$\\
\myname{} (2-Class) & 72.8\% & 1.4$\times$ & 1.7$\times$\\ 
\myname{} (3-Class) & 74.1\% & 1.3$\times$ & 1.4$\times$\\  
\myname{} (4-Class) & 74.9\% & 1.0$\times$ & 1.1$\times$\\
\bottomrule
\end{tabular}}
\caption{Comparison between the hybrid switching policy versus fixed-class switching}
\label{hybrid_perf}
\vspace{-0.2in}
\end{table}


\subsection{Perf. of Local-Only \myname{}} 
\label{sec:selector}
% \HG{We won't evaluate greedy selector anymore. Our greedy selector won't work in our hybrid micro-classifier switching setting. Instead, we are showing how can our approach work with local only scenarios.}
% \HG{The comparison in Table 1 is not fair since CACTUS is using cloud and temporal features. 3. The storage is not
% measured in the experiments. SOLUTION: report the storage overhead of our approach}

This section evaluates the end-to-end performance of the unattended operation (local-only). 
This scenario considers a heavily resource-constrained environment where communication/cloud is not available and the IoT device can fit a limited number of $\mu$Classifiers. Since FAST \cite{FAST} requires online model training and we are assuming the device is not capable of training models, it falls into category of cloud-assisted schemes and not included in this section. 
For switching between $\mu$Classifiers, the all-class model should be deployed on the device and we choose All-Class EfficientNet for this purpose (ResNet-50 is heavy for target processors). 

In order to decide which $N$ $\mu$Classifiers should be stored on the device, we used the training set and applied our hybrid switching policy while the context change detection was considered ideal. Note that the hybrid policy includes m-class $\mu$Classifiers where $m \in \{2, 3, 4\}$. Then $\mu$Classifiers (contexts) were sorted and the most frequently used N $\mu$Classifiers were stored on the device. The hybrid switching policy in the local-only setting is slightly modified and splitted into two stages. In the first stage we apply our hybrid policy on those m-class $\mu$Classifiers from all $m \in \{2, 3, 4\}$ that are available on the device . If none of them is stored on the device the second stage is activated. Here, we consider an available $\mu$Classifier which its corresponding context has the highest overlap with m classes for all $m \in \{2, 3, 4\}$ and apply our hybrid policy on these three available ones.

Table \ref{local_result} shows the accuracy and speedup on GAP8 for \myname{} and baselines. We evaluated \myname{} with 15, 20, and 30 stored $\mu$Classifiers. Results show that by only storing 30 $\mu$Classifiers, \myname{} can achieve 4.1$\times$ and 2.4$\times$ speedup for Enonkishu and Serengeti datasets respectively while the accuracy is on a par with baselines. Note that 30 $\mu$Classifiers constitue less than 1 percent of all possible $\mu$Classifiers for Serengeti dataset. Overall, with a limited number of $\mu$Classifiers \myname{} can maintain its advantage in speedup while its accuracy is either better or on a par with baselines.

\begin{table}[t]
\scalebox{0.9}{\begin{tabular}{@{}l|c|cc|cc@{}}
\toprule
Methods & {} & \multicolumn{2}{c|}{Enonkishu} & \multicolumn{2}{c}{Serengeti}\\
  &\multicolumn{1}{l|}{Storage} &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{c|}{SpeedUp} &\multicolumn{1}{c|}{Acc} & \multicolumn{1}{c}{SpeedUp} \\
  \midrule
All-Class Model& 4.8MB & 89.1\% & 1.0$\times$ & 74.6\% & 1.0$\times$\\
All-Class-Early Exit& 4.9MB & 84.6\% & 2.0$\times$ & 68.7\% & 1.5$\times$\\ 
All-Class-Pruned& 2.6MB & 81.4\% & 1.7$\times$ & 69.6\% & 1.7$\times$\\  
PALLEON \cite{palleon}& 52.1MB & 90.7\% & 1.3$\times$ & 75.1\% & 1.0$\times$\\  
\myname{} (15 $\mu$Cs)& 18.6MB & 89.5\% & 2.2$\times$ & 73.6\% & 2.0$\times$\\
\myname{} (20 $\mu$Cs)& 19.5MB & 90.1\% & 3.5$\times$ & 73.9\% & 2.2$\times$\\
\myname{} (30 $\mu$Cs)& 22.8MB & 90.2\% & 4.1$\times$ & 74.5\% & 2.4$\times$\\
\bottomrule
\end{tabular}}
\caption{End-to-End performance of Local-Only \myname{} and baselines. Speedup numbers are computed for GAP8 (Rasp. Pi0 results show a similar trend).}
\label{local_result}
\vspace{-0.2in}
\end{table}


\begin{comment}
We compare our greedy selection method against Top-K frequent $\mu$Classifiers (contexts). This scheme assumes we have prior information about the distribution of contexts. Both schemes aim to decrease the computation overhead but with different approaches. The greedy selector tries to pick the most efficient $\mu$Classifiers and finally, in its second stage, it guarantees the target accuracy is met by chosen $\mu$Classifiers. On the other hand, the Top-K selector tries to pick the most frequent contexts and store the corresponding $\mu$Classifiers in order to minimize the triggering of the all-class model which imposes a high computation cost. We show results for the Camera Trap dataset as this dataset has temporal flow (30 frames context interval) which is essential for the Top-K approach to extract prior information.

Figure~\ref{fig:late_local} shows the end-to-end latency with different numbers (K) of stored $\mu$Classifiers (averaged over 20 runs). We see that on the Raspberry Pi Zero W platform, we achieve 1.28$\times$ -- 1.42$\times$ speedup over the Top-K scheme when the number of stored $\mu$Classifiers decreases from 50 to 10 (trend on the GAP8 is similar). Results show that the greedy selection of $\mu$Classifiers is more effective than reducing the cost of triggering the all-class model even when the context interval is short (30 frames). 

Figure~\ref{fig:acc_local} shows the end-to-end accuracy with respect to the different numbers of stored $\mu$Classifiers on the device. We see \myname{} with greedy selector has the same or higher accuracy in comparison to the Top-K approach with different number of $\mu$Classifiers. It shows The second stage of the greedy selector is effective in boosting the end-to-end accuracy as it provides accuracy gain over the baseline with prior knowledge while it leads to lower overall latency. 

\end{comment}

\subsection{Ablation Study}
\label{sec:ablation}
\mypara{Effect of context change rate:}
We also evaluated how our end-to-end results change as the interval between context changes varies from every 60 frames to 4 frames on the GAP8 and Pi0 platforms using the PLACES dataset. 
Table~\ref{diff_context} shows that \myname{} maintains its advantage even with higher context change rates i.e. shorter context intervals. 
The speedup decreases slightly from 2.61--1.95$\times$ to 1.97-1.07$\times$ and accuracy gain decreases from 5.1$\%$ to 1.4$\%$ as the interval becomes smaller but \myname{} is still considerably better than the baseline.

\begin{table}[t]
\scalebox{0.93}{\begin{tabular}{@{}l|lccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{6}{c}{Context Interval} \\
 & 4 & 5 & 10 & 20 & 30 & 60\\ \midrule
Accuracy Gain & 1.4\% & 2.3\% & 4.1\% & 5.0\%& 5.4\%& 5.1\% \\
Speedup (Pi0) & 1.07$\times$& 1.18$\times$& 1.56$\times$& 1.85$\times$& 1.95$\times$& 1.95$\times$\\ 
Speedup (GAP8) & 1.97$\times$& 2.01$\times$& 2.59$\times$& 2.83$\times$& 2.81$\times$& 2.61$\times$\\  
\bottomrule
\end{tabular}}
\caption{\myname{} accuracy gain and speedup for the GAP8 with different number of context intervals in comparison to the All-Class Model on PLACES dataset.}
\label{diff_context}
\vspace{-0.2in}
\end{table}


\mypara{Scalability:}
We now look at the scalability of \myname{} with increasing the number of classes. 
% Generally, the performance of any approach drops as the number of classes increases. 
% More classes make the classification task more complex. 
Table~\ref{scalability} shows how \myname{} end-to-end performance changes relative to the All-Class Model as the reference. Note that here we employed fixed 3-class switching policy. We can achieve higher speedup if the hybrid policy is utilized. \M{should we mention due to limitation in time and resources we couldn't use hybrid policy for this evaluation?}
We see \myname{}'s accuracy gain over the All-Class Model increases as we scale up the number classes. 
The performance of All-Class Model significantly diminishes as it encompasses a broader range of classes. 
This expansion in scope leads to a widening gap in accuracy when compared to \myname{}, with the latter maintaining higher performance levels under these conditions. 
% the same which shows \myname{} maintains its advantage in terms of accuracy as the classification task scales up to 100 classes. 
Speedup on GAP8 drops from 2.3$\times$ to 1.6$\times$ since the accuracy of the all-class model decreases with increasing the number of classes and this affects the pipeline's performance and ultimately it imposes more transmission overhead. We expect this gap can be minimized by using a more powerful all-class model. It is possible to keep the speedup in the same range for high number of classes by a deliberate trade-off, utilizing the increased accuracy again to sustain the desired speed performance.


\begin{table}[t]
\tabcolsep=0.07cm
\begin{tabular}{@{}l|lccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{7}{c}{Number of Classes} \\
 & 10 & 20 & 30 & 40 & 60 & 70 & 100 \\ \midrule
Accuracy Gain& 4.4\%& 4.7\%& 4.3\%& 4.6\% & 5.3$\%$ & 5.6$\%$ & 6.5$\%$ \\
SpeedUp (GAP8)&2.33$\times$& 2.26$\times$& 2.18$\times$& 2.10$\times$ & 1.96$\times$& 1.86$\times$ & 1.63$\times$\\ 
$SD_{sampling}$ ratio& 50.0$\%$& 17.5$\%$& 10.0$\%$& 7.5$\%$ & 6.0$\%$ & 5.0$\%$ & 5.0$\%$\\ 
\bottomrule
\end{tabular}
\caption{Effect of scaling the number of covered classes on \myname{}'s performance (PLACES dataset). $SD_{sampling}$ is the ratio of $\mu$Cs used for training the kNN.}
\label{scalability}
\vspace{-0.2in}
\end{table}

% \HG{D3. the inter-class similarity metric works for measuring similarities between 3-classifers. But it might not easily distinguish between 40-classifiers. The issue is relevant because for example, there are 1000 classes in ImageNet, and a 40-classifer would still be considered as a micro-classifier. This issue is not considered in the paper because even the scalability test is conducted on datasets with only 40 classes. Furthermore, it does not necessarily work when there
% are classifiers for different number of classes. SOLUTION: extend the scalability test; update Table 4} 
% \M{Fixed, numbers in Table 4 are computed using only 3-class $\mu$Classifiers not the switching approach. I'm trying to get the numbers using switching possibly, but not sure if I can get them on-time.}

\mypara{Overhead of model training:}
Here, we report the training overhead for classification and context change detection heads. As the feature extractor is pretrained offline and frozen during training of a $\mu$Classifier's heads, we should only do the forward and backward pass for Fully Connected layers which is very fast. Hence we store the embedding for the training set on the cloud and use them for training of $\mu$Classifiers. The training overhead for Enonkishu, Camdeboo, Serengeti, and PLACES datasets are on average 5.4, 5.5, 5.7, and 3 seconds respectively. These numbers are computed for a Tesla M40 24GB GPU.
% The reason behind this negligible drop is that the accuracy all-class model on the cloud side decreases with the increase of number of classes and whenever the IoT detects the context change, the cloud all-class model may not be able to predict the correct class and provides a wrong $\mu$Classifier, and finally it dictates to more transmission overhead. A more powerful all-class model on the cloud can solve the issue. 

% Figure \ref{diff_context_change} shows how the end-to-end results change on the Raspberry Pi Zero W as the context change rates increase from 3\% to 9\%. The latency slowly increases from 88.9 to 100.6 and 297 to 316.4 milliseconds for the STL-10 and PLACES365 datasets respectively. Also, accuracy slightly decreases from 93.6 to 92.7 and 96 to 94.9 for the STL-10 and PLACES365 datasets respectively. Overall, \myname{} keeps its advantage in terms of accuracy and latency even with higher context change rates.

% On the Raspberry Pi Zero-W platform, we get the following results when comparing \myname{} to all-class EfficientNet: a) for the PLACES365 dataset, our approach provides $5\%$ accuracy gain and close to $2\times$ speedup, b) for the Camera Trap dataset, we have comparable accuracy but over $3.5\times$ lower latency, and c) for the STL-10 dataset we achieved $1.5\%$ accuracy gain and $1.2\times$ speedup.

% When comparing \myname{} to always picking the 3-class EfficientNet (the most complex $\mu$Classifier), we find that: a) For the PLACES365 dataset, we are slightly less accurate but have 2x lower latency, b) For the Camera Trap, we have $3\%$ less accuracy but $2.6\times$ speedup, and c) For the STL-10 dataset, 
% \M{Raspberry pi4 will be replaced by gap8 as we want to keep raspberry pi4 for the prototype. Also a graph with varying the context change will be added}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=3in]{figures/CameraTrapDemo.png}
%     \caption{End-to-end implementation of wild-life camera on Raspberry Pi 4B. Video URL: \url{https://anonymous.4open.science/r/CACTUS_-5BF9/README.md}}
%     \label{fig:demo}
% \end{figure}
    
\subsection{Case study: Trail camera}
\label{sec:case-study}
We also provide an end-to-end implementation of a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time on the Raspberry Pi 4B. The link \protect\footnote{ \protect\url{https://anonymous.4open.science/r/CACTUS_-5BF9/README.md}} is provided in the footnote.
In this implementation, we store $60$ $\mu$Classifiers heads and a total of four feature extractors. The total memory footprint of the models is $28$ MB  and that of the feature extractors and all-class model is $17.6$ MB. 
We use a sequence of $2100$ images from the Camera Trap dataset Enonkishu~\cite{Camera_trap_enonkishu} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 


==> Backup/Nov28/Intro-V3.tex <==
% \newpage 
\section{Introduction}

Deep learning methods have been used in many prediction tasks, such as image classification and object detection, due to their outstanding accuracy. 
To enable the economical deployment of deep learning techniques, 
there is significant interest in 
executing deep learning models on low-power embedded systems and IoT devices (e.g. \cite{lai2018enable, warden2019tinyml,mazumder2021survey}). 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.


Prior approaches to squeeze deep learning models fall into three categories.
% (summarized in Figure~\ref{fig:alternatives}). 
The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute.  
The second category is model partitioning, which executes the first few layers of a DNN on the IoT device and the remaining layers on the cloud~\cite{kang2017neurosurgeon,teerapittayanon2017distributed,choi2018deep, cohen2020lightweight, huang2020clio, itahara2021packet}.
The third category is the early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. 
Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/compression.png}
%     \caption{Prior approaches for addressing IoT resource limitations include model compression, partitioning, and early-exit. \HG{we might be able to remove this figure if space is limited}}
%     \label{fig:alternatives}
% \end{figure}

\mypara{Proposed idea: context-aware inference.} 
We argue that one dimension that has not been fully explored in prior efforts is \emph{context-aware inference}. 
Context-aware inference narrows down a prediction task to the current context -- a much shorter time window than the overall time span of the deployed task -- to improve inference efficiency. 
This is similar to how the human brain employs working memory. 
Working memory is a mental workspace where individuals can manipulate and process information relevant to the task at hand. 
It is often estimated to have a fixed capacity (of approximately three or four items’ worth of information)~\cite{luck1997capacity}. 
Despite this constraint, humans utilize this capacity judiciously by bringing into their working memory only the information that is relevant to the current context. 

Similarly, we treat the limited resources on an IoT device as a working memory. 
Instead of attempting to squeeze the original deep learning model into the memory, 
we can bring a smaller model that is relevant to the current context. 
As this paper focuses on classification tasks, we call the smaller model ``context-aware classifiers'', noted as \textit{$\mu$Classifiers}. 
% $\mu$Classifiers focus on classifying only a few relevant classes that appear in contexts and thus can be smaller than the original model that classifies all classes. 
Based on the context, the system dynamically loads the appropriate classifiers into memory, just as humans selectively populate their working memory with relevant information.


% \HG{D2. It is a bit oversimplified to only define context changes as the difference in classes. For example, it is common to see
% context changes as the increase or decrease of classes. The context could also change when the classes remain the
% same, but the samples of each class become more difficult to recognize, such as recognizing pedestrians in the daytime
% or at midnight. These contexts are also relevant as “difficulty” levels for a classifier. However, they are not considered in
% the current design. SOLUTION: clearly define context and justify that some other context definitions (e.g., early exit) are orthogonal to our approach}
% \HG{The definition of the context change is currently unclear and implicitly defined through the data. Real-world deployments
% will have multiple types of context change - from different patterns of objects observed in the field of view, to context
% change due to different weather patterns (rain, fog, snow) or light conditions (bright sunlight/overexposure in parts of
% image) that can happen over short timeframes. It is unclear how robust CACTUS image similarity, context change
% detection, or model selection methods are to the different types of context change and how quickly can the system adapt. SOLUTION: clarify our scope}

This paper defines a ``context'' as a time window where only a subset of classes (called \textit{active classes}) are likely to appear.  
A context change indicates a transition to a time window whose active classes are different from the previous context because a new class comes into the scene. 
We note that other definitions of contexts are possible but not the focus of this paper. For example, a context could also refer to a particular difficulty level of inputs for all classes and a context changes when input samples become more difficult or easier to recognize for reasons such as different weather patterns (rain, fog, snow) or light conditions (bright sunlight/overexposure). 
These definitions are orthogonal to context changes caused by variations in active classes, the focus of this paper.


Context-aware inference is particularly effective in IoT settings because, in many applications, the context can remain fairly static for extended periods.
For instance, a trail camera positioned in a forest may primarily observe the same set of animals. Similarly, a doorbell camera in a residential area is likely to capture the same types of vehicles and individuals recurrently. 
Context-aware inference could be beneficial in various other applications such as industrial monitoring systems where machinery states change infrequently or in smart agriculture where monitoring conditions may remain constant over long growing seasons. This idea holds even greater significance in environments where compute and memory resources are scarce, such as in many IoT devices.



\mypara{Challenges: } Context-aware inference trains resource-efficient $\mu$Classifiers and then dynamically executes the suitable one at runtime depending on the current context. It presents several new research challenges. 

During training, the main challenge is to efficiently create the $\mu$Classifier for every possible context. 
The total amount of contexts grows exponentially with the number of classes. 
For example, if there are 40 classes and we consider 3-class $\mu$classifiers, there are $C^{3}_{40} = 9880$ $\mu$Classifers. 
What's worse, the optimal configuration of a $\mu$Classifer depends on the similarity of classes in the context.  
A context whose classes have similar patterns would be harder to recognize and need to use a $\mu$Classifier that has a higher model capacity.  
If we consider 10 configurations per $\mu$Classifier, then nearly 100K models need to be trained to identify the optimal $\mu$Classifers for all possible contexts. 
Training $\mu$Classifiers with every configuration for each context cannot scale with a large number of configurations and classes.  


% The first challenge is to identify the most resource-efficient $\mu$Classifers for every possible context that reaches a target accuracy. 
% The total number of contexts grows exponentially with the total number of classes. 
% For example, if there are 40 classes and we consider 3-class $\mu$classifiers, there are $C^{40}_3 = 9880$ $\mu$Classifers. 
% And what's worse, the optimal configurations of the $\mu$Classifer depends on the difficulty level of the context.  
% A context whose classes have similar patterns or features would be harder to recognize and need to use a $\mu$Classifier that has higher model capacity.  





At inference time, two additional challenges need to be tackled.  
First, we need a robust and lightweight method to detect context change so that we can switch to an appropriate $\mu$Classifier for the new context. 
% A context is new when an entity that is not in the class set of the current $\mu$Classifier enters the scene.  
Since context change detection lies on the critical path of every prediction, 
the detector needs to be very fast to avoid adding significant computation overhead to the $\mu$Classifier.
Second, after a new class is detected, we need to determine which $\mu$Classifier to switch to -- that is, what are the active classes in the new context. 
We can switch to a $\mu$Classifier that handles more classes including the detected new class, to reduce the frequency of future context switches. 
However, a $\mu$Classifier with more classes tend to be more computation-intensive and thus has higher inference costs per input frame.
On the other hand, a $\mu$Classifier that recognizes only the new class can be more efficient but will cause more frequent context switches and thus higher switch costs. 
We need to design a context switching policy that considers the fundamental trade-off between the number of active classes in contexts and the overhead from context switches. 


% we also need to deal with variable connectivity to enable unattended operation as well as cloud-assisted operation.
% In particular, when cloud-assistance is unavailable or bandwidth too limited,  a subset of $\mu$Classifiers need to be pre-trained and stored locally in the limited IoT storage.


There have been a few approaches that explore context awareness, but they don't address all dimensions of the problem.
The most relevant works~\cite{palleon, han2016mcdnn} leverage class skewness in video processing to improve efficiency but have to rely on cloud servers to switch between models, limiting their applicability to devices with network connectivity. 
Other approaches assume known class skews~\cite{FAST} or tailor DNN inference to specific applications without studying how to handle context changes effectively~\cite{kang2017noscope, jiang2018chameleon, leontiadis2021s}.

\mypara{The \myname{} approach:} 
We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}\footnote{CACTUS: Context-Aware Classification Through Ultrafast Switching.}.

Our work has three major contributions. 
First, we develop an \emph{inter-class similarity} metric to estimate the difficulty in classifying the active classes in each context.
We show that this metric is highly correlated with the optimal choice of configurations for the $\mu$Classifier, and hence allows us to rapidly and cheaply estimate the best configuration for each $\mu$Classifier without incurring training costs.

Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new class. 
This separation allows us to invoke the heavyweight classifier sparingly thereby reducing the computational cost.

Third, we develop a simple yet effective context switch policy that  determines the $\mu$Classifer to switch to via a single tuning knob. 
Depending on how fast active classes change in a particular deployment environment, the tuning knob can be controlled to automatically determine the number of active classes in contexts, achieving a balance between context switching costs and the performance gain of context-aware inference. Furthermore, the policy can deal with variable connectivity between an IoT device and the cloud to enable unattended operation where the device switches between popular $\mu$Classifers cached locally only, as well as cloud-assisted operation where the device can request new $\mu$Classifers to be created and download them for new contexts.

% Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers to store on-device for unattended operation. Our method leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. 

We implement \myname{} by modifying EfficientNet-B0 \cite{efficientnet} and conduct extensive evaluation across five datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and three camera trap datasets, Enonkishu \cite{Camera_trap_enonkishu}, Camdeboo \cite{Camera_trap_camdeboo}, and Serengeti (season 4) \cite{Camera_trap_serengeti}) and multiple IoT processors (Risc-V(GAP8) \cite{URL:GAP8} and low-end ARM 11 \cite{URL:Arm11} to high-end Cortex-A77 \cite{URL:Cortex-A77}). We show that:
\begin{itemize}[leftmargin=0.24in]
    \item \myname{} reduces computational cost by up to X$\times$ while outperforming all-class EfficientNet-B0 in accuracy.
    \item Our inter-class similarity metric accurately captures the hardness of a set of classes in a $\mu$Classifier (0.86-0.97 Pearson's coefficient with classification accuracy).
    \item \myname{}'s context change detector has 10-20\% fewer false positives and false negatives than an alternate lightweight detector that uses similar FLOPs. 
    \item End-to-end results on the Raspberry Pi Zero W and GAP8 IoT processors show that \myname{} can achieve 1.6$\times$ -- 5.0$\times$ speed-up and up to $6.5\%$ gain in accuracy compared to All-Class EfficientNet. We also show that \myname{} in Local-Only setting has up to 4.1$\times$ speed-up compared to All-Class EfficientNet by storing at most 30 $\mu$Classifiers.
    
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Nov28/Intro.tex <==
% \newpage 
\section{Introduction}

There has been significant activity in recent years in optimizing deep learning methods for low-power embedded systems and IoT devices (e.g. \cite{lai2018enable, warden2019tinyml,mazumder2021survey}). 
%  vlin2021memory
% While there is great diversity in the computational capabilities (e.g. low-power microcontrollers, neural architectures and heterogeneous multi-core processors) and communication capabilities (e.g. BLE and WiFi) of these devices, they share the constraint that they are heavily resource constrained. 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.

% \mypara{Squeezing deep learning models on IoT platforms.} 
Prior approaches to squeeze deep learning models fall into three categories (summarized in Figure~\ref{fig:alternatives}). The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute. 
% Knowledge Distillation~\cite{hinton2015distilling, li2014learning} leverages the features from the larger and deeper "teacher" models to train smaller and shallower "student" models by forcing the student models to learn and capture the distribution of the features from the teacher models. 
%Other recent efforts \cite{leontiadis2021s, liu2021adaspring} focus on training dynamic networks that can adapt to input during inference by executing different sub-networks. 
% 
The second category is partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud~\cite{kang2017neurosurgeon,teerapittayanon2017distributed,choi2018deep, cohen2020lightweight, huang2020clio, itahara2021packet}
% 
The third category is early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


% Figure~\ref{fig:alternatives} shows the two classes of techniques. The first is approaches to squeeze a larger model into an IoT device's memory/compute limitations. Range of techniques including pruning, quantization, sparsification, early exit etc which have been very successful. Another line of work is on partitioning models i.e. splitting between an IoT device and a more powerful edge server/cloud. These techniques typically execute a few layers on the IoT device and remaining layers on the cloud. \DG{if focus is on local-only, we can skip mention of partition-based methods here.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations include model compression, partitioning, and early-exit.}
    \label{fig:alternatives}
\end{figure}

\mypara{Context-aware inference and its challenges:} 
We argue that one dimension that has not been explored in prior efforts is \emph{context-aware inference}. 
Our endeavor in developing context-aware inference models draws inspiration from the remarkable efficiency of the human brain, particularly, how humans employ working memory. Working memory, a fundamental cognitive mechanism, serves as a mental workspace where individuals can manipulate and process information relevant to the task at hand. Unlike an inexhaustible reservoir, it has a limited capacity. In fact, working memory is often estimated to have a fixed capacity (of approximately three or four items’ worth of information) \cite{luck1997capacity}. Despite this constraint, humans utilize this capacity judiciously. They have a knack for bringing into their working memory only the information that holds relevance for the current context. This discerning selection of information is immensely advantageous as it prevents the cognitive system from getting overwhelmed by the vast expanse of knowledge a human possesses, as much of this knowledge is often extraneous to the immediate task.

What if we borrowed idea of working memory from human cognition and integrated it into our deep learning models? We advocate for an approach that emulates the human working memory by constructing multiple, petite, context-aware classifiers (we refer to these as \textit{$\mu$Classifiers}). Each of these \textit{$\mu$Classifiers} would be akin to a segment of working memory, specialized in handling specific types of information or tasks. Based on the task at hand, the system would dynamically bring the appropriate classifiers into memory, just as humans selectively populate their working memory with relevant information.

% We argue that knowledge of the current context and the classes that are likely to be present given the current context can greatly improve performance in resource-constrained settings. 

What makes context-aware inference particularly effective and relevant in IoT settings is that, in many applications, the context can remain fairly static for extended periods.
For instance, a trail camera positioned in a forest may primarily observe the same set of animals. Similarly, a doorbell camera in a residential area is likely to capture the same types of vehicles and individuals recurrently. Context-aware inference could be beneficial in various other applications such as industrial monitoring systems where machinery states change infrequently, or in smart agriculture where monitoring conditions may remain constant over long growing seasons. This idea holds even greater significance in environments where compute and memory resources are scarce, such as in many IoT devices.


% We refer to a context-aware classifier as a $\mu$Classifier since it can focus on a subset of the overall set of classes, making it more resource-efficient and accurate.

% This paradigm shift necessitates a change in a key assumption that underlies all prior work i.e. that the classifier is trained to recognize all classes of interest and this set of classes does not change at run time.

Translating the intuitive concept of using working memory into a practical neural network model presents a plethora of challenges. Human working memory operates on a foundation of sophisticated semantic knowledge, however, our current capability in capturing context within neural networks is considerably more constrained. Thus, the first challenge is how to judiciously group classes into the current context to achieve optimal performance from a computational perspective,

% The first is that we need to minimize training overhead given the large number of $\mu$Classifiers. For example, even with only 20 classes, there are $C^{20}_3$ (1140) three-class $\mu$Classifiers and $C^{20}_4$ (4845) four-class $\mu$Classifiers that are possible (if we go with the parallel of human working memory holding three or four chunks of information). 
% In addition, there are a number of parameters to tune per class combination to optimize its size and complexity via model compression --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. %It is impractical to pre-train and optimize a huge number of $\mu$Classifers.
%As we show later, the optimal parameters depend greatly upon the specific set of classes in the $\mu$Classifier --- subsets that are easy to separate can be compressed significantly without losing accuracy whereas classes that are similar and hard to separate cannot be compressed as much. Thus, it is clearly impractical to pre-train and optimize a huge number of $\mu$Classifers.
%This separation between easy and hard class combinations is similar, in spirit, to the underlying principle in early exit models i.e. that there are easy and hard data cases but in our cases we extend this idea to class combinations.

The second challenge is that we need a robust method to detect context change so that we can switch to the appropriate $\mu$Classifier for the new context when an entity that is not in the class set of the current $\mu$Classifier enters the scene. In addition, the computational complexity of executing such a context change detector cannot be high else it can outweigh the benefits of using a context-aware $\mu$Classifier.

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the lowest computation while meeting the desired accuracy, coverage across classes of interest, and not exceeding available storage. 

\mypara{The \myname{} approach:} We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}.\footnote{\myname{} connotes the back-and-forth nature of switching between $\mu$Classifiers depending on context.}

Our work has three major contributions. First, we develop a similarity-aware kNN-based model configuration predictor to reduce training overhead. 
The core building block for our method is an \emph{inter-class similarity} metric to estimate the difficulty in classifying the set of classes in each $\mu$Classifer. 
We show that this metric is highly correlated with the choice of configurations for the model, and hence allows us to rapidly and cheaply estimate the best configuration for each classifier without going through an expensive training process for each configuration.

Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the frequency of invoking the heavyweight classifier.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.

% In this paper, we present a novel solution that addresses these problems. 
% %Our key idea is to design a lightweight mechanism for detecting context switch events, and a rapid way of determining the optimal parameters for a new $\mu$Classifier. 
% First, we define a inter-class similarity metric that captures the similarity of classes and the hardness of distinguishing them.
% A kNN takes the statistics of computed inter-class similarities as the input and predicts the optimal parameters for the $\mu$Classifier corresponding to a subset of classes. 
% %The optimal parameters for a $\mu$Classifier are the ones meeting a target accuracy with low computation. 
% Second, we add a regression head to the $\mu$Classifier as the second output head to detect context changes. 
% Since the classification and regression heads share a feature extractor, the overhead for context change detection is negligible. 
% %The regression head is supposed to output a value close to 0 for the current context and a value close to 1 for the rest of the classes.
% Third, we present a budget-limited $\mu$Classifier selector that selects the lightest $\mu$Classifiers covering all classes in the dataset while not exceeding storage available. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our-approach.png}
%     \caption{Our approach uses a context-aware classifier that determines the entities that are currently present in view of the IoT camera, determines what model parameters to use based on how ``complex'' the set of classes are, and then switches to the appropriate micro-classifer. \DG{Needs to be re-drawn to a full version across two columns - this is just a sketch}}
%     \label{fig:our-approach}
% \end{figure}

We implement \myname{} by modifying EfficientNet-B0 \cite{efficientnet} and conduct extensive evaluation across three datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}) and multiple IoT processors (Risc-V(GAP8) \cite{URL:GAP8} and low-end ARM 11 \cite{URL:Arm11} to high-end Cortex-A77 \cite{URL:Cortex-A77}). We show that:
\begin{itemize}
    \item \myname{} can provide up to 13$\times$ reduction in computational cost while outperforming all-class EfficientNet-B0 across a wide range of desired accuracy thresholds. 
    \item Our inter-class similarity metric captures the hardness of a set of classes in a $\mu$Classifier very well (0.86-0.97 Pearson's coefficient between classification accuracy and our metric).
    \item \myname{}'s context change detector has 10-20\% fewer false positives and false negatives than an alternate lightweight detector that uses similar FLOPs. It has only  3-7\% higher false positives and false negatives than a heavyweight detector that uses 2-4$\times$ more FLOPs. 
    \item End-to-end results on the Raspberry Pi Zero W and GAP8 IoT processors show that \myname{} can achieve 1.2$\times$ -- 4.4$\times$ speed-up and up to $5\%$ gain in accuracy compared to all-class EfficientNet. We also show that our greedy algorithm that selects a subset of $\mu$Classifiers to balance accuracy, FLOPs, and coverage under storage constraints has up to 1.4$\times$ speed-up compared to a solely coverage-focused method.
    
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Backup/Nov28/intro-hui.tex <==
% \newpage 
\section{Introduction}

Deep learning methods have been used in many prediction tasks, such as image classification and object detection, due to their outstanding accuracy. 
To enable economical deployment of deep learning techniques, 
there is significant interest in 
executing deep learning models on low-power embedded systems and IoT devices (e.g. \cite{lai2018enable, warden2019tinyml,mazumder2021survey}). 
These devices are heavily resource-constrained in terms of compute and storage, and typically need to operate at very low energy budgets (a few milliwatts on average) to ensure that they can run for weeks or months on battery power.


Prior approaches to squeeze deep learning models fall into three categories (summarized in Figure~\ref{fig:alternatives}). 
The first is approaches to compress the model via pruning, quantization, and knowledge distillation. 
For example, model pruning~\cite{han2015deep} and model quantization~\cite{jacob2018quantization, li2020train} techniques reduce the number of the neurons in the models or the number of the bits of the feature representation to achieve less compute.  
The second category is model partitioning, which executes the first few layers of a DNN on the IoT device and remaining layers on the cloud~\cite{kang2017neurosurgeon,teerapittayanon2017distributed,choi2018deep, cohen2020lightweight, huang2020clio, itahara2021packet}
The third category is early-exit inference which takes advantage of the fact that most data input can be classified with far less work than the entire model. 
Hence, early exit models attach exits to early layers to execute the easy cases more efficiently~\cite{teerapittayanon2016branchynet, kaya2019shallow}.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/compression.png}
    \caption{Prior approaches for addressing IoT resource limitations include model compression, partitioning, and early-exit.}
    \label{fig:alternatives}
\end{figure}

\mypara{Proposed idea: context-aware inference:} 
We argue that one complementary dimension that has not been explored in prior efforts is \emph{context-aware inference}. 
Context-aware inference narrows down a prediction task to current context -- a much shorter time window than the overall time span of the deployed task, to improve inference efficiency. 
It draws inspiration from the remarkable efficiency of the human brain, and particularly, how humans employ working memory. 
Working memory is a mental workspace where individuals can manipulate and process information relevant to the task at hand. 
It is often estimated to have a fixed capacity (of approximately three or four items’ worth of information)~\cite{luck1997capacity}. 
Despite this constraint, humans utilize this capacity judiciously by bringing into their working memory only the information that holds relevance for the current context. 

Borrowing the idea of working memory to deep learning, we can treat the limited resources on an IoT device as a working memory. 
Instead of attempting to squeeze the original deep learning model into the memory, we can bring a smaller model that is relevant for the current context. 
As this paper focuses on classification tasks, we call the smaller model ``context-aware classifier'', noted as \textit{$\mu$Classifiers}. 
$\mu$Classifiers focus on classifying only a few relevant classes that appear in contexts and thus can be smaller than the original model that classifies all classes. 
Based on the contexts, the system would dynamically bring the appropriate classifiers into memory, just as humans selectively populate their working memory with relevant information.


Context-aware inference is particularly effective in IoT settings because, in many applications, the context can remain fairly static for extended periods.
For instance, a trail camera positioned in a forest may primarily observe the same set of animals. Similarly, a doorbell camera in a residential area is likely to capture the same types of vehicles and individuals recurrently. 
Context-aware inference could be beneficial in various other applications such as industrial monitoring systems where machinery states change infrequently, or in smart agriculture where monitoring conditions may remain constant over long growing seasons. This idea holds even greater significance in environments where compute and memory resources are scarce, such as in many IoT devices.



\mypara{Challenges: } Context-aware inference poses several research challenges. 
The first challenge is how to create resource-efficient $\mu$Classifiers for every possible context. 
The total amount of contexts grows exponentially with the number of classes and the optimal $\mu$Classifier depends on the set of classes in the context -- subsets that are easy to separate can use a model with less computational efforts whereas classes that are similar and hard to separate need a model with a higher complexity. 
This calls for a metric to measure the similarity between classes and the difficulty level of a context. 

The second challenge is that we need a robust method to detect context change so that we can switch to the appropriate $\mu$Classifier for the new context when an entity that is not in the class set of the current $\mu$Classifier enters the scene. 
In addition, the computational complexity of executing such a context change detector cannot be high; otherwise, it can outweigh the benefits of using $\mu$Classifiers.

The third challenge is that $\mu$Classifiers also need to be stored on a resource-limited IoT device to switch between them at run-time. Given limited storage resources, we need an effective method to determine which subset of $\mu$Classifiers can offer the lowest computation while meeting the desired accuracy, coverage across classes of interest, and not exceeding available storage. \HG{need to update this challenge to match with the one in Overall system design.}

\mypara{The \myname{} approach:} We propose a novel paradigm for scalable and efficient context-aware classification that we refer to as \myname{}.\footnote{\myname{} connotes the back-and-forth nature of switching between $\mu$Classifiers depending on context.}\HG{Can we name the paper using the bird that is most adaptive/smart? like Pigeons, are pretty adaptive and smart. Another remote connection is we do camera trap.. so it feels like a bird-friendly project.}

Our work has three major contributions. 
First, we develop an \emph{inter-class similarity} metric to estimate the difficulty in classifying the set of classes in each context.
We show that this metric is highly correlated with the optimal choice of configurations for the $\mu$Classifier, and hence allows us to rapidly and cheaply estimate the best configuration for each $\mu$Classifier without going through an expensive training process for each configuration.



Second, we design an efficient context change adaptation pipeline by splitting the process into two parts -- a lightweight context change detector that executes on each image as a separate head attached to each $\mu$Classifer, and a more heavyweight context predictor that executes a regular all-class classifier to identify the new context. 
This separation allows us to execute context change detection on each image at a low cost:  the lightweight context change detector reduces the frequency of invoking the heavyweight classifier.

Third, we develop a greedy algorithm that chooses the best set of $\mu$Classifiers given storage limitations on the device. 
Our approach leverages the above-mentioned similarity metric to select $\mu$Classifiers that are most efficient and yet complementary to cover the desired set of classes. This method allows us to determine a minimal bag of $\mu$Classifers to store on-device.


We implement \myname{} by modifying EfficientNet-B0 \cite{efficientnet} and conduct extensive evaluation across three datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{Camera_trap_enonkishu,Camera_trap_camdeboo}) and multiple IoT processors (Risc-V(GAP8) \cite{URL:GAP8} and low-end ARM 11 \cite{URL:Arm11} to high-end Cortex-A77 \cite{URL:Cortex-A77}). We show that:
\begin{itemize}
    \item \myname{} can provide up to 13$\times$ reduction in computational cost while outperforming all-class EfficientNet-B0 across a wide range of desired accuracy thresholds. 
    \item Our inter-class similarity metric captures the hardness of a set of classes in a $\mu$Classifier very well (0.86-0.97 Pearson's coefficient between classification accuracy and our metric).
    \item \myname{}'s context change detector has 10-20\% fewer false positives and false negatives than an alternate lightweight detector that uses similar FLOPs. It has only  3-7\% higher false positives and false negatives than a heavyweight detector that uses 2-4$\times$ more FLOPs. 
    \item End-to-end results on the Raspberry Pi Zero W and GAP8 IoT processors show that \myname{} can achieve 1.2$\times$ -- 4.4$\times$ speed-up and up to $5\%$ gain in accuracy compared to all-class EfficientNet. We also show that our greedy algorithm that selects a subset of $\mu$Classifiers to balance accuracy, FLOPs, and coverage under storage constraints has up to 1.4$\times$ speed-up compared to a solely coverage-focused method.
    
    % \item Across the different compute capability of IoT processors, \myname{} could achieve better latency from 1.1x - 3.4x compared to other baselines.
    % \item \myname{} outperforms baselines on a range of IoT processors (from low-end ARM 11 \cite{} to more powerful GAP8 \cite{URL:GAP8} and Cortex-A72 \cite{Cortex-A72}), across different datasets (STL-10 \cite{STL10}, PLACES365 \cite{PLACES365}, and Camera Trap \cite{}).
\end{itemize}

% 1) What problem the paper tries to address?
% 2) Why the problem is important?
% 3) Why existing solutions are insufficient?
% 4) What is the basic idea of our solution? What are the distinctive features of our solution?
% 5) What are the challenges to make our solution work well?
% 6) How do we address those challenges?
% 7) What are the experimental results and conclusions?
% 8) What are the list of contributions this work makes?


==> Design-old.tex <==
\section{Inter-class Similarly}



\section{Configuration Prediction}
\label{sec:configuration-prediction}
% The key premise in our work is that given a total of $N$ classes, a classifier that works on only a subset of these $N$ classes can afford to be more computationally efficient compared to the classifier that works on the entire set of $N$ classes since classification tasks with fewer classes is significantly easier. 

The goal of the configuration selector is to identify the best configuration of the $\mu$Classifier for an arbitrary subset of classes. 
We note that the ``best configuration'' is defined based on application needs, i.e.  the available resources and accuracy tolerance for the application. 
For example, when resources are a priority (e.g. highly constrained IoT devices), then there may be more tolerance for lower accuracy. 
In the rest of the paper, we refer to the best configuration as the one that achieves the lowest resource demands while meeting a target accuracy $Acc_{thr}$ (as defined for the application). 

A naive way of constructing a $\mu$Classifier is to simply replace the \emph{all-class} model's classification head that targets $N$ classes with a head that targets the desired subset of classes. 
However, the resulting $\mu$Classifier provides minimal performance benefits since the computation bottleneck usually lies in the feature extractor instead of the classification head. Thus, to achieve computational savings from a $\mu$Classifier, the $\mu$Classifier needs to use a more lightweight feature extractor. This raises two questions: (1) \textit{What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? }, and (2) \textit{How to quickly identify the most efficient yet accurate $\mu$Classifier, given any subset of classes?}

% \begin{enumerate}
%     \item What configurations should we tune to have a large resource-accuracy search space of $\mu$Classifiers? 
%     \item How to quickly identify the most efficient yet accurate $\mu$Classifier, given a subset of classes?
% \end{enumerate}


\subsection{Multi-Dimensional Configuration Space}

We start by addressing the first question. 
While there are a number of techniques that can be used to compress machine learning models, we specifically look for configuration parameters that provide large dynamic range of resource-accuracy tradeoffs for $\mu$Classifiers.

We find that two methods are particularly effective for configuring $\mu$Classifiers --- image resolution and filter pruning. Varying the resolution of the image that we provide as input to the $\mu$Classifier is particularly effective because a) the computation complexity of a feature extractor decreases quadratically as resolution (height and width) decreases, and b) we find that the lower resolution inputs are sufficient when the $\mu$Classifier is separating more dissimilar classes. Filter pruning with different sparsity ratios to control the computation complexity of the feature extractor is also effective. 
In addition, we utilize post-training quantization to further lower the inference runtime and reduce the model size.

% In this work, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset).
%  can be augmented with other secondary techniques such as filter pruning and quantization for further expanding the configuration space.

% Thus, our overall configuration space is as follows. 
% In the model size dimension, we apply filter pruning with different sparsity ratio to control the computation complexity of the feature extractor. 
% In the image resolution dimension, we consider different resolutions ranging from about $58\times58$ to higher (depending on the dataset). 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.

Figure~\ref{res_size_vs_size} shows that varying both image resolution and pruning level scales down better as compute decreases compared to varying only the pruning level. Each point shows the average accuracy across all 3-class subsets of 10 classes.  We see that varying both resolution and pruning level provides us configurations with lower computation costs while accuracy remains in a reasonable range. Pruning performs poorly in the low FLOPs regime since it requires very high pruning levels which leads to very low accuracies.

\begin{figure}[h]
    \includegraphics[width=0.4\textwidth]{figures/res_size_vs_size_V3.png}
    \caption{Configuring resolution and model size (by varying the pruning level) provides us a large dynamic range in resource-accuracy tradeoffs for configuring $\mu$Classifiers. (Camera Trap dataset is used.)}
    \label{res_size_vs_size}
\end{figure}

% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. 
% As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. 
% Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.



\subsection{Inter-class similarity as a metric for resource-accuracy tradeoffs}
\label{k-nn}

The core challenge during the process of training $\mu$Classifiers is determining the most likely configuration (i.e., resolution and model sizes) without needing to train a huge number of them. 
% A $\mu$Classifier can be made computation-efficient by compressing the model via filter pruning and reducing the resolution of input images. 
Suppose there are $R$ different image resolutions and $S$ different sparsity levels, they lead to a total of $R\times S$ $\mu$Classifiers to evaluate in order to identify the best one for an arbitrary subset of classes. 
Therefore, for a classification problem with a total of $N$ classes, if we consider building $\mu$classifiers for $m$ out of $N$ classes (i.e., an \textit{m-class combination}), we will need to train a total of $C^{N}_m \times R \times S$ models to find the best $\mu$Classifier for every $m$-class combination, which can be prohibitively expensive.

% Furthermore, there is no single configuration that can fit all possible class combination well.  
% Figure~\ref{} illustrates problem. 
% We sample different combinations of three classes from the  STL image classification dataset which has a total of 10 classes. 
% The configuration of $\mu$Classifiers for the sampled combinations varies XX-XX\% in terms of computation efficiency. 
% \HG{fill in the figure and the number; fill in the figure.}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/heatmap.png}
    \caption{Heatmap shows how model complexity relates to the similarity among classes (darker $\implies$ higher accuracy). X-axis shows thirty 3-class combinations sorted from low to high similarity and Y-axis shows different models (sizes and resolutions) sorted from least to most compute complexity. We see that when classes have low similarity, even low-complexity models can achieve high accuracy, but when classes have high similarity, there is significant performance degradation for low-complexity models.}
    \label{heatmap}
\end{figure}
 
A commonly used technique for reducing the computational overhead of searching for the optimal configuration of a classifier is Neural Architecture Search (NAS \cite{NAS1,NAS2}). 
% However, this method doesn't address the problem due to two fundamental limitations. 
% First, 
although gradient-based NAS~\cite{gdas1, gdas2} can avoid the training of $R \times S$ number of $\mu$Classifiers on a given subset of classes, it still needs to examine $C^N_{m}$ number of $m$ class combinations, each of which incurs significant training overhead.
% Second, to the best of our knowledge, existing gradient-based NAS approaches usually search model architectures given a fixed image resolution and cannot simultaneously search configurations w.r.t. both image resolution and model architecture. 
Thus, we need a different method for efficiently determining the best configuration of a $\mu$Classifier.

\mypara{Key Idea:} Our key idea is to define a ``similarity'' metric that captures how similar classes are within a subset of classes. 
Our hypothesis is that two subsets of classes that have similar statistics of inter-class similarities would also share a similar $\mu$Classifier configuration. 

We design the vector ``similarity'' representation for a subset of $m$ classes based on statistics of \textit{inter-class similarities}--that is, the similarities among the $m$ classes. 
The rationale is that, if the $m$ classes are more similar to each other, the classification task addressing the $m$ classes is more difficult and thus requires classifiers with higher computation complexity.
% ; 
% if two $m$ class combinations have similar statistics of inter-class similarities, then the two combinations are likely to use similar $\mu$Classifier configuration. 

To measure the similarity between two classes, we first need to find a representation for each class. 
For each input image of a specific class, we can get its embedding from a feature extractor that is trained on all $N$ classes. 
Given a set of input images of that class, we can average the embedding of all images as the \textit{class representation}. 
We calculate Cosine Similarity between one class representation and another as the similarity between the two classes. 
The vector representation of an $m$ class combination is the mean and standard deviation of similarities among all class pairs.
Mathematically, let $s_{i, j}$ be the cosine similarity between class $i$ and class $j$. Then the representation of an m class combination $C$, where $|C|=m$, is:
\begin{equation}
    [\text{mean}(\{s_{i, j}\}), \text{std}(\{s_{i, j}\})], i, j \in C. \label{eq:rep_vector}
\end{equation}

\mypara{Does similarity capture resource-accuracy tradeoffs?} 
Figure~\ref{heatmap} shows that the ``similarity'' metric generally tracks the resource-accuracy tradeoffs. We sample 30 different 3-class combinations from the  STL-10 image classification dataset. We sort these combinations in terms of their mean similarity (Eq \ref{eq:rep_vector}) from low to high (X-axis). 
The Y-axis shows the model complexity of $\mu$Classifiers measured by FLOPs. 
Each entry in the heatmap reports the accuracy of the $\mu$Classifier with a specific FLOPs for a 3-class combination (darker is higher accuracy). 

When the mean of inter-class similarities is low, the classes are easily separable, hence even low-resource models can obtain similar accuracy as their high-resource counterparts. But when the mean of inter-class similarities is high, the classes are hard to separate, hence there is a significant accuracy gap between low-resource and high-resource models.
% 
Thus, we see that the similarity metric that we have defined tracks resource-accuracy tradeoffs quite effectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knn_train.png}
    \caption{To build the training dataset for the kNN, we (a) use similarity-directed (SD) sampling to select $x$ subsets of classes, and determine the best configuration for each subset as the ground truth label (e.g., Config3 and Config4); and (b) for each subset, calculate the mean and std of inter-class similarities to get its vector representation.}
    \label{fig:kNN-training}
\end{figure}

\subsection{kNN-based configuration selection}
\label{sec:knn}
Given that inter-class similarity accurately tracks resource-accuracy trade-offs of a $\mu$Classifier, we can use a kNN-based predictor to predict which configuration to choose for a given combination of classes. 
As shown in Figure~\ref{fig:kNN-training}, the kNN takes as input the vector representation (Eq.~\ref{eq:rep_vector}) of the desired $m$ class combination and predicts the configuration that is most efficient for the combination. 


% \mypara{Similarity-directed sampling.} 
The challenge of training the kNN in a resource-efficient manner is to build an effective training set. 
On the one hand, we want the samples to have a good coverage of the spectrum of $m$-class combinations so that we can predict the best configuration of the remaining combinations accurately. This is critical to ensure the performance of kNN--based prediction. 
On the other hand, we want as small amount of samples as possible because for each sample, we need to train all possible $\mu$classifiers to identify the best one. 
Thus, the training costs grow linearly with the number of samples we selected. 

To sample efficiently, we propose a \textbf{similarity-directed sampling} scheme that samples at different levels of hardness in the training dataset. 
First, we compute the mean of pair-wise similarity for all combinations. 
We then cluster them into four groups of similarity (quartiles). We then sample randomly from each cluster to gather enough data samples for training the kNN.
Compared to random sampling, our empirical evaluation on three datasets demonstrates that similarity-directed sampling can reduce 25-66\% of samples while getting similar prediction accuracy.  



% \mypara{Input for kNN training.} The input to train the kNN comprises the vector representation (Eq.~\ref{eq:rep_vector}) for the chosen m-class subsets and their best $\mu$Classifier configuration. We note that the ``best configuration'' is defined based on the application needs i.e the resources available and accuracy tolerance for the application. For example, when resources are a priority (e.g. highly constrained IoT device), then there may be more tolerance for lower accuracy. 
% \DG{We need a figure to show this stage}


% Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{\HG{change this table to figure}}
% \label{sampling}
% \end{table}

\section{Budget-limited $\mu$C selection}
% \HG{we do not have an evaluation section corresponding to the classifier selection component} 
So far, we have looked at how the kNN can be used to determine the best $\mu$Classifier configuration for an $m$-class combination. 
However, we may not be able to train and/or store all $m$-class subsets. This raises another question:
\textit{How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes?}
% \begin{enumerate}
%     \item How should we quickly identify the best subsets to choose from among the $C^N_m$ $m$-class subsets of all $N$ classes.
% \end{enumerate}


\subsection{The $\mu$Classifier selection problem}
The best set of $m$-class $\mu$Classifiers to store on a device should be able to cover all classes that can possibly occur in a scene, and achieve the highest classification accuracy and computation efficiency than any other sets. 
The rationale of covering as many classes as possible is to enable smooth switching between $\mu$Classifiers -- that is, at least one $\mu$Classifier should work in any possible context. 

The problem can be re-phrased as a combinatorial optimization problem: given a set of $m$-class $\mu$Classifiers, each with a classification accuracy and resource consumption, determine which $m$-class $\mu$Classifiers to include in the collection so that the total resource consumption is minimized while each model meets a target accuracy threshold and the collection meets some class coverage requirement. The problem can be proved to be at least NP-hard by reducing it to a knapsack problem~\cite{salkin1975knapsack}. 
We next elaborate on our greedy algorithm to approximate the optimal solution. 

% \M{Our solution has a different objective in comparison to the stated problem. The Problem says we want to maximize accuracy s.t a budget limit. But our approach aims to minimize computation s.t that the accuracy over a threshold. Do you agree?}
 
\subsection{Greedy $\mu$classifier selection} 




% k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}\HG{I added the above subsection 5.1}

% \mypara{Greedy $\mu$classifier selection.} 
% The greedy algorithm heuristically selects the best set of $n$ $\mu$Classifiers where $n$ is a specified parameter that is chosen based on storage or other constraints. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined.

Assume that the IoT device can fit $n$ $\mu$Classifiers. 
The greedy algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset. 
If it cannot cover all $N$, then we restrict the process to the most frequent classes that occur within $N$. 

Then, the greedy method proceeds in two stages.
First, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. 
In the first stage, the method identifies the $\mu$Classifier with the highest FLOPs in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPs over set $C$ doesn't decrease compared to the previous iteration. 
Note that this selection procedure is done solely with the predictions from the kNN and does not involve training of the $\mu$Classifiers.

At this point, $n$ $\mu$Classifiers with low computation are chosen and are trained so we know their actual accuracy. 
Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. 
If this is the case, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy while maintaining the coverage of $N$. Since the selection is based on kNN prediction, we again need to go through the process of training the newly selected model to check if the accuracy requirement ($Acc_{thr}$) is satisfied.
% In the first iteration, we don't know the accuracy of available $\mu$Classifiers as they are not trained. 
% As a result, we start with the lightest available $\mu$Classifier and train it to check the accuracy condition. 
If so, the replacement happens; otherwise, the process repeats and the next lightest $\mu$Classifier will be selected and trained. 
% and checked until the replacement happens. 
% Now the average accuracy of $\mu$Classifiers in set $C$ is again computed to check if it reaches the $Acc_{thr}$. 
This process continues until the $Acc_{thr}$ threshold is met. 
In our experience, kNN has high accuracy, hence the number of times a $\mu$Classifier in the selected set needs to be replaced is very low.

\mypara{Optimizing storage requirements:} 
Since $\mu$Classifiers that operate on the same model size (same pruning level) share the same model weights, we can further reduce storage requirements by storing one feature extractor per model size, and then only storing the classification and context change detection heads for each chosen $\mu$Classifier. 

% only a limited number of $\mu$Classifiers out of the final set C were trained as the second stage finishes fast due to the high accuracy of the kNN. In other words, kNN performs poorly on only a small portion of the combinations in set C at the end of the first stage, and those $\mu$Classifiers should be replaced to adjust the average accuracy.

% \subsection{Local and Edge-cloud} 

% We now look at how the budget-limited $\mu$Classifier selection process can be leveraged in the context of IoT deployments.

% \mypara{Local processing on IoT devices.} The first scenario is when the IoT device is operating autonomously. Since IoT devices are resource-limited and on-demand training of classifiers is expensive, we need to pre-load a set of $\mu$Classifiers on the device prior to deployment. 

% The main challenge is storage since IoT devices have limited storage space and thus cannot afford to keep hundreds or thousands of $\mu$Classifiers locally. 
% Thus, we need to use the budget-limited $\mu$Classifier selection process to select an optimal set of $\mu$Classifiers to load on a device (given storage limitations) such that the device can switch between them to make accurate predictions. 

% During inference, the choice of the full-class model to run for context change detection depends on available resources. On single-core low-power platforms, the full-class model also needs to be resource constrained hence a lightweight model like full-class EfficientNet can be used as the switching model.

% On heterogenous multicore ultra-low power processors (e.g. NXP's i.MX family with Cortex-A7 and Cortex-M4 cores), the full-class model can be a more computationally heavy model like ResNet since it can use the more powerful core upon detecting context change.

% \mypara{Edge-cloud assisted IoT devices.} 
% Our system is also useful when an IoT device is operating with edge-cloud support. In this scenario, the IoT device locally executes the $\mu$Classifier and transmits images to the edge-cloud when it detects a context change. 
% The edge-cloud uses a more powerful model to determine whether a new class needs to be added to the $\mu$Classifier. 
% It then uses the kNN to decide the configuration parameters for the new $\mu$Classifier and trains the model on the fly. The parameters of the trained model are then downloaded to the IoT device.

% Despite the fact that edge-cloud resources are plentiful, it is still beneficial to cache a few $\mu$Classifiers on the IoT device to reduce the frequency with which model parameters need to be downloaded via a wireless link. Frequent wireless communication consumes energy and bandwidth and incurs additional latency of switching between models. 
% The edge-cloud can use the budget-limited $\mu$Classifier selection procedure to decide which models to cache at the IoT device given its resource limitations.


\section{Context-aware Switching}
\label{context_change}

An essential part of making our system work is precisely detecting context change and, once detected, rapidly switching to the right $\mu$Classifier for the new context. 
A context change happens when an input image frame falls into an unknown class that is not covered by the current $\mu$Classifier. 
Since context change detection lies on the critical path of every prediction, the detector should be very fast.  

\mypara{Detecting context change:} 
The first step in context-aware switching is detecting when the current context has changed. Detecting context changes for a $\mu$Classifier is essentially the same as detecting out-of-distribution samples, which falls into the area of uncertainty estimation~\cite{ensemble1,mcdrop1,testtime1,testtime2,maxsoft1,naff1,naff2,aff1,aff2,aff3}. 
Although many approaches have been proposed for uncertainty estimation, most of them are computationally intensive and thus cannot be applied in a real-time scenario (see Section~\ref{related}).  
Among all the approaches, Maximum Softmax Probability~\cite{maxsoft1} is the cheapest way to capture out-of-distribution samples. 
However, as we show later, this method doesn't have a satisfying performance in our work as the false positive and false negative rates are high. 

In this work, we introduce a regression-based context change detector. 
Specifically, a regression head is added to the $\mu$Classifier as the second output head alongside the classification head. 
The regressor outputs a value around 0 for the classes on which the $\mu$Classifier is trained and a value around 1 for all other classes i.e. for a new context. Both the classification and regression heads share the feature extractor of the $\mu$Classifier and thus the additional computation overhead introduced by the regressor is negligible. 
Since the output of the regressor is a continuous value, a threshold, $\theta$, is needed to distinguish between the current context and the new context. 
This threshold is dataset-dependent and tunable considering the trade-off between the ratio of false positives and false negatives. 
We set $\theta=0.5$ by default.

\mypara{Classifier switching:} The second step is switching from the current $\mu$classifier to one appropriate to the new context. For this, we need to first determine what are the new class(es) that are in the scene. This is accomplished by an \emph{all-class} model that determines which are the classes that need to be included in the new $\mu$classifier. Once this is determined, we use a simple technique where the last $p$ predictions made by the pipeline are observed and the farthest predicted class among the previous set of classes is substituted by the new ones. 

As described in \S\ref{sec:overview}, the \emph{all-class} model can be either executed locally or at the edge cloud depending on connectivity. Executing the all-class model at the edge cloud allows us to use more powerful and more accurate models for determining the classes in the current context, which in turn can lead to more precise switching. 

% \section{Budget-limited $\mu$C selection} 

% We now turn to another resource dimension i.e. storage constraints on an IoT device. A device could have limited storage space and thus cannot afford to keep all $\mu$Classifiers locally. Thus, a key step is to select the optimal set of $\mu$Classifiers to load on a device such that the device can switch between them to make accurate predictions. 

% Note that this problem is important whether the IoT device is operating autonomously or with edge-cloud support. In the latter case, it is still beneficial to cache the optimal set of $\mu$Classifiers to reduce the frequency with which model parameters need to be downloaded via a wireless link (which consumes energy and bandwidth).

% % k-NN provides us $\mu$Classifiers, each corresponding to an m class combination. In the situation that there is no network, the device can only rely on the stored $\mu$Classifers. In order to switch between the $\mu$Classifiers, the all-class model should be executed on the device which imposes a high latency as no filter pruning is applied on this model and it utilizes the full-resolution images. To partially compensate for the overhead of the all-class model, we should select n $\mu$Classifiers with the least average computation overhead while they cover all N classes of the dataset. In case the network is available, storing $\mu$Classifiers on the device is optional as the cloud is able to transmit the $\mu$Classifiers to the device.

% The problem of selecting an optimal $\mu$Classifier set needs to consider the implications of resource-accuracy tradeoffs on switching overhead and missed detections.
% A $\mu$Classifer may be computationally cheaper than another, but it may have a higher False Positive Rate (FPR). This higher false positive rate will trigger the \emph{all-class} model more often and increases the overall latency. We also need to consider the False Negative Rate (FNR) since this can decrease latency but at the cost of missing context changes. In order to consider the effect of the FPR and FNR, we compute the expected FLOPs for each $\mu$Classifier considering a fixed context change rate and calculated FPR and FNR on the validation set. The formula is shown below:

% \begin{equation}
%   \label{exp_comp}
%   \begin{aligned}[b]
%   &F_i= CCR\times\left(FNR\times f_i + (1-FNR)\times(f_i+f_{full})\right) +\\
%   &(1-CCR)\times\left(FPR\times(f_i+f_{full}) + (1-FPR)\times f_i\right)
%  \end{aligned}
% \end{equation}

% In equation \ref{exp_comp}, $CCR$ is the context change rate, $f_i$ is the FLOPs of the $\mu Classifier_{i}$ and $f_{full}$ is the FLOPs of the all-class model. $F_i$ calculates the expected compute cost for an image if $\mu Classifier_{i}$ is deployed on the device.

% \DG{We need something here about why the problem is NP Hard and needs a greedy approximation.}

% \mypara{Greedy $\mu$classifier selection.} 
% Our greedy algorithm heuristically selects the best set of $\mu Classifiers$ that fit within the storage constraints of the IoT device. kNN predicts $\mu$Classifiers for all combinations, then these $\mu$Classifiers will be trained and their accuracy, FPR, and FNR are calculated. Using FPR and FNR, the expected FLOPs (Eq \ref{exp_comp}) for each $\mu$Classifier is determined. Let us assume that the IoT device can fit $n$ $\mu$Classifiers. The algorithm starts by initializing the set $C$ with $n$ random $\mu$Classifiers that cover the $N$ classes of the dataset (if it cannot cover all $N$, then we pick the most frequent subset that it can cover). 

% Then, the greedy method proceeds in two stages --- first, it optimizes the computation while maintaining coverage, and second, it compensates for errors in the kNN prediction. In the first stage, the method identifies the $\mu$Classifier with the highest expected FLOPS in set $C$ and replaces it with the lightest available $\mu$Classifier that maintains the coverage of $N$ for the updated set $C$. This process continues until the average of expected FLOPS over set $C$ doesn't decrease compared to the previous iteration.

% At this point, $n$ $\mu$Classifiers with low computation are chosen. Since the kNN is not a perfect predictor, some predicted $\mu$Classifiers may not meet the target accuracy. To address this, our method picks the $\mu$Classifier with the lowest task accuracy in set $C$ and replaces it with the lightest available $\mu$Classifier with a higher task accuracy maintaining the coverage of $N$. Now the average accuracy of $\mu$Classifiers in set $C$ is computed to check if it reaches the $Acc_{thr}$. If not, this process continues until the threshold is met.

%  \begin{algorithm}
%         \caption{GreeComp}
%         \label{Alg1}
% \begin{flushleft}
%         \textbf{INPUT} 
%         \\$N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs; $C_{sel}$: selected $\mu$Classifiers; COV: Coverage of selected set.
% \end{flushleft}
%         \begin{algorithmic}[1]
%             \State  Initialize $C_{sel}$ with $n$ random $\mu$Cs s.t COV($C_{sel}$)== $N$
%             \While{$Avg_{Flops}(C_{updated}<Avg_{Flop}(C_{sel})$}
%                 \State $c_{max} \leftarrow$ Classifier with max cost in $C_{sel}$
%                 \For{$m \notin C_{sel}$}
%                     \State $C_{try} = (C-c_{max})\cup m$
%                     \If {$COV(C_{try}) == N \land Acc(C_{try}) < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                     \EndIf
%                 \EndFor
%             \EndWhile
%             \State Train classifiers in set $C_{selected}$
%             \State \DG{the second stage comes here}
%             \While{$Acc_{C_{sel}} < Acc_{thr}(C_{sel})$}
%                 \State $c_{min} \leftarrow$ Classifier with min acc in $C_{sel}$
%                 \For{$m \notin C_{sel} \land COV(C_{sel}-c_{min}+m) == N$}
%                     \State Train $m$ \If{Acc($C_{sel}-c_{min}+m < Acc_{thr}$}
%                         \State $C_{updated} = C_{try}$
%                         \State \DG{incomplete}
%         \end{algorithmic}
% \begin{flushleft}            
%         \textbf{OUTPUT}
%         \\$C$: Chosen Set of Combinations   
% \end{flushleft}           
%     \end{algorithm}


\begin{comment}
 \begin{algorithm}
        \caption{Budget-limited $\mu$Classifier Selection}
        \label{Alg1}
\begin{flushleft}
        \textbf{INPUT} 
        \\$S$: $\mu$Cs sorted by FLOPs, $N$: Num of classes in the dataset, $n$: Num of desired $\mu$Cs, $COV$: Coverage of the selected set
\end{flushleft}
        \begin{algorithmic}[1]
            \State  Initialize $C$ with $n$ random $\mu$Cs s.t $COV(C)==N$
            \State Initialize $Comp_{new}=0$ and $Comp_{old}=1$
            \While{$Comp_{new}<Comp_{old}$}
            \State $Comp_{old}=Comp_{avg}(C)$ \Comment{Average of FLOPs over C}
            \State $m=Comp_{max}(C)$ \Comment{$\mu$C with highest FLOPs in $C$}
            \State $idx=Index(m)$ \Comment{index of $m$ in $S$}
            \For{$i=1$ to $idx$}
            \If{$S[i] \notin C \land COV(C-m + S[i])==N$}
            %\State del $m$ from $C$
            %\State add $S[i]$ to $C$
            \State $C=C-m + S[i]$
            \State break
            \EndIf
            \EndFor
            \State $Comp_{new}=Comp_{avg}(C)$
            \EndWhile    
            \State Train $\mu$Classifiers in C and get the accuracy
            \While{$Acc_{Avg}(C)<Acc_{thr}$}
            \State $l, acc_l=Acc_{min}(C)$ \Comment{least accurate $\mu C$ and its acc}
            \For{$i=1$ to $|S|$}
            \State Train S[i] and get its accuracy (if not yet trained) 
            \If{$S[i] \notin C \land A[i]>acc_l$}
            %\State del $l$ from $C$
            %\State add $S[i]$ to $C$
            \If{$COV(C-l + S[i])==N$}
            \State $C=C-l + S[i]$
            \State break
            \EndIf
            \EndIf
            \EndFor
            \EndWhile                 
        \end{algorithmic}
\begin{flushleft}            
        \textbf{OUTPUT}
        \\$C$: Chosen Set of Combinations   
\end{flushleft}           
    \end{algorithm}
\end{comment}


 
% In any classification problem, the confusion matrix shows that some classes are easier to handle and the classifier labels them with high accuracy while there may be a class that a bigger number of its samples is misclassified by other classes. It can be explained by the fact that some classes have a higher similarity and hence the model struggles to distinguish them for a portion of their samples. Consider there are three classes, bird, dog, and cat, obviously a dog looks much more similar to a cat than a bird. To classify dogs and cats a more complex model needs to be employed while a simpler model can handle the classification task of birds and dogs. As a result, it is not efficient to employ a single model for different sets of classes. To demonstrate that, we picked ten combinations of three classes from the STL-10 dataset and tested multiple models on them. 

% Figure \ref{our_vs_other} shows that a fixed configuration cannot be both efficient in computation and accurate for every set of classes. All 120 combinations of three classes from the STL-10 dataset were divided into 10 clusters. We calculated the mean of pair-wise similarities for a combination and we used these values to cluster 120 combinations into equal-size clusters. Each point represents the average accuracy in a cluster. We can see that the blue line shows a consistent accuracy of around $93\%$. This consistency is achieved by picking a configuration with the least FLOPS while it has accuracy over a threshold. If we assume the desired accuracy is close to $93\%$, the fixed model represented by the green curve only works for the first few clusters. On the other hand, the fixed model corresponding to the red curve doesn't meet our target accuracy for the last three clusters. As a result, a scheme is needed to choose the right model for each set of classes. 

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/our_vs_other_v2.png}
%     \caption{Accuracy of five models on ten distinct combinations of three classes from STL-10 dataset}
%     \label{our_vs_other}
% \end{figure}

% \subsection{Inter-Class Similarity Measurement:}
% \label{similarity}
% To measure the similarity between two classes, we first need to find a representation for each class. The output vector of the oracle’s feature extractor is picked to represent a class, which we will refer to as a feature vector in the following. To be more consistent and reduce the effect of any noise, $K$ samples are randomly selected from each class and the average of their feature vector is used for the representation. The cosine distance computes the similarity between the feature vector of two classes (The closer the cosine distance to 1, the more similar the two classes are).

% \subsubsection{Configurations for Efficient Model Selection:}
% IoT nodes are limited in computation resources and it is not rational to use a single complex model for all possible sets of classes. The variety in hardness of different sets of classes motivated us to look for a way to assign each set the most efficient model. We considered two knobs for controlling model complexity and its required computation overhead, the image resolution and the number of filters in convolutional layers.

% As the effect of image resolution on a convolutional neural network's computation overhead is near quadratic it is a very top choice for reducing a network's FLOPS. Pruning is a popular technique to decrease the model's computation cost, reduce its size, and make it more memory efficient with a small accuracy drop. 
% Generally, pruning can be categorized into structured and unstructured methods. In unstructured pruning methods, a convolutional neural network is sparsified by converting weights with a small magnitude into zeros \cite{upruning1,upruning2}. 
% This results in unstructured sparsities and specialized hardware and software are needed to speed up the inference runtime. As a result, unstructured pruning is not a good fit for our work as we are not aiming for a specific hardware or processor. On the other hand, structured pruning techniques \cite{spruning1,spruning2}, which crop unimportant filters in convolutional layers do not need specialized hardware. As the entire filters are deleted it can effectively make the inference time faster and decrease the needed amount of memory for storing the model's weights and intermediate representations.


% Among different criteria for pruning the filters, approaches using $\ell2,1-norm$ \cite{str_p1,str_p2} have shown remarkable results despite being simple and straightforward. 
% In our work, filters are ranked based on their $\ell1-norm$ values and those which fall below the user-defined cut-off will be pruned. 
% By specifying different pruning cut-offs we can have several levels ($M$) of model size and complexity. 
% We applied the filter pruning on the pre-trained ImageNet weights for the EfficientNet-B0 model. 
% Image resolution plays a huge role in computation overhead as its effect is nearly quadratic and even a minor downsampling can highly reduce a model's FLOPS. As the second knob, several resolutions ($N$) are considered so that in total we can have $M\times N$ different configurations to be assigned to each set of classes. Figure \ref{res_size_vs_size} shows model size with image resolution can highly broaden the configuration space compares to the model size. These two knobs cover a big range of FLOPS while the accuracy is in a reasonable range. 
% We utilized post-training quantization to further lower the inference runtime and reduce the model size.


% \subsubsection{k-NN as the Model Selector:}
% \label{sec4.4.3}
% In the proposed framework, a k-NN is responsible for choosing the most efficient model configuration. However, the popular technique for discovering the optimal network architecture for a specific need is the Neural Architecture Search (NAS). NAS consists of three major components, search space, the optimization method, and the evaluation method. The search space contains candidate networks and the optimization method decides how to search among those candidates. The evaluation method is a tool for the optimizer to test the networks and decides the search direction until it meets the predefined objectives. However, NAS is very slow and computationally expensive \cite{nas1} as it explores a lot of solutions with different levels of complexity. Also, it's not possible to vary resolution in existing gradient-based NAS approaches while changing resolution is a top variable for shrinking a network's computation burden. On the other hand, k-NN is quite fast and suitable for real-time applications.

% The k-NN's input is supposed to be statistics of pair-wise similarities and the output (label) is an efficient configuration delivering high accuracy and low computation. To label a set of classes we pick a configuration with the smallest FLOPS meeting inequality \ref{ineq1}:
% \begin{equation}
%     \label{eq1}
%     A(x)=\{Acc(x,baseline), Acc(x,cfg_1), ..., Acc(x,cfg_{|Config|})\}
% \end{equation}
% \begin{equation}
%     \label{eq2}
%     Accuracy_{thr} = \underset{x \in tr\_ds}{median}[median(A(x))]
% \end{equation}
% \begin{equation}
%     \label{ineq1}
%     Accuracy(C,cfg_i)\geq Accuracy_{thr} 
% \end{equation}
% in the above inequality, $C$ refers to the set of target classes, $Config$ is the configuration space, $cfg_i \in Config$. In equation \ref{eq2}, $tr\_ds$ represents all sets of classes in the training dataset. Based on inequality \ref{ineq1}, we are looking for the lightest model giving test accuracy over the threshold accuracy. The user can control the computation overhead by changing Margin p as it directly affects labels. A high margin leads to models with higher FLOPS while a small margin tends to pick configurations with a lower number of FLOPS. In our work, we considered EfficientNet-B0 with no downsampled input covering all classes as the reference. The selected configuration determines the $\mu$Classifier for the target set of classes $C$.


% For k-NN inputs, different statistics were examined and two of them showed promising performance. Consider $C=\{c_i,c_j,c_k\}$ as a set of classes. In section \ref{similarity}, we explained how the similarity between two classes is computed using the cosine distance. For $C$ there are three pair-wise similarities, $similarity(c_i,c_j), similarity(c_i,c_k)$, and $similarity(c_j,c_k)$. The mean and standard deviation of these three numbers are the statistics we feed to k-NN as the input.


% A dataset should be prepared to train the k-NN based on what has been explained above. Assume a dataset consists of twenty classes, hence there are 1140 combinations of three classes for this dataset. For each of these combinations, $M\times N$ $\mu$Classifiers should be trained and then tested to compute the accuracy so we can pick the most efficient $\mu$Classifier for each of them. 
% Since it is highly time-consuming, only a small subset of combinations should be selected to prepare a dataset for training the k-NN. 
% To sample efficiently, We propose a similarity-directed sampling scheme to include different levels of hardness in the training dataset. The mean of pair-wise similarity is computed for all combinations and we cluster them based on their $33\%$ and $66\%$ percentiles. Then we sample randomly from each cluster to gather enough data samples for training the k-NN. Table **** shows that the similarity-directed sampling trains a more accurate k-NN compared to random sampling based on the mean accuracy difference between the predicted $\mu$Classifier and the efficient $\mu$Classifier over the test set and it is the case for the number of FLOPS as well.
% \begin{table}[h]
% \begin{tabular}{@{}l|ccc@{}}
% \toprule
% Number of Samples & \multicolumn{2}{c}{Accuracy Difference}  \\
%   &\multicolumn{1}{c|}{Similarity-Directed} & \multicolumn{1}{c}{Random}\\ 
% \midrule
% 20 & -0.876\% \textpm 0.496 & -1.136\% \textpm 0.526 \\
% 40 & -0.870\% \textpm 0.318 & -0.994\% \textpm 0.337 \\
% 60 & -0.814\% \textpm 0.258 & -0.892\% \textpm 0.251 \\
% 100 & -0.804\% \textpm 0.201 & -0.824\% \textpm 0.195 \\
% 150 & -0.789\% \textpm 0.173 & -0.802\% \textpm 0.172 \\
% 200 & -0.769\% \textpm 0.146 & -0.780\% \textpm 0.133 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{sampling}
% \end{table}



% \section{$\mu$Classifier Constructor}
% k-NN outputs an efficient configuration and the corresponding $\mu$Classifier should be trained so we can transmit it to IoT. 
% The feature extractor for every model size ($M$) was once trained (fine-tuned) on all classes before and its weights are stored in the cloud and the IoT. 
% As a result, the feature extractors are initialized using their corresponding stored weights and are frozen during the training of classification and context change detector heads. 
% Experiments have shown this initialization is good enough so we don't need to train the feature extractor again. It also makes the training process much faster as the dominant part of the network is not needed to be trained. The mentioned two heads will be quantized after being trained to lessen transmission latency. Finally, the classification and context change detector heads and feature extractor ID will be transmitted to the IoT. IoT will load the feature extractor corresponding to the transmitted ID and connect it to the two received output heads.
% \label{new_model}




==> Discussion.tex <==
\section{Discussion}

==> Implementation.tex <==

\section{Implementation}\DG{THIS SECTION HAS BEEN MOVED INTO EVAL SINCE ITS TOO SHORT TO BE STANDALONE}
We tested \myname{} on three IoT accelerators and processors using three datasets. The implementation details are described below.

An NVIDIA Tesla M40 24GB GPU was used for training models and as the edge-cloud in some of our experiments. 

We implement the \myname{} pipeline on three different IoT devices --- Raspberry Pi 4B, Raspberry Pi Zero W and GAP8. We generate \textbf{TensorFlow Lite} models using the default optimization and int-8 quantization to reduce model size and the execution latency. 

For profiling on Raspberry Pi 4B and Zero W, we utilize the \textbf{TVM} framework \cite{} to tune the operation orders to reduce the execution latency for the Arm Cores. 

For the profiling on GAP8, we use the GAP8 tool chain \cite{} to transform the \textbf{TensorFlow Lite} models into C code by fusing the operations. 

On all the platforms, we profile the execution latency of the models of the different configurations on the different datasets.

% \mypara{Configuration.} \DG{Since the giant table of configurations was removed, that is no longer described anywhere…can you add a summary of that here (there was another spot where Hui's comment mentioned it)}

\mypara{Local implementation optimizations.} \DG{We never really describe for “local” that we optimize further by storing only four feature extractors (one for each resolution) and then store only the two heads...that needs to be mentioned and some numbers should be added.}


% \mypara{Case study: Trail camera.} While resource usage depends on the number of models and configurations, we provide end-to-end memory benchmarks for one implementation instance on the Raspberry Pi 4B running at $1$ GHz (see \cite{} for a video demo). The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows a working end-to-end system.

% \mypara{Case study: Trail camera.} While resource usage depends on the number of models and configurations, we provide end-to-end memory benchmarks for one implementation instance on the Raspberry Pi 4B running at $1$ GHz (see \cite{} for a video demo). The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows a working end-to-end system.

% In this implementation, we store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. 

\mypara{Open source code.} If accepted, we will make our code on all above platforms openly available so that others can build on this work.

% \mypara{Case study: Trail camera.} In order to better visualize how the \myname{} pipeline works, we built a demo on the Raspberry Pi 4B running at $1$ GHz. The application is a wild-life camera that can be deployed in the wild to capture images of animals or birds and classify them in real-time. The video in \cite{} shows an example.

% In this implementation, We store $60$ $\mu$Classifiers and the feature extractors. The total memory footprint is $28$ MB and that of the feature extractors and full models is $17.6$ MB. We use a sequence of $2400$ images from the Camera Trap dataset \cite{Camera_trap_enonkishu,Camera_trap_camdeboo} to visualize the demo but we can also directly obtain input from the Raspberry Pi camera. Given the current context, we resize the captured images into $4$ different sizes: $100$, $160$, $240$, $320$ and use the corresponding feature extractors and $\mu$Classifiers to generate the classification results and regression results. 

% For the regression results, we use a threshold of $0.6$ to trigger the context change. When the regression results are smaller than $0.6$, we consider the current context might not be appropriate anymore and trigger the full model to do the inference again. The full model is latency-heavy on the Raspberry Pi 4B which will cost more than $600$ ms. The all-class model uses the image of the size $320$ as input and will generate the classification results of $11$ classes. Based on the classification results, we will find the most proper context. We find the new combinations of 3-class in a First-In-First-Out(\textbf{FIFO}) manner by removing the oldest classes and adding the latest predicted classes. If the new combination has no valid $\mu$Classifiers, we will iteratively remove the second and third oldest classes instead of the first one. If there is no valid combination using the heuristic, we will randomly sample one valid combination containing the predicted class. 

% When the regression results are larger than the threshold, we will remain on the current context and accept the predicted $3$-class results. Overall, we find out that we could achieve $82\%$ accuracy and $16\%$ rate of triggering the all-class models.




==> Outline/outline.tex <==
\section*{Outline: }

\mypara{page allocation for a 12 page paper}
\begin{itemize}
    \item intro: 2 page 
    \item motivation: 2 pages 
    \item design: 4 pages 
    \item eval: 3-4 pages 
    \item others(related work, conclusion): 1 page
\end{itemize}

\section*{Case for Context-aware Micro-classifiers}

Many methods exist to reduce the computational cost of executing classifiers of IoT devices. We argue that each of these have their limitations when scaled down to small processors/resources.

\mypara{Limits of alternate approaches} Existing techniques include a) squeezing the size of the classifier using a variety of model compression techniques, or b) using early exit to reduce computation cost. Both have limits.
\begin{itemize}
\item \emph{Graph: Accuracy vs Size.} Show that a 10 or 20 class classifier will lose accuracy quickly if squeezed below some threshold size for either method (under some resource constraints in terms of number of layers/parameters)

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/Acc_vs_Model_Size.png}
%     \caption{Accuracy Drops as the model gets smaller (Places Dataset)}
%     \label{fig:accuracy_vs_model_size}
% \end{figure}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/STL_All_Config.png}
    \caption{Accuracy Drops when models get squeezed and resolution is decreased - Blue: 3 Classes, Red: 10 Classes}
    \label{fig:accuracy_vs_size}
\end{figure}


\item Fewer classes is better. Classifiers with fewer classes is better from performance perspective.
\end{itemize}

\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/STL_Acc_vs_Classes.png}
    \caption{Accuracy Drops as the classifier coverage increases (STL Dataset)}
    \label{fig:accuracy_vs_classes}
\end{figure}

\mypara{Temporal correlation in classes} In many static deployments, there is significant temporal stability and context change is not frequent. 
\begin{itemize}
    \item \emph{Graph: Median #classes vs Temporal window.} For different temporal windows (30min, 1hr, 2hr, 3 hr, etc), show the median number of classes that occur. Use camera-trap dataset.
\end{itemize}


\begin{figure}[h!!!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/CDF_Temporal.png}
    \caption{CDF for number of unique classes in different temporal windows (Camera Trap Dataset)}
    \label{fig:CDF_Temporal}
\end{figure}


\mypara{Our idea: Context-aware Micro-classifiers.} To scale down in resources, our idea is to use context-aware $\mu$Classifiers combined with context change detection. Context-aware $\mu$Classifiers consume less resources and can offer \textcolor{red}{higher accuracy} in resource-constrained settings. But they introduce new problem --- need to switch to a different set of classes when detecting that the context has changed. However, as shown above, there is temporal consistency, so context don't change very frequently for static sensor deployments.

\section{Design Challenges}

$\mu$Classifiers introduce several new design challenges.

\mypara{Challenge 1: How should we decide the appropriate model for a micro-classifier for an arbitrary subset of classes?}

\begin{itemize}
\item \textbf{decide the right model architecture for a given set of classes.} Larger model achieves higher accuracy but minimal performance gain; smaller model achieves higher performance gain but could suffer from accuracy drop. Show the trade-offs between model complexity v.s. accuracy v.s. performance benefit. [Table~\ref{fig:uC-performance}]
% Different sets of classes have different optimum model parameters. Show that the choice of the optimum parameters can make a significant performance difference.
\item \textbf{many combinations of classes: combinatorial space; different combinations have different appropriate model complexity} Cannot pre-train models for every possible subset of classes. show that pre-training all possible combinations to identify the appropriate model is prohibitive (or a bad idea): Each combination of classs has N model options; total combination variants are M, the entire model to train is $N^M$. [Our solution: KNN for configuration prediction, trained on a subset of combinations (say 20$\%$)]
\end{itemize}

\mypara{Challenge 2: How to reliably detect context change to switch between micro-classifiers?}

\begin{itemize}
\item In the absence of reliable context change detection, can lose accuracy (false negatives) and increase overhead (false positives). Accuracy drop and Overhead of context change detection has to be low. [Our solution: linear regressor-based prediction.]
\end{itemize}

% \mypara{Challenge 3: How to rapidly training a new classifier for the current context i.e. set of classes that occur in the current context?}

% \begin{itemize}
% \item In the absence of reliable context change detection, can lose accuracy. 
% \item Overhead of context change detection has to be low.
% \end{itemize}

\section*{Design}

\mypara{Overview [1 page]}
\begin{itemize}
\item Overall figure showing the microclassifier + multiple heads + (optional cloud-side or local) context-change detection
\item describe the entire pipeline/flow. 
\end{itemize}

\mypara{Micro-classifier configuration prediction [2 pages]}
\begin{itemize}
\item What is our configuration space? we choose resolution/size instead of just size. why? Add figure: x-axis is FLOPS; y-axis is accuracy; two curves - one for resolution + size; one curve - only by varying size.  
\item Why does the configuration need to be carefully selected for each set of classes in the micro-classifier? show that a bad selection leads to poor results...or a default selection is far from optimal. Add a figure: x-axis: XXnumber of different class combination, y-axis: accuracy; several curves, each corresponds to a fixed configuration; expected: there is no single configuration that can fit all class combination well. This motivate us to search the best configuration for each single class combination.  
\item how to find the best configuration for each combination of classes? NAS v.s. KNN. NAS has two limitations: 1) too expensive because identifying the best configuration using NAS requires training XX of DNNs sampled from the configuration space; 2）cannot vary resolution in existing gradient-based NAS approach. 
\item We describe the basic idea of our approach: KNN-based predictor. Two challenges to address: (1) what is the representation for each class combination: solution: a new ``similarity'' metric such that each class is represented as a vector \[mean pair-wise similarity, std\]
\item (2) how to generate the training dataset for KNN? We sample a set of class combinations and train all the configurations for each class combination to select the best one. The question is how to sample effectively? One option is random sampling; we propose similarity-directed sampling. Evaluation: random v.s. similarity-directed sampling. Expected: similarity-directed sampling is more sample efficient--that is, given the same amount of training dataset, similarity-directed sampling  has higher test accuracy. Another perspective: how many samples is need to achieve the same accuracy. 
\item Notes: Highlight a) how do we predict micro-classifier for each combo of classes, b) our choice for how to make it configurable (resolution/size)


\end{itemize}


\mypara{Context Change Detection [0.5 page]}
\begin{itemize}
\item List two potential solutions and mention that they won't work. The first potential solution is to have another NN trained for detecting changes. Mention several research papers in this direction. Cons: additional costs; 
\item The second potential solution is to use the softmax value + threshold. Cons: less accurate. 
\item Our proposed solution: extra context change detection head. Add a table: compare the three approaches to show our solution is the best. 
\item implementation issues: (1) where do we want to context change to happen? Option 1: on device; More compute but works in cases where no communication available. Option 2: on cloud. Pro: less compute on device but need to communicate with the cloud.
\end{itemize}

\section*{Evaluation}

\subsection{Micro-classifier evaluation.} 

\mypara{Eval of similarity metric.} How well does our similarity metric capture actual difficulty level of combining the class. Show scatterplot of similarity metric vs accuracy of the 3-class classifier - maybe using EfficientNet and lower resolution. Then report the pearson correlation coefficient between them.

\mypara{Eval of config selector.} Compare accuracy and speedup of model that uses configuration parameters selected using kNN to full resolution 3-class EfficientNet.

\begin{table*}[ht]
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{3}{c|}{Camera Trap} & \multicolumn{3}{c|}{STL} & \multicolumn{3}{c}{PLACES} \\
 & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Speedup} & \multicolumn{1}{l|}{Mem}  & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Speedup} & \multicolumn{1}{l|}{Mem} & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Speedup} & \multicolumn{1}{l}{Mem} \\ \midrule
Easy & -4.29\% & 10.03$\times$ & -$\times$ & -5.446\% & 3.430$\times$ & -$\times$ & -2.421\% & 5.184$\times$ & -$\times$\\
Hard & -2.41\% & 5.19$\times$ & -$\times$ & -2.861\% & 1.887$\times$ & -$\times$ & -1.033\% & 2.865$\times$ & -$\times$ \\
\midrule
All & -3.35\% & 7.61$\times$ & -$\times$ & -4.153\% & 2.658$\times$ & -$\times$ & -1.727\% & 4.025$\times$ & -$\times$ \\
\midrule
\end{tabular}
\caption{How well does the config selector perform against the most powerful model (full resolution 3-class EfficientNet)? }
\label{fig:uC_full3-performance}
\end{table*}

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.904$)\label{fig:CameraTrap_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Acc_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL ($r=-0.974$) \label{fig:STL_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Acc_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES ($r=-0.857$)\label{fig:Places_acc_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Acc_Vs_Similarity_V2.png}}}%
    \caption{Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets.}
\label{fig:acc_vs_sim}
\end{figure*}



\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($r=-0.934$)\label{fig:CameraTrap_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_SpeedUp_Vs_Similarity_V2.png}}}%
    \subfloat[\centering STL ($r=-0.973$) \label{fig:STL_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_Speedup_Vs_Similarity_V2.png}}}%
    % \qquad
    \subfloat[\centering PLACES ($r=-0.81$)\label{fig:Places_speedup_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_Speedup_Vs_Similarity_V2.png}}}%
    \caption{Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets - Speedup against full resolution 3-class or All-Class EfficientNet (Table~\ref{fig:uC_full3-performance})}
\label{fig:speedup_vs_sim}
\end{figure*}


\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap ($Acc = 93\%$)\label{fig:CameraTrap_Acc_Diff_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_VAcc_Vs_Similarity.png}}}%
    \subfloat[\centering STL ($Acc = 93\%$) \label{fig:STL_Acc_Diff_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/STL_VAcc_Vs_Similarity.png}}}%
    % \qquad
    \subfloat[\centering PLACES ($Acc = 97\%$)\label{fig:Places_Acc_Diff_vs_similarity}]{{\includegraphics[width=.32\textwidth]{figures/Places_VAcc_Vs_Similarity.png}}}%
    \caption{Our configuration selector can closely follow the most efficient configuration; the most efficient configurations have noisy pattern around the predefined accuracy criteria for labeling}
\label{fig:Acc_Diff_vs_sim}
\end{figure*}


\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap \label{fig:CameraTrap_Boxplot_Speedup}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Boxplot_Speedup.png}}}%
    \subfloat[\centering STL
    \label{fig:STL_Boxplot_Speedup}]{{\includegraphics[width=.32\textwidth]{figures/STL_Boxplot_Speedup.png}}}%
    % \qquad
    \subfloat[\centering PLACES \label{fig:Places_Boxplot_Speedup}]{{\includegraphics[width=.32\textwidth]{figures/Places_Boxplot_Speedup.png}}}%
    \caption{Our inter-class similarity metric closely mirrors the actual difficulty level of combining the classes across all three datasets - Speedup against full resolution 3-class or All-Class EfficientNet (Table~\ref{fig:uC_full3-performance})}
\label{fig:Acc_Diff_vs_sim}
\end{figure*}

\begin{figure*}[t]%
    \centering
    \subfloat[\centering Camera Trap \label{fig:CameraTrap_Boxplot_Accuracy}]{{\includegraphics[width=.32\textwidth]{figures/Camera_Trap_Boxplot_Accuracy.png}}}%
    \subfloat[\centering STL
    \label{fig:STL_Boxplot_Accuracy}]{{\includegraphics[width=.32\textwidth]{figures/STL_Boxplot_Accuracy.png}}}%
    % \qquad
    \subfloat[\centering PLACES \label{fig:Places_Boxplot_Accuracy}]{{\includegraphics[width=.32\textwidth]{figures/Places_Boxplot_Accuracy.png}}}%
    \caption{Our configuration selector can closely follow the most efficient configuration; the most efficient configurations have noisy pattern around the predefined accuracy criteria for labeling}
\label{fig:Acc_Diff_vs_sim}
\end{figure*}

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/STL_Acc_Vs_Similarity.png}
%     \caption{STL Dataset / How well does our Inter-class similarity metric capture actual difficulty level of combining the classes?}
%     \label{fig:STL_acc_vs_similarity}
% \end{figure}

% \begin{figure}[h!!!]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/Places_Acc_Vs_Similarity.png}
%     \caption{Places Dataset / How well does our Inter-class similarity metric capture actual difficulty level of combining the classes?}
%     \label{fig:Places_acc_vs_similarity}
% \end{figure}

\mypara{Model complexity v.s. accuracy v.s. performance benefit:} Show results to illustrate tradeoff described in challenge 1(a). Table~\ref{fig:uC-performance} shows performance against the best of the rest but it would be good to have some overall results too that show the overall three-way tradeoff across all methods. some possibilities: \DG{Mohammad - can you generate boxplot graphs corresponding to the first bullet below - you probably have the data for this.}

\begin{itemize}
    \item Three boxplot graphs --- (a) Boxplot of accuracy; (b) model complexity; and (c) performance benefit (one for each scheme in Table~\ref{fig:uC-performance}). \HG{Figure 5: Expected insight from the box plot:  the speedup we can achieve depends on the difficulties of the class combinations (measured with similarity). For easy 3-class combination, we can get higher speedups compared to all-class efficientnet (3-class efficientnet) without losing much accuracy; for harder 3-class combination, our speedup is smaller and we still don't lose accuracy.   Figure 6: For accuracy, our predicted micro-classifier has small variance in the difference between micro-classfier's accuracy v.s. 3-class full resolution efficientnet's accuracy, no matter what difficulty level it is.   two curves: 1 curve from grouth truth micro-classifier: the goal is to show that there are naturally some noise caused by class difficulties; 2nd curve from our predicted micro-classifier: the goal is to show that our predicted model has consistent accuracy gap compared to the full resolution 3-class efficientnet. } 
    \item If we want to collapse into single figure, maybe Model complexity (x-axis); Accuracy (y-axis); Scatterplot with color coding representing the performance benefit. The kNN-selected scheme marked with an X. But we can start with the three boxplots.
\end{itemize}



\mypara{Comparison against baselines.} We evaluate different baselines across all datasets and show gains of our approach against the best of the baselines (Table~\ref{fig:uC-performance}).

\begin{table*}[ht]
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL} & \multicolumn{2}{c}{PLACES} \\
 & Acc & \multicolumn{1}{l|}{Speedup} & Acc & \multicolumn{1}{l|}{Speedup} & Acc & \multicolumn{1}{l}{Speedup} \\ \midrule
vs. Most efficient $\mu$C & -1.138\% & 1.742$\times$ & -0.358\% & 1.058$\times$ & -0.895\% & 1.255$\times$\\
vs 3-class EfficientNet (full res) & -3.346\% & 7.215$\times$ & -4.153\% & 2.658$\times$ & -1.727\% & 4.025$\times$ \\
vs. All-class EfficientNet (full res) & +9.005\% & 7.215$\times$ & +0.677\% & 2.658$\times$ & +5.38\% & 4.025$\times$\\
vs. All-class Early Exit (full res) & +11.172\% & 3.586$\times$ & +1.377\% & 1.394$\times$ & -\% & -$\times$\\
\midrule
Predicted $\mu$C vs best of above & -\% & -$\times$ & -\% & -$\times$ & -\% & -$\times$ \\
\midrule
\end{tabular}
\caption{Shows performance of 
the gains against each baseline and the in the row labeled ``All'', the gains against the best baseline. \HG{ baseline accuracy (full resolution 10-class efficientnet on the three classes) Expected accuracy results:  most efficient micro-classier and also our predicted micro-classifier get similar or even higher accuracy as the full resolution 10-calss efficientnet, but we are able to achieve very high speedup, similar to the most efficient micro-classifier. }}
\label{fig:uC-performance}
\end{table*}

\subsection{Context change detection evaluation}

\mypara{Context change triggering accuracy.} How well do we detect changes in context. Table~\ref{fig:comparison of trigger-accuracy} shows the results. 


\begin{table*}[ht]
\begin{tabular}{@{}p{2in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL} & \multicolumn{2}{c}{PLACES} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
vs. Most efficient $\mu$C & -0.456\% & -0.121\% & -0.301\% & -0.058\% & +0.337\% & +0.543\% \\
vs. 3-class EfficientNet (full res) & +3.091\% & +4.614\%  & +7.418\% & +6.671\%  & +3.713\% & +2.367\%  \\
%vs. Idealized $\mu$Classifier --- EfficientNet (full res) + most recent classes & 6\% & 2\%  & -\% & -\%  & -\% & -\%  \\
% vs. 10-class EfficientNet (full res) & 6\% & 2\%  & 8\% & 2\%  & 7\% & 2\% \\
% vs. 10-class Early Exit (full res) & 6\% & 2\%  & 8\% & 2\%  & 7\% & 2\% \\
% vs. 10-class Partitioning (full res) & 6\% & 2\%  & 8\% & 1.2$\times$ & 7\% & 2\% \\
\midrule
\end{tabular}
\caption{Context change trigger false positives and false negatives of different approaches. The Camera Trap dataset is longitudinal, for others, we just jumble up the images}
\label{fig:comparison of trigger-accuracy}
\end{table*}




\begin{table*}[ht]
\begin{tabular}{@{}p{2in}|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method\end{tabular}} & \multicolumn{2}{c|}{Camera Trap} & \multicolumn{2}{c|}{STL} & \multicolumn{2}{c}{PLACES} \\
 & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c|}{FN} & FP & \multicolumn{1}{c}{FN} \\ \midrule
Our Approach (predicted $\mu$C) & 12.663\% & 13.139\% & 13.535\% & 11.099\% & 8.914\% & 8.185\% \\
Most efficient $\mu$C & 13.119\% & 13.260\% & 13.836\% & 11.157\% & 8.577\% & 7.642\% \\
3-class EfficientNet (full res) & 9.572\% & 8.525\%  & 6.117\% & 4.428\%  & 5.201\% & 5.818\%  \\

\midrule
\end{tabular}
\caption{Context change trigger false positives and false negatives of different approaches. The Camera Trap dataset is longitudinal, for others, we just jumble up the images}
\label{fig:trigger-accuracy}
\end{table*}





\mypara{Context change detection evaluation.} We evaluate context change across all datasets and show gains of our approach against the best of the baselines (Table~\ref{fig:uC-across-datasets}).

\begin{table*}[h]
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Platform\end{tabular}} & \multicolumn{3}{c|}{Predicted $\mu$C} & \multicolumn{3}{c|}{Baseline 1} & \multicolumn{3}{c|}{Baseline 2} & \multicolumn{3}{c}{Baseline 3} \\
 & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency} & Power & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency} & Power & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency} & Power & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{Latency} & Power\\ \midrule
GAP8 & 66\% & 1.2s$\times$ & 8mW & .. & .. & .. & .. & .. & .. & .. & .. & ..\\
Raspberry PI  & 66\% & 1.2s$\times$ & 8mW & .. & .. & .. & .. & .. & .. & .. & .. & ..\\
Nordic N53  & 66\% & 1.2s$\times$ & 8mW & .. & .. & .. & .. & .. & .. & .. & .. & ..\\
\midrule
\end{tabular}
\caption{Table shows the performance of various methods on different embedded processors. Dataset is the camera-trap dataset.}
\label{fig:uC-across-datasets}
\end{table*}



\subsection{End-to-End evaluation}

\mypara{Local switching.} Show performance of local switching between context-aware $\mu$Classifers on platform (e.g. GAP8 or Rasp Pi), using the camera trap dataset. Assume a subset of the 3-class models are locally stored. Table ~\ref{fig:local-switching}. Notice that here we are using the most efficient $\mu$C, not the configuration determined by KNN.


\begin{table*}[h]
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
 Methods &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy\\ \midrule
Most efficient $\mu$C (20MB) & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
Most efficient $\mu$C (30MB) & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
Most efficient $\mu$C (40MB) & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
10-class EfficientNet (full res)  & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
10-class Early Exit (full res)  & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
\midrule
\end{tabular}
\caption{Local Switching; Show performance of local switching case based on the number of stored $\mu$Cs}
\label{fig:local-switching}
\end{table*}


\mypara{Cloud-based switching.} Show performance of cloud-based switching example on Raspberry PI + wireless link to server, using say the Camera Trap, Table~\ref{fig:End-to-end} and ~\ref{fig:End-to-end2}. 



\begin{table*}[h]
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
 Methods &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Energy\\ \midrule
Our Method & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
Most efficient $\mu$C & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
3-class EfficientNet (full res)  & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
10-class EfficientNet (full res)  & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
10-class Early Exit (full res)  & 66\% & 1.2$\times$ & 8mW & .. & .. & .. & .. & .. & .. \\
\midrule
\end{tabular}
\caption{End-to-End Performance of all methods on a Camera Trap recording.}
\label{fig:End-to-end}
\end{table*}



\begin{table*}[h]
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{8$\%$ Context Change} & \multicolumn{3}{c|}{6$\%$ Context Change} & \multicolumn{3}{c}{2$\%$ Context Change} \\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Flops (M)\\ \midrule
Our Method & 91.433\% & 284 & 42.709 & 92.766\% & 208 & 45.648 & 94.033\% & 102 & 44.564 \\
Most efficient $\mu$C & -\% & -$\times$ & .. & .. & .. & .. & .. & .. & .. \\
3-class EfficientNet (full res)  & -\% & -$\times$ & .. & .. & .. & .. & .. & .. & .. \\
10-class EfficientNet (full res)  & 91.433\% & -$\times$ & 74 & 91.433\% & .. & 74 & 91.433\% & .. & 74 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}
\caption{Table shows how the performance varies based on the frequency of context change. Dataset is STL. Labeling > Baseline + 1$\%$}
\label{fig:End-to-end2}
\end{table*}


\begin{table*}[h]
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
Methods & \multicolumn{3}{c|}{100$\%$ Oracle} &  \multicolumn{3}{c}{EfficientNet Oracle} \\
  &\multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Flops (M) & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{\#Switches} & Flops (M)\\ \midrule
Our Method & 90.375\% & 70 & 165 & 81\% & 107 & 217 \\
Most efficient $\mu$C & -\% & -$\times$ & .. & .. & .. & .. \\
3-class EfficientNet (full res)  & -\% & -$\times$ & .. & .. & .. & .. \\
10-class EfficientNet (full res)  & 83\% & -$\times$ & 810 & 83\% & .. & 810 \\
%10-class Early Exit (full res)  & 90.733\% & -$\times$ & .. & 90.733\% & .. & .. & 90.733\% & .. & .. \\
\midrule
\end{tabular}
\caption{Table shows how the performance varies based on the oracle performance. Dataset is Camera Trap. Labeling > Baseline + 5$\%$, 3$\%$ Context Change}
\label{fig:End-to-end3}
\end{table*}

==> Scenario.tex <==
\section{Pipeline Scenarios}

We identify that our pipelines not only are compatible with any model partitioning methods by leveraging the parallel transmission as we described in our design but also can work standalone as non-blocking inference pipelines. The main difference between the above two scenarios is whether the granularity module is included \ref{}: under the enhancement scenarios, our methods are leveraged to enhance the model split methods and will wait to merge all the features before the split point so that only one inference result will be given for the single input; under the non-blocking scenarios, our methods are generating results in a finer grained granularity and therefore multiple inference results are generated along the way to the possible early stop or the split point. Because we are not blocked by waiting for the features to be transmitted under the latter scenarios, we identify it as non-blocking inference pipelines. 

\mypara{Enhancing partitioned edge-cloud models:} Our methods can be used to enhance the partitioned edge-cloud models to fully utilize the parallelism of transmission and execution on IoT devices. 

\Jin{A Figure to show campatiblity of partition-model}

For example, Figure~\ref{} shows how the partitioned models can be enhanced by our module. The pipeline when used as enhancement will use our IoT design and part of the cloud design described in Sec~\ref{}. We denote the point when the features are transmitted from the edge to the clouds as the transmission point. Instead of a single transmission point in the traditional model split methods, our methods as enhancement make every layer before the split point as a potential transmission point to transmit some features to cloud. Cloud also requires feature encoders and feature aggregate modules to encode and aggregate the features received from the IoT devices. After receiving all the features before the partition points, our methods will generate an inference results.

\mypara{Latency-aware Partition-free models:}
Our method could not only perform as an enhancement to the model split methods but could also be a non-blocking latency-aware deployment of deep learning models. The model split methods is constrained by the partition points because the models deployed on the IoT devices will always be executed until the split point and then the features generated at the split point will be transmitted to the clouds. However, for latency-sensitive applications, the constraint can be inflexible. Our methods, because of the parallelism between the data transmission and model execution on IoT devices, are not constrained by partition points - we could stop the execution of the models after any layer as long as the performance given the received data reaches the expectation - namely latency-aware inference in a non-blocking manner. 

Furthermore, the possibility of determining where to stop the pipeline rather than restricted from the split points, enables the extra flexibility of dynamic on-clouds early-exit. 
